Learning to Configure Computer Networks with Neural Algorithmic Reasoning

We present a new method for scaling automatic configuration of computer networks. The key idea is to relax the computationally hard search problem of finding a configuration that satisfies a given specification into an approximate objective amenable to learning-based techniques. Based on this idea, we train a neural algorithmic model which learns to generate configurations likely to (fully or partially) satisfy a given specification under existing routing protocols. By relaxing the rigid satisfaction guarantees, our approach (i) enables greater flexibility: it is protocol-agnostic, enables cross-protocol reasoning, and does not depend on hardcoded rules; and (ii) finds configurations for much larger computer networks than previously possible. Our learned synthesizer is up to 490x faster than state-of-the-art SMT-based methods, while producing configurations which on average satisfy more than 93% of the provided requirements.

==> diff/git-latexdiff.33774/new/acronyms.tex <==
\DeclareAcronym{AS}{
    short = AS,
    long = autonomous system,
    short-plural = es ,
    long-plural = s
}

==> diff/git-latexdiff.33774/new/sections/0_abstract.tex <==
% Context
Computer networks employ a number of different protocols to enable efficient routing. However, due to the complexity of multiple interacting protocols, it can be hard for network operators to implement high-level routing policies and requirements. Network configuration synthesis promises to address this situation by automatically generating configurations that satisfy a provided specification. However, existing synthesis methods are often limited to single-protocol reasoning, depend on protocol-specific and hand-coded synthesis rules, and are difficult to scale due to the SMT-based methods they employ. In this work we present a rather different, learning-based method for addressing the configuration synthesis challenge, one based on the recently proposed paradigm of neural algorithmic reasoning. Our framework is protocol-agnostic, enables cross-protocol reasoning and does not depend on any hardcoded synthesis rules. To evaluate, we instantiate our framework for the case of BGP/OSPF synthesis. Our experiments show we can synthesize configurations with a very high degree of specification consistency while observing speedups of up to $500\times$ compared to a state-of-the-art SMT-based synthesis tool.


==> diff/git-latexdiff.33774/new/sections/1_intro.tex <==
\section{Introduction}
\label{sec:introduction}

The backbone of the internet consists of many connected computer networks operated by different internet service providers (ISPs) and other large organizations. These networks rely on a number of protocols to enable effective and policy-driven routing of traffic. Based on router-level configurations, the protocols perform a distributed computation to construct a network's forwarding state. However, the relatively low-level router configuration makes it hard for network operators to directly enforce network-wide policies and requirements. This often leads to misconfiguration, which can cause global outages such as the recent hours-long blackout of the entire Facebook platform \cite{janardhan2021} and comparable events \cite{mccarthy_2019}.
%
\paragraph{Configuration Synthesis} This situation has triggered a number of research efforts regarding the synthesis of network configurations \cite{el2018netcomplete,beckett2017network,narain2008declarative}. Configuration synthesis is concerned with the task of automatically generating router-level configurations given a set of high-level requirements. However, this synthesis problem can be very hard to solve, since network configurations typically consist of a considerable number of tunable parameters, where the execution of several interacting protocols yields the overall forwarding state. An effective synthesis tool must thus account for this fact and be able to reason across multiple protocols.

\paragraph{SMT-based Synthesis} Some of the most successful efforts in providing cross-protocol synthesis capabilities are based on satisfiability modulo theory (SMT) solvers \cite{el2018netcomplete,el2017network}. While SMT-based synthesis is a promising method, it comes with a number of limitations:
% \item protocol-specific
% fully hand-coded synthesis rules, a lot of implementation effort, cross-protocol support extra complicated
(1) SMT-based synthesizers are hand-crafted and highly protocol-specific. To implement synthesis, we must first express our networking model, protocol semantics including vendor and device specific behavior in terms of first-order logic constraints. This is a time-intensive and complicated process, requiring lots of expert knowledge.
%  model-dependent: synthesis is reasoning on the level of some assumed model which may not reflect the real world: even if a configuration is synthesized based on some spec, it may behave differently and violate spec in practice
Further, (2) logic-based modelling introduces a disconnect between the synthesis tool and real-world behavior \cite{birkner2021metha}. More specifically, synthesized configurations may satisfy a provided specification within a formal framework, but may not behave the same way in the real world.
% can be very slow
And, (3) SMT-based synthesis can be very slow or fail to complete, especially when reasoning about large network topologies. In practice however, network operators reconfigure their networks on a daily basis \cite{vissicchio2012improving}, which means an effective synthesis tool must be fast.

% \item fully learned, no hand-coded synthesis rules (model-free), very flexible to adapt to more/new protocols
% \item protocol-agnostic, cross-protocol
\paragraph{Neural Algorithmic Reasoning for Synthesis} Recent work on neural algorithmic reasoning (NAR) proposes to replace traditional algorithms with neural networks to learn improved algorithmic procedures \cite{velivckovic2021neural}.
It has been shown to be a powerful and fast algorithmic approximation method for a number of graph-related \cite{velivckovic2019neural} and combinatorial optimization problems \cite{cappart2021combinatorial}. Further, due to its learned nature, NAR allows for learning procedures directly from (real-world) data, without the need for manual feature extraction. Overall, this positions NAR as an attractive method to obtain a fast, fully-learned synthesis procedure, which entirely avoids the need for a formal model or any hand-crafted synthesis rules. Based on this promising outlook, this paper explores how to apply the NAR paradigm to the problem of network configuration synthesis.

To that end, we propose a \textbf{new learning-based framework for configuration synthesis} as an alternative to SMT-based approaches. Our framework is protocol-agnostic, enables cross-protocol reasoning and avoids the need to manually provide synthesis rules. We build upon the idea of NAR, and train a graph-based processor neural network to learn a synthesis procedure in latent space. A key challenge in a multi-protocol setting is the diversity of different protocols and configuration parameters. To this end, we implement a generic embedding scheme based on Datalog-like facts and program sketching \cite{solar2008program}, which allows us to easily adapt our framework to new protocols. Further, our synthesis model produces a whole distribution of network configurations. As a consequence, we can directly sample multiple alternative synthesis outputs, which is not possible with standard SMT solvers. We apply our framework to a non-trivial synthesis setting where both the Border Gateway Protocol (BGP) and the Open Shortest Path First (OSPF) protocol are used. We demonstrate that our learned synthesis tool is up to~$500\times$ faster than a state-of-the-art SMT-based synthesizer, while producing configurations which on average enjoy more than 91\% satisfaction of the provided specification.

\paragraph{Main Contributions} Our core contributions are:
\vspace{-5pt}
\begin{itemize}
    \setlength{\itemsep}{5pt}
    \setlength{\parskip}{0pt}
    \item A learning-based framework for network configuration synthesis based on neural algorithmic reasoning.
    \item A neural network architecture for learning synthesizer models which relies on a generic graph-based encoding of network topologies and configurations.
    \item An extensive evaluation of our learning-based synthesizer, in terms of both precision and scalability, on the challenging setting where both the BGP and OSPF protocols are involved.
\end{itemize}

\section{Framework Overview}
\label{sec:overview}

\begin{figure}
    \begin{center}
        \includegraphics[width=0.45\textwidth]{figures/synthesizer-overview.pdf}
    \end{center}
    \caption{An overview of our learning-based synthesis framework.}
    \label{fig:learning-based-synthesis}
\end{figure}

%As an example, consider \cref{fig:network-fwd-tree} (c) which illustrates the forwarding plane of some traffic class reachable via external peer $E$ or $F$ in our example network. Each router of the network forwards traffic along some of its outgoing links. In practice, a number of protocols are used to populate a router's routing tables. For the instantiation of our synthesis framework however, we focus on OSPF and BGP.

In the following, we discuss the fundamentals and core steps of our learning-based framework as illustrated in \cref{fig:learning-based-synthesis}.

\paragraph{Network Configuration} In this work, we consider the configuration synthesis problem at the level of the so-called \emph{forwarding plane} of a network. This means we look at how each router forwards traffic, given a packet with a certain destination. The forwarding plane is determined by a distributed computation whose exact semantics depend on the different routing protocols in use. To adapt the forwarding behavior, network operators change configuration parameters at the router-level (e.g. link weights), such that running the protocols results in the desired forwarding plane. Given this context, we define the problem of configuration synthesis as follows.

\paragraph{Configuration Synthesis} The configuration synthesis problem corresponds to automatically generating these router-level configurations, such that a set of given requirements about the forwarding plane is satisfied. Typical requirements include reachability, traffic isolation and other forwarding properties. 

\paragraph{Dataset} To train a synthesizer model, we first generate a dataset of input/output samples for the synthesis problem. For this, we rely on a generative pipeline as shown in the top of \cref{fig:learning-based-synthesis}. First, we sample a random network configuration for some topology using a uniform generative process. Then, we simulate the involved protocols to obtain the corresponding forwarding plane. Next, we extract a specification by randomly selecting properties that hold for the computed forwarding plane. This leaves us with a specification and topology as input and corresponding configuration as the output to a synthesis problem.

\paragraph{Simulation} Depending on the protocols in use, one implements simulation code to compute the forwarding plane induced by a sampled configuration. Although this step is protocol-specific, the overall implementation effort is much lower compared to SMT-based synthesis. Protocols are typically well-defined algorithms which can be simulated, whereas the alternative of implementing a synthesizer often requires expert knowledge about SMT solvers. In practice, our framework may also be adapted to use a real-world network router to compute the behavior of a configuration, thereby capturing the real-world behavior directly.

\paragraph{Neural Synthesizer Model} Based on the generated dataset, we train a graph neural network (GNN) to perform synthesis. For this, the network's input consists of a topology, a specification and a configuration sketch where to-be-synthesized parameters are omitted. Following the NAR paradigm, we first encode this synthesizer input in latent space. Then, we apply an iterative processor network which relies on the graph attention mechanism to propagate information \cite{velivckovic2017graph}. Last, we apply a decoder network to predict the values of omitted configuration parameters, thereby synthesizing a corresponding configuration. To remain protocol-agnostic, our model is generic with respect to the input format, using an intermediate representation based on Datalog-like facts.
%
\paragraph{Relaxed Specification Consistency} Since parts of the configuration synthesis problems are known to be NP-hard \cite{fortz2000internet}, any precise synthesis method will run into scalability issues, just like SMT-based methods. However, practical synthesis must be fast and scalable to accommodate the size of real-world networks and the frequency at which configurations need to be updated \cite{vissicchio2012improving}. In our learning-based framework, we therefore employ a fixed-size neural network architecture which always runs in polynomial time. While this indeed enables fast synthesis times, we cannot expect our neural system to be as precise as SMT methods. Therefore, to assess the synthesis capabilities of our learning-based system, we rely on the notion of \emph{relaxed~specification~consistency}. More specifically, we do not just check whether a configuration satisfies a specification or not, but also measure the degree up to which a synthesized configuration satisfies a specification (e.g. via the number of satisfied requirements). 

This "soft" understanding of a specification allows us to evaluate neural synthesis systems which may not always produce fully consistent configurations. Further, we argue that configurations with less than $100\%$ consistency are still very useful in practice, as they provide a good starting point for additional adjustments by network operators. Future work may improve the precision of neural synthesis by exploiting partial synthesis methods \cite{el2018netcomplete} to obtain fully consistent solutions, given a partially consistent configuration. However, note also that even exact SMT-based synthesizers may not always produce fully consistent solutions, due to differences between the formal protocol model and the one running on a given real-world router where the configuration is to be deployed \cite{birkner2021metha}.

\paragraph{Instantiation} Our learning-based synthesis framework is generic with respect to the routing protocols in use. This means, it can be instantiated to many different synthesis settings. To do this, users merely provide a drop-in replacement for the simulation component as shown in \cref{fig:learning-based-synthesis}, while other components such as the neural model architecture itself can be directly re-used.

%More specifically, we employ a slightly modified variant which operates on a graph-based encoding of a specification, topology and configuration parameters.

%  \begin{figure*}
%      \centering
%      \includegraphics[width=0.85\textwidth]{figures/system-overview.pdf}
%      \caption{An overview of our synthesis system: (1) First, we use a generic embedding scheme to transform a network topology, protocol configuration sketches and the specification given as Datalog-like facts to a latent input representation. Next, we apply a learned (2) Processor GNN and obtain a latent synthesis output. Last, we apply a (3) Decoder Network to obtain a distribution over possible values per unknown parameter in our configuration.}
%      \label{fig:overview-model}
% \end{figure*}
%

In this paper, we first discuss the architecture of our neural synthesis model. In follow-up sections, we instantiate our framework  for the case of BGP/OSPF configuration synthesis, and evaluate the resulting instantiation by comparing it to a state-of-the-art SMT-based synthesizer.

% \begin{itemize}
%     \item effort: need to implement simulation code to generate dataset to learn from (typically well-defined in protocol specs, much easier than implementing synthesis directly)
%     \item can be sampled (multiple alternative solutions, not easily possible with SMT-based methods)
%     \item much faster than SMT-based synthesis
% \end{itemize}

% Requirements:
% \begin{itemize}
%     \item protocol-agnostic
%     \item fully learned, no hand-coded synthesis rules
%     \item define: strict specification vs. relaxed specification
% \end{itemize} 

==> diff/git-latexdiff.33774/new/sections/2_model.tex <==
\section{Neural Synthesis Model}
\label{sec:model}


We now present the architecture of our graph-based neural synthesizer model, illustrated in \cref{fig:overview-model}. First, in \cref{sec:graph-embedding} we introduce our generic graph-based encoding, which allows us to embed network topologies, protocol configuration and the specification into a latent space. Then, in \cref{sec:graph-transformer} we present the architecture of the processor network which we train to perform the synthesis task. Finally, in \cref{sec:decoding-sampling} we discuss how to sample network configurations from the resulting latent synthesis output.

\begin{figure}
    \begin{minipage}[t]{0.21\textwidth}
    \begin{lstlisting}[basicstyle=\ttfamily\small, escapeinside={(*}{*)}]
router(A)
router(B)
(...)

connected(A,B,2)
connected(A,C,?)(*\blackcircled{1}*)
(...)
    \end{lstlisting}
\end{minipage}
\begin{minipage}[t]{0.21\textwidth}
    \begin{lstlisting}[basicstyle=\ttfamily\small, escapeinside={(*}{*)}]
network(N1)
bgp_route(E,N1,2,3,1,0,1)

fwd(A,B,N1)
not fwd(B,A,N1)
(...)
    \end{lstlisting}
\end{minipage}
    \caption{A snippet of a fact base sketch encoding a network's topology, parameters such as link weights (\texttt{connected} facts) and a specification (\texttt{fwd} facts).}
    \label{fig:datalog-encoding}
\end{figure}

\begin{figure}[t]
    \centering
    \includegraphics[width=0.25\textwidth]{figures/synth-architecture.png}
    \caption{The neural synthesizer model architecture.}
    \label{fig:architecture}
\end{figure}

\subsection{Fact Base Embedding}
\label{sec:graph-embedding}
To remain network protocol-agnostic in our model architecture, we implement a generic graph-based encoding of Datalog-like facts, similar to knowledge graphs \cite{rosso2020beyond}. This means that we first encode topologies, configurations and specifications as a set of Datalog-like facts and then employ a generic embedding.
%We chose Datalog facts as the input format of our synthesis approach for its flexibility, wide-spread use in Program Analysis and use in previous work on configuration synthesis \cite{el2017network}.

\paragraph{Fact Base} A set of Datalog-like facts, as depicted in \cref{fig:datalog-encoding}, serves as the input \emph{fact base} $\mathcal{F}$ to our synthesizer model. $\mathcal{F}$ is a set of facts $f(a_0, \dots, a_n)$ where arguments may be constants (e.g. A or B) or integer literals. Further, each fact in a fact base has a corresponding truth value denoted as $[f(a)]_{\mathcal{B}}$. For instance, from the fact base in \cref{fig:datalog-encoding} we can derive $[fwd(A,B,N1)]_{\mathcal{B}} = \text{\texttt{true}}$ and $[fwd(B,A,N1)]_{\mathcal{B}} = \text{\texttt{false}}$.

\paragraph{Consistency} We represent a network's topology, the protocol configuration and parameters as well as the specification, all in a single fact base. Given the semantics of the protocols in use, we can then check whether the specification encoded in a fact base is satisfied by the provided configuration. To quantify, we define the notion of relaxed specification consistency, as discussed earlier, with respect to a fact base: Given a fact base $\mathcal{F}$, a subset of specification facts $S \subset \mathcal{F}$ and protocol semantics $\mathcal{P}$, the \emph{consistency} of a fact base is defined as the relative number of satisfied facts in $S$ with respect to the forwarding plane obtained via $\mathcal{P}$. The contents of $S$ depend on the concrete instantiation of the synthesizer model. For an example of possible specification facts, see our instantiation of the synthesizer model for BGP/OSPF in \cref{sec:training}.

\begin{figure*}
    \footnotesize
    \def\arraystretch{1.4}
    \begin{tabular}{lr}
        %$T_f: T_1 \times \dots \times T_n$ & \textit{(fact type declaration)}\\
        $emb(f) := \mathbf{V_f}$ & \textit{(learned fact type embedding)}\\
        $emb(b) := \mathbf{W_{\text{bool}}}\;onehot(b)$ & \textit{(learned boolean embedding)}\\
        $emb(f,i,v) := \mathbf{W_{f_i}}\;onehot(v)$ & \textit{(learned integer embedding)}\\
        $emb(f,i,?) := \mathbf{V_{hole}}$ & \textit{(learned hole embedding)}\vspace{2pt}\\
        $\mathlarger{
        h_c := \sum_{f(c) \in \mathcal{F}}
        emb(f)
        }$ & \textit{(constant embedding)}\vspace{2pt}\\
        $h_{f(a_0, \dots, a_n)} := emb(f) + emb([f(a_0, \dots, a_n)]_{\mathcal{B}}) + \mathlarger{
        \sum_{(i,v) \in \mathcal{I}(f(a_0, \dots, a_n))}
        emb(f, i, v)
        }$\hspace{-1.2cm} & \textit{(fact embedding)}\\
        $\mathcal{I}(f(a_0, \dots, a_n)) := \{(i,v) \; | \; f(a_0, \dots, a_{i-1}, v, \dots, a_n) \in \mathcal{F} \wedge v:Int \wedge i \in \mathbb{N}$ \}& \textit{(integer arguments)}\vspace{2pt}\\
        $N_i(h_c) := \{h_f \; | \; \exists i \in \mathbb{N} . f(a_0, \dots, a_{i-1}, c, a_{i+1}, \dots, a_n) \in \mathcal{F}\}$& \textit{(i-th neighborhood of constant node)} \\
        $N_i(h_f) := \{h_c \; | \; \exists i \in \mathbb{N} . f(a_0, \dots, a_{i-1}, c, a_{i+1}, \dots, a_n) \in \mathcal{F}\}$& \textit{(i-th neighborhood of fact node)} \\
    \end{tabular}
    \caption{Translating a fact base $\mathcal{F}$ to node features. $f$ denotes a predicate, $v$ integer values, $b$ boolean values as 0 or 1, $i$ argument indices and $[f(a)]_{\mathcal{B}}$ the truth value of a fact. }
    \label{fig:graph-embedding}
\end{figure*}

%discuss embedding as shown in \cref{fig:datalog-encoding}. Note how this makes fact bases a suitable input to standard GNN architectures.

\paragraph{Fact Base Sketching} In a synthesis setting, we are confronted with incomplete fact bases, i.e. the specification and topology is given but the network configuration is to be synthesized. For these cases, we also consider fact bases with unknown parameters inspired by the idea of program sketching in program synthesis \cite{solar2008program}. More specifically, users may replace an unknown integer argument of a fact by a \texttt{?} symbol, indicating a value to be synthesized. Using this mechanic, we can represent the synthesis input as an incomplete fact base which encodes to-be-synthesized values as unknown parameters. As an example, consider \cref{fig:datalog-encoding} \blackcircled{1}, where the link weight between router nodes \texttt{A} and \texttt{C} is represented as an unknown parameter.

\paragraph{Embedding} We employ a structurally-defined embedding scheme to transform a fact base into a graph with node features as required for processing with graph neural networks. Given a fact base $\mathcal{F}$, we apply the rules in \cref{fig:graph-embedding} to obtain node features and adjacency information. Both a fact $f$ and a constant $c$ are represented as distinct nodes with features $h_c$ and $h_f$, respectively. The relationships between facts and constants is encoded as node adjacency as defined by the neighborhood functions $N_i$.

We use multiple neighborhood functions, i.e. multiple types of edges, to encode the argument position of a constant occurring in a fact. Hence, the number of neighborhood functions corresponds to the maximum number of arguments in a single fact, e.g. 3 in \cref{fig:datalog-encoding}. Integer arguments and unary facts are directly accounted for in the respective node or fact embedding. To handle unknown parameters, we replace the corresponding $emb(...)$ term with the learned $\mathbf{V_{hole}}$ embedding.

Considering the embedding function $emb$, the learned parameters of our embedding are $\mathbf{V_f} \in \mathbb{R}^D$ per fact type in~$\mathcal{F}$, $\mathbf{W_{\text{bool}}} \in \mathbb{R}^{D \times 2}$ for boolean values, $\mathbf{W_{f_i}} \in \mathbb{R}^{D \times N}$ per integer argument of fact type $f$ and $\mathbf{V_{hole}} \in \mathbb{R}^D$ to represent unknown parameters. Hyperparameter $D$ represents the dimension of the latent space the synthesizer model operates in and $N$ specifies the number of supported integer values. An example of applying this embedding scheme to a simple fact base is given in \cref{fig:graph-encoding-example}.

\begin{figure}
    \begin{minipage}[t]{0.2\textwidth}
        \centering
        \footnotesize
        \textbf{Fact Base}
        \begin{lstlisting}[basicstyle=\ttfamily\small]
router(A)
router(B)

conn(A, B, 12)
        \end{lstlisting}
    \end{minipage}
    \begin{minipage}[t]{0.15\textwidth}
        \centering
        \textbf{Graph}\\
        \vspace{5pt}
        \includegraphics[width=0.7\textwidth]{figures/graph-encoding.pdf}
    \end{minipage}\\
    \centering\\
    \vspace{10pt}
    \textbf{Node Features}\\
    \vspace{10pt}
    \begin{minipage}[t]{0.5\textwidth}
        $\begin{array}{rcl}
        h_A &:=& emb(router) = \mathbf{V_{\text{router}}}\\
        h_B &:=& emb(router) = \mathbf{V_{\text{router}}}\\
        h_{\text{conn(A,B,12)}} &:=& emb(conn) + emb(conn, 2, 12)\\
        &:=& \mathbf{V_{\text{conn}}} + \mathbf{W_{conn_2}} onehot(12)
    \end{array}$
    \end{minipage}
    \caption{An example of embedding a simple fact base using the embedding scheme of \cref{fig:graph-embedding}. The shown graph illustrates the neighborhoods $N_0$ and $N_1$ induced by the \texttt{conn} fact.}
    \label{fig:graph-encoding-example}
\end{figure}

\begin{figure}
    $$
    \begin{array}{rcl}
    z_j &:=& h_j + Drop(\mathlarger{\sum_{N_i}} h'_{GAT_i})\\
    h'_j &:=& FFN(Norm(z_j))\vspace{11pt}\\
    FFN(x_j) &:=& Norm(Lin2(Drop(Lin1(x_j)))))
    \end{array}
    $$
    \caption{
        The recurrence relation of a node $j$'s representation $h_j$. $h'_{GAT_i}$ represents the output of a graph attention layer operating with neighborhood $N_i$ according to \cite{velivckovic2017graph}, $h_j$ the representation of node $j$ at the previous step. $Norm$ refers to batch normalization \cite{ioffe2015batch}, $Drop$ to dropout regularization \cite{hinton2012improving} and $Lin1$ and $Lin2$ to linear layers with an inner dimension of $4N$.
    }
    \label{fig:recurrence}
\end{figure}

\subsection{Synthesizer Model}
\label{sec:graph-transformer}

For an illustration of the synthesizer model's architecture, please see Figure~\ref{fig:architecture}. Given a fact base $\mathcal{F}$ we first apply our embedding scheme as described in \cref{sec:graph-embedding}. We then employ a 2-layer GNN-based encoder network to produce the latent representation of a synthesis input.
Given this representation, a processors network is trained to perform the actual synthesis task in high-dimensional space. Last, we apply a set of decoder networks, to obtain the synthesized values of unknown parameter, given the latent synthesis~output.

%In this context, the synthesis problem for network configurations corresponds to completing partially provided fact bases.

% \paragraph{High-Level Architecture}

% We employ the high-level architecture to obtain the latent synthesis output $y_\mathcal{F}$:
% $$
% \begin{array}{rcl}
%     \mathbf{x_{\mathcal{F}}} &:=& Encoder(Embedding(\mathcal{F}))\\
%     \mathbf{y_{\mathcal{F}}} &:=& Processor(\mathbf{x_{\mathcal{F}}} + \mathbf{z})\\
%     z_i &\sim& \mathcal{N}(0,1)
% \end{array}
% $$
% \todo{z is only added for $i<N/2$}

% $Embedding$ corresponds to the graph-based embedding as discussed in \cref{sec:graph-embedding} and $Encoder$ is a 2-layer graph attention module. $Processor$

\paragraph{Encoding} The encoder GNN operates on the embedded representation of a fact base. It produces the high-dimensional representation of a synthesis input as required for the processor network. We additionally apply noise to the first half of the units of the latent representation via $\mathbf{z}$, as a source of non-determinism. According to our experiments this improves model performance and we hypothesize this is due to the synthesis problem having more than one solution in most cases.

\paragraph{Iterative Processor} The processor network is modelled as an iterative process. It consists of a 6-layer graph attention module which we apply for a total of 4 iterations. In the framework of neural algorithmic reasoning, this iterative computational structure encodes an inductive bias towards an iterative solution to the synthesis problem. Because of this bias, our processor network essentially learns an algorithmic procedure which iteratively synthesizes the values of unknown parameters in a fact base.

\paragraph{Graph Attention Layer} In the GNNs we employ, we rely on a composed variant of the graph attention layer as introduced by \cite{velivckovic2017graph}. We employ multiple graph attention layers in lockstep, one per neighborhood $N_i$ defined by our graph embedding (cf. \cref{sec:graph-embedding}), and combine the intermediate results after each step. Specifically, the recurrence relation of a node $j$'s representation $h_j$ is defined as shown in \cref{fig:recurrence}. These mechanics of combining the results of the different graph attention layers $h'_{GAT_i}$, directly corresponds to how multiple attention heads are combined in the original Transformer architecture \cite{vaswani2017attention}.

\paragraph{Argument Decoder Networks} To synthesize the values of unknown parameters, the model maintains a set of decoder networks. That is, it provides one decoder network per integer argument per fact type in a fact base. When decoding, the network is applied to the latent synthesis output of the corresponding fact node. For example, a synthesizer model which operates on the fact base in \cref{fig:datalog-encoding}, would provide a decoder network $D_{\text{connected}_2}: \mathbb{R}^D \rightarrow \mathbb{R^N}$ to decode values for the third argument of a \texttt{conn} fact. In our experiments, decoder networks are implemented as simple multi-layer perceptron models.

\paragraph{Supervision Signal} During training, we mask all fact arguments that represent to-be-synthesized configuration parameters in our synthesis setting. As a supervision signal we use the masked values as the ground-truth and apply a negative log-likelihood loss function to the output distribution of the corresponding argument decoder networks.

%The synthesizer model learns a conditional distribution of fact bases which are consistent with respect to the protocols' semantics.

%\todo{introduce synthesis as a completion problem of an encoded fact base (a la BERT). Introduce masking, introduce decoding of integer and truth values. Synthesis is learning a conditional distribution of consistent fact bases.}

%Using this method, we obtain the node features $h_c$ per constant, $h_f$ per fact and adjacency information in terms of node neighborhood functions $N_i(h_c)$ and $N_i(h_f)$. Overall, this encoding makes a fact base suitable for processing using standard graph neural networks.

%- Brief description of the Graph Transformer Model
\subsection{Multi-Shot Sampling}
\label{sec:decoding-sampling}

%Multi-Stage Parameter Sampling (sampling methods: topk, high-temp, low-temp)
To sample concrete values from the output distributions over unknown parameters, we apply a multi-shot sampling strategy. That is, we sample values only for a subset of unknown parameters, insert them in our input fact base and run the synthesis model again. We repeat this process until no more unknown parameters remain. This multi-shot sampling strategy allows the model to incorporate the concrete values of previously synthesized parameters in its computation. In our evaluation in \cref{sec:evaluation}, we include a comparison of how this compares to sampling all unknown parameters at once.

%In a fact base with multiple holes, we apply the corresponding decoder networks to obtain a value distribution for each integer hole. However, instead of sampling all integer holes in one


==> diff/git-latexdiff.33774/new/sections/3_bgp_ospf.tex <==
\section{BGP/OSPF Synthesis}
\label{sec:bgp-ospf}

\newcommand{\as}{\ac{AS}~}
\newcommand{\ases}{\acp{AS}~}

\newcommand{\squareann}{{\tiny$\blacksquare\;$}}
\newcommand{\triangleann}{{\small$\blacktriangle\;$}}

\begin{figure*}
    \centering
    \includegraphics[width=0.95\textwidth]{figures/networks-all.pdf}
    \caption{(a) An illustration of a small AS network, including internal peers (blue), external peers (purple), BGP sessions as well as physical links. (b) The propagation of two BGP announcement across the network. (c) The resulting forwarding plane after applying BGP and OSPF.}
    \label{fig:network-fwd-tree}
\end{figure*}

We now discuss an instantiation of our learning-based framework for the case of BGP and OSPF protocols. In \cref{sec:synthesis-setting} we introduce a basic networking model, BGP and OSPF protocols and the synthesis setting. Given this model, \cref{sec:training} describes how to generate a corresponding dataset of input/output samples and train a synthesizer model.
%This shall serve as a prerequisite to the instantiation of our learning-based synthesis framework for the BGP and OSPF protocol in \cref{sec:training}.

\subsection{Synthesis Setting}
\label{sec:synthesis-setting}

\paragraph{Graphical Model} We assume an abstract network model which can be represented as an undirected graph as shown in \cref{fig:network-fwd-tree} (a). We always consider a set of internal routers (A, B, C, D in \cref{fig:network-fwd-tree}) as well as a set of adjacent external routers (E, F  in \cref{fig:network-fwd-tree}). The group of internal routers forms the \emph{\as} under consideration whereas external routers belong to other adjacent \ases. In practice, an \as represents an administrative domain controlled by a single operator. 

\paragraph{Forwarding Plane} For an example of a possible forwarding plane in this abstract model, consider \cref{fig:network-fwd-tree} (c) which illustrates the forwarding plane of traffic destined towards some destination reachable via external peer $E$ or $F$. Each router of the network forwards traffic along some of its outgoing links. In practice, a number of protocols are used to compute the forwarding plane. However, here we focus on OSPF and BGP.

\paragraph{OSPF} The OSPF protocol \cite{moy1994ospf} is a link-state protocol, typically used as an interior gateway protocol~(IGP), i.e., to route traffic within an \ac{AS}. Given link weights per physical link in the network, OSPF simply routes traffic along the shortest path towards the destination.

\paragraph{BGP} The BGP protocol \cite{rekhter1994border} on the other hand is a path-vector protocol used to exchange reachability information mostly on the level of \acp{AS}.
%These are groups of routers typically operated by a single party (e.g. an ISP).
When using BGP, a routing destination announces its existence to other \ases and routers, by sending out a BGP announcement. Receivers of such announcements may then choose to pass them on to other \acp{AS}, redistribute them internally and/or modify them. Instead of communicating along physical links directly, the BGP protocol requires manually configured BGP sessions among routers of the \as and external peers, as indicated by the BGP session edges in \cref{fig:network-fwd-tree}(a).
%\todo{more discussion of eBGP vs iBGP and support for route reflection (more of an implementation detail, maybe only mention in dataset generation where simulation code is discussed)}.

%\paragraph{BGP Decision Procedure}~
%\todo{discuss decision procedure}
In case a router receives more than one announcement for a destination, a designated BGP decision process is applied to determine a single best route. \cref{fig:bgp-decision} shows the ordered list of comparison criteria of this decision process. The different criteria depend different properties of a route announcements, including the IGP cost towards the routing destination. As a consequence, when used together, OSPF as IGP protocol and BGP will interact. %Note also that BGP is an iterative process which needs multiple rounds of propagation to converge.

\paragraph{Example}
%\todo{run through simple BGP+OSPF example of computing the forwarding plane}
To better understand BGP/OSPF routing, consider the simple example given in \cref{fig:network-fwd-tree} (b). Here, our example \as imports BGP announcements \squareann and \triangleann from E and F respectively. Both represent a route to the same destination. As shown, both announcements have a so-called local preference of 2. For simplicity, we ignore other properties such as the AS path length, Origin and MED in this example. The announcements are propagated among BGP neighbors and the best route is selected according to the decision procedure in \cref{fig:bgp-decision}. See \cref{fig:network-fwd-tree} (b) for an illustration of the intermediate states of this propagation process. As both announcements have a local preference of 2, rule 1 of the decision process is not used. Instead, in round 2, node B selects \squareann over \triangleann due to a lower IGP cost of 2 via egress node A as compared to 3 via egress node D (rule 6). Node D selects \triangleann over \squareann, since it learns this route directly from an external peer (rule 5). After Round 3, the BGP propagation process converges to a stable state and we can derive the forwarding plane as shown in \cref{fig:network-fwd-tree} (c).


%, as well as external peers E and F which belong to other \acp{AS}. External peers are routers which are connected via eBGP sessions to routers of the \ac{AS} under consideration. They announce BGP routes to their neighbors, which are propagated within the network

%\paragraph{BGP/OSPF Configuration Synthesis} We phrase the BGP/OSPF configuration synthesis problem on the level of the forwarding plane. This means that users provide a specification which constraints the set of allowed forwarding planes. This includes predicates which enforce forwarding paths, block forwarding paths or assert higher-level properties like traffic isolation and reachability. Given such a specification, we consider network configuration synthesis as the task of configuring OSPF and BGP in a way that produces a forwarding plane which satisfies the provided specification.

\paragraph{BGP/OSPF Configuration Synthesis} According to our general synthesis framework, we consider the BGP/OSPF configuration synthesis problem at the level of the forwarding plane. However, we further also define the set of synthesized parameters: For OSPF we synthesize link weights as explored in a wide range of existing work (e.g. \cite{el2018netcomplete,fortz2000internet}. For BGP, the set of parameters is not defined as clearly: Depending on the requirements of a network operator, one may employ custom BGP import and export policies at every router of a network to implement complex behavior. However, in this instantiation we focus on a simplified setting, where we assume BGP route announcements to only be modified when imported into the \as from an external peer. Previous work has already pointed out that this is a reasonable assumption which holds for the majority of real-world networks \cite{caesar2005bgp,cittadini2010doing, steffen2020probabilistic}.

\begin{figure}
    \small{
    \begin{enumerate}
        \setlength{\itemsep}{0pt}
        \setlength{\parskip}{0pt}
        \item Highest Local preference
        \item Lowest AS path length
        \item Prefer Origin (IGP $>$ EBGP $>$ INCOMPLETE)
        \item Lowest Multi-exit discriminator (MED)
        \item External over internal announcements
        \item Lowest IGP cost to egress
        \item Lowest BGP peer id (tie breaker)
    \end{enumerate}}
    \vspace{-15pt}
    \caption{The BGP decision process \cite{rekhter1994border}. The shown rules are applied in order until a single best BGP announcements remains.}
    \label{fig:bgp-decision}
\end{figure}

\subsection{Dataset Generation and Training}
\label{sec:training}
To train a synthesizer model, we need a large number of fact bases encoding a variety of network topologies, configurations and forwarding specifications. Further, we must provide the model with target values for unknown parameters as a supervision signal. This section discusses how we construct such a dataset for BGP/OSPF synthesis.
%Further, we provide an example of what a corresponding fact base looks like, including a description of the supported specification language.

\paragraph{Dataset Generation} To obtain network configurations and corresponding forwarding specifications we employ a generative process: We first randomly configure BGP and OSPF parameters for some topology. Then we simulate the OSPF and BGP protocol and compute the resulting forwarding plane. Based on this, we extract a forwarding specification which fixes a random subset of forwarding paths, reachability and isolation properties that are satisfied by the forwarding plane.

\paragraph{Topologies} For training, our dataset is based on random topologies with $16$-$24$ routers. We generate the physical layout of these graphs by triangulation of uniformly sampled points in two-dimensional space.

\paragraph{Simulation} To compute the forwarding plane given an OSPF and BGP configuration, we simulate the protocols. For OSPF, we implement shortest path computation to obtain the forwarding plane. For BGP, we implement the full BGP decision process as shown in \cref{fig:bgp-decision}, except for the MED attribute. In addition to the basic networking model discussed in \cref{sec:synthesis-setting}, we implement support for eBGP and iBGP, fully-meshed BGP session layouts as well as layouts relying on route reflection. For more details of these BGP concepts see \cite{bates2000rr}.

%Note that the synthesizer model will reason on the level of the provided training samples. That is, to improve the overall synthesis quality in a real-world setting, it is helpful to implement simulation code which behaves very similar to real-world networks. Another promising approach would be to extract training samples from real-world networks, thereby circumventing the need for simulation, however, we leave this as future work.

%While this can be a considerable effort, it is typically an easier task than to implement the synthesizer directly. The concrete semantics of protocols and their simulation is a well-defined procedure, whereas implementing efficient synthesis tools is still an open problem.

\paragraph{Fact Base Encoding} We encode synthesis input using a small set of facts. For an example of a corresponding fact base see \cref{fig:bgp-ospf-fact-base}. We use the \texttt{router}, \texttt{external} and \texttt{network} facts to mark routers, external peers and routing destinations respectively. Physical links between routers are encoded as \texttt{connected(R1,R2,W)} facts where \texttt{W} denotes the OSPF link weight. Further, we rely on \texttt{ibgp}, \texttt{ebgp}, \texttt{route\_reflector} and \texttt{bgp\_route} facts to represent different types of BGP sessions and imported routes. Using the notion of unknown parameters as discussed in \cref{sec:graph-embedding}, we encode configuration parameters, e.g., properties of imported routes or OSPF link weights.

\paragraph{Specification Language} We support a small specification language with three types of forwarding predicates:

\begin{itemize}
    \setlength{\itemsep}{0pt}
    \setlength{\parskip}{2pt}
    \item \texttt{fwd(R1, Net, R2)} specifies that router \texttt{R1} forwards traffic destined for \texttt{Net} to its neighbor \texttt{R2}.
    \item \texttt{reachable(R1, Net, R2)} specifies that traffic destined for \texttt{Net} that passes through \texttt{R1} also passes through \texttt{R2} before reaching its destination.
    \item \texttt{trafficIsolation(R1, R2, N1, N2)} specifies that it must not hold that $[fwd(R1,R2,N1)]_{\mathcal{B}} \wedge [fwd(R1,R2,N2)]_{\mathcal{B}}$.
\end{itemize}

In the negative case of each predicate, the opposite must hold true for the fact to be satisfied. This specification language can easily be extended by including new specification predicates in the dataset generation process. One must simply provide a method of extracting positive and negative cases of a specification fact from a given forwarding plane. Once included in the training dataset of a synthesizer model, the resulting synthesis system will be able to consider specifications relying on the new type of predicates.

% \todo{info on loss function, optimizer, etc.}
\paragraph{Training} We generate a dataset of $10,240$ input/output samples and instantiate our synthesizer model with a hidden dimension $D$ of $64$. For optimization, we use the Adam optimizer \cite{kingma2014adam} with a learning rate of $10^{-4}$. We stop training after the specification consistency on a validation dataset no longer increases at $\sim2800$ epochs.

\begin{figure}
\begin{minipage}[t]{0.22\textwidth}
\begin{lstlisting}[basicstyle=\ttfamily\tiny]
# topology and configuration
router(c5)
router(c3)
router(c1)
router(c0)
network(c6)
network(c7)

external(c8)
external(c9)
external(c10)
external(c11)
external(c12)
external(c13)

route_reflector(c2)
route_reflector(c4)

connected(c2,c4,?)
connected(c2,c5,?)
connected(c2,c3,?)
connected(c4,c5,?)
connected(c4,c3,?)
connected(c4,c0,?)
connected(c5,c1,?)
connected(c5,c0,?)
connected(c3,c0,?)
connected(c3,c1,?)
connected(c1,c0,?)

ibgp(c2,c4)
ibgp(c2,c5)
ibgp(c2,c0)
ibgp(c2,c1)
ibgp(c4,c3)
ibgp(c4,c4)
\end{lstlisting}
\end{minipage}
\begin{minipage}[t]{0.2\textwidth}
\begin{lstlisting}[basicstyle=\ttfamily\tiny]
ebgp(c2,c12)
ebgp(c5,c9)
ebgp(c5,c10)
ebgp(c5,c13)
ebgp(c0,c8)
ebgp(c0,c11)

bgp_route(c8,c6,?,?,1,?,1,8)
bgp_route(c9,c6,?,?,0,?,1,9)
bgp_route(c10,c6,?,?,0,?,1,10)
bgp_route(c11,c7,?,?,0,?,1,11)
bgp_route(c12,c7,?,?,0,?,1,12)
bgp_route(c13,c7,?,?,2,?,1,13)

# forwarding specification
fwd(c0,c6,c3)
fwd(c3,c6,c2)
fwd(c2,c6,c4)
not fwd(c3,c6,c0)
not fwd(c0,c6,c11)
not fwd(c11,c6,c0)

not trafficIsolation(c1,c0,c7,c6)
not trafficIsolation(c1,c0,c7,c6)
trafficIsolation(c0,c3,c6,c7)
trafficIsolation(c0,c3,c6,c7)

reachable(c5,c6,c10)
reachable(c1,c6,c4)
not reachable(c0,c6,c5)
reachable(c5,c6,c10)
\end{lstlisting}
\end{minipage}
\caption{An example of a fact base encoding a topology, a sketch of a BGP and OSPF configuration and a forwarding specification.}
\label{fig:bgp-ospf-fact-base}
\end{figure} 

==> diff/git-latexdiff.33774/new/sections/4_evaluation.tex <==
\section{Evaluation}
\label{sec:evaluation}

We trained a synthesizer model to perform configuration synthesis for BGP and OSPF. We now assess the performance of the resulting neural synthesizer with respect to two core metrics: (1) the quality of synthesized configurations in terms of their consistency with the provided forwarding specifications (\cref{sec:synthesis-quality}), and (ii) the time a learned synthesizer takes when compared to the state-of-the-art SMT-based synthesizer NetComplete \cite{el2018netcomplete} (\cref{sec:synthesis-vs-smt}).

\paragraph{Dataset} We compare across three datasets: Small, Medium and Large. Each dataset represents 8 real-world topologies, sampled from the Topology Zoo \cite{knight2011internet}, where the number of nodes lies between 0-34, 34-68 and 68-170 respectively. To obtain forwarding specifications for the sampled topologies, we use our generative pipeline as discussed in \cref{sec:training}. In each topology, we do synthesis for 4 different traffic classes (routing destinations) at a time.

\paragraph{Experimental Setup} We run all our experiments on an Ubuntu Linux machine with an Intel(R)~Core(TM)~i9-9900X~@~3.50GHz processor, 64GB of system memory and an NVIDIA GeForce RTX 3080 GPU with 10GB of video~memory.

\subsection{Synthesis Quality}
\label{sec:synthesis-quality}
To assess our learned synthesizer, we examine its behavior with increasingly large topologies and specifications.

\paragraph{Specifications} Using the same generative model as described in \cref{sec:training}, we generate forwarding specifications for the topologies in our three datasets with each specification constructed from $3 \times n$ requirements, one per supported predicate type:  \texttt{fwd} requirements correspond to specifying or blocking a forwarding path using multiple \texttt{fwd} predicates whereas \texttt{reachable} and \texttt{trafficIsolation} requirements each translate to a single specification fact. We compare across increasingly large specifications of $3\times 2$, $3\times 8$ and $3 \times 16$ requirements, respectively.

\paragraph{Methodology} For each pair of topology and specification, we run our synthesizer 5 times and report the network configurations with the highest overall consistency value. For sampling, we rely on our multi-shot sampling strategy where we randomly group the unknown parameters of a configuration into 4 groups (4-shot sampling).

\paragraph{Results} We summarize our results in \cref{fig:eval-consistency}. On average, our synthesis model produces network configurations that are $>91\%$ consistent with the provided forwarding specifications across all datasets and sizes of specifications. When only few requirements are given, the synthesizer model even succeeds in producing fully-consistent configurations. We observe a slightly decreasing consistency with increasingly large topologies.

%\texttt{fwd} facts are satisfied more easily, whereas \texttt{reachable} and \texttt{trafficIsolation} facts are violated more often.

\paragraph{Multi-Shot Sampling} In \cref{fig:eval-consistency-baseline}, we report the average specification consistency using our multi-shot sampling strategy as compared to sampling all unknown parameters at once. As a baseline we have also sampled random configurations from a uniform distribution (per parameter) and compute the corresponding specification consistency. Over the baseline, our synthesizer model shows clear improvement and multi-shot sampling further increases consistency.

\begin{figure*}
    \begin{center}
        \textbf{Specification Consistency}\\
        \footnotesize
        \begin{tabular}{rrcccccccccc}
        \toprule
        \multicolumn{2}{c}{Dataset} & \tiny\texttt{fwd} & \tiny\texttt{reachable}  & \tiny\texttt{trafficIsolation} & Overall & $\emptyset$     No. Full Matches & $\emptyset$ No. $>90\%$ Matches\\
        \midrule
        $3\times 2$ requirements & Small & 0.95 & 0.94 & 1.00 & \textbf{0.95} & 0.62 & 0.62\\
& Medium & 0.96 & 1.00 & 0.94 & \textbf{0.96} & 0.88 & 0.88\\
& Large & 0.94 & 0.94 & 1.00 & \textbf{0.93} & 0.62 & 0.62\\
\midrule
$3\times 8$ requirements & Small & 0.97 & 0.98 & 0.97 & \textbf{0.98} & 0.50 & 1.00\\
& Medium & 0.99 & 0.95 & 1.00 & \textbf{0.98} & 0.50 & 1.00\\
& Large & 0.96 & 0.95 & 0.91 & \textbf{0.94} & 0.38 & 0.88\\
\midrule
$3\times 16$ requirements & Small & 0.97 & 0.89 & 0.95 & \textbf{0.94} & 0.38 & 0.75\\
& Medium & 0.98 & 0.97 & 0.97 & \textbf{0.98} & 0.38 & 1.00\\
& Large & 0.92 & 0.88 & 0.95 & \textbf{0.91} & 0.12 & 0.50\\
    \end{tabular}\end{center}
    \caption{Average specification consistency of the network configurations synthesized by our trained synthesizer model. Per sample we run the synthesizer with a specification of $3\times N$ requirements, where the specifications always include $N$ requirements per supported predicate type (\texttt{fwd}, \texttt{reachable}, \texttt{trafficIsolation}).}
    \label{fig:eval-consistency}
\end{figure*}

\begin{figure}
    \begin{center}
        \footnotesize
        \begin{tabular}{rrcccccccccc}
        &  & \multicolumn{2}{c}{Neural}\\
        & Random & 1-Shot & 4-shot\\
        \toprule
        Small & 0.83 & 0.92 & \textbf{0.94} \\
        Medium & 0.88 & 0.95 & \textbf{0.98} \\
        Large & 0.78 & 0.88 & \textbf{0.91} \\
    \end{tabular}\end{center}
    \caption{Average specification consistency with $3\times 16$ requirements when sampling configurations randomly from a uniform distribution and 1-shot/4-shot sampling using our synthesizer model.}
    \label{fig:eval-consistency-baseline}
\end{figure}

\begin{figure*}[ht]
    \footnotesize
    \begin{center}
        \textbf{BGP Synthesis Time}
        \footnotesize
        \begin{tabular}{rrccccccccc}
        \toprule
        &&\multicolumn{3}{c}{Synthesis Time (s)} & \multicolumn{2}{c}{Accuracy (Neural)} \\
        \multicolumn{2}{l}{\# Requirements} & NetComplete & Neural (CPU) & Speedup &$\emptyset$ Consistency& $\emptyset$ No. Full Matches\\
        \midrule
    2 requirements &Small & 18.073s & 0.641s & \textbf{28.2x} & 0.969 & 0.875\\
        &Medium & 60.864s & 2.748s & \textbf{22.2x} & 0.939 & 0.75\\
        &Large & 1389.485s\tiny{  7/8 TO} & 22.301s & \textbf{62.3x} & 0.989 & 0.875\\
    \midrule
    8 requirements &Small & 247.691s & 1.065s & \textbf{232.5x} & 0.96 & 0.75\\
        &Medium & $>$25m\tiny{  8/8 TO} & 3.47s & \textbf{432.2x} & 0.968 & 0.5\\
        &Large & $>$25m\tiny{  8/8 TO} & 30.961s & \textbf{48.4x} & 0.969 & 0.75\\
    \midrule
    16 requirements &Small & 1416.828s\tiny{  7/8 TO} & 2.528s & \textbf{560.5x} & 0.926 & 0.25\\
        &Medium & $>$25m\tiny{  8/8 TO} & 5.481s & \textbf{273.7x} & 0.947 & 0.25\\
        &Large & $>$25m\tiny{  8/8 TO} & 69.092s & \textbf{21.7x} & 0.959 & 0.25\\
    \end{tabular}\end{center}
    \caption{Comparing consistency and synthesis time of our method (Neural) with the SMT-based state-of-art synthesis tool NetComplete. The notation {\tiny{n/8 TO}} indicates the number of timed out synthesis runs out of 8 (25+ minutes).}
    \label{fig:evaluation-compare-bgp}
\end{figure*}

\begin{figure*}[ht]
    \begin{center}
        \footnotesize
        \textbf{OSPF Synthesis Time}\\
        \footnotesize
        \begin{tabular}{rrccccccccc}
        \toprule
        &&\multicolumn{3}{c}{Synthesis Time (s)} & \multicolumn{2}{c}{Accuracy (Neural)} \\
        \multicolumn{2}{l}{} & NetComplete & Neural (GPU) & Speedup &$\emptyset$ Consistency& $\emptyset$ No. Full Matches\\
        \midrule
    2 requirements &Small & 0.265s & 0.091s & \textbf{2.9x} & 1.000 & 1.00\\
     &Medium & 0.404s & 0.098s & \textbf{4.1x} & 1.000 & 1.00\\
     &Large & 0.944s & 0.14s & \textbf{6.7x} & 1.000 & 1.00\\
    \midrule
    8 requirements &Small & 0.876s & 0.164s & \textbf{5.3x} & 0.982 & 0.75\\
     &Medium & 1.517s & 0.103s & \textbf{14.7x} & 1.000 & 1.00\\
     &Large & 3.505s & 0.316s & \textbf{11.1x} & 0.981 & 0.50\\
    \midrule
    16 requirements &Small & 1.65s & 0.21s & \textbf{7.9x} & 0.991 & 0.625\\
     &Medium & 2.646s & 0.245s & \textbf{10.8x} & 0.989 & 0.50\\
     &Large & $>$566.636s+\tiny{  3/8 TO} & 0.233s & \textbf{2430.4x} & 0.987 & 0.875\\
    \end{tabular}\end{center}
    \caption{Comparing consistency and synthesis time of our method (Neural) with the SMT-based OSPF synthesis tool NetComplete. The notation {\tiny{n/8 TO}} indicates the number of timed out synthesis runs out of 8 (25+ minutes).}
    \label{fig:evaluation-compare-ospf}
\end{figure*}


\subsection{Comparison to SMT-based Synthesis}
\label{sec:synthesis-vs-smt}

%To provide a comparison of our learned BGP/OSPF synthesizer with SMT-based methods,
We now compare the synthesis time of the learned neural synthesizer with those of NetComplte, a state-of-art configuration synthesis tool based on SMT-solvers \cite{el2018netcomplete}.

\paragraph{Specifications} As the type of supported requirements in NetComplete does not fully align with our model, we restrict this comparison to specifications which only include forwarding paths (i.e. \texttt{fwd} predicates). Further, NetComplete does not support cross-protocol synthesis as in our case and instead requires users to specify for each requirement the protocol to use for its implementation. To bridge this gap, we split the generated forwarding requirements into BGP and OSPF paths for a corresponding NetComplete specification.
%\todo{note on NetComplete installing policies at all routers, not only the edges of the AS}

\paragraph{Methodology} We compare both OSPF synthesis and BGP/OSPF-synthesis. We configure our trained synthesizer model to do OSPF synthesis by only predicting link weights. For each pair of topology and specification, we report the total time of running our synthesizer 4 times using 4-shot sampling, whereas for consistency we report the best out of the 4 runs. For NetComplete, we run the synthesizer with a timeout of 25 minutes. In case a NetComplete attempt times out, we report 25 minutes as a lower bound for its runtime.

\paragraph{OSPF Synthesis Time Results} We document the results of comparing OSPF synthesis time in \cref{fig:evaluation-compare-ospf}. Our synthesizer model achieves a speedup of 2-10x over NetComplete. With 16 requirements and dataset Large this speedup even increases to $2000\times$. Further, our model achieves very high consistency with the provided specification, often producing fully-consistent configurations.

\paragraph{BGP/OSPF Synthesis Time Results} In \cref{fig:evaluation-compare-bgp} we show the comparison of BGP/OSPF synthesis time. Our synthesizer model outperforms NetComplete by multiple orders of magnitude. We observe a speedup of $20-560\times$ which appears to increase with the size of topology and specification. Further, the average specification consistency of the synthesized configurations is greater than $92\%$ across all datasets, even for large topologies. In many cases, our synthesizer model produces fully-consistent configurations, especially with small topologies and specifications. In comparison, NetComplete times out on more than half of the synthesis tasks which means that we can only observe a lower bound of speedup in these cases. Note that our synthesizer model is running on a CPU due to memory restrictions with large topologies. However, running it on a GPU results in even greater speedups (up to $1000\times$, cf. \cref{app:sec:bgp-gpu-performance}). 

==> diff/git-latexdiff.33774/new/sections/5_related_work.tex <==
\section{Related Work}
\label{sec:related-work}

\paragraph{Traditional Configuration Synthesis} 
%A range of existing work is concerned with network configuration synthesis. 
Next to methods based on compilation such as Propane/PropaneAT \cite{beckett2017network}, there are a number of configuration synthesis methods based on constraint solving: Examples include ConfigAssure \cite{narain2008declarative}, SyNet \cite{el2017network} and NetComplete \cite{el2018netcomplete}. Due to their hand-coded nature, these methods are highly protocol-specific and can be very slow due to the solvers they employ. Although some of them allow for cross-protocol reasoning, this is not implemented as transparently as in our framework and users must specify per requirement which protocol to use for its implementation. In contrast, our approach has lower precision but allows for fully transparent cross-protocol reasoning, meaning forwarding requirements are not protocol-bound and the synthesizer chooses how to implement them. Further, our learned BGP/OSPF synthesis tool exhibits much lower synthesis times as compared to an SMT-based tool like NetComplete.

% \begin{itemize}
%     \item NetComplete, SyNet
%     \item Propane, PropaneAT
%     \item DeepBGP
% \end{itemize}

\paragraph{GNNs and Networking} DeepBGP \cite{bahnasy2020deepbgp} relies on GNNs and reinforcement learning to do configuration synthesis. However, it is limited to BGP configuration synthesis and is slower than SMT-based synthesis according to the author's evaluation. In contrast, our learning-based framework is cross-protocol, does not rely on reinforcement learning and provides better synthesis performance. Apart from configuration synthesis, GNNs have also been applied to other problems in the networking domain. For example, the authors of RouteNet \cite{rusek2020routenet} use GNNs to predict performance metrics of network configurations. Other work that is concerned with learning improved protocols includes Q-Routing \cite{boyan1994packet} or more modern approaches such as the Graph-Query Neural Network architecture \cite{geyer2018learning}.

\paragraph{Neural Algorithmic Reasoning} 
Neural algorithmic reasoning (NAR) as proposed in \cite{velivckovic2021neural}, describes the idea of replacing traditional algorithms with neural networks to learn improved algorithmic procedures. Exemplary work includes graph-related algorithms \cite{velivckovic2019neural} or solvers for combinatorial optimization problems \cite{cappart2021combinatorial,joshi2020learning,selsam2019guiding}. Our synthesis framework is the first applications of NAR to the networking domain and relies on the NAR-native encode-process-decode architecture. According to the hierarchy of NAR approaches in \cite{cappart2021combinatorial}, our method is an algorithm-level approach, as we do not supervise on intermediate steps. Although, such step-level methods promise better generalization, it is not clear what an intermediate result of a general synthesis procedure would be. However, future work on a step-level approach may further improve synthesis quality.

% \begin{itemize}
%     \item RouteNet
%     \item GraphNET
%     \item Learning and generating distributed routing protocols using graph-based deep learning
%     \item Unveiling the potential of Graph Neural Networks for network modeling and optimization in SDN
% \end{itemize}

==> diff/git-latexdiff.33774/new/sections/6_conclusion.tex <==
\setlength{\parskip}{6pt plus4mm minus4mm}
\section{Conclusion}
\label{sec:conclusion}
We presented a learning-based framework for configuration synthesis based on the idea of neural algorithmic reasoning. To assess the effectiveness of the system, we instantiated it for the case of BGP/OSPF synthesis. In contrast to traditional synthesis methods, our system supports transparent cross-protocol reasoning and learns synthesis rules only from data. Using our system, synthesis is sped up by a factor of up to $500\times$ when compared to SMT-based methods. Further, our evaluation demonstrates that the resulting synthesis tool provides excellent synthesis quality, producing configurations with high specification consistency. Overall, our results illustrate that exploring the direction of learning-based network configuration synthesis is a promising direction, enabling new cross-protocol reasoning capabilities and great performance improvements. Promising future work includes construction of hybrid systems, integrating both neural models and SMT-based approaches to obtain the best of both worlds.

==> diff/git-latexdiff.33774/old/acronyms.tex <==
\DeclareAcronym{AS}{
    short = AS,
    long = autonomous system,
    short-plural = es ,
    long-plural = s
}

==> diff/git-latexdiff.33774/old/sections/0_abstract.tex <==
% Context
Computer networks employ a number of different protocols to enable efficient routing. However, due to the complexity of multiple interacting protocols, it can be hard for network operators to implement high-level routing policies and requirements. Network configuration synthesis promises to address this situation by automatically generating configurations that satisfy a provided specification. However, existing synthesis methods are often limited to single-protocol reasoning, depend on protocol-specific and hand-coded synthesis rules, and are difficult to scale due to the SMT-based methods they employ. In this work we present a rather different, learning-based method for addressing the configuration synthesis challenge, one based on the recently proposed paradigm of neural algorithmic reasoning. Our framework is protocol-agnostic, enables cross-protocol reasoning and does not depend on any hardcoded synthesis rules. To evaluate, we instantiate our framework for the case of BGP/OSPF synthesis. Our experiments show we can synthesize configurations with a very high degree of specification consistency while observing speedups of up to $500\times$ compared to a state-of-the-art SMT-based synthesis tool.


==> diff/git-latexdiff.33774/old/sections/1_intro.tex <==
\section{Introduction}
\label{sec:introduction}

The backbone of the internet consists of many connected computer networks operated by different internet service providers (ISPs) and other large organizations. These networks rely on a number of protocols to enable effective and policy-driven routing of traffic. Based on router-level configurations, the protocols perform a distributed computation to construct a network's forwarding state. However, the relatively low-level router configuration makes it hard for network operators to directly enforce network-wide policies and requirements. This often leads to misconfiguration, which can cause global outages such as the recent hours-long blackout of the entire Facebook platform \cite{janardhan2021} and comparable events \cite{mccarthy_2019}.
%
\paragraph{Configuration Synthesis} This situation has triggered a number of research efforts regarding the synthesis of network configurations \cite{el2018netcomplete,beckett2017network,narain2008declarative}. Configuration synthesis is concerned with the task of automatically generating router-level configurations given a set of high-level requirements. However, this synthesis problem can be very hard to solve, since network configurations typically consist of a considerable number of tunable parameters, where the execution of several interacting protocols yields the overall forwarding state. An effective synthesis tool must thus account for this fact and be able to reason across multiple protocols.

\paragraph{SMT-based Synthesis} Some of the most successful efforts in providing cross-protocol synthesis capabilities are based on satisfiability modulo theory (SMT) solvers \cite{el2018netcomplete,el2017network}. While SMT-based synthesis is a promising method, it comes with a number of limitations:
% \item protocol-specific
% fully hand-coded synthesis rules, a lot of implementation effort, cross-protocol support extra complicated
(1) SMT-based synthesizers are hand-crafted and highly protocol-specific. To implement synthesis, we must first express our networking model, protocol semantics including vendor and device specific behavior in terms of first-order logic constraints. This is a time-intensive and complicated process, requiring lots of expert knowledge.
%  model-dependent: synthesis is reasoning on the level of some assumed model which may not reflect the real world: even if a configuration is synthesized based on some spec, it may behave differently and violate spec in practice
Further, (2) logic-based modelling introduces a disconnect between the synthesis tool and real-world behavior \cite{birkner2021metha}. More specifically, synthesized configurations may satisfy a provided specification within a formal framework, but may not behave the same way in the real world.
% can be very slow
And, (3) SMT-based synthesis can be very slow or fail to complete, especially when reasoning about large network topologies. In practice however, network operators reconfigure their networks on a daily basis \cite{vissicchio2012improving}, which means an effective synthesis tool must be fast.

% \item fully learned, no hand-coded synthesis rules (model-free), very flexible to adapt to more/new protocols
% \item protocol-agnostic, cross-protocol
\paragraph{Neural Algorithmic Reasoning for Synthesis} Recent work on neural algorithmic reasoning (NAR) proposes to replace traditional algorithms with neural networks to learn improved algorithmic procedures \cite{velivckovic2021neural}.
It has been shown to be a powerful and fast algorithmic approximation method for a number of graph-related \cite{velivckovic2019neural} and combinatorial optimization problems \cite{cappart2021combinatorial}. Further, due to its learned nature, NAR allows for learning procedures directly from (real-world) data, without the need for manual feature extraction. Overall, this positions NAR as an attractive method to obtain a fast, fully-learned synthesis procedure, which entirely avoids the need for a formal model or any hand-crafted synthesis rules. Based on this promising outlook, this paper explores how to apply NAR to the problem of network configuration synthesis.

We propose a \textbf{new learning-based framework for configuration synthesis} as an alternative to SMT-based approaches. Our framework is protocol-agnostic, enables cross-protocol reasoning and avoids the need to manually provide synthesis rules. Instead of implementing the synthesizer explicitly, we replace it by an iterative graph neural network which is trained on input/output samples of specifications, topologies and configurations.
%While our approach still requires some protocol-specific implementation efforts, it is limited to implementing the simulation of the involved protocols.
Our method is highly flexible due to its generic nature and can be extended to any protocol. Further, the synthesizer model learns a whole distribution of network configurations. As a consequence, we can even sample multiple alternative configurations, which is not possible with standard SMT solvers. We apply our framework to a synthesis setting where both the Border Gateway Protocol (BGP) and the Open Shortest Path First (OSPF) protocol are used. Our learned synthesis tool is up to~$500\times$ faster than a state-of-the-art SMT-based synthesizer, while producing configurations which satisfy more than 90\% of the provided specification.

\paragraph{Contributions} Our core contributions are:
\vspace{-5pt}
\begin{itemize}
    \setlength{\itemsep}{5pt}
    \setlength{\parskip}{0pt}
    \item A learning-based framework for network configuration synthesis based on neural algorithmic reasoning.
    \item A neural network architecture for learning synthesizer models which relies on a generic graph-based encoding of network topologies and configurations.
    \item An evaluation of synthesis quality and time when instantiating our framework for BGP/OSPF.
\end{itemize}

\section{Overview}
\label{sec:overview}

\begin{figure}
    \begin{center}
        \includegraphics[width=0.45\textwidth]{figures/synthesizer-overview.pdf}
    \end{center}
    \caption{An overview of our learning-based synthesis framework.}
    \label{fig:learning-based-synthesis}
\end{figure}

We first discuss the core concepts of our learning-based synthesis framework. This includes a number of steps as illustrated in \cref{fig:learning-based-synthesis}.

\paragraph{Dataset} To train a synthesizer model, we first generate a dataset of input/output samples. For this, we rely on a generative pipeline as shown in the top of \cref{fig:learning-based-synthesis}. First, we sample a random network configuration for some topology using a uniform generative process. Then, we simulate the involved protocols to obtain the corresponding routing behavior. Next, we extract a specification by randomly selecting properties that hold for the simulated routing behavior. This leaves us with a pair of specification and network configuration which can be added to a dataset of training~samples.

\paragraph{Simulation} Depending on the protocols in use, one implements simulation code to compute the routing behavior based on a randomly sampled configuration. Although this step of our approach is protocol-specific, the overall implementation effort is much lower compared to SMT-based synthesis. Protocols are typically well-defined algorithms which can be simulated, whereas the the alternative of implementing a synthesizer directly often requires expert knowledge about SMT solvers. In practice, our framework may also be adapted to use a real-world network to compute the routing behavior of a configuration, thereby learning the synthesis procedure directly from real-world behavior.

% \paragraph{Extracting Specifications} To extract a specification, we randomly sample properties, given some concrete routing behavior. According to our experiments, this simple strategy suffices to obtain a diverse dataset of specifications and configurations.

\paragraph{Model} We train a graph neural network to perform synthesis. According to the idea of NAR, we first encode the synthesizer input in latent space. Then, we apply an iterative processor network which relies on the graph attention mechanism to propagate information \cite{velivckovic2017graph}. Last, we apply a decoder network to extract the synthesized network configuration. To remain protocol-agnostic, our model is generic with respect to the input format, using an intermediate representation based on Datalog-like facts.

%More specifically, we employ a slightly modified variant which operates on a graph-based encoding of a specification, topology and configuration parameters.

\paragraph{Relaxed Specification Consistency} Parts of the configuration synthesis problems are known to be NP-hard \cite{fortz2000internet}. In contrast, our learning-based framework depends on a fixed-size neural network architecture running in polynomial time. Hence, we expect neural synthesis to be less precise than SMT methods and propose the notion of \emph{relaxed~specification~consistency}: To assess the performance of a neural synthesis tool, we do not only consider a configuration to either satisfy a specification or not. Instead, we measure the degree up to which a synthesized configuration satisfies a specification, e.g. via the relative number of satisfied requirements. This "soft" understanding of a specification allows us to evaluate neural synthesis systems which may not always produce fully specification-consistent configurations. Nonetheless, we argue that configurations with less than $100\%$ consistency are still very useful in practice, as they provide a good starting point for further manual tweaking by network operators. A similar tweaking process may also be required with SMT solutions, due to differences between the formal model and real-world behavior.

\paragraph{Outline} In this paper, we first discuss the architecture of our synthesizer model in \cref{sec:model}. Based on this, we demonstrate how to instantiate our framework for the case of BGP/OSPF configuration synthesis in \cref{sec:bgp-ospf}. Further, we evaluate the resulting synthesis tool in \cref{sec:evaluation} and compare it to a comparable SMT-based tool. Last, \cref{sec:conclusion} concludes this paper.

% \begin{itemize}
%     \item effort: need to implement simulation code to generate dataset to learn from (typically well-defined in protocol specs, much easier than implementing synthesis directly)
%     \item can be sampled (multiple alternative solutions, not easily possible with SMT-based methods)
%     \item much faster than SMT-based synthesis
% \end{itemize}

% Requirements:
% \begin{itemize}
%     \item protocol-agnostic
%     \item fully learned, no hand-coded synthesis rules
%     \item define: strict specification vs. relaxed specification
% \end{itemize} 

==> diff/git-latexdiff.33774/old/sections/2_model.tex <==
\section{Model}
\label{sec:model}

 \begin{figure*}
     \centering
     \includegraphics[width=0.85\textwidth]{figures/system-overview.pdf}
     \caption{An overview of our synthesis system: (1) First, we use a generic embedding scheme to transform a network topology, protocol configuration sketches and the specification given as Datalog-like facts to a latent input representation. Next, we apply a learned (2) Processor GNN and obtain a latent synthesis output. Last, we apply a (3) Decoder Network to obtain a distribution over possible values per unknown parameter in our configuration.} 
     \label{fig:overview-model}
\end{figure*}

This section presents the architecture of our graph-based synthesizer model. 
An overview of the system is given in \cref{fig:overview-model}. 
\cref{sec:graph-embedding} introduces the generic graph-based encoding, which allows us to embed network topologies, protocol configuration and the specification into latent space. \cref{sec:graph-transformer}~overviews the architecture of the processor network which we train to perform the synthesis task. Last, \cref{sec:decoding-sampling} outlines how we sample network configurations from the resulting latent synthesis output.

\begin{figure}
    \begin{minipage}[t]{0.21\textwidth}
    \begin{lstlisting}[basicstyle=\ttfamily\small, escapeinside={(*}{*)}]
router(A)
router(B)
(...)

connected(A,B,2)
connected(A,C,?)(*\blackcircled{1}*)
(...)
    \end{lstlisting}
\end{minipage}
\begin{minipage}[t]{0.21\textwidth}
    \begin{lstlisting}[basicstyle=\ttfamily\small, escapeinside={(*}{*)}]
network(N1)
bgp_route(E,N1,2,3,1,0,1)

fwd(A,B,N1)
not fwd(B,A,N1)
(...)
    \end{lstlisting}
\end{minipage}
    \caption{A snippet of a fact base sketch encoding a network's topology, parameters such as link weights (\texttt{connected} facts) and a specification (\texttt{fwd} facts).}
    \label{fig:datalog-encoding}
\end{figure}

\begin{figure}[t]
    \centering
    \includegraphics[width=0.25\textwidth]{figures/synth-architecture.png}
    \caption{The synthesizer model architecture.}
    \label{fig:architecture}
\end{figure}

\subsection{Fact Base Embedding}
\label{sec:graph-embedding}
To remain protocol-agnostic in our model architecture, we implement a generic graph-based encoding of Datalog-like facts, similar to knowledge graphs \cite{rosso2020beyond}. This means, we first encode topologies, configurations and specifications as a set of Datalog-like facts and then employ a generic embedding. 
%We chose Datalog facts as the input format of our synthesis approach for its flexibility, wide-spread use in Program Analysis and use in previous work on configuration synthesis \cite{el2017network}.

\paragraph{Fact Base} A set of Datalog-like facts as depicted in \cref{fig:datalog-encoding} serves as the input \emph{fact base} $\mathcal{F}$ to our synthesizer model. $\mathcal{F}$ is a set of facts $f(a_0, \dots, a_n)$ where arguments may be constants (e.g. A or B) or integer literals. Further, each fact in a fact base has a corresponding truth value denoted as $[f(a)]_{\mathcal{B}}$. For instance, from the fact base in \cref{fig:datalog-encoding} we can derive $[fwd(A,B,N1)]_{\mathcal{B}} = \text{\texttt{true}}$ and $[fwd(B,A,N1)]_{\mathcal{B}} = \text{\texttt{false}}$.

\paragraph{Consistency} We represent a network's topology, the protocol configuration and parameters as well as the specification, all in a single fact base. Given the semantics of the protocols in use, we can then check whether the specification encoded in a fact base is satisfied by the provided configuration. To quantify, we define the notion of relaxed specification consistency, as initially discussed, with respect to a fact base: Given a fact base $\mathcal{F}$, a subset of specification facts $S \subset \mathcal{F}$ and protocol semantics $\mathcal{P}$, the \emph{consistency} of a fact base is defined as the relative number of satisfied facts in $S$ with respect to the routing behavior obtained via $\mathcal{P}$. The contents of $S$ depends on the concrete instantiation of the synthesizer model. For an example of possible specification facts, see our instantiation of the synthesizer model for BGP/OSPF in \cref{sec:training}.

\begin{figure*}
    \def\arraystretch{1.5}
    \begin{tabular}{lr}
        %$T_f: T_1 \times \dots \times T_n$ & \textit{(fact type declaration)}\\
        $emb(f) := \mathbf{V_f}$ & \textit{(learned fact type embedding)}\\
        $emb(b) := \mathbf{W_{\text{bool}}}\;onehot(b)$ & \textit{(learned boolean embedding)}\\
        $emb(f,i,v) := \mathbf{W_{f_i}}\;onehot(v)$ & \textit{(learned integer embedding)}\\
        $emb(f,i,?) := \mathbf{V_{hole}}$ & \textit{(learned hole embedding)}\vspace{10pt}\\
        $\mathlarger{
        h_c := \sum_{f(c) \in \mathcal{F}}
        emb(f)
        }$ & \textit{(constant embedding)}\vspace{10pt}\\
        $h_{f(a_0, \dots, a_n)} := emb(f) + emb([f(a_0, \dots, a_n)]_{\mathcal{B}}) + \mathlarger{
        \sum_{(i,v) \in \mathcal{I}(f(a_0, \dots, a_n))} 
        emb(f, i, v)
        }$\hspace{-1.2cm} & \textit{(fact embedding)}\\
        $\mathcal{I}(f(a_0, \dots, a_n)) := \{(i,v) \; | \; f(a_0, \dots, a_{i-1}, v, \dots, a_n) \in \mathcal{F} \wedge v:Int \wedge i \in \mathbb{N}$ \}& \textit{(integer arguments)}\vspace{10pt}\\
        $N_i(h_c) := \{h_f \; | \; \exists i \in \mathbb{N} . f(a_0, \dots, a_{i-1}, c, a_{i+1}, \dots, a_n) \in \mathcal{F}\}$& \textit{(i-th neighborhood of constant node)} \\
        $N_i(h_f) := \{h_c \; | \; \exists i \in \mathbb{N} . f(a_0, \dots, a_{i-1}, c, a_{i+1}, \dots, a_n) \in \mathcal{F}\}$& \textit{(i-th neighborhood of fact node)} \\
    \end{tabular}
    \caption{Translating a fact base $\mathcal{F}$ to node features. $f$ denotes a predicate, $v$ integer values, $b$ boolean values as 0 or 1, $i$ argument indices and $[f(a)]_{\mathcal{B}}$ the truth value of a fact. }
    \label{fig:graph-embedding}
\end{figure*}

%discuss embedding as shown in \cref{fig:datalog-encoding}. Note how this makes fact bases a suitable input to standard GNN architectures.

\paragraph{Fact Base Sketching} In a synthesis setting, we are confronted with incomplete fact bases, i.e. the specification and topology is given but the network configuration is to be synthesized. For these cases, we also consider fact bases with unknown parameters inspired by the idea of program sketching in program synthesis \cite{solar2008program}. More specifically, users may replace an unknown integer argument of a fact by a \texttt{?} symbol, indicating a value to be synthesized. Using this mechanic, we can represent the synthesis input as an incomplete fact base which encodes to-be-synthesized values as unknown parameters. As an example, consider \cref{fig:datalog-encoding} \blackcircled{1}, where the link weight between router nodes \texttt{A} and \texttt{C} is represented as an unknown parameter.

\paragraph{Embedding} We employ a structurally-defined embedding scheme to transform a fact base into a graph with node features as required for processing with graph neural networks. Given a fact base $\mathcal{F}$, we apply the rules in \cref{fig:graph-embedding} to obtain node features and adjacency information. Both a fact $f$ and a constant $c$ are represented as distinct nodes with features $h_c$ and $h_f$ respectively. The relationships between facts and constants is encoded as node adjacency as defined by the neighborhood functions $N_i$. 

We use multiple neighborhood functions, i.e. multiple types of edges, to encode the argument position of a constant occurring in a fact. Hence, the number of neighborhood functions corresponds to the maximum number of arguments in a single fact, e.g. 3 in \cref{fig:datalog-encoding}. Integer arguments and unary facts are directly accounted for in the respective node or fact embedding. To handle unknown parameters, we replace the corresponding $emb(...)$ term with the learned $\mathbf{V_{hole}}$ embedding.

Considering the embedding function $emb$, the learned parameters of our embedding are $\mathbf{V_f} \in \mathbb{R}^D$ per fact type in~$\mathcal{F}$, $\mathbf{W_{\text{bool}}} \in \mathbb{R}^{D \times 2}$ for boolean values, $\mathbf{W_{f_i}} \in \mathbb{R}^{D \times N}$ per integer argument of fact type $f$ and $\mathbf{V_{hole}} \in \mathbb{R}^D$ to represent unknown parameters. Hyperparameter $D$ represents the dimension of the latent space the synthesizer model operates in and $N$ specifies the number of supported integer values. An example of applying this embedding scheme to a simple fact base is given in \cref{fig:graph-encoding-example}.

\begin{figure}
    \begin{minipage}[t]{0.2\textwidth}
        \centering
        \footnotesize
        \textbf{Fact Base}
        \begin{lstlisting}[basicstyle=\ttfamily\small]
router(A)
router(B)

conn(A, B, 12)
        \end{lstlisting}
    \end{minipage}
    \begin{minipage}[t]{0.15\textwidth}
        \centering
        \textbf{Graph}\\
        \vspace{5pt}
        \includegraphics[width=0.7\textwidth]{figures/graph-encoding.pdf}
    \end{minipage}\\
    \centering\\
    \vspace{10pt}
    \textbf{Node Features}\\
    \vspace{10pt}
    \begin{minipage}[t]{0.5\textwidth}
        $\begin{array}{rcl}
        h_A &:=& emb(router) = \mathbf{V_{\text{router}}}\\
        h_B &:=& emb(router) = \mathbf{V_{\text{router}}}\\
        h_{\text{conn(A,B,12)}} &:=& emb(conn) + emb(conn, 2, 12)\\
        &:=& \mathbf{V_{\text{conn}}} + \mathbf{W_{conn_2}} onehot(12)
    \end{array}$
    \end{minipage}
    \caption{An example of embedding a simple fact base using the embedding scheme of \cref{fig:graph-embedding}. The shown graph illustrates the neighborhoods $N_0$ and $N_1$ induced by the \texttt{conn} fact.}
    \label{fig:graph-encoding-example}
\end{figure}

\begin{figure}
    $$
    \begin{array}{rcl}
    z_j &:=& h_j + Drop(\mathlarger{\sum_{N_i}} h'_{GAT_i})\\
    h'_j &:=& FFN(Norm(z_j))\vspace{11pt}\\
    FFN(x_j) &:=& Norm(Lin2(Drop(Lin1(x_j)))))
    \end{array}
    $$
    \caption{
        The recurrence relation of a node $j$'s representation $h_j$. $h'_{GAT_i}$ represents the output of a graph attention layer operating with neighborhood $N_i$ according to \cite{velivckovic2017graph}, $h_j$ the representation of node $j$ at the previous step. $Norm$ refers to batch normalization \cite{ioffe2015batch}, $Drop$ to dropout regularization \cite{hinton2012improving} and $Lin1$ and $Lin2$ to linear layers with an inner dimension of $4N$.
    }
    \label{fig:recurrence}
\end{figure}

\subsection{Synthesizer Model}
\label{sec:graph-transformer}

For an illustration of the synthesizer model's architecture, please see Figure~\ref{fig:architecture}. Given a fact base $\mathcal{F}$ we first apply our embedding scheme as described in \cref{sec:graph-embedding}. We then employ a 2-layer GNN-based encoder network to produce the latent representation of a synthesis input. 
Given this representation, a processors network is trained to perform the actual synthesis task in high-dimensional space. Last, we apply a set of decoder networks, to obtain the synthesized values of unknown parameter, given the latent synthesis~output.

%In this context, the synthesis problem for network configurations corresponds to completing partially provided fact bases.

% \paragraph{High-Level Architecture}  

% We employ the high-level architecture to obtain the latent synthesis output $y_\mathcal{F}$:
% $$
% \begin{array}{rcl}
%     \mathbf{x_{\mathcal{F}}} &:=& Encoder(Embedding(\mathcal{F}))\\
%     \mathbf{y_{\mathcal{F}}} &:=& Processor(\mathbf{x_{\mathcal{F}}} + \mathbf{z})\\
%     z_i &\sim& \mathcal{N}(0,1)
% \end{array}
% $$
% \todo{z is only added for $i<N/2$}

% $Embedding$ corresponds to the graph-based embedding as discussed in \cref{sec:graph-embedding} and $Encoder$ is a 2-layer graph attention module. $Processor$ 

\paragraph{Encoding} The encoder GNN operates on the embedded representation of a fact base. It produces the high-dimensional representation of a synthesis input as required for the processor network. We additionally apply noise to the first half of the units of the latent representation via $\mathbf{z}$, as a source of non-determinism. According to our experiments this improves model performance and we hypothesize this is due to the synthesis problem having more than one solution in most cases.

\paragraph{Processor} The processor network is modelled as an iterative process. For this, we apply the same 6-layer graph attention module for a total of 4 iterations.
In the framework of neural algorithmic reasoning, this iterative computational structure encodes an inductive bias towards an iterative solution to the synthesis problem. Because of this bias, our processor network essentially learns an algorithmic procedure which iteratively synthesizes the values of unknown parameters in a fact base.

\paragraph{Graph Attention Layer} In the GNNs we employ, we rely on a composed variant of the graph attention layer as introduced by \cite{velivckovic2017graph}. We employ multiple graph attention layers in lockstep, one per neighborhood $N_i$ defined by our graph embedding (cf. \cref{sec:graph-embedding}), and combine the intermediate results after each step. More specifically, the recurrence relation of a node $j$'s representation $h_j$ is defined as shown in \cref{fig:recurrence}. These mechanics of combining the results of the different graph attention layers $h'_{GAT_i}$, directly corresponds to how multiple attention heads are combined in the original Transformer architecture \cite{vaswani2017attention}.

\paragraph{Argument Decoder Networks} To synthesize the value of unknown parameters, the model maintains a set of decoder networks. That is, it provides one decoder network per integer argument per fact type in a fact base. When decoding, the network is applied to the latent synthesis output of the corresponding fact node. For example, a synthesizer model which operates on the fact base in \cref{fig:graph-encoding-example}, would provide a decoder network $D_{\text{conn}_2}: \mathbb{R}^D \rightarrow \mathbb{R^N}$ to decode values for the third argument of a \texttt{conn} fact. In our experiments, decoder networks are implemented as simple multi-layer perceptron models.

%The synthesizer model learns a conditional distribution of fact bases which are consistent with respect to the protocols' semantics. 

%\todo{introduce synthesis as a completion problem of an encoded fact base (a la BERT). Introduce masking, introduce decoding of integer and truth values. Synthesis is learning a conditional distribution of consistent fact bases.}

%Using this method, we obtain the node features $h_c$ per constant, $h_f$ per fact and adjacency information in terms of node neighborhood functions $N_i(h_c)$ and $N_i(h_f)$. Overall, this encoding makes a fact base suitable for processing using standard graph neural networks. 

%- Brief description of the Graph Transformer Model
\subsection{Multi-Shot Sampling}
\label{sec:decoding-sampling}

%Multi-Stage Parameter Sampling (sampling methods: topk, high-temp, low-temp)
To sample concrete values from the output distributions over unknown parameters, we apply a multi-shot sampling strategy. More specifically, we sample values only for a subset of unknown parameters, insert them in our input fact base and run the synthesis model again. We repeat this process until no more unknown parameters remain. This multi-shot sampling strategy allows the model to incorporate the concrete values of previously synthesized parameters in its computation. In our evaluation in \cref{sec:evaluation}, we include a comparison of how this compares to sampling all unknown parameters at once.

%In a fact base with multiple holes, we apply the corresponding decoder networks to obtain a value distribution for each integer hole. However, instead of sampling all integer holes in one 


==> diff/git-latexdiff.33774/old/sections/3_bgp_ospf.tex <==
\section{BGP/OSPF Synthesis}
\label{sec:bgp-ospf}

\newcommand{\as}{\ac{AS}~}
\newcommand{\ases}{\acp{AS}~}

\newcommand{\squareann}{{\tiny$\blacksquare\;$}}
\newcommand{\triangleann}{{\small$\blacktriangle\;$}}

\begin{figure*}
    \centering
    \includegraphics[width=0.95\textwidth]{figures/networks-all.pdf}
    \caption{(a) An illustration of a small AS network, including internal peers (blue), external peers (purple), BGP sessions as well as physical links. (b) The propagation of two BGP announcement across the network. (c) The resulting forwarding plane after applying BGP and OSPF.}
    \label{fig:network-fwd-tree}
\end{figure*}

This section discusses how we instantiate our learning-based synthesis framework for the case of the BGP and OSPF protocol. \cref{sec:synthesis-setting} first introduces a basic networking model, the BGP and OSPF protocol as well as the synthesis setting. Given this model, \cref{sec:training} describes how to generate a corresponding dataset of input/output samples and train a synthesizer model.
%This shall serve as a prerequisite to the instantiation of our learning-based synthesis framework for the BGP and OSPF protocol in \cref{sec:training}.

\subsection{Synthesis Setting}
\label{sec:synthesis-setting}

\paragraph{Graphical Model} We assume an abstract network model which can be represented as an undirected graph as shown in \cref{fig:network-fwd-tree} (a). We always consider a set of internal routers (A, B, C, D in \cref{fig:network-fwd-tree}) as well as a set of adjacent external routers (E, F  in \cref{fig:network-fwd-tree}). The group of internal routers forms the \emph{\as} under consideration whereas external routers belong to other adjacent \ases. In practice, an \as represents an administrative domain controlled by a single operator.

\paragraph{Forwarding Plane} We focus on the \emph{forwarding plane} of a network. This means we are interested in how a router forwards packets given incoming traffic of different traffic classes. For this, each router maintains a routing table which determines which of its outgoing edges is used to forward packets of a certain traffic class. As an example, consider \cref{fig:network-fwd-tree} (c) which illustrates the forwarding plane of some traffic class reachable via external peer $E$ or $F$ in our example network. Each router of the network forwards traffic along some of its outgoing links. In practice, a number of protocols are used to populate a router's routing tables. For the instantiation of our synthesis framework however, we focus on OSPF and BGP.

\paragraph{OSPF} The OSPF protocol \cite{moy1994ospf} is a link-state protocol which is typically used as a interior gateway protocol~(IGP), i.e. it is used to route traffic within an \ac{AS}. Given link weights per physical link in the network, the OSPF protocol simply routes traffic along the shortest path towards the destination.

\paragraph{BGP} The BGP protocol \cite{rekhter1994border} on the other hand, is a path-vector protocol which is used to exchange reachability information mostly on the level \acp{AS}. 
%These are groups of routers typically operated by a single party (e.g. an ISP). 
When using BGP, a routing destination announces its existence to other \ases and routers, by sending out a BGP announcement. Receivers of such announcements may then choose to pass them on to other \acp{AS}, redistribute them internally and/or modify them. Instead of communicating along physical links directly, the BGP protocol requires manually configured BGP sessions among routers of the \as and external peers, as indicated by the BGP session edges in \cref{fig:network-fwd-tree}(a). 
%\todo{more discussion of eBGP vs iBGP and support for route reflection (more of an implementation detail, maybe only mention in dataset generation where simulation code is discussed)}.

%\paragraph{BGP Decision Procedure}~
%\todo{discuss decision procedure}
In case a router receives more than one announcement for a destination, a designated BGP decision process is applied to determine a single best route. \cref{fig:bgp-decision} shows the ordered list of comparison criteria of this decision process. The different criteria depend different properties of a route announcements, including the IGP cost towards the routing destination. As a consequence, when used together, OSPF as IGP protocol and BGP will interact. %Note also that BGP is an iterative process which needs multiple rounds of propagation to converge.

\paragraph{Example}
%\todo{run through simple BGP+OSPF example of computing the forwarding plane} 
To better understand BGP/OSPF routing, consider the simple example given in \cref{fig:network-fwd-tree} (b). Here, our example \as imports BGP announcements \squareann and \triangleann from E and F respectively. Both represent a route to the same destination. As shown, both announcements have a so-called local preference of 2. For simplicity, we ignore other properties such as the AS path length, Origin and MED in this example. The announcements are propagated among BGP neighbors and the best route is selected according to the decision procedure in \cref{fig:bgp-decision}. See \cref{fig:network-fwd-tree} (b) for an illustration of the intermediate states of this propagation process. As both announcements have a local preference of 2, rule 1 of the decision process is not used. Instead, in round 2, node B selects \squareann over \triangleann due to a lower IGP cost of 2 via egress node A as compared to 3 via egress node D (rule 6). Node D selects \triangleann over \squareann, since it learns this route directly from an external peer (rule 5). After Round 3, the BGP propagation process converges to a stable state and we can derive the forwarding plane as shown in \cref{fig:network-fwd-tree} (c). 


%, as well as external peers E and F which belong to other \acp{AS}. External peers are routers which are connected via eBGP sessions to routers of the \ac{AS} under consideration. They announce BGP routes to their neighbors, which are propagated within the network

\paragraph{Problem Statement} We phrase the BGP/OSPF configuration synthesis problem on the level of the forwarding plane. This means that users provide a specification which constraints the set of allowed forwarding planes. This includes predicates which enforce forwarding paths, block forwarding paths or assert higher-level properties like traffic isolation and reachability. Given such a specification, we consider network configuration synthesis as the task of configuring OSPF and BGP in a way that produces a forwarding plane which satisfies the provided specification.

\paragraph{Search Space} To limit the space of candidate configurations, we define the set of synthesized parameters: For OSPF we synthesize link weights as explored in a wide range of existing work (e.g. \cite{el2018netcomplete,fortz2000internet}. BGP parameters on the other hand are not defined as clearly: Depending on the requirements of a network operator, one may employ custom BGP import and export policies at every router of a network to implement complex behavior. However, in this work we focus on a simplified setting, where we assume BGP route announcements to only be modified when imported into the \as from an external peer. Previous work has already pointed out, that this is a reasonable assumption which holds for a majority of real-world networks \cite{caesar2005bgp,cittadini2010doing, steffen2020probabilistic}. 

\begin{figure}
    \small{
    \begin{enumerate}
        \setlength{\itemsep}{0pt}
        \setlength{\parskip}{0pt}
        \item Highest Local preference
        \item Lowest AS path length
        \item Prefer Origin (IGP $>$ EBGP $>$ INCOMPLETE)
        \item Lowest Multi-exit discriminator (MED)
        \item External over internal announcements
        \item Lowest IGP cost to egress
        \item Lowest BGP peer id (tie breaker)
    \end{enumerate}}
    \vspace{-15pt}
    \caption{The BGP decision process \cite{rekhter1994border}. The shown rules are applied in order until a single best BGP announcements remains.}
    \label{fig:bgp-decision}
\end{figure}

\subsection{Dataset Generation and Training}
\label{sec:training}
To train a synthesizer model, we need a large number of fact bases encoding a variety of network topologies, configurations and forwarding specifications. Further, we must provide the model with target values for unknown parameters as a supervision signal. This section discusses how we construct such a dataset for BGP/OSPF synthesis. 
%Further, we provide an example of what a corresponding fact base looks like, including a description of the supported specification language.

\paragraph{Dataset Generation} To obtain network configurations and corresponding forwarding specifications we employ a generative process: We first randomly configure BGP and OSPF parameters for some topology. Then we simulate the OSPF and BGP protocol and compute the resulting forwarding plane. Based on this, we extract a forwarding specification which fixes a random subset of forwarding paths, reachability and isolation properties that are satisfied by the forwarding plane.

\paragraph{Topologies} For training, our dataset is based on random topologies with $16$-$24$ routers. We generate the physical layout of these graphs by triangulation of uniformly sampled points in two-dimensional space.

\paragraph{Simulation} To compute the forwarding plane given an OSPF and BGP configuration, we simulate the protocols. For OSPF, we implement shortest path computation to obtain the forwarding plane. For BGP, we implement the full BGP decision process as shown in \cref{fig:bgp-decision}, except for the MED attribute. In addition to the basic networking model discussed in \cref{sec:synthesis-setting}, we implement support for eBGP and iBGP, fully-meshed BGP session layouts as well as layouts relying on route reflection. For more details of these BGP concepts see \cite{bates2000rr}.

%Note that the synthesizer model will reason on the level of the provided training samples. That is, to improve the overall synthesis quality in a real-world setting, it is helpful to implement simulation code which behaves very similar to real-world networks. Another promising approach would be to extract training samples from real-world networks, thereby circumventing the need for simulation, however, we leave this as future work.

%While this can be a considerable effort, it is typically an easier task than to implement the synthesizer directly. The concrete semantics of protocols and their simulation is a well-defined procedure, whereas implementing efficient synthesis tools is still an open problem.

\paragraph{Fact Base Encoding} We encode synthesis input using a small set of facts. For an example of a corresponding fact base see \cref{fig:bgp-ospf-fact-base}. We use the \texttt{router}, \texttt{external} and \texttt{network} facts to mark routers, external peers and routing destinations respectively. Physical links between routers are encoded as \texttt{connected(R1,R2,W)} facts where \texttt{W} denotes the OSPF link weight. Further, we rely on \texttt{ibgp}, \texttt{ebgp}, \texttt{route\_reflector} and \texttt{bgp\_route} facts to represent different types of BGP sessions and imported routes. Using the notion of unknown parameters as discussed in \cref{sec:graph-embedding}, we encode configuration parameters such as the properties of imported routes and OSPF link weights.

\paragraph{Specification Language} We support a small specification language with three types of forwarding predicates:

\begin{itemize}
    \setlength{\itemsep}{0pt}
    \setlength{\parskip}{2pt}
    \item \texttt{fwd(R1, Net, R2)} specifies that router \texttt{R1} forwards traffic destined for \texttt{Net} to its neighbor \texttt{R2}.
    \item \texttt{reachable(R1, Net, R2)} specifies that traffic destined for \texttt{Net} that passes through \texttt{R1} also passes through \texttt{R2} before reaching its destination.
    \item \texttt{trafficIsolation(R1, R2, N1, N2)} specifies that it must not hold that $[fwd(R1,R2,N1)]_{\mathcal{B}} \wedge [fwd(R1,R2,N2)]_{\mathcal{B}}$.
\end{itemize}
 
In the negative case of each predicate, the opposite must hold true for the fact to be satisfied. This specification language can easily be extended by including new specification predicates in the dataset generation process. One must simply provide a method of extracting positive and negative cases of a specification fact from a given forwarding plane. Once included in the training dataset of a synthesizer model, the resulting synthesis system will be able to consider specifications relying on the new type of predicates.

% \todo{info on loss function, optimizer, etc.}
\paragraph{Training} We generate a dataset of $10,240$ input/output samples and instantiate our synthesizer model with a hidden dimension $D$ of $64$. For optimization, we use the Adam optimizer \cite{kingma2014adam} with a learning rate of $10^{-4}$, applying negative log-likelihood loss to the decoder networks' outputs. We stop training after the specification consistency on a validation dataset no longer increases at around $\sim2800$ epochs.

\begin{figure}
\begin{minipage}[t]{0.22\textwidth}
\begin{lstlisting}[basicstyle=\ttfamily\tiny]
# topology and configuration
router(c5)
router(c3)
router(c1)
router(c0)
network(c6)
network(c7)

external(c8)
external(c9)
external(c10)
external(c11)
external(c12)
external(c13)

route_reflector(c2)
route_reflector(c4)

connected(c2,c4,?)
connected(c2,c5,?)
connected(c2,c3,?)
connected(c4,c5,?)
connected(c4,c3,?)
connected(c4,c0,?)
connected(c5,c1,?)
connected(c5,c0,?)
connected(c3,c0,?)
connected(c3,c1,?)
connected(c1,c0,?)

ibgp(c2,c4)
ibgp(c2,c5)
ibgp(c2,c0)
ibgp(c2,c1)
ibgp(c4,c3)
ibgp(c4,c4)
\end{lstlisting}
\end{minipage}
\begin{minipage}[t]{0.2\textwidth}
\begin{lstlisting}[basicstyle=\ttfamily\tiny]
ebgp(c2,c12)
ebgp(c5,c9)
ebgp(c5,c10)
ebgp(c5,c13)
ebgp(c0,c8)
ebgp(c0,c11)

bgp_route(c8,c6,?,?,1,?,1,8)
bgp_route(c9,c6,?,?,0,?,1,9)
bgp_route(c10,c6,?,?,0,?,1,10)
bgp_route(c11,c7,?,?,0,?,1,11)
bgp_route(c12,c7,?,?,0,?,1,12)
bgp_route(c13,c7,?,?,2,?,1,13)

# forwarding specification
fwd(c0,c6,c3)
fwd(c3,c6,c2)
fwd(c2,c6,c4)
not fwd(c3,c6,c0)
not fwd(c0,c6,c11)
not fwd(c11,c6,c0)

not trafficIsolation(c1,c0,c7,c6)
not trafficIsolation(c1,c0,c7,c6)
trafficIsolation(c0,c3,c6,c7)
trafficIsolation(c0,c3,c6,c7)

reachable(c5,c6,c10)
reachable(c1,c6,c4)
not reachable(c0,c6,c5)
reachable(c5,c6,c10)
\end{lstlisting}
\end{minipage}
\caption{An example of a fact base encoding a topology, a sketch of a BGP and OSPF configuration and a forwarding specification.}
\label{fig:bgp-ospf-fact-base}
\end{figure}

==> diff/git-latexdiff.33774/old/sections/4_evaluation.tex <==
\section{Evaluation}
\label{sec:evaluation}

We have trained a synthesizer model to perform configuration synthesis for BGP and OSPF. In this section, we assess the performance of the resulting synthesis tool with respect to two core metrics: (1) We evaluate the quality of the synthesized configurations in terms of their consistency with the provided forwarding specifications in \cref{sec:synthesis-quality}. And (2), we evaluate the synthesis time of a learned synthesizer as compared to the state-of-the-art SMT-based synthesis tool NetComplete \cite{el2018netcomplete} in \cref{sec:synthesis-vs-smt}.

\paragraph{Dataset} We compare across three datasets: Small, Medium and Large. Each dataset represents 8 real-world topologies, sampled from the Topology Zoo \cite{knight2011internet}, where the number of nodes lies between 0-34, 34-68 and 68-170 respectively. To obtain forwarding specifications for the sampled topologies, we use our generative pipeline as discussed in \cref{sec:training}. In each topology, we do synthesis for 4 different traffic classes (routing destinations) at a time.

\paragraph{Experimental Setup} We run all our experiments on an Ubuntu Linux machine with an Intel(R)~Core(TM)~i9-9900X~@~3.50GHz processor, 64GB of system memory and an NVIDIA GeForce RTX 3080 GPU with 10GB of video~memory.

\subsection{Synthesis Quality}
\label{sec:synthesis-quality}
To assess the limitations of our learned synthesizer in a BGP/OSPF setting, we examine its behavior with increasingly large topologies and specifications. 

\paragraph{Specifications} Using the same generative model as described in \cref{sec:training}, we generate forwarding specifications for the topologies in our three datasets. More specifically, each specification is constructed from $3 \times n$ requirements, one per supported predicate type: A \texttt{fwd} requirements corresponds to specifying or blocking a forwarding path using multiple \texttt{fwd} predicates whereas \texttt{reachable} and \texttt{trafficIsolation} requirements translate to a single specification fact each. We compare across increasingly large specifications of $3\times 2$, $3\times 8$ and $3 \times 16$ requirements respectively. 

\paragraph{Methodology} For each pair of topology and specification, we run our synthesizer model 5 times and report the network configurations with the highest overall consistency value. For sampling, we rely on our multi-shot sampling strategy where we randomly group the unknown parameters of a configuration into 4 groups (4-shot sampling).

\paragraph{Results} We summarize our results in \cref{fig:eval-consistency}. On average, our synthesis model produces network configurations that are $>91\%$ consistent with the provided forwarding specifications across all datasets and sizes of specifications. When only few requirements are given, the synthesizer model even succeeds in producing fully-consistent configurations. We observe a slightly decreasing consistency with increasingly large topologies. 

%\texttt{fwd} facts are satisfied more easily, whereas \texttt{reachable} and \texttt{trafficIsolation} facts are violated more often. 

\paragraph{Multi-Shot Sampling} In \cref{fig:eval-consistency-baseline}, we report the average specification consistency using our multi-shot sampling strategy as compared to sampling all unknown parameters at once. As a baseline we have also sampled random configurations from a uniform distribution (per parameter) and compute the corresponding specification consistency. Over the baseline, our synthesizer model shows clear improvement and multi-shot sampling further increases consistency.

\begin{figure*}
    \begin{center}
        \textbf{Specification Consistency}\\
        \footnotesize
        \begin{tabular}{rrcccccccccc}
        \toprule
        \multicolumn{2}{c}{Dataset} & \tiny\texttt{fwd} & \tiny\texttt{reachable}  & \tiny\texttt{trafficIsolation} & Overall & $\emptyset$     No. Full Matches & $\emptyset$ No. $>90\%$ Matches\\
        \midrule
        $3\times 2$ requirements & Small & 0.95 & 0.94 & 1.00 & \textbf{0.95} & 0.62 & 0.62\\
& Medium & 0.96 & 1.00 & 0.94 & \textbf{0.96} & 0.88 & 0.88\\
& Large & 0.94 & 0.94 & 1.00 & \textbf{0.93} & 0.62 & 0.62\\
\midrule
$3\times 8$ requirements & Small & 0.97 & 0.98 & 0.97 & \textbf{0.98} & 0.50 & 1.00\\
& Medium & 0.99 & 0.95 & 1.00 & \textbf{0.98} & 0.50 & 1.00\\
& Large & 0.96 & 0.95 & 0.91 & \textbf{0.94} & 0.38 & 0.88\\
\midrule
$3\times 16$ requirements & Small & 0.97 & 0.89 & 0.95 & \textbf{0.94} & 0.38 & 0.75\\
& Medium & 0.98 & 0.97 & 0.97 & \textbf{0.98} & 0.38 & 1.00\\
& Large & 0.92 & 0.88 & 0.95 & \textbf{0.91} & 0.12 & 0.50\\
    \end{tabular}\end{center}
    \caption{Average specification consistency of the network configurations synthesized by our trained synthesizer model. Per sample we run the synthesizer with a specification of $3\times N$ requirements, where the specifications always include $N$ requirements per supported predicate type (\texttt{fwd}, \texttt{reachable}, \texttt{trafficIsolation}).}
    \label{fig:eval-consistency}
\end{figure*}

\begin{figure}
    \begin{center}
        \footnotesize
        \begin{tabular}{rrcccccccccc}
        &  & \multicolumn{2}{c}{Neural}\\
        & Random & 1-Shot & 4-shot\\
        \toprule
        Small & 0.83 & 0.92 & \textbf{0.94} \\
        Medium & 0.88 & 0.95 & \textbf{0.98} \\
        Large & 0.78 & 0.88 & \textbf{0.91} \\
    \end{tabular}\end{center}
    \caption{Average specification consistency with $3\times 16$ requirements when sampling configurations randomly from a uniform distribution and 1-shot/4-shot sampling using our synthesizer model.}
    \label{fig:eval-consistency-baseline}
\end{figure}
    
\begin{figure*}[ht]
    \footnotesize
    \begin{center}
        \textbf{BGP Synthesis Time}
        \footnotesize
        \begin{tabular}{rrccccccccc}
        \toprule
        &&\multicolumn{3}{c}{Synthesis Time (s)} & \multicolumn{2}{c}{Accuracy (Neural)} \\
        \multicolumn{2}{l}{\# Requirements} & NetComplete & Neural (CPU) & Speedup &$\emptyset$ Consistency& $\emptyset$ No. Full Matches\\
        \midrule
    2 requirements &Small & 18.073s & 0.641s & \textbf{28.2x} & 0.969 & 0.875\\
        &Medium & 60.864s & 2.748s & \textbf{22.2x} & 0.939 & 0.75\\
        &Large & 1389.485s\tiny{  7/8 TO} & 22.301s & \textbf{62.3x} & 0.989 & 0.875\\
    \midrule
    8 requirements &Small & 247.691s & 1.065s & \textbf{232.5x} & 0.96 & 0.75\\
        &Medium & $>$25m\tiny{  8/8 TO} & 3.47s & \textbf{432.2x} & 0.968 & 0.5\\
        &Large & $>$25m\tiny{  8/8 TO} & 30.961s & \textbf{48.4x} & 0.969 & 0.75\\
    \midrule
    16 requirements &Small & 1416.828s\tiny{  7/8 TO} & 2.528s & \textbf{560.5x} & 0.926 & 0.25\\
        &Medium & $>$25m\tiny{  8/8 TO} & 5.481s & \textbf{273.7x} & 0.947 & 0.25\\
        &Large & $>$25m\tiny{  8/8 TO} & 69.092s & \textbf{21.7x} & 0.959 & 0.25\\
    \end{tabular}\end{center}
    \caption{Comparing consistency and synthesis time of our method (Neural) with the SMT-based state-of-art synthesis tool NetComplete. The notation {\tiny{n/8 TO}} indicates the number of timed out synthesis runs out of 8 (25+ minutes).}
    \label{fig:evaluation-compare-bgp}
\end{figure*}

\begin{figure*}[ht]
    \begin{center}
        \footnotesize
        \textbf{OSPF Synthesis Time}\\
        \footnotesize
        \begin{tabular}{rrccccccccc}
        \toprule
        &&\multicolumn{3}{c}{Synthesis Time (s)} & \multicolumn{2}{c}{Accuracy (Neural)} \\
        \multicolumn{2}{l}{} & NetComplete & Neural (GPU) & Speedup &$\emptyset$ Consistency& $\emptyset$ No. Full Matches\\
        \midrule
    2 requirements &Small & 0.265s & 0.091s & \textbf{2.9x} & 1.000 & 1.00\\
     &Medium & 0.404s & 0.098s & \textbf{4.1x} & 1.000 & 1.00\\
     &Large & 0.944s & 0.14s & \textbf{6.7x} & 1.000 & 1.00\\
    \midrule
    8 requirements &Small & 0.876s & 0.164s & \textbf{5.3x} & 0.982 & 0.75\\
     &Medium & 1.517s & 0.103s & \textbf{14.7x} & 1.000 & 1.00\\
     &Large & 3.505s & 0.316s & \textbf{11.1x} & 0.981 & 0.50\\
    \midrule
    16 requirements &Small & 1.65s & 0.21s & \textbf{7.9x} & 0.991 & 0.625\\
     &Medium & 2.646s & 0.245s & \textbf{10.8x} & 0.989 & 0.50\\
     &Large & $>$566.636s+\tiny{  3/8 TO} & 0.233s & \textbf{2430.4x} & 0.987 & 0.875\\
    \end{tabular}\end{center}
    \caption{Comparing consistency and synthesis time of our method (Neural) with the SMT-based OSPF synthesis tool NetComplete. The notation {\tiny{n/8 TO}} indicates the number of timed out synthesis runs out of 8 (25+ minutes).}
    \label{fig:evaluation-compare-ospf}
\end{figure*}
    

\subsection{Comparison to SMT-based Synthesis}
\label{sec:synthesis-vs-smt}

%To provide a comparison of our learned BGP/OSPF synthesizer with SMT-based methods, 
We compare the synthesis time of the learned synthesizer with the state-of-art configuration synthesis tool NetComplete \cite{el2018netcomplete}.

\paragraph{Specifications} Since the type of supported requirements in NetComplete does not fully align with our model, we restrict this comparison to specifications which only include forwarding paths (i.e. \texttt{fwd} predicates). Further, NetComplete does not support cross-protocol synthesis as in our case and instead requires users to specify for each requirements which protocol to use for its implementation. To bridge this gap, we split the generated forwarding requirements into BGP and OSPF paths for a corresponding NetComplete specification.
%\todo{note on NetComplete installing policies at all routers, not only the edges of the AS}

\paragraph{Methodology} We compare both OSPF synthesis and BGP/OSPF-synthesis. We configure our trained synthesizer model to do OSPF synthesis by only predicting link weights. For each pair of topology and specification, we report the total time of running our synthesizer 4 times using 4-shot sampling, whereas for consistency we report the best out of the 4 runs. For NetComplete, we run the synthesizer with a timeout of 25 minutes. In case the NetComplete synthesis attempt times out, we report 25 minutes as a lower bound for the actual NetComplete runtime.

\paragraph{OSPF Synthesis Time Results} We document the results of comparing OSPF synthesis time in \cref{fig:evaluation-compare-ospf}. Our synthesizer model achieves a speedup of 2-10x over NetComplete's counter-example guided SMT-based method. With 16 requirements and dataset Large this speedup even increases to $2000\times$. Further, our model achieves very high consistency with the provided specification, often even producing fully-consistent configurations.

\paragraph{BGP/OSPF Synthesis Time Results} See \cref{fig:evaluation-compare-bgp} for the comparison of the BGP/OSPF synthesis time. Our synthesizer model outperforms NetComplete by multiple orders of magnitude. We observe a speedup of $20-560\times$ which appears to increase with the size of topology and specification. Further, the average specification consistency of the synthesized configurations is greater than $92\%$ across all datasets, even for large topologies. In many cases, our synthesizer model even produces fully-consistent configurations, especially with small topologies and specifications. In comparison, NetComplete times out on more than half of the synthesis tasks which means that we can only observe a lower bound of speedup in these cases. Note that our synthesizer model is running on a CPU due to memory restrictions with large topologies. However, running it on a GPU results in even greater speedups (up to $1000\times$, cf. \cref{app:sec:bgp-gpu-performance}). 

==> diff/git-latexdiff.33774/old/sections/5_related_work.tex <==
\section{Related Work}
\label{sec:related-work}

\paragraph{Traditional Configuration Synthesis} 
%A range of existing work is concerned with network configuration synthesis. 
Next to methods based on compilation such as Propane/PropaneAT \cite{beckett2017network}, there are a number of configuration synthesis methods based on constraint solving: Examples include ConfigAssure \cite{narain2008declarative}, SyNet \cite{el2017network} and NetComplete \cite{el2018netcomplete}. Due to their hand-coded nature, these methods are highly protocol-specific and can be very slow due to the solvers they employ. Although some of them allow for cross-protocol reasoning, this is not implemented as transparently as in our framework and users must specify per requirement which protocol to use for its implementation. In contrast, our approach has lower precision but allows for fully transparent cross-protocol reasoning, meaning forwarding requirements are not protocol-bound and the synthesizer chooses how to implement them. Further, our learned BGP/OSPF synthesis tool exhibits much lower synthesis times as compared to an SMT-based tool like NetComplete.

% \begin{itemize}
%     \item NetComplete, SyNet
%     \item Propane, PropaneAT
%     \item DeepBGP
% \end{itemize}

\paragraph{GNNs and Networking} DeepBGP \cite{bahnasy2020deepbgp} relies on GNNs and reinforcement learning to do configuration synthesis. However, it is limited to BGP configuration synthesis and is slower than SMT-based synthesis according to the author's evaluation. In contrast, our learning-based framework is cross-protocol, does not rely on reinforcement learning and provides better synthesis performance. Apart from configuration synthesis, GNNs have also been applied to other problems in the networking domain. For example, the authors of RouteNet \cite{rusek2020routenet} use GNNs to predict performance metrics of network configurations. Other work that is concerned with learning improved protocols includes Q-Routing \cite{boyan1994packet} or more modern approaches such as the Graph-Query Neural Network architecture \cite{geyer2018learning}.

\paragraph{Neural Algorithmic Reasoning} 
Neural algorithmic reasoning (NAR) as proposed in \cite{velivckovic2021neural}, describes the idea of replacing traditional algorithms with neural networks to learn improved algorithmic procedures. Exemplary work includes graph-related algorithms \cite{velivckovic2019neural} or solvers for combinatorial optimization problems \cite{cappart2021combinatorial,joshi2020learning,selsam2019guiding}. Our synthesis framework is the first applications of NAR to the networking domain and relies on the NAR-native encode-process-decode architecture. According to the hierarchy of NAR approaches in \cite{cappart2021combinatorial}, our method is an algorithm-level approach, as we do not supervise on intermediate steps. Although, such step-level methods promise better generalization, it is not clear what an intermediate result of a general synthesis procedure would be. However, future work on a step-level approach may further improve synthesis quality.

% \begin{itemize}
%     \item RouteNet
%     \item GraphNET
%     \item Learning and generating distributed routing protocols using graph-based deep learning
%     \item Unveiling the potential of Graph Neural Networks for network modeling and optimization in SDN
% \end{itemize}

==> diff/git-latexdiff.33774/old/sections/6_conclusion.tex <==
\setlength{\parskip}{6pt plus4mm minus4mm}
\section{Conclusion}
\label{sec:conclusion}
We presented a learning-based framework for configuration synthesis based on the idea of neural algorithmic reasoning. To assess the effectiveness of the system, we instantiated it for the case of BGP/OSPF synthesis. In contrast to traditional synthesis methods, our system supports transparent cross-protocol reasoning and learns synthesis rules completely from data. Using our system, synthesis is sped up by a factor of up to $500\times$ when compared to SMT-based methods. Further, our evaluation demonstrates that the resulting synthesis tool provides very good synthesis quality, producing configurations with high specification consistency. Overall, our results show that learning-based network configuration synthesis is a promising direction, enabling new cross-protocol reasoning capabilities and great performance improvements. For future work, we see a lot of promise in constructing hybrid systems, integrating both our neural model and SMT-based synthesis to address the decreased precision of a neural model.

==> diff/git-latexdiff.33882/new/acronyms.tex <==
\DeclareAcronym{AS}{
    short = AS,
    long = autonomous system,
    short-plural = es ,
    long-plural = s
}

==> diff/git-latexdiff.33882/new/sections/0_abstract.tex <==
% Context
Computer networks employ a number of different protocols to enable efficient routing. However, due to the complexity of multiple interacting protocols, it can be hard for network operators to implement high-level routing policies and requirements. Network configuration synthesis promises to address this situation by automatically generating configurations that satisfy a provided specification. However, existing synthesis methods are often limited to single-protocol reasoning, depend on protocol-specific and hand-coded synthesis rules, and are difficult to scale due to the SMT-based methods they employ. In this work we present a rather different, learning-based method for addressing the configuration synthesis challenge, one based on the recently proposed paradigm of neural algorithmic reasoning. Our framework is protocol-agnostic, enables cross-protocol reasoning and does not depend on any hardcoded synthesis rules. To evaluate, we instantiate our framework for the case of BGP/OSPF synthesis. Our experiments show we can synthesize configurations with a very high degree of specification consistency while observing speedups of up to $500\times$ compared to a state-of-the-art SMT-based synthesis tool.


==> diff/git-latexdiff.33882/new/sections/1_intro.tex <==
\section{Introduction}
\label{sec:introduction}

The backbone of the internet consists of many connected computer networks operated by different internet service providers (ISPs) and other large organizations. These networks rely on a number of protocols to enable effective and policy-driven routing of traffic. Based on router-level configurations, the protocols perform a distributed computation to construct a network's forwarding state. However, the relatively low-level router configuration makes it hard for network operators to directly enforce network-wide policies and requirements. This often leads to misconfiguration, which can cause global outages such as the recent hours-long blackout of the entire Facebook platform \cite{janardhan2021} and comparable events \cite{mccarthy_2019}.
%
\paragraph{Configuration Synthesis} This situation has triggered a number of research efforts regarding the synthesis of network configurations \cite{el2018netcomplete,beckett2017network,narain2008declarative}. Configuration synthesis is concerned with the task of automatically generating router-level configurations given a set of high-level requirements. However, this synthesis problem can be very hard to solve, since network configurations typically consist of a considerable number of tunable parameters, where the execution of several interacting protocols yields the overall forwarding state. An effective synthesis tool must thus account for this fact and be able to reason across multiple protocols.

\paragraph{SMT-based Synthesis} Some of the most successful efforts in providing cross-protocol synthesis capabilities are based on satisfiability modulo theory (SMT) solvers \cite{el2018netcomplete,el2017network}. While SMT-based synthesis is a promising method, it comes with a number of limitations:
% \item protocol-specific
% fully hand-coded synthesis rules, a lot of implementation effort, cross-protocol support extra complicated
(1) SMT-based synthesizers are hand-crafted and highly protocol-specific. To implement synthesis, we must first express our networking model, protocol semantics including vendor and device specific behavior in terms of first-order logic constraints. This is a time-intensive and complicated process, requiring lots of expert knowledge.
%  model-dependent: synthesis is reasoning on the level of some assumed model which may not reflect the real world: even if a configuration is synthesized based on some spec, it may behave differently and violate spec in practice
Further, (2) logic-based modelling introduces a disconnect between the synthesis tool and real-world behavior \cite{birkner2021metha}. More specifically, synthesized configurations may satisfy a provided specification within a formal framework, but may not behave the same way in the real world.
% can be very slow
And, (3) SMT-based synthesis can be very slow or fail to complete, especially when reasoning about large network topologies. In practice however, network operators reconfigure their networks on a daily basis \cite{vissicchio2012improving}, which means an effective synthesis tool must be fast.

% \item fully learned, no hand-coded synthesis rules (model-free), very flexible to adapt to more/new protocols
% \item protocol-agnostic, cross-protocol
\paragraph{Neural Algorithmic Reasoning for Synthesis} Recent work on neural algorithmic reasoning (NAR) proposes to replace traditional algorithms with neural networks to learn improved algorithmic procedures \cite{velivckovic2021neural}.
It has been shown to be a powerful and fast algorithmic approximation method for a number of graph-related \cite{velivckovic2019neural} and combinatorial optimization problems \cite{cappart2021combinatorial}. Further, due to its learned nature, NAR allows for learning procedures directly from (real-world) data, without the need for manual feature extraction. Overall, this positions NAR as an attractive method to obtain a fast, fully-learned synthesis procedure, which entirely avoids the need for a formal model or any hand-crafted synthesis rules. Based on this promising outlook, this paper explores how to apply the NAR paradigm to the problem of network configuration synthesis.

To that end, we propose a \textbf{new learning-based framework for configuration synthesis} as an alternative to SMT-based approaches. Our framework is protocol-agnostic, enables cross-protocol reasoning and avoids the need to manually provide synthesis rules. We build upon the idea of NAR, and train a graph-based processor neural network to learn a synthesis procedure in latent space. A key challenge in a multi-protocol setting is the diversity of different protocols and configuration parameters. To this end, we implement a generic embedding scheme based on Datalog-like facts and program sketching \cite{solar2008program}, which allows us to easily adapt our framework to new protocols. Further, our synthesis model produces a whole distribution of network configurations. As a consequence, we can directly sample multiple alternative synthesis outputs, which is not possible with standard SMT solvers. We apply our framework to a non-trivial synthesis setting where both the Border Gateway Protocol (BGP) and the Open Shortest Path First (OSPF) protocol are used. We demonstrate that our learned synthesis tool is up to~$500\times$ faster than a state-of-the-art SMT-based synthesizer, while producing configurations which on average enjoy more than 91\% satisfaction of the provided specification.

\paragraph{Main Contributions} Our core contributions are:
\vspace{-5pt}
\begin{itemize}
    \setlength{\itemsep}{5pt}
    \setlength{\parskip}{0pt}
    \item A learning-based framework for network configuration synthesis based on neural algorithmic reasoning.
    \item A neural network architecture for learning synthesizer models which relies on a generic graph-based encoding of network topologies and configurations.
    \item An extensive evaluation of our learning-based synthesizer, in terms of both precision and scalability, on the challenging setting where both the BGP and OSPF protocols are involved.
\end{itemize}

\section{Framework Overview}
\label{sec:overview}

\begin{figure}
    \begin{center}
        \includegraphics[width=0.45\textwidth]{figures/synthesizer-overview.pdf}
    \end{center}
    \caption{An overview of our learning-based synthesis framework.}
    \label{fig:learning-based-synthesis}
\end{figure}

%As an example, consider \cref{fig:network-fwd-tree} (c) which illustrates the forwarding plane of some traffic class reachable via external peer $E$ or $F$ in our example network. Each router of the network forwards traffic along some of its outgoing links. In practice, a number of protocols are used to populate a router's routing tables. For the instantiation of our synthesis framework however, we focus on OSPF and BGP.

In the following, we discuss the fundamentals and core steps of our learning-based framework as illustrated in \cref{fig:learning-based-synthesis}.

\paragraph{Network Configuration} In this work, we consider the configuration synthesis problem at the level of the so-called \emph{forwarding plane} of a network. This means we look at how each router forwards traffic, given a packet with a certain destination. The forwarding plane is determined by a distributed computation whose exact semantics depend on the different routing protocols in use. To adapt the forwarding behavior, network operators change configuration parameters at the router-level (e.g. link weights), such that running the protocols results in the desired forwarding plane. Given this context, we define the problem of configuration synthesis as follows.

\paragraph{Configuration Synthesis} The configuration synthesis problem corresponds to automatically generating these router-level configurations, such that a set of given requirements about the forwarding plane is satisfied. Typical requirements include reachability, traffic isolation and other forwarding properties. 

\paragraph{Dataset} To train a synthesizer model, we first generate a dataset of input/output samples for the synthesis problem. For this, we rely on a generative pipeline as shown in the top of \cref{fig:learning-based-synthesis}. First, we sample a random network configuration for some topology using a uniform generative process. Then, we simulate the involved protocols to obtain the corresponding forwarding plane. Next, we extract a specification by randomly selecting properties that hold for the computed forwarding plane. This leaves us with a specification and topology as input and corresponding configuration as the output to a synthesis problem.

\paragraph{Simulation} Depending on the protocols in use, one implements simulation code to compute the forwarding plane induced by a sampled configuration. Although this step is protocol-specific, the overall implementation effort is much lower compared to SMT-based synthesis. Protocols are typically well-defined algorithms which can be simulated, whereas the alternative of implementing a synthesizer often requires expert knowledge about SMT solvers. In practice, our framework may also be adapted to use a real-world network router to compute the behavior of a configuration, thereby capturing the real-world behavior directly.

\paragraph{Neural Synthesizer Model} Based on the generated dataset, we train a graph neural network (GNN) to perform synthesis. For this, the network's input consists of a topology, a specification and a configuration sketch where to-be-synthesized parameters are omitted. Following the NAR paradigm, we first encode this synthesizer input in latent space. Then, we apply an iterative processor network which relies on the graph attention mechanism to propagate information \cite{velivckovic2017graph}. Last, we apply a decoder network to predict the values of omitted configuration parameters, thereby synthesizing a corresponding configuration. To remain protocol-agnostic, our model is generic with respect to the input format, using an intermediate representation based on Datalog-like facts.
%
\paragraph{Relaxed Specification Consistency} Since parts of the configuration synthesis problems are known to be NP-hard \cite{fortz2000internet}, any precise synthesis method will run into scalability issues, just like SMT-based methods. However, practical synthesis must be fast and scalable to accommodate the size of real-world networks and the frequency at which configurations need to be updated \cite{vissicchio2012improving}. In our learning-based framework, we therefore employ a fixed-size neural network architecture which always runs in polynomial time. While this indeed enables fast synthesis times, we cannot expect our neural system to be as precise as SMT methods. Therefore, to assess the synthesis capabilities of our learning-based system, we rely on the notion of \emph{relaxed~specification~consistency}. More specifically, we do not just check whether a configuration satisfies a specification or not, but also measure the degree up to which a synthesized configuration satisfies a specification (e.g. via the number of satisfied requirements). 

This "soft" understanding of a specification allows us to evaluate neural synthesis systems which may not always produce fully consistent configurations. Further, we argue that configurations with less than $100\%$ consistency are still very useful in practice, as they provide a good starting point for additional adjustments by network operators. Future work may improve the precision of neural synthesis by exploiting partial synthesis methods \cite{el2018netcomplete} to obtain fully consistent solutions, given a partially consistent configuration. However, note also that even exact SMT-based synthesizers may not always produce fully consistent solutions, due to differences between the formal protocol model and the one running on a given real-world router where the configuration is to be deployed \cite{birkner2021metha}.

\paragraph{Instantiation} Our learning-based synthesis framework is generic with respect to the routing protocols in use. This means, it can be instantiated to many different synthesis settings. To do this, users merely provide a drop-in replacement for the simulation component as shown in \cref{fig:learning-based-synthesis}, while other components such as the neural model architecture itself can be directly re-used.

%More specifically, we employ a slightly modified variant which operates on a graph-based encoding of a specification, topology and configuration parameters.

%  \begin{figure*}
%      \centering
%      \includegraphics[width=0.85\textwidth]{figures/system-overview.pdf}
%      \caption{An overview of our synthesis system: (1) First, we use a generic embedding scheme to transform a network topology, protocol configuration sketches and the specification given as Datalog-like facts to a latent input representation. Next, we apply a learned (2) Processor GNN and obtain a latent synthesis output. Last, we apply a (3) Decoder Network to obtain a distribution over possible values per unknown parameter in our configuration.}
%      \label{fig:overview-model}
% \end{figure*}
%

In this paper, we first discuss the architecture of our neural synthesis model. In follow-up sections, we instantiate our framework  for the case of BGP/OSPF configuration synthesis, and evaluate the resulting instantiation by comparing it to a state-of-the-art SMT-based synthesizer.

% \begin{itemize}
%     \item effort: need to implement simulation code to generate dataset to learn from (typically well-defined in protocol specs, much easier than implementing synthesis directly)
%     \item can be sampled (multiple alternative solutions, not easily possible with SMT-based methods)
%     \item much faster than SMT-based synthesis
% \end{itemize}

% Requirements:
% \begin{itemize}
%     \item protocol-agnostic
%     \item fully learned, no hand-coded synthesis rules
%     \item define: strict specification vs. relaxed specification
% \end{itemize} 

==> diff/git-latexdiff.33882/new/sections/2_model.tex <==
\section{Neural Synthesis Model}
\label{sec:model}


We now present the architecture of our graph-based neural synthesizer model, illustrated in \cref{fig:overview-model}. First, in \cref{sec:graph-embedding} we introduce our generic graph-based encoding, which allows us to embed network topologies, protocol configuration and the specification into a latent space. Then, in \cref{sec:graph-transformer} we present the architecture of the processor network which we train to perform the synthesis task. Finally, in \cref{sec:decoding-sampling} we discuss how to sample network configurations from the resulting latent synthesis output.

\begin{figure}
    \begin{minipage}[t]{0.21\textwidth}
    \begin{lstlisting}[basicstyle=\ttfamily\small, escapeinside={(*}{*)}]
router(A)
router(B)
(...)

connected(A,B,2)
connected(A,C,?)(*\blackcircled{1}*)
(...)
    \end{lstlisting}
\end{minipage}
\begin{minipage}[t]{0.21\textwidth}
    \begin{lstlisting}[basicstyle=\ttfamily\small, escapeinside={(*}{*)}]
network(N1)
bgp_route(E,N1,2,3,1,0,1)

fwd(A,B,N1)
not fwd(B,A,N1)
(...)
    \end{lstlisting}
\end{minipage}
    \caption{A snippet of a fact base sketch encoding a network's topology, parameters such as link weights (\texttt{connected} facts) and a specification (\texttt{fwd} facts).}
    \label{fig:datalog-encoding}
\end{figure}

\begin{figure}[t]
    \centering
    \includegraphics[width=0.25\textwidth]{figures/synth-architecture.png}
    \caption{The neural synthesizer model architecture.}
    \label{fig:architecture}
\end{figure}

\subsection{Fact Base Embedding}
\label{sec:graph-embedding}
To remain network protocol-agnostic in our model architecture, we implement a generic graph-based encoding of Datalog-like facts, similar to knowledge graphs \cite{rosso2020beyond}. This means that we first encode topologies, configurations and specifications as a set of Datalog-like facts and then employ a generic embedding.
%We chose Datalog facts as the input format of our synthesis approach for its flexibility, wide-spread use in Program Analysis and use in previous work on configuration synthesis \cite{el2017network}.

\paragraph{Fact Base} A set of Datalog-like facts, as depicted in \cref{fig:datalog-encoding}, serves as the input \emph{fact base} $\mathcal{F}$ to our synthesizer model. $\mathcal{F}$ is a set of facts $f(a_0, \dots, a_n)$ where arguments may be constants (e.g. A or B) or integer literals. Further, each fact in a fact base has a corresponding truth value denoted as $[f(a)]_{\mathcal{B}}$. For instance, from the fact base in \cref{fig:datalog-encoding} we can derive $[fwd(A,B,N1)]_{\mathcal{B}} = \text{\texttt{true}}$ and $[fwd(B,A,N1)]_{\mathcal{B}} = \text{\texttt{false}}$.

\paragraph{Consistency} We represent a network's topology, the protocol configuration and parameters as well as the specification, all in a single fact base. Given the semantics of the protocols in use, we can then check whether the specification encoded in a fact base is satisfied by the provided configuration. To quantify, we define the notion of relaxed specification consistency, as discussed earlier, with respect to a fact base: Given a fact base $\mathcal{F}$, a subset of specification facts $S \subset \mathcal{F}$ and protocol semantics $\mathcal{P}$, the \emph{consistency} of a fact base is defined as the relative number of satisfied facts in $S$ with respect to the forwarding plane obtained via $\mathcal{P}$. The contents of $S$ depend on the concrete instantiation of the synthesizer model. For an example of possible specification facts, see our instantiation of the synthesizer model for BGP/OSPF in \cref{sec:training}.

\begin{figure*}
    \footnotesize
    \def\arraystretch{1.4}
    \begin{tabular}{lr}
        %$T_f: T_1 \times \dots \times T_n$ & \textit{(fact type declaration)}\\
        $emb(f) := \mathbf{V_f}$ & \textit{(learned fact type embedding)}\\
        $emb(b) := \mathbf{W_{\text{bool}}}\;onehot(b)$ & \textit{(learned boolean embedding)}\\
        $emb(f,i,v) := \mathbf{W_{f_i}}\;onehot(v)$ & \textit{(learned integer embedding)}\\
        $emb(f,i,?) := \mathbf{V_{hole}}$ & \textit{(learned hole embedding)}\vspace{2pt}\\
        $\mathlarger{
        h_c := \sum_{f(c) \in \mathcal{F}}
        emb(f)
        }$ & \textit{(constant embedding)}\vspace{2pt}\\
        $h_{f(a_0, \dots, a_n)} := emb(f) + emb([f(a_0, \dots, a_n)]_{\mathcal{B}}) + \mathlarger{
        \sum_{(i,v) \in \mathcal{I}(f(a_0, \dots, a_n))}
        emb(f, i, v)
        }$\hspace{-1.2cm} & \textit{(fact embedding)}\\
        $\mathcal{I}(f(a_0, \dots, a_n)) := \{(i,v) \; | \; f(a_0, \dots, a_{i-1}, v, \dots, a_n) \in \mathcal{F} \wedge v:Int \wedge i \in \mathbb{N}$ \}& \textit{(integer arguments)}\vspace{2pt}\\
        $N_i(h_c) := \{h_f \; | \; \exists i \in \mathbb{N} . f(a_0, \dots, a_{i-1}, c, a_{i+1}, \dots, a_n) \in \mathcal{F}\}$& \textit{(i-th neighborhood of constant node)} \\
        $N_i(h_f) := \{h_c \; | \; \exists i \in \mathbb{N} . f(a_0, \dots, a_{i-1}, c, a_{i+1}, \dots, a_n) \in \mathcal{F}\}$& \textit{(i-th neighborhood of fact node)} \\
    \end{tabular}
    \caption{Translating a fact base $\mathcal{F}$ to node features. $f$ denotes a predicate, $v$ integer values, $b$ boolean values as 0 or 1, $i$ argument indices and $[f(a)]_{\mathcal{B}}$ the truth value of a fact. }
    \label{fig:graph-embedding}
\end{figure*}

%discuss embedding as shown in \cref{fig:datalog-encoding}. Note how this makes fact bases a suitable input to standard GNN architectures.

\paragraph{Fact Base Sketching} In a synthesis setting, we are confronted with incomplete fact bases, i.e. the specification and topology is given but the network configuration is to be synthesized. For these cases, we also consider fact bases with unknown parameters inspired by the idea of program sketching in program synthesis \cite{solar2008program}. More specifically, users may replace an unknown integer argument of a fact by a \texttt{?} symbol, indicating a value to be synthesized. Using this mechanic, we can represent the synthesis input as an incomplete fact base which encodes to-be-synthesized values as unknown parameters. As an example, consider \cref{fig:datalog-encoding} \blackcircled{1}, where the link weight between router nodes \texttt{A} and \texttt{C} is represented as an unknown parameter.

\paragraph{Embedding} We employ a structurally-defined embedding scheme to transform a fact base into a graph with node features as required for processing with graph neural networks. Given a fact base $\mathcal{F}$, we apply the rules in \cref{fig:graph-embedding} to obtain node features and adjacency information. Both a fact $f$ and a constant $c$ are represented as distinct nodes with features $h_c$ and $h_f$, respectively. The relationships between facts and constants is encoded as node adjacency as defined by the neighborhood functions $N_i$.

We use multiple neighborhood functions, i.e. multiple types of edges, to encode the argument position of a constant occurring in a fact. Hence, the number of neighborhood functions corresponds to the maximum number of arguments in a single fact, e.g. 3 in \cref{fig:datalog-encoding}. Integer arguments and unary facts are directly accounted for in the respective node or fact embedding. To handle unknown parameters, we replace the corresponding $emb(...)$ term with the learned $\mathbf{V_{hole}}$ embedding.

Considering the embedding function $emb$, the learned parameters of our embedding are $\mathbf{V_f} \in \mathbb{R}^D$ per fact type in~$\mathcal{F}$, $\mathbf{W_{\text{bool}}} \in \mathbb{R}^{D \times 2}$ for boolean values, $\mathbf{W_{f_i}} \in \mathbb{R}^{D \times N}$ per integer argument of fact type $f$ and $\mathbf{V_{hole}} \in \mathbb{R}^D$ to represent unknown parameters. Hyperparameter $D$ represents the dimension of the latent space the synthesizer model operates in and $N$ specifies the number of supported integer values. An example of applying this embedding scheme to a simple fact base is given in \cref{fig:graph-encoding-example}.

\begin{figure}
    \begin{minipage}[t]{0.2\textwidth}
        \centering
        \footnotesize
        \textbf{Fact Base}
        \begin{lstlisting}[basicstyle=\ttfamily\small]
router(A)
router(B)

conn(A, B, 12)
        \end{lstlisting}
    \end{minipage}
    \begin{minipage}[t]{0.15\textwidth}
        \centering
        \textbf{Graph}\\
        \vspace{5pt}
        \includegraphics[width=0.7\textwidth]{figures/graph-encoding.pdf}
    \end{minipage}\\
    \centering\\
    \vspace{10pt}
    \textbf{Node Features}\\
    \vspace{10pt}
    \begin{minipage}[t]{0.5\textwidth}
        $\begin{array}{rcl}
        h_A &:=& emb(router) = \mathbf{V_{\text{router}}}\\
        h_B &:=& emb(router) = \mathbf{V_{\text{router}}}\\
        h_{\text{conn(A,B,12)}} &:=& emb(conn) + emb(conn, 2, 12)\\
        &:=& \mathbf{V_{\text{conn}}} + \mathbf{W_{conn_2}} onehot(12)
    \end{array}$
    \end{minipage}
    \caption{An example of embedding a simple fact base using the embedding scheme of \cref{fig:graph-embedding}. The shown graph illustrates the neighborhoods $N_0$ and $N_1$ induced by the \texttt{conn} fact.}
    \label{fig:graph-encoding-example}
\end{figure}

\begin{figure}
    $$
    \begin{array}{rcl}
    z_j &:=& h_j + Drop(\mathlarger{\sum_{N_i}} h'_{GAT_i})\\
    h'_j &:=& FFN(Norm(z_j))\vspace{11pt}\\
    FFN(x_j) &:=& Norm(Lin2(Drop(Lin1(x_j)))))
    \end{array}
    $$
    \caption{
        The recurrence relation of a node $j$'s representation $h_j$. $h'_{GAT_i}$ represents the output of a graph attention layer operating with neighborhood $N_i$ according to \cite{velivckovic2017graph}, $h_j$ the representation of node $j$ at the previous step. $Norm$ refers to batch normalization \cite{ioffe2015batch}, $Drop$ to dropout regularization \cite{hinton2012improving} and $Lin1$ and $Lin2$ to linear layers with an inner dimension of $4N$.
    }
    \label{fig:recurrence}
\end{figure}

\subsection{Synthesizer Model}
\label{sec:graph-transformer}

For an illustration of the synthesizer model's architecture, please see Figure~\ref{fig:architecture}. Given a fact base $\mathcal{F}$ we first apply our embedding scheme as described in \cref{sec:graph-embedding}. We then employ a 2-layer GNN-based encoder network to produce the latent representation of a synthesis input.
Given this representation, a processors network is trained to perform the actual synthesis task in high-dimensional space. Last, we apply a set of decoder networks, to obtain the synthesized values of unknown parameter, given the latent synthesis~output.

%In this context, the synthesis problem for network configurations corresponds to completing partially provided fact bases.

% \paragraph{High-Level Architecture}

% We employ the high-level architecture to obtain the latent synthesis output $y_\mathcal{F}$:
% $$
% \begin{array}{rcl}
%     \mathbf{x_{\mathcal{F}}} &:=& Encoder(Embedding(\mathcal{F}))\\
%     \mathbf{y_{\mathcal{F}}} &:=& Processor(\mathbf{x_{\mathcal{F}}} + \mathbf{z})\\
%     z_i &\sim& \mathcal{N}(0,1)
% \end{array}
% $$
% \todo{z is only added for $i<N/2$}

% $Embedding$ corresponds to the graph-based embedding as discussed in \cref{sec:graph-embedding} and $Encoder$ is a 2-layer graph attention module. $Processor$

\paragraph{Encoding} The encoder GNN operates on the embedded representation of a fact base. It produces the high-dimensional representation of a synthesis input as required for the processor network. We additionally apply noise to the first half of the units of the latent representation via $\mathbf{z}$, as a source of non-determinism. According to our experiments this improves model performance and we hypothesize this is due to the synthesis problem having more than one solution in most cases.

\paragraph{Iterative Processor} The processor network is modelled as an iterative process. It consists of a 6-layer graph attention module which we apply for a total of 4 iterations. In the framework of neural algorithmic reasoning, this iterative computational structure encodes an inductive bias towards an iterative solution to the synthesis problem. Because of this bias, our processor network essentially learns an algorithmic procedure which iteratively synthesizes the values of unknown parameters in a fact base.

\paragraph{Graph Attention Layer} In the GNNs we employ, we rely on a composed variant of the graph attention layer as introduced by \cite{velivckovic2017graph}. We employ multiple graph attention layers in lockstep, one per neighborhood $N_i$ defined by our graph embedding (cf. \cref{sec:graph-embedding}), and combine the intermediate results after each step. Specifically, the recurrence relation of a node $j$'s representation $h_j$ is defined as shown in \cref{fig:recurrence}. These mechanics of combining the results of the different graph attention layers $h'_{GAT_i}$, directly corresponds to how multiple attention heads are combined in the original Transformer architecture \cite{vaswani2017attention}.

\paragraph{Argument Decoder Networks} To synthesize the values of unknown parameters, the model maintains a set of decoder networks. That is, it provides one decoder network per integer argument per fact type in a fact base. When decoding, the network is applied to the latent synthesis output of the corresponding fact node. For example, a synthesizer model which operates on the fact base in \cref{fig:datalog-encoding}, would provide a decoder network $D_{\text{connected}_2}: \mathbb{R}^D \rightarrow \mathbb{R^N}$ to decode values for the third argument of a \texttt{conn} fact. In our experiments, decoder networks are implemented as simple multi-layer perceptron models.

\paragraph{Supervision Signal} During training, we mask all fact arguments that represent to-be-synthesized configuration parameters in our synthesis setting. As a supervision signal we use the masked values as the ground-truth and apply a negative log-likelihood loss function to the output distribution of the corresponding argument decoder networks.

%The synthesizer model learns a conditional distribution of fact bases which are consistent with respect to the protocols' semantics.

%\todo{introduce synthesis as a completion problem of an encoded fact base (a la BERT). Introduce masking, introduce decoding of integer and truth values. Synthesis is learning a conditional distribution of consistent fact bases.}

%Using this method, we obtain the node features $h_c$ per constant, $h_f$ per fact and adjacency information in terms of node neighborhood functions $N_i(h_c)$ and $N_i(h_f)$. Overall, this encoding makes a fact base suitable for processing using standard graph neural networks.

%- Brief description of the Graph Transformer Model
\subsection{Multi-Shot Sampling}
\label{sec:decoding-sampling}

%Multi-Stage Parameter Sampling (sampling methods: topk, high-temp, low-temp)
To sample concrete values from the output distributions over unknown parameters, we apply a multi-shot sampling strategy. That is, we sample values only for a subset of unknown parameters, insert them in our input fact base and run the synthesis model again. We repeat this process until no more unknown parameters remain. This multi-shot sampling strategy allows the model to incorporate the concrete values of previously synthesized parameters in its computation. In our evaluation in \cref{sec:evaluation}, we include a comparison of how this compares to sampling all unknown parameters at once.

%In a fact base with multiple holes, we apply the corresponding decoder networks to obtain a value distribution for each integer hole. However, instead of sampling all integer holes in one


==> diff/git-latexdiff.33882/new/sections/3_bgp_ospf.tex <==
\section{BGP/OSPF Synthesis}
\label{sec:bgp-ospf}

\newcommand{\as}{\ac{AS}~}
\newcommand{\ases}{\acp{AS}~}

\newcommand{\squareann}{{\tiny$\blacksquare\;$}}
\newcommand{\triangleann}{{\small$\blacktriangle\;$}}

\begin{figure*}
    \centering
    \includegraphics[width=0.95\textwidth]{figures/networks-all.pdf}
    \caption{(a) An illustration of a small AS network, including internal peers (blue), external peers (purple), BGP sessions as well as physical links. (b) The propagation of two BGP announcement across the network. (c) The resulting forwarding plane after applying BGP and OSPF.}
    \label{fig:network-fwd-tree}
\end{figure*}

We now discuss an instantiation of our learning-based framework for the case of BGP and OSPF protocols. In \cref{sec:synthesis-setting} we introduce a basic networking model, BGP and OSPF protocols and the synthesis setting. Given this model, \cref{sec:training} describes how to generate a corresponding dataset of input/output samples and train a synthesizer model.
%This shall serve as a prerequisite to the instantiation of our learning-based synthesis framework for the BGP and OSPF protocol in \cref{sec:training}.

\subsection{Synthesis Setting}
\label{sec:synthesis-setting}

\paragraph{Graphical Model} We assume an abstract network model which can be represented as an undirected graph as shown in \cref{fig:network-fwd-tree} (a). We always consider a set of internal routers (A, B, C, D in \cref{fig:network-fwd-tree}) as well as a set of adjacent external routers (E, F  in \cref{fig:network-fwd-tree}). The group of internal routers forms the \emph{\as} under consideration whereas external routers belong to other adjacent \ases. In practice, an \as represents an administrative domain controlled by a single operator. 

\paragraph{Forwarding Plane} For an example of a possible forwarding plane in this abstract model, consider \cref{fig:network-fwd-tree} (c) which illustrates the forwarding plane of traffic destined towards some destination reachable via external peer $E$ or $F$. Each router of the network forwards traffic along some of its outgoing links. In practice, a number of protocols are used to compute the forwarding plane. However, here we focus on OSPF and BGP.

\paragraph{OSPF} The OSPF protocol \cite{moy1994ospf} is a link-state protocol, typically used as an interior gateway protocol~(IGP), i.e., to route traffic within an \ac{AS}. Given link weights per physical link in the network, OSPF simply routes traffic along the shortest path towards the destination.

\paragraph{BGP} The BGP protocol \cite{rekhter1994border} on the other hand is a path-vector protocol used to exchange reachability information mostly on the level of \acp{AS}.
%These are groups of routers typically operated by a single party (e.g. an ISP).
When using BGP, a routing destination announces its existence to other \ases and routers, by sending out a BGP announcement. Receivers of such announcements may then choose to pass them on to other \acp{AS}, redistribute them internally and/or modify them. Instead of communicating along physical links directly, the BGP protocol requires manually configured BGP sessions among routers of the \as and external peers, as indicated by the BGP session edges in \cref{fig:network-fwd-tree}(a).
%\todo{more discussion of eBGP vs iBGP and support for route reflection (more of an implementation detail, maybe only mention in dataset generation where simulation code is discussed)}.

%\paragraph{BGP Decision Procedure}~
%\todo{discuss decision procedure}
In case a router receives more than one announcement for a destination, a designated BGP decision process is applied to determine a single best route. \cref{fig:bgp-decision} shows the ordered list of comparison criteria of this decision process. The different criteria depend different properties of a route announcements, including the IGP cost towards the routing destination. As a consequence, when used together, OSPF as IGP protocol and BGP will interact. %Note also that BGP is an iterative process which needs multiple rounds of propagation to converge.

\paragraph{Example}
%\todo{run through simple BGP+OSPF example of computing the forwarding plane}
To better understand BGP/OSPF routing, consider the simple example given in \cref{fig:network-fwd-tree} (b). Here, our example \as imports BGP announcements \squareann and \triangleann from E and F respectively. Both represent a route to the same destination. As shown, both announcements have a so-called local preference of 2. For simplicity, we ignore other properties such as the AS path length, Origin and MED in this example. The announcements are propagated among BGP neighbors and the best route is selected according to the decision procedure in \cref{fig:bgp-decision}. See \cref{fig:network-fwd-tree} (b) for an illustration of the intermediate states of this propagation process. As both announcements have a local preference of 2, rule 1 of the decision process is not used. Instead, in round 2, node B selects \squareann over \triangleann due to a lower IGP cost of 2 via egress node A as compared to 3 via egress node D (rule 6). Node D selects \triangleann over \squareann, since it learns this route directly from an external peer (rule 5). After Round 3, the BGP propagation process converges to a stable state and we can derive the forwarding plane as shown in \cref{fig:network-fwd-tree} (c).


%, as well as external peers E and F which belong to other \acp{AS}. External peers are routers which are connected via eBGP sessions to routers of the \ac{AS} under consideration. They announce BGP routes to their neighbors, which are propagated within the network

%\paragraph{BGP/OSPF Configuration Synthesis} We phrase the BGP/OSPF configuration synthesis problem on the level of the forwarding plane. This means that users provide a specification which constraints the set of allowed forwarding planes. This includes predicates which enforce forwarding paths, block forwarding paths or assert higher-level properties like traffic isolation and reachability. Given such a specification, we consider network configuration synthesis as the task of configuring OSPF and BGP in a way that produces a forwarding plane which satisfies the provided specification.

\paragraph{BGP/OSPF Configuration Synthesis} According to our general synthesis framework, we consider the BGP/OSPF configuration synthesis problem at the level of the forwarding plane. However, we further also define the set of synthesized parameters: For OSPF we synthesize link weights as explored in a wide range of existing work (e.g. \cite{el2018netcomplete,fortz2000internet}. For BGP, the set of parameters is not defined as clearly: Depending on the requirements of a network operator, one may employ custom BGP import and export policies at every router of a network to implement complex behavior. However, in this instantiation we focus on a simplified setting, where we assume BGP route announcements to only be modified when imported into the \as from an external peer. Previous work has already pointed out that this is a reasonable assumption which holds for the majority of real-world networks \cite{caesar2005bgp,cittadini2010doing, steffen2020probabilistic}.

\begin{figure}
    \small{
    \begin{enumerate}
        \setlength{\itemsep}{0pt}
        \setlength{\parskip}{0pt}
        \item Highest Local preference
        \item Lowest AS path length
        \item Prefer Origin (IGP $>$ EBGP $>$ INCOMPLETE)
        \item Lowest Multi-exit discriminator (MED)
        \item External over internal announcements
        \item Lowest IGP cost to egress
        \item Lowest BGP peer id (tie breaker)
    \end{enumerate}}
    \vspace{-15pt}
    \caption{The BGP decision process \cite{rekhter1994border}. The shown rules are applied in order until a single best BGP announcements remains.}
    \label{fig:bgp-decision}
\end{figure}

\subsection{Dataset Generation and Training}
\label{sec:training}
To train a synthesizer model, we need a large number of fact bases encoding a variety of network topologies, configurations and forwarding specifications. Further, we must provide the model with target values for unknown parameters as a supervision signal. This section discusses how we construct such a dataset for BGP/OSPF synthesis.
%Further, we provide an example of what a corresponding fact base looks like, including a description of the supported specification language.

\paragraph{Dataset Generation} To obtain network configurations and corresponding forwarding specifications we employ a generative process: We first randomly configure BGP and OSPF parameters for some topology. Then we simulate the OSPF and BGP protocol and compute the resulting forwarding plane. Based on this, we extract a forwarding specification which fixes a random subset of forwarding paths, reachability and isolation properties that are satisfied by the forwarding plane.

\paragraph{Topologies} For training, our dataset is based on random topologies with $16$-$24$ routers. We generate the physical layout of these graphs by triangulation of uniformly sampled points in two-dimensional space.

\paragraph{Simulation} To compute the forwarding plane given an OSPF and BGP configuration, we simulate the protocols. For OSPF, we implement shortest path computation to obtain the forwarding plane. For BGP, we implement the full BGP decision process as shown in \cref{fig:bgp-decision}, except for the MED attribute. In addition to the basic networking model discussed in \cref{sec:synthesis-setting}, we implement support for eBGP and iBGP, fully-meshed BGP session layouts as well as layouts relying on route reflection. For more details of these BGP concepts see \cite{bates2000rr}.

%Note that the synthesizer model will reason on the level of the provided training samples. That is, to improve the overall synthesis quality in a real-world setting, it is helpful to implement simulation code which behaves very similar to real-world networks. Another promising approach would be to extract training samples from real-world networks, thereby circumventing the need for simulation, however, we leave this as future work.

%While this can be a considerable effort, it is typically an easier task than to implement the synthesizer directly. The concrete semantics of protocols and their simulation is a well-defined procedure, whereas implementing efficient synthesis tools is still an open problem.

\paragraph{Fact Base Encoding} We encode synthesis input using a small set of facts. For an example of a corresponding fact base see \cref{fig:bgp-ospf-fact-base}. We use the \texttt{router}, \texttt{external} and \texttt{network} facts to mark routers, external peers and routing destinations respectively. Physical links between routers are encoded as \texttt{connected(R1,R2,W)} facts where \texttt{W} denotes the OSPF link weight. Further, we rely on \texttt{ibgp}, \texttt{ebgp}, \texttt{route\_reflector} and \texttt{bgp\_route} facts to represent different types of BGP sessions and imported routes. Using the notion of unknown parameters as discussed in \cref{sec:graph-embedding}, we encode configuration parameters, e.g., properties of imported routes or OSPF link weights.

\paragraph{Specification Language} We support a small specification language with three types of forwarding predicates:

\begin{itemize}
    \setlength{\itemsep}{0pt}
    \setlength{\parskip}{2pt}
    \item \texttt{fwd(R1, Net, R2)} specifies that router \texttt{R1} forwards traffic destined for \texttt{Net} to its neighbor \texttt{R2}.
    \item \texttt{reachable(R1, Net, R2)} specifies that traffic destined for \texttt{Net} that passes through \texttt{R1} also passes through \texttt{R2} before reaching its destination.
    \item \texttt{trafficIsolation(R1, R2, N1, N2)} specifies that it must not hold that $[fwd(R1,R2,N1)]_{\mathcal{B}} \wedge [fwd(R1,R2,N2)]_{\mathcal{B}}$.
\end{itemize}

In the negative case of each predicate, the opposite must hold true for the fact to be satisfied. This specification language can easily be extended by including new specification predicates in the dataset generation process. One must simply provide a method of extracting positive and negative cases of a specification fact from a given forwarding plane. Once included in the training dataset of a synthesizer model, the resulting synthesis system will be able to consider specifications relying on the new type of predicates.

% \todo{info on loss function, optimizer, etc.}
\paragraph{Training} We generate a dataset of $10,240$ input/output samples and instantiate our synthesizer model with a hidden dimension $D$ of $64$. For optimization, we use the Adam optimizer \cite{kingma2014adam} with a learning rate of $10^{-4}$. We stop training after the specification consistency on a validation dataset no longer increases at $\sim2800$ epochs.

\begin{figure}
\begin{minipage}[t]{0.22\textwidth}
\begin{lstlisting}[basicstyle=\ttfamily\tiny]
# topology and configuration
router(c5)
router(c3)
router(c1)
router(c0)
network(c6)
network(c7)

external(c8)
external(c9)
external(c10)
external(c11)
external(c12)
external(c13)

route_reflector(c2)
route_reflector(c4)

connected(c2,c4,?)
connected(c2,c5,?)
connected(c2,c3,?)
connected(c4,c5,?)
connected(c4,c3,?)
connected(c4,c0,?)
connected(c5,c1,?)
connected(c5,c0,?)
connected(c3,c0,?)
connected(c3,c1,?)
connected(c1,c0,?)

ibgp(c2,c4)
ibgp(c2,c5)
ibgp(c2,c0)
ibgp(c2,c1)
ibgp(c4,c3)
ibgp(c4,c4)
\end{lstlisting}
\end{minipage}
\begin{minipage}[t]{0.2\textwidth}
\begin{lstlisting}[basicstyle=\ttfamily\tiny]
ebgp(c2,c12)
ebgp(c5,c9)
ebgp(c5,c10)
ebgp(c5,c13)
ebgp(c0,c8)
ebgp(c0,c11)

bgp_route(c8,c6,?,?,1,?,1,8)
bgp_route(c9,c6,?,?,0,?,1,9)
bgp_route(c10,c6,?,?,0,?,1,10)
bgp_route(c11,c7,?,?,0,?,1,11)
bgp_route(c12,c7,?,?,0,?,1,12)
bgp_route(c13,c7,?,?,2,?,1,13)

# forwarding specification
fwd(c0,c6,c3)
fwd(c3,c6,c2)
fwd(c2,c6,c4)
not fwd(c3,c6,c0)
not fwd(c0,c6,c11)
not fwd(c11,c6,c0)

not trafficIsolation(c1,c0,c7,c6)
not trafficIsolation(c1,c0,c7,c6)
trafficIsolation(c0,c3,c6,c7)
trafficIsolation(c0,c3,c6,c7)

reachable(c5,c6,c10)
reachable(c1,c6,c4)
not reachable(c0,c6,c5)
reachable(c5,c6,c10)
\end{lstlisting}
\end{minipage}
\caption{An example of a fact base encoding a topology, a sketch of a BGP and OSPF configuration and a forwarding specification.}
\label{fig:bgp-ospf-fact-base}
\end{figure} 

==> diff/git-latexdiff.33882/new/sections/4_evaluation.tex <==
\section{Evaluation}
\label{sec:evaluation}

We trained a synthesizer model to perform configuration synthesis for BGP and OSPF. We now assess the performance of the resulting neural synthesizer with respect to two core metrics: (1) the quality of synthesized configurations in terms of their consistency with the provided forwarding specifications (\cref{sec:synthesis-quality}), and (ii) the time a learned synthesizer takes when compared to the state-of-the-art SMT-based synthesizer NetComplete \cite{el2018netcomplete} (\cref{sec:synthesis-vs-smt}).

\paragraph{Dataset} We compare across three datasets: Small, Medium and Large. Each dataset represents 8 real-world topologies, sampled from the Topology Zoo \cite{knight2011internet}, where the number of nodes lies between 0-34, 34-68 and 68-170 respectively. To obtain forwarding specifications for the sampled topologies, we use our generative pipeline as discussed in \cref{sec:training}. In each topology, we do synthesis for 4 different traffic classes (routing destinations) at a time.

\paragraph{Experimental Setup} We run all our experiments on an Ubuntu Linux machine with an Intel(R)~Core(TM)~i9-9900X~@~3.50GHz processor, 64GB of system memory and an NVIDIA GeForce RTX 3080 GPU with 10GB of video~memory.

\subsection{Synthesis Quality}
\label{sec:synthesis-quality}
To assess our learned synthesizer, we examine its behavior with increasingly large topologies and specifications.

\paragraph{Specifications} Using the same generative model as described in \cref{sec:training}, we generate forwarding specifications for the topologies in our three datasets with each specification constructed from $3 \times n$ requirements, one per supported predicate type:  \texttt{fwd} requirements correspond to specifying or blocking a forwarding path using multiple \texttt{fwd} predicates whereas \texttt{reachable} and \texttt{trafficIsolation} requirements each translate to a single specification fact. We compare across increasingly large specifications of $3\times 2$, $3\times 8$ and $3 \times 16$ requirements, respectively.

\paragraph{Methodology} For each pair of topology and specification, we run our synthesizer 5 times and report the network configurations with the highest overall consistency value. For sampling, we rely on our multi-shot sampling strategy where we randomly group the unknown parameters of a configuration into 4 groups (4-shot sampling).

\paragraph{Results} We summarize our results in \cref{fig:eval-consistency}. On average, our synthesis model produces network configurations that are $>91\%$ consistent with the provided forwarding specifications across all datasets and sizes of specifications. When only few requirements are given, the synthesizer model even succeeds in producing fully-consistent configurations. We observe a slightly decreasing consistency with increasingly large topologies.

%\texttt{fwd} facts are satisfied more easily, whereas \texttt{reachable} and \texttt{trafficIsolation} facts are violated more often.

\paragraph{Multi-Shot Sampling} In \cref{fig:eval-consistency-baseline}, we report the average specification consistency using our multi-shot sampling strategy as compared to sampling all unknown parameters at once. As a baseline we have also sampled random configurations from a uniform distribution (per parameter) and compute the corresponding specification consistency. Over the baseline, our synthesizer model shows clear improvement and multi-shot sampling further increases consistency.

\begin{figure*}
    \begin{center}
        \textbf{Specification Consistency}\\
        \footnotesize
        \begin{tabular}{rrcccccccccc}
        \toprule
        \multicolumn{2}{c}{Dataset} & \tiny\texttt{fwd} & \tiny\texttt{reachable}  & \tiny\texttt{trafficIsolation} & Overall & $\emptyset$     No. Full Matches & $\emptyset$ No. $>90\%$ Matches\\
        \midrule
        $3\times 2$ requirements & Small & 0.95 & 0.94 & 1.00 & \textbf{0.95} & 0.62 & 0.62\\
& Medium & 0.96 & 1.00 & 0.94 & \textbf{0.96} & 0.88 & 0.88\\
& Large & 0.94 & 0.94 & 1.00 & \textbf{0.93} & 0.62 & 0.62\\
\midrule
$3\times 8$ requirements & Small & 0.97 & 0.98 & 0.97 & \textbf{0.98} & 0.50 & 1.00\\
& Medium & 0.99 & 0.95 & 1.00 & \textbf{0.98} & 0.50 & 1.00\\
& Large & 0.96 & 0.95 & 0.91 & \textbf{0.94} & 0.38 & 0.88\\
\midrule
$3\times 16$ requirements & Small & 0.97 & 0.89 & 0.95 & \textbf{0.94} & 0.38 & 0.75\\
& Medium & 0.98 & 0.97 & 0.97 & \textbf{0.98} & 0.38 & 1.00\\
& Large & 0.92 & 0.88 & 0.95 & \textbf{0.91} & 0.12 & 0.50\\
    \end{tabular}\end{center}
    \caption{Average specification consistency of the network configurations synthesized by our trained synthesizer model. Per sample we run the synthesizer with a specification of $3\times N$ requirements, where the specifications always include $N$ requirements per supported predicate type (\texttt{fwd}, \texttt{reachable}, \texttt{trafficIsolation}).}
    \label{fig:eval-consistency}
\end{figure*}

\begin{figure}
    \begin{center}
        \footnotesize
        \begin{tabular}{rrcccccccccc}
        &  & \multicolumn{2}{c}{Neural}\\
        & Random & 1-Shot & 4-shot\\
        \toprule
        Small & 0.83 & 0.92 & \textbf{0.94} \\
        Medium & 0.88 & 0.95 & \textbf{0.98} \\
        Large & 0.78 & 0.88 & \textbf{0.91} \\
    \end{tabular}\end{center}
    \caption{Average specification consistency with $3\times 16$ requirements when sampling configurations randomly from a uniform distribution and 1-shot/4-shot sampling using our synthesizer model.}
    \label{fig:eval-consistency-baseline}
\end{figure}

\begin{figure*}[ht]
    \footnotesize
    \begin{center}
        \textbf{BGP Synthesis Time}
        \footnotesize
        \begin{tabular}{rrccccccccc}
        \toprule
        &&\multicolumn{3}{c}{Synthesis Time (s)} & \multicolumn{2}{c}{Accuracy (Neural)} \\
        \multicolumn{2}{l}{\# Requirements} & NetComplete & Neural (CPU) & Speedup &$\emptyset$ Consistency& $\emptyset$ No. Full Matches\\
        \midrule
    2 requirements &Small & 18.073s & 0.641s & \textbf{28.2x} & 0.969 & 0.875\\
        &Medium & 60.864s & 2.748s & \textbf{22.2x} & 0.939 & 0.75\\
        &Large & 1389.485s\tiny{  7/8 TO} & 22.301s & \textbf{62.3x} & 0.989 & 0.875\\
    \midrule
    8 requirements &Small & 247.691s & 1.065s & \textbf{232.5x} & 0.96 & 0.75\\
        &Medium & $>$25m\tiny{  8/8 TO} & 3.47s & \textbf{432.2x} & 0.968 & 0.5\\
        &Large & $>$25m\tiny{  8/8 TO} & 30.961s & \textbf{48.4x} & 0.969 & 0.75\\
    \midrule
    16 requirements &Small & 1416.828s\tiny{  7/8 TO} & 2.528s & \textbf{560.5x} & 0.926 & 0.25\\
        &Medium & $>$25m\tiny{  8/8 TO} & 5.481s & \textbf{273.7x} & 0.947 & 0.25\\
        &Large & $>$25m\tiny{  8/8 TO} & 69.092s & \textbf{21.7x} & 0.959 & 0.25\\
    \end{tabular}\end{center}
    \caption{Comparing consistency and synthesis time of our method (Neural) with the SMT-based state-of-art synthesis tool NetComplete. The notation {\tiny{n/8 TO}} indicates the number of timed out synthesis runs out of 8 (25+ minutes).}
    \label{fig:evaluation-compare-bgp}
\end{figure*}

\begin{figure*}[ht]
    \begin{center}
        \footnotesize
        \textbf{OSPF Synthesis Time}\\
        \footnotesize
        \begin{tabular}{rrccccccccc}
        \toprule
        &&\multicolumn{3}{c}{Synthesis Time (s)} & \multicolumn{2}{c}{Accuracy (Neural)} \\
        \multicolumn{2}{l}{} & NetComplete & Neural (GPU) & Speedup &$\emptyset$ Consistency& $\emptyset$ No. Full Matches\\
        \midrule
    2 requirements &Small & 0.265s & 0.091s & \textbf{2.9x} & 1.000 & 1.00\\
     &Medium & 0.404s & 0.098s & \textbf{4.1x} & 1.000 & 1.00\\
     &Large & 0.944s & 0.14s & \textbf{6.7x} & 1.000 & 1.00\\
    \midrule
    8 requirements &Small & 0.876s & 0.164s & \textbf{5.3x} & 0.982 & 0.75\\
     &Medium & 1.517s & 0.103s & \textbf{14.7x} & 1.000 & 1.00\\
     &Large & 3.505s & 0.316s & \textbf{11.1x} & 0.981 & 0.50\\
    \midrule
    16 requirements &Small & 1.65s & 0.21s & \textbf{7.9x} & 0.991 & 0.625\\
     &Medium & 2.646s & 0.245s & \textbf{10.8x} & 0.989 & 0.50\\
     &Large & $>$566.636s+\tiny{  3/8 TO} & 0.233s & \textbf{2430.4x} & 0.987 & 0.875\\
    \end{tabular}\end{center}
    \caption{Comparing consistency and synthesis time of our method (Neural) with the SMT-based OSPF synthesis tool NetComplete. The notation {\tiny{n/8 TO}} indicates the number of timed out synthesis runs out of 8 (25+ minutes).}
    \label{fig:evaluation-compare-ospf}
\end{figure*}


\subsection{Comparison to SMT-based Synthesis}
\label{sec:synthesis-vs-smt}

%To provide a comparison of our learned BGP/OSPF synthesizer with SMT-based methods,
We now compare the synthesis time of the learned neural synthesizer with those of NetComplte, a state-of-art configuration synthesis tool based on SMT-solvers \cite{el2018netcomplete}.

\paragraph{Specifications} As the type of supported requirements in NetComplete does not fully align with our model, we restrict this comparison to specifications which only include forwarding paths (i.e. \texttt{fwd} predicates). Further, NetComplete does not support cross-protocol synthesis as in our case and instead requires users to specify for each requirement the protocol to use for its implementation. To bridge this gap, we split the generated forwarding requirements into BGP and OSPF paths for a corresponding NetComplete specification.
%\todo{note on NetComplete installing policies at all routers, not only the edges of the AS}

\paragraph{Methodology} We compare both OSPF synthesis and BGP/OSPF-synthesis. We configure our trained synthesizer model to do OSPF synthesis by only predicting link weights. For each pair of topology and specification, we report the total time of running our synthesizer 4 times using 4-shot sampling, whereas for consistency we report the best out of the 4 runs. For NetComplete, we run the synthesizer with a timeout of 25 minutes. In case a NetComplete attempt times out, we report 25 minutes as a lower bound for its runtime.

\paragraph{OSPF Synthesis Time Results} We document the results of comparing OSPF synthesis time in \cref{fig:evaluation-compare-ospf}. Our synthesizer model achieves a speedup of 2-10x over NetComplete. With 16 requirements and dataset Large this speedup even increases to $2000\times$. Further, our model achieves very high consistency with the provided specification, often producing fully-consistent configurations.

\paragraph{BGP/OSPF Synthesis Time Results} In \cref{fig:evaluation-compare-bgp} we show the comparison of BGP/OSPF synthesis time. Our synthesizer model outperforms NetComplete by multiple orders of magnitude. We observe a speedup of $20-560\times$ which appears to increase with the size of topology and specification. Further, the average specification consistency of the synthesized configurations is greater than $92\%$ across all datasets, even for large topologies. In many cases, our synthesizer model produces fully-consistent configurations, especially with small topologies and specifications. In comparison, NetComplete times out on more than half of the synthesis tasks which means that we can only observe a lower bound of speedup in these cases. Note that our synthesizer model is running on a CPU due to memory restrictions with large topologies. However, running it on a GPU results in even greater speedups (up to $1000\times$, cf. \cref{app:sec:bgp-gpu-performance}). 

==> diff/git-latexdiff.33882/new/sections/5_related_work.tex <==
\section{Related Work}
\label{sec:related-work}

\paragraph{Traditional Configuration Synthesis} 
%A range of existing work is concerned with network configuration synthesis. 
Next to methods based on compilation such as Propane/PropaneAT \cite{beckett2017network}, there are a number of configuration synthesis methods based on constraint solving: Examples include ConfigAssure \cite{narain2008declarative}, SyNet \cite{el2017network} and NetComplete \cite{el2018netcomplete}. Due to their hand-coded nature, these methods are highly protocol-specific and can be very slow due to the solvers they employ. Although some of them allow for cross-protocol reasoning, this is not implemented as transparently as in our framework and users must specify per requirement which protocol to use for its implementation. In contrast, our approach has lower precision but allows for fully transparent cross-protocol reasoning, meaning forwarding requirements are not protocol-bound and the synthesizer chooses how to implement them. Further, our learned BGP/OSPF synthesis tool exhibits much lower synthesis times as compared to an SMT-based tool like NetComplete.

% \begin{itemize}
%     \item NetComplete, SyNet
%     \item Propane, PropaneAT
%     \item DeepBGP
% \end{itemize}

\paragraph{GNNs and Networking} DeepBGP \cite{bahnasy2020deepbgp} relies on GNNs and reinforcement learning to do configuration synthesis. However, it is limited to BGP configuration synthesis and is slower than SMT-based synthesis according to the author's evaluation. In contrast, our learning-based framework is cross-protocol, does not rely on reinforcement learning and provides better synthesis performance. Apart from configuration synthesis, GNNs have also been applied to other problems in the networking domain. For example, the authors of RouteNet \cite{rusek2020routenet} use GNNs to predict performance metrics of network configurations. Other work that is concerned with learning improved protocols includes Q-Routing \cite{boyan1994packet} or more modern approaches such as the Graph-Query Neural Network architecture \cite{geyer2018learning}.

\paragraph{Neural Algorithmic Reasoning} 
Neural algorithmic reasoning (NAR) as proposed in \cite{velivckovic2021neural}, describes the idea of replacing traditional algorithms with neural networks to learn improved algorithmic procedures. Exemplary work includes graph-related algorithms \cite{velivckovic2019neural} or solvers for combinatorial optimization problems \cite{cappart2021combinatorial,joshi2020learning,selsam2019guiding}. Our synthesis framework is the first applications of NAR to the networking domain and relies on the NAR-native encode-process-decode architecture. According to the hierarchy of NAR approaches in \cite{cappart2021combinatorial}, our method is an algorithm-level approach, as we do not supervise on intermediate steps. Although, such step-level methods promise better generalization, it is not clear what an intermediate result of a general synthesis procedure would be. However, future work on a step-level approach may further improve synthesis quality.

% \begin{itemize}
%     \item RouteNet
%     \item GraphNET
%     \item Learning and generating distributed routing protocols using graph-based deep learning
%     \item Unveiling the potential of Graph Neural Networks for network modeling and optimization in SDN
% \end{itemize}

==> diff/git-latexdiff.33882/new/sections/6_conclusion.tex <==
\setlength{\parskip}{6pt plus4mm minus4mm}
\section{Conclusion}
\label{sec:conclusion}
We presented a learning-based framework for configuration synthesis based on the idea of neural algorithmic reasoning. To assess the effectiveness of the system, we instantiated it for the case of BGP/OSPF synthesis. In contrast to traditional synthesis methods, our system supports transparent cross-protocol reasoning and learns synthesis rules only from data. Using our system, synthesis is sped up by a factor of up to $500\times$ when compared to SMT-based methods. Further, our evaluation demonstrates that the resulting synthesis tool provides excellent synthesis quality, producing configurations with high specification consistency. Overall, our results illustrate that exploring the direction of learning-based network configuration synthesis is a promising direction, enabling new cross-protocol reasoning capabilities and great performance improvements. Promising future work includes construction of hybrid systems, integrating both neural models and SMT-based approaches to obtain the best of both worlds.

==> diff/git-latexdiff.33882/old/acronyms.tex <==
\DeclareAcronym{AS}{
    short = AS,
    long = autonomous system,
    short-plural = es ,
    long-plural = s
}

==> diff/git-latexdiff.33882/old/sections/0_abstract.tex <==
% Context
Computer networks employ a number of different protocols to enable efficient routing. However, due to the complexity of multiple interacting protocols, it can be hard for network operators to implement high-level routing policies and requirements. Network configuration synthesis promises to address this situation by automatically generating configurations that satisfy a provided specification. However, existing synthesis methods are often limited to single-protocol reasoning, depend on protocol-specific and hand-coded synthesis rules, and are difficult to scale due to the SMT-based methods they employ. In this work we present a rather different, learning-based method for addressing the configuration synthesis challenge, one based on the recently proposed paradigm of neural algorithmic reasoning. Our framework is protocol-agnostic, enables cross-protocol reasoning and does not depend on any hardcoded synthesis rules. To evaluate, we instantiate our framework for the case of BGP/OSPF synthesis. Our experiments show we can synthesize configurations with a very high degree of specification consistency while observing speedups of up to $500\times$ compared to a state-of-the-art SMT-based synthesis tool.


==> diff/git-latexdiff.33882/old/sections/1_intro.tex <==
\section{Introduction}
\label{sec:introduction}

The backbone of the internet consists of many connected computer networks operated by different internet service providers (ISPs) and other large organizations. These networks rely on a number of protocols to enable effective and policy-driven routing of traffic. Based on router-level configurations, the protocols perform a distributed computation to construct a network's forwarding state. However, the relatively low-level router configuration makes it hard for network operators to directly enforce network-wide policies and requirements. This often leads to misconfiguration, which can cause global outages such as the recent hours-long blackout of the entire Facebook platform \cite{janardhan2021} and comparable events \cite{mccarthy_2019}.
%
\paragraph{Configuration Synthesis} This situation has triggered a number of research efforts regarding the synthesis of network configurations \cite{el2018netcomplete,beckett2017network,narain2008declarative}. Configuration synthesis is concerned with the task of automatically generating router-level configurations given a set of high-level requirements. However, this synthesis problem can be very hard to solve, since network configurations typically consist of a considerable number of tunable parameters, where the execution of several interacting protocols yields the overall forwarding state. An effective synthesis tool must thus account for this fact and be able to reason across multiple protocols.

\paragraph{SMT-based Synthesis} Some of the most successful efforts in providing cross-protocol synthesis capabilities are based on satisfiability modulo theory (SMT) solvers \cite{el2018netcomplete,el2017network}. While SMT-based synthesis is a promising method, it comes with a number of limitations:
% \item protocol-specific
% fully hand-coded synthesis rules, a lot of implementation effort, cross-protocol support extra complicated
(1) SMT-based synthesizers are hand-crafted and highly protocol-specific. To implement synthesis, we must first express our networking model, protocol semantics including vendor and device specific behavior in terms of first-order logic constraints. This is a time-intensive and complicated process, requiring lots of expert knowledge.
%  model-dependent: synthesis is reasoning on the level of some assumed model which may not reflect the real world: even if a configuration is synthesized based on some spec, it may behave differently and violate spec in practice
Further, (2) logic-based modelling introduces a disconnect between the synthesis tool and real-world behavior \cite{birkner2021metha}. More specifically, synthesized configurations may satisfy a provided specification within a formal framework, but may not behave the same way in the real world.
% can be very slow
And, (3) SMT-based synthesis can be very slow or fail to complete, especially when reasoning about large network topologies. In practice however, network operators reconfigure their networks on a daily basis \cite{vissicchio2012improving}, which means an effective synthesis tool must be fast.

% \item fully learned, no hand-coded synthesis rules (model-free), very flexible to adapt to more/new protocols
% \item protocol-agnostic, cross-protocol
\paragraph{Neural Algorithmic Reasoning for Synthesis} Recent work on neural algorithmic reasoning (NAR) proposes to replace traditional algorithms with neural networks to learn improved algorithmic procedures \cite{velivckovic2021neural}.
It has been shown to be a powerful and fast algorithmic approximation method for a number of graph-related \cite{velivckovic2019neural} and combinatorial optimization problems \cite{cappart2021combinatorial}. Further, due to its learned nature, NAR allows for learning procedures directly from (real-world) data, without the need for manual feature extraction. Overall, this positions NAR as an attractive method to obtain a fast, fully-learned synthesis procedure, which entirely avoids the need for a formal model or any hand-crafted synthesis rules. Based on this promising outlook, this paper explores how to apply the NAR paradigm to the problem of network configuration synthesis.

To that end, we propose a \textbf{new learning-based framework for configuration synthesis} as an alternative to SMT-based approaches. Our framework is protocol-agnostic, enables cross-protocol reasoning and avoids the need to manually provide synthesis rules. Instead of implementing the synthesizer explicitly, we replace it by an iterative graph neural network which is trained on input/output samples of specifications, topologies and configurations.
%While our approach still requires some protocol-specific implementation efforts, it is limited to implementing the simulation of the involved protocols.
Our method is highly flexible due to its generic nature and can be extended to any protocol. Further, the synthesizer model learns a whole distribution of network configurations. As a consequence, we can directly sample multiple alternative configurations, not possible with standard SMT solvers. We apply our framework to a non-trivial synthesis setting where both the Border Gateway Protocol (BGP) and the Open Shortest Path First (OSPF) protocol are used. We demonstrate that our learned synthesis tool is up to~$500\times$ faster than a state-of-the-art SMT-based synthesizer, while producing configurations which enjoy more than 90\% satisfaction of the given specification.

\paragraph{Main Contributions} Our core contributions are:
\vspace{-5pt}
\begin{itemize}
    \setlength{\itemsep}{5pt}
    \setlength{\parskip}{0pt}
    \item A learning-based framework for network configuration synthesis based on neural algorithmic reasoning.
    \item A neural network architecture for learning synthesizer models which relies on a generic graph-based encoding of network topologies and configurations.
    \item An extensive evaluation of our learning-based synthesizer, in terms of both precision and scalability, on the challenging setting where both BGP and OSPF protocols are involved.
\end{itemize}

\section{Overview}
\label{sec:overview}

\begin{figure}
    \begin{center}
        \includegraphics[width=0.45\textwidth]{figures/synthesizer-overview.pdf}
    \end{center}
    \caption{An overview of our learning-based synthesis framework.}
    \label{fig:learning-based-synthesis}
\end{figure}

We first discuss the core concepts behind our learning-based synthesis framework, illustrated in \cref{fig:learning-based-synthesis}.

\paragraph{Dataset} To train a synthesizer model, we first generate a dataset of input/output samples. For this, we rely on a generative pipeline as shown in the top of \cref{fig:learning-based-synthesis}. First, we sample a random network configuration for some topology using a uniform generative process. Then, we simulate the involved protocols to obtain the corresponding routing behavior. Next, we extract a specification by randomly selecting properties that hold for the simulated routing behavior. This leaves us with a pair of (specification, configuration) added to a dataset of training~samples.

\paragraph{Simulation} Depending on the protocols in use, one implements simulation code to compute the routing behavior induced by a sampled configuration. Although this step is protocol-specific, the overall implementation effort is much lower compared to SMT-based synthesis. Protocols are typically well-defined algorithms which can be simulated, whereas the alternative of implementing a synthesizer often requires expert knowledge about SMT solvers. In practice, our framework may also be adapted to use a real-world network router to compute the behavior of a configuration, thereby capturing the real-world behavior directly.

\paragraph{Neural Synthesizer Model} Given a dataset of pairs each consisting of a configuration and a specification, we now train a graph neural network on this dataset to perform synthesis: given a specification, it tries to predict the configuration. Following the NAR paradigm, we first encode the synthesizer input (specification) in latent space. Then, we apply an iterative processor network which relies on the graph attention mechanism to propagate information \cite{velivckovic2017graph}. Last, we apply a decoder network to extract the synthesized configuration. To remain protocol-agnostic, our model is generic with respect to the input format, using an intermediate representation based on Datalog-like facts.

%More specifically, we employ a slightly modified variant which operates on a graph-based encoding of a specification, topology and configuration parameters.



 \begin{figure*}
     \centering
     \includegraphics[width=0.85\textwidth]{figures/system-overview.pdf}
     \caption{An overview of our synthesis system: (1) First, we use a generic embedding scheme to transform a network topology, protocol configuration sketches and the specification given as Datalog-like facts to a latent input representation. Next, we apply a learned (2) Processor GNN and obtain a latent synthesis output. Last, we apply a (3) Decoder Network to obtain a distribution over possible values per unknown parameter in our configuration.}
     \label{fig:overview-model}
\end{figure*}

\paragraph{Relaxed Specification Consistency} Parts of the configuration synthesis problems are known to be NP-hard \cite{fortz2000internet}. In contrast, our learning-based framework depends on a fixed-size neural network architecture running in polynomial time. Hence, we expect neural synthesis to be less precise than SMT methods and propose the notion of \emph{relaxed~specification~consistency}. That is, to assess the performance of a neural synthesizer, we not only consider if a configuration satisfies a specification, but also the degree up to which it satisfies a specification (e.g., via the relative number of satisfied requirements). This ``soft'' understanding of a specification allows us to evaluate neural synthesis systems which may not always produce fully specification-consistent configurations. Nonetheless, we argue that configurations with less than $100\%$ consistency are still very useful in practice as they provide a good starting point for further manual adjustment by network operators. Note that a similar adjustment process may also be required with SMT-based synthesizers, due to differences between the formal protocol model and the one running on a given real-world router where the configuration is to be deployed.

Next, we discuss the architecture of our neural synthesis framework. In follow-up sections, we instantiate this framework for the case of BGP/OSPF configuration synthesis, and evaluate the resulting instantiation by comparing it to a state-of-the-art SMT-based synthesizer.

% \begin{itemize}
%     \item effort: need to implement simulation code to generate dataset to learn from (typically well-defined in protocol specs, much easier than implementing synthesis directly)
%     \item can be sampled (multiple alternative solutions, not easily possible with SMT-based methods)
%     \item much faster than SMT-based synthesis
% \end{itemize}

% Requirements:
% \begin{itemize}
%     \item protocol-agnostic
%     \item fully learned, no hand-coded synthesis rules
%     \item define: strict specification vs. relaxed specification
% \end{itemize} 

==> diff/git-latexdiff.33882/old/sections/2_model.tex <==
\section{Neural Synthesis Framework}
\label{sec:model}


We now present the architecture of our graph-based neural synthesizer model, illustrated in \cref{fig:overview-model}. First, in \cref{sec:graph-embedding} we introduce our generic graph-based encoding, which allows us to embed network topologies, protocol configuration and the specification into a latent space. Then, in \cref{sec:graph-transformer} we present the architecture of the processor network which we train to perform the synthesis task. Finally, in \cref{sec:decoding-sampling} we discuss how to sample network configurations from the resulting latent synthesis output.

\begin{figure}
    \begin{minipage}[t]{0.21\textwidth}
    \begin{lstlisting}[basicstyle=\ttfamily\small, escapeinside={(*}{*)}]
router(A)
router(B)
(...)

connected(A,B,2)
connected(A,C,?)(*\blackcircled{1}*)
(...)
    \end{lstlisting}
\end{minipage}
\begin{minipage}[t]{0.21\textwidth}
    \begin{lstlisting}[basicstyle=\ttfamily\small, escapeinside={(*}{*)}]
network(N1)
bgp_route(E,N1,2,3,1,0,1)

fwd(A,B,N1)
not fwd(B,A,N1)
(...)
    \end{lstlisting}
\end{minipage}
    \caption{A snippet of a fact base sketch encoding a network's topology, parameters such as link weights (\texttt{connected} facts) and a specification (\texttt{fwd} facts).}
    \label{fig:datalog-encoding}
\end{figure}

\begin{figure}[t]
    \centering
    \includegraphics[width=0.25\textwidth]{figures/synth-architecture.png}
    \caption{The neural synthesizer model architecture.}
    \label{fig:architecture}
\end{figure}

\subsection{Fact Base Embedding}
\label{sec:graph-embedding}
To remain network protocol-agnostic in our model architecture, we implement a generic graph-based encoding of Datalog-like facts, similar to knowledge graphs \cite{rosso2020beyond}. This means that we first encode topologies, configurations and specifications as a set of Datalog-like facts and then employ a generic embedding.
%We chose Datalog facts as the input format of our synthesis approach for its flexibility, wide-spread use in Program Analysis and use in previous work on configuration synthesis \cite{el2017network}.

\paragraph{Fact Base} A set of Datalog-like facts, as depicted in \cref{fig:datalog-encoding}, serves as the input \emph{fact base} $\mathcal{F}$ to our synthesizer model. $\mathcal{F}$ is a set of facts $f(a_0, \dots, a_n)$ where arguments may be constants (e.g. A or B) or integer literals. Further, each fact in a fact base has a corresponding truth value denoted as $[f(a)]_{\mathcal{B}}$. For instance, from the fact base in \cref{fig:datalog-encoding} we can derive $[fwd(A,B,N1)]_{\mathcal{B}} = \text{\texttt{true}}$ and $[fwd(B,A,N1)]_{\mathcal{B}} = \text{\texttt{false}}$.

\paragraph{Consistency} We represent a network's topology, the protocol configuration and parameters as well as the specification, all in a single fact base. Given the semantics of the protocols in use, we can then check whether the specification encoded in a fact base is satisfied by the provided configuration. To quantify, we define the notion of relaxed specification consistency, as discussed earlier, with respect to a fact base: Given a fact base $\mathcal{F}$, a subset of specification facts $S \subset \mathcal{F}$ and protocol semantics $\mathcal{P}$, the \emph{consistency} of a fact base is defined as the relative number of satisfied facts in $S$ with respect to the routing behavior obtained via $\mathcal{P}$. The contents of $S$ depend on the concrete instantiation of the synthesizer model. For an example of possible specification facts, see our instantiation of the synthesizer model for BGP/OSPF in \cref{sec:training}.

\begin{figure*}
    \def\arraystretch{1.5}
    \begin{tabular}{lr}
        %$T_f: T_1 \times \dots \times T_n$ & \textit{(fact type declaration)}\\
        $emb(f) := \mathbf{V_f}$ & \textit{(learned fact type embedding)}\\
        $emb(b) := \mathbf{W_{\text{bool}}}\;onehot(b)$ & \textit{(learned boolean embedding)}\\
        $emb(f,i,v) := \mathbf{W_{f_i}}\;onehot(v)$ & \textit{(learned integer embedding)}\\
        $emb(f,i,?) := \mathbf{V_{hole}}$ & \textit{(learned hole embedding)}\vspace{10pt}\\
        $\mathlarger{
        h_c := \sum_{f(c) \in \mathcal{F}}
        emb(f)
        }$ & \textit{(constant embedding)}\vspace{10pt}\\
        $h_{f(a_0, \dots, a_n)} := emb(f) + emb([f(a_0, \dots, a_n)]_{\mathcal{B}}) + \mathlarger{
        \sum_{(i,v) \in \mathcal{I}(f(a_0, \dots, a_n))}
        emb(f, i, v)
        }$\hspace{-1.2cm} & \textit{(fact embedding)}\\
        $\mathcal{I}(f(a_0, \dots, a_n)) := \{(i,v) \; | \; f(a_0, \dots, a_{i-1}, v, \dots, a_n) \in \mathcal{F} \wedge v:Int \wedge i \in \mathbb{N}$ \}& \textit{(integer arguments)}\vspace{10pt}\\
        $N_i(h_c) := \{h_f \; | \; \exists i \in \mathbb{N} . f(a_0, \dots, a_{i-1}, c, a_{i+1}, \dots, a_n) \in \mathcal{F}\}$& \textit{(i-th neighborhood of constant node)} \\
        $N_i(h_f) := \{h_c \; | \; \exists i \in \mathbb{N} . f(a_0, \dots, a_{i-1}, c, a_{i+1}, \dots, a_n) \in \mathcal{F}\}$& \textit{(i-th neighborhood of fact node)} \\
    \end{tabular}
    \caption{Translating a fact base $\mathcal{F}$ to node features. $f$ denotes a predicate, $v$ integer values, $b$ boolean values as 0 or 1, $i$ argument indices and $[f(a)]_{\mathcal{B}}$ the truth value of a fact. }
    \label{fig:graph-embedding}
\end{figure*}

%discuss embedding as shown in \cref{fig:datalog-encoding}. Note how this makes fact bases a suitable input to standard GNN architectures.

\paragraph{Fact Base Sketching} In a synthesis setting, we are confronted with incomplete fact bases, i.e. the specification and topology is given but the network configuration is to be synthesized. For these cases, we also consider fact bases with unknown parameters inspired by the idea of program sketching in program synthesis \cite{solar2008program}. More specifically, users may replace an unknown integer argument of a fact by a \texttt{?} symbol, indicating a value to be synthesized. Using this mechanic, we can represent the synthesis input as an incomplete fact base which encodes to-be-synthesized values as unknown parameters. As an example, consider \cref{fig:datalog-encoding} \blackcircled{1}, where the link weight between router nodes \texttt{A} and \texttt{C} is represented as an unknown parameter.

\paragraph{Embedding} We employ a structurally-defined embedding scheme to transform a fact base into a graph with node features as required for processing with graph neural networks. Given a fact base $\mathcal{F}$, we apply the rules in \cref{fig:graph-embedding} to obtain node features and adjacency information. Both a fact $f$ and a constant $c$ are represented as distinct nodes with features $h_c$ and $h_f$, respectively. The relationships between facts and constants is encoded as node adjacency as defined by the neighborhood functions $N_i$.

We use multiple neighborhood functions, i.e. multiple types of edges, to encode the argument position of a constant occurring in a fact. Hence, the number of neighborhood functions corresponds to the maximum number of arguments in a single fact, e.g. 3 in \cref{fig:datalog-encoding}. Integer arguments and unary facts are directly accounted for in the respective node or fact embedding. To handle unknown parameters, we replace the corresponding $emb(...)$ term with the learned $\mathbf{V_{hole}}$ embedding.

Considering the embedding function $emb$, the learned parameters of our embedding are $\mathbf{V_f} \in \mathbb{R}^D$ per fact type in~$\mathcal{F}$, $\mathbf{W_{\text{bool}}} \in \mathbb{R}^{D \times 2}$ for boolean values, $\mathbf{W_{f_i}} \in \mathbb{R}^{D \times N}$ per integer argument of fact type $f$ and $\mathbf{V_{hole}} \in \mathbb{R}^D$ to represent unknown parameters. Hyperparameter $D$ represents the dimension of the latent space the synthesizer model operates in and $N$ specifies the number of supported integer values. An example of applying this embedding scheme to a simple fact base is given in \cref{fig:graph-encoding-example}.

\begin{figure}
    \begin{minipage}[t]{0.2\textwidth}
        \centering
        \footnotesize
        \textbf{Fact Base}
        \begin{lstlisting}[basicstyle=\ttfamily\small]
router(A)
router(B)

conn(A, B, 12)
        \end{lstlisting}
    \end{minipage}
    \begin{minipage}[t]{0.15\textwidth}
        \centering
        \textbf{Graph}\\
        \vspace{5pt}
        \includegraphics[width=0.7\textwidth]{figures/graph-encoding.pdf}
    \end{minipage}\\
    \centering\\
    \vspace{10pt}
    \textbf{Node Features}\\
    \vspace{10pt}
    \begin{minipage}[t]{0.5\textwidth}
        $\begin{array}{rcl}
        h_A &:=& emb(router) = \mathbf{V_{\text{router}}}\\
        h_B &:=& emb(router) = \mathbf{V_{\text{router}}}\\
        h_{\text{conn(A,B,12)}} &:=& emb(conn) + emb(conn, 2, 12)\\
        &:=& \mathbf{V_{\text{conn}}} + \mathbf{W_{conn_2}} onehot(12)
    \end{array}$
    \end{minipage}
    \caption{An example of embedding a simple fact base using the embedding scheme of \cref{fig:graph-embedding}. The shown graph illustrates the neighborhoods $N_0$ and $N_1$ induced by the \texttt{conn} fact.}
    \label{fig:graph-encoding-example}
\end{figure}

\begin{figure}
    $$
    \begin{array}{rcl}
    z_j &:=& h_j + Drop(\mathlarger{\sum_{N_i}} h'_{GAT_i})\\
    h'_j &:=& FFN(Norm(z_j))\vspace{11pt}\\
    FFN(x_j) &:=& Norm(Lin2(Drop(Lin1(x_j)))))
    \end{array}
    $$
    \caption{
        The recurrence relation of a node $j$'s representation $h_j$. $h'_{GAT_i}$ represents the output of a graph attention layer operating with neighborhood $N_i$ according to \cite{velivckovic2017graph}, $h_j$ the representation of node $j$ at the previous step. $Norm$ refers to batch normalization \cite{ioffe2015batch}, $Drop$ to dropout regularization \cite{hinton2012improving} and $Lin1$ and $Lin2$ to linear layers with an inner dimension of $4N$.
    }
    \label{fig:recurrence}
\end{figure}

\subsection{Synthesizer Model}
\label{sec:graph-transformer}

For an illustration of the synthesizer model's architecture, please see Figure~\ref{fig:architecture}. Given a fact base $\mathcal{F}$ we first apply our embedding scheme as described in \cref{sec:graph-embedding}. We then employ a 2-layer GNN-based encoder network to produce the latent representation of a synthesis input.
Given this representation, a processors network is trained to perform the actual synthesis task in high-dimensional space. Last, we apply a set of decoder networks, to obtain the synthesized values of unknown parameter, given the latent synthesis~output.

%In this context, the synthesis problem for network configurations corresponds to completing partially provided fact bases.

% \paragraph{High-Level Architecture}

% We employ the high-level architecture to obtain the latent synthesis output $y_\mathcal{F}$:
% $$
% \begin{array}{rcl}
%     \mathbf{x_{\mathcal{F}}} &:=& Encoder(Embedding(\mathcal{F}))\\
%     \mathbf{y_{\mathcal{F}}} &:=& Processor(\mathbf{x_{\mathcal{F}}} + \mathbf{z})\\
%     z_i &\sim& \mathcal{N}(0,1)
% \end{array}
% $$
% \todo{z is only added for $i<N/2$}

% $Embedding$ corresponds to the graph-based embedding as discussed in \cref{sec:graph-embedding} and $Encoder$ is a 2-layer graph attention module. $Processor$

\paragraph{Encoding} The encoder GNN operates on the embedded representation of a fact base. It produces the high-dimensional representation of a synthesis input as required for the processor network. We additionally apply noise to the first half of the units of the latent representation via $\mathbf{z}$, as a source of non-determinism. According to our experiments this improves model performance and we hypothesize this is due to the synthesis problem having more than one solution in most cases.

\paragraph{Iterative Processor} The processor network is modelled as an iterative process. For this, we apply the same 6-layer graph attention module for a total of 4 iterations.
In the framework of neural algorithmic reasoning, this iterative computational structure encodes an inductive bias towards an iterative solution to the synthesis problem. Because of this bias, our processor network essentially learns an algorithmic procedure which iteratively synthesizes the values of unknown parameters in a fact base.

\paragraph{Graph Attention Layer} In the GNNs we employ, we rely on a composed variant of the graph attention layer as introduced by \cite{velivckovic2017graph}. We employ multiple graph attention layers in lockstep, one per neighborhood $N_i$ defined by our graph embedding (cf. \cref{sec:graph-embedding}), and combine the intermediate results after each step. Specifically, the recurrence relation of a node $j$'s representation $h_j$ is defined as shown in \cref{fig:recurrence}. These mechanics of combining the results of the different graph attention layers $h'_{GAT_i}$, directly corresponds to how multiple attention heads are combined in the original Transformer architecture \cite{vaswani2017attention}.

\paragraph{Argument Decoder Networks} To synthesize the values of unknown parameters, the model maintains a set of decoder networks. That is, it provides one decoder network per integer argument per fact type in a fact base. When decoding, the network is applied to the latent synthesis output of the corresponding fact node. For example, a synthesizer model which operates on the fact base in \cref{fig:graph-encoding-example}, would provide a decoder network $D_{\text{conn}_2}: \mathbb{R}^D \rightarrow \mathbb{R^N}$ to decode values for the third argument of a \texttt{conn} fact. In our experiments, decoder networks are implemented as simple multi-layer perceptron models.

%The synthesizer model learns a conditional distribution of fact bases which are consistent with respect to the protocols' semantics.

%\todo{introduce synthesis as a completion problem of an encoded fact base (a la BERT). Introduce masking, introduce decoding of integer and truth values. Synthesis is learning a conditional distribution of consistent fact bases.}

%Using this method, we obtain the node features $h_c$ per constant, $h_f$ per fact and adjacency information in terms of node neighborhood functions $N_i(h_c)$ and $N_i(h_f)$. Overall, this encoding makes a fact base suitable for processing using standard graph neural networks.

%- Brief description of the Graph Transformer Model
\subsection{Multi-Shot Sampling}
\label{sec:decoding-sampling}

%Multi-Stage Parameter Sampling (sampling methods: topk, high-temp, low-temp)
To sample concrete values from the output distributions over unknown parameters, we apply a multi-shot sampling strategy. That is, we sample values only for a subset of unknown parameters, insert them in our input fact base and run the synthesis model again. We repeat this process until no more unknown parameters remain. This multi-shot sampling strategy allows the model to incorporate the concrete values of previously synthesized parameters in its computation. In our evaluation in \cref{sec:evaluation}, we include a comparison of how this compares to sampling all unknown parameters at once.

%In a fact base with multiple holes, we apply the corresponding decoder networks to obtain a value distribution for each integer hole. However, instead of sampling all integer holes in one


==> diff/git-latexdiff.33882/old/sections/3_bgp_ospf.tex <==
\section{BGP/OSPF Synthesis}
\label{sec:bgp-ospf}

\newcommand{\as}{\ac{AS}~}
\newcommand{\ases}{\acp{AS}~}

\newcommand{\squareann}{{\tiny$\blacksquare\;$}}
\newcommand{\triangleann}{{\small$\blacktriangle\;$}}

\begin{figure*}
    \centering
    \includegraphics[width=0.95\textwidth]{figures/networks-all.pdf}
    \caption{(a) An illustration of a small AS network, including internal peers (blue), external peers (purple), BGP sessions as well as physical links. (b) The propagation of two BGP announcement across the network. (c) The resulting forwarding plane after applying BGP and OSPF.}
    \label{fig:network-fwd-tree}
\end{figure*}

We now discuss an instantiation of our learning-based framework for the case of BGP and OSPF protocols. In \cref{sec:synthesis-setting} we introduce a basic networking model, BGP and OSPF protocols and the synthesis setting. Given this model, \cref{sec:training} describes how to generate a corresponding dataset of input/output samples and train a synthesizer model.
%This shall serve as a prerequisite to the instantiation of our learning-based synthesis framework for the BGP and OSPF protocol in \cref{sec:training}.

\subsection{Synthesis Setting}
\label{sec:synthesis-setting}

\paragraph{Graphical Model} We assume an abstract network model which can be represented as an undirected graph as shown in \cref{fig:network-fwd-tree} (a). We always consider a set of internal routers (A, B, C, D in \cref{fig:network-fwd-tree}) as well as a set of adjacent external routers (E, F  in \cref{fig:network-fwd-tree}). The group of internal routers forms the \emph{\as} under consideration whereas external routers belong to other adjacent \ases. In practice, an \as represents an administrative domain controlled by a single operator.

\paragraph{Forwarding Plane} We focus on the \emph{forwarding plane} of a network. This means we are interested in how a router forwards packets given incoming traffic of different traffic classes. For this, each router maintains a routing table which determines which of its outgoing edges is used to forward packets of a certain traffic class. As an example, consider \cref{fig:network-fwd-tree} (c) which illustrates the forwarding plane of some traffic class reachable via external peer $E$ or $F$ in our example network. Each router of the network forwards traffic along some of its outgoing links. In practice, a number of protocols are used to populate a router's routing tables. For the instantiation of our synthesis framework however, we focus on OSPF and BGP.

\paragraph{OSPF} The OSPF protocol \cite{moy1994ospf} is a link-state protocol, typically used as an interior gateway protocol~(IGP), i.e., to route traffic within an \ac{AS}. Given link weights per physical link in the network, OSPF simply routes traffic along the shortest path towards the destination.

\paragraph{BGP} The BGP protocol \cite{rekhter1994border} on the other hand is a path-vector protocol used to exchange reachability information mostly on the level of \acp{AS}.
%These are groups of routers typically operated by a single party (e.g. an ISP).
When using BGP, a routing destination announces its existence to other \ases and routers, by sending out a BGP announcement. Receivers of such announcements may then choose to pass them on to other \acp{AS}, redistribute them internally and/or modify them. Instead of communicating along physical links directly, the BGP protocol requires manually configured BGP sessions among routers of the \as and external peers, as indicated by the BGP session edges in \cref{fig:network-fwd-tree}(a).
%\todo{more discussion of eBGP vs iBGP and support for route reflection (more of an implementation detail, maybe only mention in dataset generation where simulation code is discussed)}.

%\paragraph{BGP Decision Procedure}~
%\todo{discuss decision procedure}
In case a router receives more than one announcement for a destination, a designated BGP decision process is applied to determine a single best route. \cref{fig:bgp-decision} shows the ordered list of comparison criteria of this decision process. The different criteria depend different properties of a route announcements, including the IGP cost towards the routing destination. As a consequence, when used together, OSPF as IGP protocol and BGP will interact. %Note also that BGP is an iterative process which needs multiple rounds of propagation to converge.

\paragraph{Example}
%\todo{run through simple BGP+OSPF example of computing the forwarding plane}
To better understand BGP/OSPF routing, consider the simple example given in \cref{fig:network-fwd-tree} (b). Here, our example \as imports BGP announcements \squareann and \triangleann from E and F respectively. Both represent a route to the same destination. As shown, both announcements have a so-called local preference of 2. For simplicity, we ignore other properties such as the AS path length, Origin and MED in this example. The announcements are propagated among BGP neighbors and the best route is selected according to the decision procedure in \cref{fig:bgp-decision}. See \cref{fig:network-fwd-tree} (b) for an illustration of the intermediate states of this propagation process. As both announcements have a local preference of 2, rule 1 of the decision process is not used. Instead, in round 2, node B selects \squareann over \triangleann due to a lower IGP cost of 2 via egress node A as compared to 3 via egress node D (rule 6). Node D selects \triangleann over \squareann, since it learns this route directly from an external peer (rule 5). After Round 3, the BGP propagation process converges to a stable state and we can derive the forwarding plane as shown in \cref{fig:network-fwd-tree} (c).


%, as well as external peers E and F which belong to other \acp{AS}. External peers are routers which are connected via eBGP sessions to routers of the \ac{AS} under consideration. They announce BGP routes to their neighbors, which are propagated within the network

\paragraph{Problem Statement: Configuration Synthesis} We phrase the BGP/OSPF configuration synthesis problem on the level of the forwarding plane. This means that users provide a specification which constraints the set of allowed forwarding planes. This includes predicates which enforce forwarding paths, block forwarding paths or assert higher-level properties like traffic isolation and reachability. Given such a specification, we consider network configuration synthesis as the task of configuring OSPF and BGP in a way that produces a forwarding plane which satisfies the provided specification.

\paragraph{Search Space} To limit the space of candidate configurations, we define the set of synthesized parameters: For OSPF we synthesize link weights as explored in a wide range of existing work (e.g. \cite{el2018netcomplete,fortz2000internet}. BGP parameters on the other hand are not defined as clearly: Depending on the requirements of a network operator, one may employ custom BGP import and export policies at every router of a network to implement complex behavior. However, in this work we focus on a simplified setting, where we assume BGP route announcements to only be modified when imported into the \as from an external peer. Previous work has already pointed out that this is a reasonable assumption which holds for the majority of real-world networks \cite{caesar2005bgp,cittadini2010doing, steffen2020probabilistic}.

\begin{figure}
    \small{
    \begin{enumerate}
        \setlength{\itemsep}{0pt}
        \setlength{\parskip}{0pt}
        \item Highest Local preference
        \item Lowest AS path length
        \item Prefer Origin (IGP $>$ EBGP $>$ INCOMPLETE)
        \item Lowest Multi-exit discriminator (MED)
        \item External over internal announcements
        \item Lowest IGP cost to egress
        \item Lowest BGP peer id (tie breaker)
    \end{enumerate}}
    \vspace{-15pt}
    \caption{The BGP decision process \cite{rekhter1994border}. The shown rules are applied in order until a single best BGP announcements remains.}
    \label{fig:bgp-decision}
\end{figure}

\subsection{Dataset Generation and Training}
\label{sec:training}
To train a synthesizer model, we need a large number of fact bases encoding a variety of network topologies, configurations and forwarding specifications. Further, we must provide the model with target values for unknown parameters as a supervision signal. This section discusses how we construct such a dataset for BGP/OSPF synthesis.
%Further, we provide an example of what a corresponding fact base looks like, including a description of the supported specification language.

\paragraph{Dataset Generation} To obtain network configurations and corresponding forwarding specifications we employ a generative process: We first randomly configure BGP and OSPF parameters for some topology. Then we simulate the OSPF and BGP protocol and compute the resulting forwarding plane. Based on this, we extract a forwarding specification which fixes a random subset of forwarding paths, reachability and isolation properties that are satisfied by the forwarding plane.

\paragraph{Topologies} For training, our dataset is based on random topologies with $16$-$24$ routers. We generate the physical layout of these graphs by triangulation of uniformly sampled points in two-dimensional space.

\paragraph{Simulation} To compute the forwarding plane given an OSPF and BGP configuration, we simulate the protocols. For OSPF, we implement shortest path computation to obtain the forwarding plane. For BGP, we implement the full BGP decision process as shown in \cref{fig:bgp-decision}, except for the MED attribute. In addition to the basic networking model discussed in \cref{sec:synthesis-setting}, we implement support for eBGP and iBGP, fully-meshed BGP session layouts as well as layouts relying on route reflection. For more details of these BGP concepts see \cite{bates2000rr}.

%Note that the synthesizer model will reason on the level of the provided training samples. That is, to improve the overall synthesis quality in a real-world setting, it is helpful to implement simulation code which behaves very similar to real-world networks. Another promising approach would be to extract training samples from real-world networks, thereby circumventing the need for simulation, however, we leave this as future work.

%While this can be a considerable effort, it is typically an easier task than to implement the synthesizer directly. The concrete semantics of protocols and their simulation is a well-defined procedure, whereas implementing efficient synthesis tools is still an open problem.

\paragraph{Fact Base Encoding} We encode synthesis input using a small set of facts. For an example of a corresponding fact base see \cref{fig:bgp-ospf-fact-base}. We use the \texttt{router}, \texttt{external} and \texttt{network} facts to mark routers, external peers and routing destinations respectively. Physical links between routers are encoded as \texttt{connected(R1,R2,W)} facts where \texttt{W} denotes the OSPF link weight. Further, we rely on \texttt{ibgp}, \texttt{ebgp}, \texttt{route\_reflector} and \texttt{bgp\_route} facts to represent different types of BGP sessions and imported routes. Using the notion of unknown parameters as discussed in \cref{sec:graph-embedding}, we encode configuration parameters, e.g., properties of imported routes or OSPF link weights.

\paragraph{Specification Language} We support a small specification language with three types of forwarding predicates:

\begin{itemize}
    \setlength{\itemsep}{0pt}
    \setlength{\parskip}{2pt}
    \item \texttt{fwd(R1, Net, R2)} specifies that router \texttt{R1} forwards traffic destined for \texttt{Net} to its neighbor \texttt{R2}.
    \item \texttt{reachable(R1, Net, R2)} specifies that traffic destined for \texttt{Net} that passes through \texttt{R1} also passes through \texttt{R2} before reaching its destination.
    \item \texttt{trafficIsolation(R1, R2, N1, N2)} specifies that it must not hold that $[fwd(R1,R2,N1)]_{\mathcal{B}} \wedge [fwd(R1,R2,N2)]_{\mathcal{B}}$.
\end{itemize}

In the negative case of each predicate, the opposite must hold true for the fact to be satisfied. This specification language can easily be extended by including new specification predicates in the dataset generation process. One must simply provide a method of extracting positive and negative cases of a specification fact from a given forwarding plane. Once included in the training dataset of a synthesizer model, the resulting synthesis system will be able to consider specifications relying on the new type of predicates.

% \todo{info on loss function, optimizer, etc.}
\paragraph{Training} We generate a dataset of $10,240$ input/output samples and instantiate our synthesizer model with a hidden dimension $D$ of $64$. For optimization, we use the Adam optimizer \cite{kingma2014adam} with a learning rate of $10^{-4}$, applying negative log-likelihood loss to the decoder networks' outputs. We stop training after the specification consistency on a validation dataset no longer increases at around $\sim2800$ epochs.

\begin{figure}
\begin{minipage}[t]{0.22\textwidth}
\begin{lstlisting}[basicstyle=\ttfamily\tiny]
# topology and configuration
router(c5)
router(c3)
router(c1)
router(c0)
network(c6)
network(c7)

external(c8)
external(c9)
external(c10)
external(c11)
external(c12)
external(c13)

route_reflector(c2)
route_reflector(c4)

connected(c2,c4,?)
connected(c2,c5,?)
connected(c2,c3,?)
connected(c4,c5,?)
connected(c4,c3,?)
connected(c4,c0,?)
connected(c5,c1,?)
connected(c5,c0,?)
connected(c3,c0,?)
connected(c3,c1,?)
connected(c1,c0,?)

ibgp(c2,c4)
ibgp(c2,c5)
ibgp(c2,c0)
ibgp(c2,c1)
ibgp(c4,c3)
ibgp(c4,c4)
\end{lstlisting}
\end{minipage}
\begin{minipage}[t]{0.2\textwidth}
\begin{lstlisting}[basicstyle=\ttfamily\tiny]
ebgp(c2,c12)
ebgp(c5,c9)
ebgp(c5,c10)
ebgp(c5,c13)
ebgp(c0,c8)
ebgp(c0,c11)

bgp_route(c8,c6,?,?,1,?,1,8)
bgp_route(c9,c6,?,?,0,?,1,9)
bgp_route(c10,c6,?,?,0,?,1,10)
bgp_route(c11,c7,?,?,0,?,1,11)
bgp_route(c12,c7,?,?,0,?,1,12)
bgp_route(c13,c7,?,?,2,?,1,13)

# forwarding specification
fwd(c0,c6,c3)
fwd(c3,c6,c2)
fwd(c2,c6,c4)
not fwd(c3,c6,c0)
not fwd(c0,c6,c11)
not fwd(c11,c6,c0)

not trafficIsolation(c1,c0,c7,c6)
not trafficIsolation(c1,c0,c7,c6)
trafficIsolation(c0,c3,c6,c7)
trafficIsolation(c0,c3,c6,c7)

reachable(c5,c6,c10)
reachable(c1,c6,c4)
not reachable(c0,c6,c5)
reachable(c5,c6,c10)
\end{lstlisting}
\end{minipage}
\caption{An example of a fact base encoding a topology, a sketch of a BGP and OSPF configuration and a forwarding specification.}
\label{fig:bgp-ospf-fact-base}
\end{figure} 

==> diff/git-latexdiff.33882/old/sections/4_evaluation.tex <==
\section{Evaluation}
\label{sec:evaluation}

We trained a synthesizer model to perform configuration synthesis for BGP and OSPF. We now assess the performance of the resulting neural synthesizer with respect to two core metrics: (1) the quality of synthesized configurations in terms of their consistency with the provided forwarding specifications (\cref{sec:synthesis-quality}), and (ii) the time a learned synthesizer takes when compared to the state-of-the-art SMT-based synthesizer NetComplete \cite{el2018netcomplete} (\cref{sec:synthesis-vs-smt}).

\paragraph{Dataset} We compare across three datasets: Small, Medium and Large. Each dataset represents 8 real-world topologies, sampled from the Topology Zoo \cite{knight2011internet}, where the number of nodes lies between 0-34, 34-68 and 68-170 respectively. To obtain forwarding specifications for the sampled topologies, we use our generative pipeline as discussed in \cref{sec:training}. In each topology, we do synthesis for 4 different traffic classes (routing destinations) at a time.

\paragraph{Experimental Setup} We run all our experiments on an Ubuntu Linux machine with an Intel(R)~Core(TM)~i9-9900X~@~3.50GHz processor, 64GB of system memory and an NVIDIA GeForce RTX 3080 GPU with 10GB of video~memory.

\subsection{Synthesis Quality}
\label{sec:synthesis-quality}
To assess our learned synthesizer, we examine its behavior with increasingly large topologies and specifications.

\paragraph{Specifications} Using the same generative model as described in \cref{sec:training}, we generate forwarding specifications for the topologies in our three datasets with each specification constructed from $3 \times n$ requirements, one per supported predicate type:  \texttt{fwd} requirements correspond to specifying or blocking a forwarding path using multiple \texttt{fwd} predicates whereas \texttt{reachable} and \texttt{trafficIsolation} requirements each translate to a single specification fact. We compare across increasingly large specifications of $3\times 2$, $3\times 8$ and $3 \times 16$ requirements, respectively.

\paragraph{Methodology} For each pair of topology and specification, we run our synthesizer 5 times and report the network configurations with the highest overall consistency value. For sampling, we rely on our multi-shot sampling strategy where we randomly group the unknown parameters of a configuration into 4 groups (4-shot sampling).

\paragraph{Results} We summarize our results in \cref{fig:eval-consistency}. On average, our synthesis model produces network configurations that are $>91\%$ consistent with the provided forwarding specifications across all datasets and sizes of specifications. When only few requirements are given, the synthesizer model even succeeds in producing fully-consistent configurations. We observe a slightly decreasing consistency with increasingly large topologies.

%\texttt{fwd} facts are satisfied more easily, whereas \texttt{reachable} and \texttt{trafficIsolation} facts are violated more often.

\paragraph{Multi-Shot Sampling} In \cref{fig:eval-consistency-baseline}, we report the average specification consistency using our multi-shot sampling strategy as compared to sampling all unknown parameters at once. As a baseline we have also sampled random configurations from a uniform distribution (per parameter) and compute the corresponding specification consistency. Over the baseline, our synthesizer model shows clear improvement and multi-shot sampling further increases consistency.

\begin{figure*}
    \begin{center}
        \textbf{Specification Consistency}\\
        \footnotesize
        \begin{tabular}{rrcccccccccc}
        \toprule
        \multicolumn{2}{c}{Dataset} & \tiny\texttt{fwd} & \tiny\texttt{reachable}  & \tiny\texttt{trafficIsolation} & Overall & $\emptyset$     No. Full Matches & $\emptyset$ No. $>90\%$ Matches\\
        \midrule
        $3\times 2$ requirements & Small & 0.95 & 0.94 & 1.00 & \textbf{0.95} & 0.62 & 0.62\\
& Medium & 0.96 & 1.00 & 0.94 & \textbf{0.96} & 0.88 & 0.88\\
& Large & 0.94 & 0.94 & 1.00 & \textbf{0.93} & 0.62 & 0.62\\
\midrule
$3\times 8$ requirements & Small & 0.97 & 0.98 & 0.97 & \textbf{0.98} & 0.50 & 1.00\\
& Medium & 0.99 & 0.95 & 1.00 & \textbf{0.98} & 0.50 & 1.00\\
& Large & 0.96 & 0.95 & 0.91 & \textbf{0.94} & 0.38 & 0.88\\
\midrule
$3\times 16$ requirements & Small & 0.97 & 0.89 & 0.95 & \textbf{0.94} & 0.38 & 0.75\\
& Medium & 0.98 & 0.97 & 0.97 & \textbf{0.98} & 0.38 & 1.00\\
& Large & 0.92 & 0.88 & 0.95 & \textbf{0.91} & 0.12 & 0.50\\
    \end{tabular}\end{center}
    \caption{Average specification consistency of the network configurations synthesized by our trained synthesizer model. Per sample we run the synthesizer with a specification of $3\times N$ requirements, where the specifications always include $N$ requirements per supported predicate type (\texttt{fwd}, \texttt{reachable}, \texttt{trafficIsolation}).}
    \label{fig:eval-consistency}
\end{figure*}

\begin{figure}
    \begin{center}
        \footnotesize
        \begin{tabular}{rrcccccccccc}
        &  & \multicolumn{2}{c}{Neural}\\
        & Random & 1-Shot & 4-shot\\
        \toprule
        Small & 0.83 & 0.92 & \textbf{0.94} \\
        Medium & 0.88 & 0.95 & \textbf{0.98} \\
        Large & 0.78 & 0.88 & \textbf{0.91} \\
    \end{tabular}\end{center}
    \caption{Average specification consistency with $3\times 16$ requirements when sampling configurations randomly from a uniform distribution and 1-shot/4-shot sampling using our synthesizer model.}
    \label{fig:eval-consistency-baseline}
\end{figure}

\begin{figure*}[ht]
    \footnotesize
    \begin{center}
        \textbf{BGP Synthesis Time}
        \footnotesize
        \begin{tabular}{rrccccccccc}
        \toprule
        &&\multicolumn{3}{c}{Synthesis Time (s)} & \multicolumn{2}{c}{Accuracy (Neural)} \\
        \multicolumn{2}{l}{\# Requirements} & NetComplete & Neural (CPU) & Speedup &$\emptyset$ Consistency& $\emptyset$ No. Full Matches\\
        \midrule
    2 requirements &Small & 18.073s & 0.641s & \textbf{28.2x} & 0.969 & 0.875\\
        &Medium & 60.864s & 2.748s & \textbf{22.2x} & 0.939 & 0.75\\
        &Large & 1389.485s\tiny{  7/8 TO} & 22.301s & \textbf{62.3x} & 0.989 & 0.875\\
    \midrule
    8 requirements &Small & 247.691s & 1.065s & \textbf{232.5x} & 0.96 & 0.75\\
        &Medium & $>$25m\tiny{  8/8 TO} & 3.47s & \textbf{432.2x} & 0.968 & 0.5\\
        &Large & $>$25m\tiny{  8/8 TO} & 30.961s & \textbf{48.4x} & 0.969 & 0.75\\
    \midrule
    16 requirements &Small & 1416.828s\tiny{  7/8 TO} & 2.528s & \textbf{560.5x} & 0.926 & 0.25\\
        &Medium & $>$25m\tiny{  8/8 TO} & 5.481s & \textbf{273.7x} & 0.947 & 0.25\\
        &Large & $>$25m\tiny{  8/8 TO} & 69.092s & \textbf{21.7x} & 0.959 & 0.25\\
    \end{tabular}\end{center}
    \caption{Comparing consistency and synthesis time of our method (Neural) with the SMT-based state-of-art synthesis tool NetComplete. The notation {\tiny{n/8 TO}} indicates the number of timed out synthesis runs out of 8 (25+ minutes).}
    \label{fig:evaluation-compare-bgp}
\end{figure*}

\begin{figure*}[ht]
    \begin{center}
        \footnotesize
        \textbf{OSPF Synthesis Time}\\
        \footnotesize
        \begin{tabular}{rrccccccccc}
        \toprule
        &&\multicolumn{3}{c}{Synthesis Time (s)} & \multicolumn{2}{c}{Accuracy (Neural)} \\
        \multicolumn{2}{l}{} & NetComplete & Neural (GPU) & Speedup &$\emptyset$ Consistency& $\emptyset$ No. Full Matches\\
        \midrule
    2 requirements &Small & 0.265s & 0.091s & \textbf{2.9x} & 1.000 & 1.00\\
     &Medium & 0.404s & 0.098s & \textbf{4.1x} & 1.000 & 1.00\\
     &Large & 0.944s & 0.14s & \textbf{6.7x} & 1.000 & 1.00\\
    \midrule
    8 requirements &Small & 0.876s & 0.164s & \textbf{5.3x} & 0.982 & 0.75\\
     &Medium & 1.517s & 0.103s & \textbf{14.7x} & 1.000 & 1.00\\
     &Large & 3.505s & 0.316s & \textbf{11.1x} & 0.981 & 0.50\\
    \midrule
    16 requirements &Small & 1.65s & 0.21s & \textbf{7.9x} & 0.991 & 0.625\\
     &Medium & 2.646s & 0.245s & \textbf{10.8x} & 0.989 & 0.50\\
     &Large & $>$566.636s+\tiny{  3/8 TO} & 0.233s & \textbf{2430.4x} & 0.987 & 0.875\\
    \end{tabular}\end{center}
    \caption{Comparing consistency and synthesis time of our method (Neural) with the SMT-based OSPF synthesis tool NetComplete. The notation {\tiny{n/8 TO}} indicates the number of timed out synthesis runs out of 8 (25+ minutes).}
    \label{fig:evaluation-compare-ospf}
\end{figure*}


\subsection{Comparison to SMT-based Synthesis}
\label{sec:synthesis-vs-smt}

%To provide a comparison of our learned BGP/OSPF synthesizer with SMT-based methods,
We now compare the synthesis time of the learned neural synthesizer with those of NetComplte, a state-of-art configuration synthesis tool based on SMT-solvers \cite{el2018netcomplete}.

\paragraph{Specifications} As the type of supported requirements in NetComplete does not fully align with our model, we restrict this comparison to specifications which only include forwarding paths (i.e. \texttt{fwd} predicates). Further, NetComplete does not support cross-protocol synthesis as in our case and instead requires users to specify for each requirement the protocol to use for its implementation. To bridge this gap, we split the generated forwarding requirements into BGP and OSPF paths for a corresponding NetComplete specification.
%\todo{note on NetComplete installing policies at all routers, not only the edges of the AS}

\paragraph{Methodology} We compare both OSPF synthesis and BGP/OSPF-synthesis. We configure our trained synthesizer model to do OSPF synthesis by only predicting link weights. For each pair of topology and specification, we report the total time of running our synthesizer 4 times using 4-shot sampling, whereas for consistency we report the best out of the 4 runs. For NetComplete, we run the synthesizer with a timeout of 25 minutes. In case a NetComplete attempt times out, we report 25 minutes as a lower bound for its runtime.

\paragraph{OSPF Synthesis Time Results} We document the results of comparing OSPF synthesis time in \cref{fig:evaluation-compare-ospf}. Our synthesizer model achieves a speedup of 2-10x over NetComplete. With 16 requirements and dataset Large this speedup even increases to $2000\times$. Further, our model achieves very high consistency with the provided specification, often producing fully-consistent configurations.

\paragraph{BGP/OSPF Synthesis Time Results} In \cref{fig:evaluation-compare-bgp} we show the comparison of BGP/OSPF synthesis time. Our synthesizer model outperforms NetComplete by multiple orders of magnitude. We observe a speedup of $20-560\times$ which appears to increase with the size of topology and specification. Further, the average specification consistency of the synthesized configurations is greater than $92\%$ across all datasets, even for large topologies. In many cases, our synthesizer model produces fully-consistent configurations, especially with small topologies and specifications. In comparison, NetComplete times out on more than half of the synthesis tasks which means that we can only observe a lower bound of speedup in these cases. Note that our synthesizer model is running on a CPU due to memory restrictions with large topologies. However, running it on a GPU results in even greater speedups (up to $1000\times$, cf. \cref{app:sec:bgp-gpu-performance}). 

==> diff/git-latexdiff.33882/old/sections/5_related_work.tex <==
\section{Related Work}
\label{sec:related-work}

\paragraph{Traditional Configuration Synthesis} 
%A range of existing work is concerned with network configuration synthesis. 
Next to methods based on compilation such as Propane/PropaneAT \cite{beckett2017network}, there are a number of configuration synthesis methods based on constraint solving: Examples include ConfigAssure \cite{narain2008declarative}, SyNet \cite{el2017network} and NetComplete \cite{el2018netcomplete}. Due to their hand-coded nature, these methods are highly protocol-specific and can be very slow due to the solvers they employ. Although some of them allow for cross-protocol reasoning, this is not implemented as transparently as in our framework and users must specify per requirement which protocol to use for its implementation. In contrast, our approach has lower precision but allows for fully transparent cross-protocol reasoning, meaning forwarding requirements are not protocol-bound and the synthesizer chooses how to implement them. Further, our learned BGP/OSPF synthesis tool exhibits much lower synthesis times as compared to an SMT-based tool like NetComplete.

% \begin{itemize}
%     \item NetComplete, SyNet
%     \item Propane, PropaneAT
%     \item DeepBGP
% \end{itemize}

\paragraph{GNNs and Networking} DeepBGP \cite{bahnasy2020deepbgp} relies on GNNs and reinforcement learning to do configuration synthesis. However, it is limited to BGP configuration synthesis and is slower than SMT-based synthesis according to the author's evaluation. In contrast, our learning-based framework is cross-protocol, does not rely on reinforcement learning and provides better synthesis performance. Apart from configuration synthesis, GNNs have also been applied to other problems in the networking domain. For example, the authors of RouteNet \cite{rusek2020routenet} use GNNs to predict performance metrics of network configurations. Other work that is concerned with learning improved protocols includes Q-Routing \cite{boyan1994packet} or more modern approaches such as the Graph-Query Neural Network architecture \cite{geyer2018learning}.

\paragraph{Neural Algorithmic Reasoning} 
Neural algorithmic reasoning (NAR) as proposed in \cite{velivckovic2021neural}, describes the idea of replacing traditional algorithms with neural networks to learn improved algorithmic procedures. Exemplary work includes graph-related algorithms \cite{velivckovic2019neural} or solvers for combinatorial optimization problems \cite{cappart2021combinatorial,joshi2020learning,selsam2019guiding}. Our synthesis framework is the first applications of NAR to the networking domain and relies on the NAR-native encode-process-decode architecture. According to the hierarchy of NAR approaches in \cite{cappart2021combinatorial}, our method is an algorithm-level approach, as we do not supervise on intermediate steps. Although, such step-level methods promise better generalization, it is not clear what an intermediate result of a general synthesis procedure would be. However, future work on a step-level approach may further improve synthesis quality.

% \begin{itemize}
%     \item RouteNet
%     \item GraphNET
%     \item Learning and generating distributed routing protocols using graph-based deep learning
%     \item Unveiling the potential of Graph Neural Networks for network modeling and optimization in SDN
% \end{itemize}

==> diff/git-latexdiff.33882/old/sections/6_conclusion.tex <==
\setlength{\parskip}{6pt plus4mm minus4mm}
\section{Conclusion}
\label{sec:conclusion}
We presented a learning-based framework for configuration synthesis based on the idea of neural algorithmic reasoning. To assess the effectiveness of the system, we instantiated it for the case of BGP/OSPF synthesis. In contrast to traditional synthesis methods, our system supports transparent cross-protocol reasoning and learns synthesis rules only from data. Using our system, synthesis is sped up by a factor of up to $500\times$ when compared to SMT-based methods. Further, our evaluation demonstrates that the resulting synthesis tool provides excellent synthesis quality, producing configurations with high specification consistency. Overall, our results illustrate that exploring the direction of learning-based network configuration synthesis is a promising direction, enabling new cross-protocol reasoning capabilities and great performance improvements. Promising future work includes construction of hybrid systems, integrating both neural models and SMT-based approaches to obtain the best of both worlds.

==> diff/git-latexdiff.34107/new/acronyms.tex <==
\DeclareAcronym{AS}{
    short = AS,
    long = autonomous system,
    short-plural = es ,
    long-plural = s
}

==> diff/git-latexdiff.34107/new/sections/0_abstract.tex <==
% Context
Computer networks employ a number of different protocols to enable efficient routing. However, due to the complexity of multiple interacting protocols, it can be hard for network operators to implement high-level routing policies and requirements. Network configuration synthesis promises to address this situation by automatically generating configurations that satisfy a provided specification. However, existing synthesis methods are often limited to single-protocol reasoning, depend on protocol-specific and hand-coded synthesis rules, and are difficult to scale due to the SMT-based methods they employ. In this work we present a rather different, learning-based method for addressing the configuration synthesis challenge, one based on the recently proposed paradigm of neural algorithmic reasoning. Our framework is protocol-agnostic, enables cross-protocol reasoning and does not depend on any hardcoded synthesis rules. To evaluate, we instantiate our framework for the case of BGP/OSPF synthesis. Our experiments show we can synthesize configurations with a very high degree of specification consistency while observing speedups of up to $500\times$ compared to a state-of-the-art SMT-based synthesis tool.


==> diff/git-latexdiff.34107/new/sections/1_intro.tex <==
\section{Introduction}
\label{sec:introduction}

The backbone of the internet consists of many connected computer networks operated by different internet service providers (ISPs) and other large organizations. These networks rely on a number of protocols to enable effective and policy-driven routing of traffic. Based on router-level configurations, the protocols perform a distributed computation to construct a network's forwarding state. However, the relatively low-level router configuration makes it hard for network operators to directly enforce network-wide policies and requirements. This often leads to misconfiguration, which can cause global outages such as the recent hours-long blackout of the entire Facebook platform \cite{janardhan2021} and comparable events \cite{mccarthy_2019}.
%
\paragraph{Configuration Synthesis} This situation has triggered a number of research efforts regarding the synthesis of network configurations \cite{el2018netcomplete,beckett2017network,narain2008declarative}. Configuration synthesis is concerned with the task of automatically generating router-level configurations given a set of high-level requirements. However, this synthesis problem can be very hard to solve, since network configurations typically consist of a considerable number of tunable parameters, where the execution of several interacting protocols yields the overall forwarding state. An effective synthesis tool must thus account for this fact and be able to reason across multiple protocols.

\paragraph{SMT-based Synthesis} Some of the most successful efforts in providing cross-protocol synthesis capabilities are based on satisfiability modulo theory (SMT) solvers \cite{el2018netcomplete,el2017network}. While SMT-based synthesis is a promising method, it comes with a number of limitations:
% \item protocol-specific
% fully hand-coded synthesis rules, a lot of implementation effort, cross-protocol support extra complicated
(1) SMT-based synthesizers are hand-crafted and highly protocol-specific. To implement synthesis, we must first express our networking model, protocol semantics including vendor and device specific behavior in terms of first-order logic constraints. This is a time-intensive and complicated process, requiring lots of expert knowledge.
%  model-dependent: synthesis is reasoning on the level of some assumed model which may not reflect the real world: even if a configuration is synthesized based on some spec, it may behave differently and violate spec in practice
Further, (2) logic-based modelling introduces a disconnect between the synthesis tool and real-world behavior \cite{birkner2021metha}. More specifically, synthesized configurations may satisfy a provided specification within a formal framework, but may not behave the same way in the real world.
% can be very slow
And, (3) SMT-based synthesis can be very slow or fail to complete, especially when reasoning about large network topologies. In practice however, network operators reconfigure their networks on a daily basis \cite{vissicchio2012improving}, which means an effective synthesis tool must be fast.

% \item fully learned, no hand-coded synthesis rules (model-free), very flexible to adapt to more/new protocols
% \item protocol-agnostic, cross-protocol
\paragraph{Neural Algorithmic Reasoning for Synthesis} Recent work on neural algorithmic reasoning (NAR) proposes to replace traditional algorithms with neural networks to learn improved algorithmic procedures \cite{velivckovic2021neural}.
It has been shown to be a powerful and fast algorithmic approximation method for a number of graph-related \cite{velivckovic2019neural} and combinatorial optimization problems \cite{cappart2021combinatorial}. Further, due to its learned nature, NAR allows for learning procedures directly from (real-world) data, without the need for manual feature extraction. Overall, this positions NAR as an attractive method to obtain a fast, fully-learned synthesis procedure, which entirely avoids the need for a formal model or any hand-crafted synthesis rules. Based on this promising outlook, this paper explores how to apply the NAR paradigm to the problem of network configuration synthesis.

To that end, we propose a \textbf{new learning-based framework for configuration synthesis} as an alternative to SMT-based approaches. Our framework is protocol-agnostic, enables cross-protocol reasoning and avoids the need to manually provide synthesis rules. We build upon the idea of NAR, and train a graph-based processor neural network to learn a synthesis procedure in latent space. A key challenge in a multi-protocol setting is the diversity of different protocols and configuration parameters. To this end, we implement a generic embedding scheme based on Datalog-like facts and program sketching \cite{solar2008program}, which allows us to easily adapt our framework to new protocols. Further, our synthesis model produces a whole distribution of network configurations. As a consequence, we can directly sample multiple alternative synthesis outputs, which is not possible with standard SMT solvers. We apply our framework to a non-trivial synthesis setting where both the Border Gateway Protocol (BGP) and the Open Shortest Path First (OSPF) protocol are used. We demonstrate that our learned synthesis tool is up to~$500\times$ faster than a state-of-the-art SMT-based synthesizer, while producing configurations which on average enjoy more than 91\% satisfaction of the provided specification.

\paragraph{Main Contributions} Our core contributions are:
\vspace{-5pt}
\begin{itemize}
    \setlength{\itemsep}{5pt}
    \setlength{\parskip}{0pt}
    \item A learning-based framework for network configuration synthesis based on neural algorithmic reasoning.
    \item A neural network architecture for learning synthesizer models which relies on a generic graph-based encoding of network topologies and configurations.
    \item An extensive evaluation of our learning-based synthesizer, in terms of both precision and scalability, on the challenging setting where both the BGP and OSPF protocols are involved.
\end{itemize}

\section{Framework Overview}
\label{sec:overview}

\begin{figure}
    \begin{center}
        \includegraphics[width=0.45\textwidth]{figures/synthesizer-overview.pdf}
    \end{center}
    \caption{An overview of our learning-based synthesis framework.}
    \label{fig:learning-based-synthesis}
\end{figure}

%As an example, consider \cref{fig:network-fwd-tree} (c) which illustrates the forwarding plane of some traffic class reachable via external peer $E$ or $F$ in our example network. Each router of the network forwards traffic along some of its outgoing links. In practice, a number of protocols are used to populate a router's routing tables. For the instantiation of our synthesis framework however, we focus on OSPF and BGP.

In the following, we discuss the fundamentals and core steps of our learning-based framework as illustrated in \cref{fig:learning-based-synthesis}.

\paragraph{Network Configuration} In this work, we consider the configuration synthesis problem at the level of the so-called \emph{forwarding plane} of a network. This means we look at how each router forwards traffic, given a packet with a certain destination. The forwarding plane is determined by a distributed computation whose exact semantics depend on the different routing protocols in use. To adapt the forwarding behavior, network operators change configuration parameters at the router-level (e.g. link weights), such that running the protocols results in the desired forwarding plane. Given this context, we define the problem of configuration synthesis as follows.

\paragraph{Configuration Synthesis} The configuration synthesis problem corresponds to automatically generating these router-level configurations, such that a set of given requirements about the forwarding plane is satisfied. Typical requirements include reachability, traffic isolation and other forwarding properties. 

\paragraph{Dataset} To train a synthesizer model, we first generate a dataset of input/output samples for the synthesis problem. For this, we rely on a generative pipeline as shown in the top of \cref{fig:learning-based-synthesis}. First, we sample a random network configuration for some topology using a uniform generative process. Then, we simulate the involved protocols to obtain the corresponding forwarding plane. Next, we extract a specification by randomly selecting properties that hold for the computed forwarding plane. This leaves us with a specification and topology as input and corresponding configuration as the output to a synthesis problem.

\paragraph{Simulation} Depending on the protocols in use, one implements simulation code to compute the forwarding plane induced by a sampled configuration. Although this step is protocol-specific, the overall implementation effort is much lower compared to SMT-based synthesis. Protocols are typically well-defined algorithms which can be simulated, whereas the alternative of implementing a synthesizer often requires expert knowledge about SMT solvers. In practice, our framework may also be adapted to use a real-world network router to compute the behavior of a configuration, thereby capturing the real-world behavior directly.

\paragraph{Neural Synthesizer Model} Based on the generated dataset, we train a graph neural network (GNN) to perform synthesis. For this, the network's input consists of a topology, a specification and a configuration sketch where to-be-synthesized parameters are omitted. Following the NAR paradigm, we first encode this synthesizer input in latent space. Then, we apply an iterative processor network which relies on the graph attention mechanism to propagate information \cite{velivckovic2017graph}. Last, we apply a decoder network to predict the values of omitted configuration parameters, thereby synthesizing a corresponding configuration. To remain protocol-agnostic, our model is generic with respect to the input format, using an intermediate representation based on Datalog-like facts.
%
\paragraph{Relaxed Specification Consistency} Since parts of the configuration synthesis problems are known to be NP-hard \cite{fortz2000internet}, any precise synthesis method will run into scalability issues, just like SMT-based methods. However, practical synthesis must be fast and scalable to accommodate the size of real-world networks and the frequency at which configurations need to be updated \cite{vissicchio2012improving}. In our learning-based framework, we therefore employ a fixed-size neural network architecture which always runs in polynomial time. While this indeed enables fast synthesis times, we cannot expect our neural system to be as precise as SMT methods. Therefore, to assess the synthesis capabilities of our learning-based system, we rely on the notion of \emph{relaxed~specification~consistency}. More specifically, we do not just check whether a configuration satisfies a specification or not, but also measure the degree up to which a synthesized configuration satisfies a specification (e.g. via the number of satisfied requirements). 

This "soft" understanding of a specification allows us to evaluate neural synthesis systems which may not always produce fully consistent configurations. Further, we argue that configurations with less than $100\%$ consistency are still very useful in practice, as they provide a good starting point for additional adjustments by network operators. Future work may improve the precision of neural synthesis by exploiting partial synthesis methods \cite{el2018netcomplete} to obtain fully consistent solutions, given a partially consistent configuration. However, note also that even exact SMT-based synthesizers may not always produce fully consistent solutions, due to differences between the formal protocol model and the one running on a given real-world router where the configuration is to be deployed \cite{birkner2021metha}.

\paragraph{Instantiation} Our learning-based synthesis framework is generic with respect to the routing protocols in use. This means, it can be instantiated to many different synthesis settings. To do this, users merely provide a drop-in replacement for the simulation component as shown in \cref{fig:learning-based-synthesis}, while other components such as the neural model architecture itself can be directly re-used.

%More specifically, we employ a slightly modified variant which operates on a graph-based encoding of a specification, topology and configuration parameters.

%  \begin{figure*}
%      \centering
%      \includegraphics[width=0.85\textwidth]{figures/system-overview.pdf}
%      \caption{An overview of our synthesis system: (1) First, we use a generic embedding scheme to transform a network topology, protocol configuration sketches and the specification given as Datalog-like facts to a latent input representation. Next, we apply a learned (2) Processor GNN and obtain a latent synthesis output. Last, we apply a (3) Decoder Network to obtain a distribution over possible values per unknown parameter in our configuration.}
%      \label{fig:overview-model}
% \end{figure*}
%

In this paper, we first discuss the architecture of our neural synthesis model. In follow-up sections, we instantiate our framework  for the case of BGP/OSPF configuration synthesis, and evaluate the resulting instantiation by comparing it to a state-of-the-art SMT-based synthesizer.

% \begin{itemize}
%     \item effort: need to implement simulation code to generate dataset to learn from (typically well-defined in protocol specs, much easier than implementing synthesis directly)
%     \item can be sampled (multiple alternative solutions, not easily possible with SMT-based methods)
%     \item much faster than SMT-based synthesis
% \end{itemize}

% Requirements:
% \begin{itemize}
%     \item protocol-agnostic
%     \item fully learned, no hand-coded synthesis rules
%     \item define: strict specification vs. relaxed specification
% \end{itemize} 

==> diff/git-latexdiff.34107/new/sections/2_model.tex <==
\section{Neural Synthesis Model}
\label{sec:model}


We now present the architecture of our graph-based neural synthesizer model, illustrated in \cref{fig:overview-model}. First, in \cref{sec:graph-embedding} we introduce our generic graph-based encoding, which allows us to embed network topologies, protocol configuration and the specification into a latent space. Then, in \cref{sec:graph-transformer} we present the architecture of the processor network which we train to perform the synthesis task. Finally, in \cref{sec:decoding-sampling} we discuss how to sample network configurations from the resulting latent synthesis output.

\begin{figure}
    \begin{minipage}[t]{0.21\textwidth}
    \begin{lstlisting}[basicstyle=\ttfamily\small, escapeinside={(*}{*)}]
router(A)
router(B)
(...)

connected(A,B,2)
connected(A,C,?)(*\blackcircled{1}*)
(...)
    \end{lstlisting}
\end{minipage}
\begin{minipage}[t]{0.21\textwidth}
    \begin{lstlisting}[basicstyle=\ttfamily\small, escapeinside={(*}{*)}]
network(N1)
bgp_route(E,N1,2,3,1,0,1)

fwd(A,B,N1)
not fwd(B,A,N1)
(...)
    \end{lstlisting}
\end{minipage}
    \caption{A snippet of a fact base sketch encoding a network's topology, parameters such as link weights (\texttt{connected} facts) and a specification (\texttt{fwd} facts).}
    \label{fig:datalog-encoding}
\end{figure}

\begin{figure}[t]
    \centering
    \includegraphics[width=0.25\textwidth]{figures/synth-architecture.png}
    \caption{The neural synthesizer model architecture.}
    \label{fig:architecture}
\end{figure}

\subsection{Fact Base Embedding}
\label{sec:graph-embedding}
To remain network protocol-agnostic in our model architecture, we implement a generic graph-based encoding of Datalog-like facts, similar to knowledge graphs \cite{rosso2020beyond}. This means that we first encode topologies, configurations and specifications as a set of Datalog-like facts and then employ a generic embedding.
%We chose Datalog facts as the input format of our synthesis approach for its flexibility, wide-spread use in Program Analysis and use in previous work on configuration synthesis \cite{el2017network}.

\paragraph{Fact Base} A set of Datalog-like facts, as depicted in \cref{fig:datalog-encoding}, serves as the input \emph{fact base} $\mathcal{F}$ to our synthesizer model. $\mathcal{F}$ is a set of facts $f(a_0, \dots, a_n)$ where arguments may be constants (e.g. A or B) or integer literals. Further, each fact in a fact base has a corresponding truth value denoted as $[f(a)]_{\mathcal{B}}$. For instance, from the fact base in \cref{fig:datalog-encoding} we can derive $[fwd(A,B,N1)]_{\mathcal{B}} = \text{\texttt{true}}$ and $[fwd(B,A,N1)]_{\mathcal{B}} = \text{\texttt{false}}$.

\paragraph{Consistency} We represent a network's topology, the protocol configuration and parameters as well as the specification, all in a single fact base. Given the semantics of the protocols in use, we can then check whether the specification encoded in a fact base is satisfied by the provided configuration. To quantify, we define the notion of relaxed specification consistency, as discussed earlier, with respect to a fact base: Given a fact base $\mathcal{F}$, a subset of specification facts $S \subset \mathcal{F}$ and protocol semantics $\mathcal{P}$, the \emph{consistency} of a fact base is defined as the relative number of satisfied facts in $S$ with respect to the forwarding plane obtained via $\mathcal{P}$. The contents of $S$ depend on the concrete instantiation of the synthesizer model. For an example of possible specification facts, see our instantiation of the synthesizer model for BGP/OSPF in \cref{sec:training}.

\begin{figure*}
    \footnotesize
    \def\arraystretch{1.4}
    \begin{tabular}{lr}
        %$T_f: T_1 \times \dots \times T_n$ & \textit{(fact type declaration)}\\
        $emb(f) := \mathbf{V_f}$ & \textit{(learned fact type embedding)}\\
        $emb(b) := \mathbf{W_{\text{bool}}}\;onehot(b)$ & \textit{(learned boolean embedding)}\\
        $emb(f,i,v) := \mathbf{W_{f_i}}\;onehot(v)$ & \textit{(learned integer embedding)}\\
        $emb(f,i,?) := \mathbf{V_{hole}}$ & \textit{(learned hole embedding)}\vspace{2pt}\\
        $\mathlarger{
        h_c := \sum_{f(c) \in \mathcal{F}}
        emb(f)
        }$ & \textit{(constant embedding)}\vspace{2pt}\\
        $h_{f(a_0, \dots, a_n)} := emb(f) + emb([f(a_0, \dots, a_n)]_{\mathcal{B}}) + \mathlarger{
        \sum_{(i,v) \in \mathcal{I}(f(a_0, \dots, a_n))}
        emb(f, i, v)
        }$\hspace{-1.2cm} & \textit{(fact embedding)}\\
        $\mathcal{I}(f(a_0, \dots, a_n)) := \{(i,v) \; | \; f(a_0, \dots, a_{i-1}, v, \dots, a_n) \in \mathcal{F} \wedge v:Int \wedge i \in \mathbb{N}$ \}& \textit{(integer arguments)}\vspace{2pt}\\
        $N_i(h_c) := \{h_f \; | \; \exists i \in \mathbb{N} . f(a_0, \dots, a_{i-1}, c, a_{i+1}, \dots, a_n) \in \mathcal{F}\}$& \textit{(i-th neighborhood of constant node)} \\
        $N_i(h_f) := \{h_c \; | \; \exists i \in \mathbb{N} . f(a_0, \dots, a_{i-1}, c, a_{i+1}, \dots, a_n) \in \mathcal{F}\}$& \textit{(i-th neighborhood of fact node)} \\
    \end{tabular}
    \caption{Translating a fact base $\mathcal{F}$ to node features. $f$ denotes a predicate, $v$ integer values, $b$ boolean values as 0 or 1, $i$ argument indices and $[f(a)]_{\mathcal{B}}$ the truth value of a fact. }
    \label{fig:graph-embedding}
\end{figure*}

%discuss embedding as shown in \cref{fig:datalog-encoding}. Note how this makes fact bases a suitable input to standard GNN architectures.

\paragraph{Fact Base Sketching} In a synthesis setting, we are confronted with incomplete fact bases, i.e. the specification and topology is given but the network configuration is to be synthesized. For these cases, we also consider fact bases with unknown parameters inspired by the idea of program sketching in program synthesis \cite{solar2008program}. More specifically, users may replace an unknown integer argument of a fact by a \texttt{?} symbol, indicating a value to be synthesized. Using this mechanic, we can represent the synthesis input as an incomplete fact base which encodes to-be-synthesized values as unknown parameters. As an example, consider \cref{fig:datalog-encoding} \blackcircled{1}, where the link weight between router nodes \texttt{A} and \texttt{C} is represented as an unknown parameter.

\paragraph{Embedding} We employ a structurally-defined embedding scheme to transform a fact base into a graph with node features as required for processing with graph neural networks. Given a fact base $\mathcal{F}$, we apply the rules in \cref{fig:graph-embedding} to obtain node features and adjacency information. Both a fact $f$ and a constant $c$ are represented as distinct nodes with features $h_c$ and $h_f$, respectively. The relationships between facts and constants is encoded as node adjacency as defined by the neighborhood functions $N_i$.

We use multiple neighborhood functions, i.e. multiple types of edges, to encode the argument position of a constant occurring in a fact. Hence, the number of neighborhood functions corresponds to the maximum number of arguments in a single fact, e.g. 3 in \cref{fig:datalog-encoding}. Integer arguments and unary facts are directly accounted for in the respective node or fact embedding. To handle unknown parameters, we replace the corresponding $emb(...)$ term with the learned $\mathbf{V_{hole}}$ embedding.

Considering the embedding function $emb$, the learned parameters of our embedding are $\mathbf{V_f} \in \mathbb{R}^D$ per fact type in~$\mathcal{F}$, $\mathbf{W_{\text{bool}}} \in \mathbb{R}^{D \times 2}$ for boolean values, $\mathbf{W_{f_i}} \in \mathbb{R}^{D \times N}$ per integer argument of fact type $f$ and $\mathbf{V_{hole}} \in \mathbb{R}^D$ to represent unknown parameters. Hyperparameter $D$ represents the dimension of the latent space the synthesizer model operates in and $N$ specifies the number of supported integer values. An example of applying this embedding scheme to a simple fact base is given in \cref{fig:graph-encoding-example}.

\begin{figure}
    \begin{minipage}[t]{0.2\textwidth}
        \centering
        \footnotesize
        \textbf{Fact Base}
        \begin{lstlisting}[basicstyle=\ttfamily\small]
router(A)
router(B)

conn(A, B, 12)
        \end{lstlisting}
    \end{minipage}
    \begin{minipage}[t]{0.15\textwidth}
        \centering
        \textbf{Graph}\\
        \vspace{5pt}
        \includegraphics[width=0.7\textwidth]{figures/graph-encoding.pdf}
    \end{minipage}\\
    \centering\\
    \vspace{10pt}
    \textbf{Node Features}\\
    \vspace{10pt}
    \begin{minipage}[t]{0.5\textwidth}
        $\begin{array}{rcl}
        h_A &:=& emb(router) = \mathbf{V_{\text{router}}}\\
        h_B &:=& emb(router) = \mathbf{V_{\text{router}}}\\
        h_{\text{conn(A,B,12)}} &:=& emb(conn) + emb(conn, 2, 12)\\
        &:=& \mathbf{V_{\text{conn}}} + \mathbf{W_{conn_2}} onehot(12)
    \end{array}$
    \end{minipage}
    \caption{An example of embedding a simple fact base using the embedding scheme of \cref{fig:graph-embedding}. The shown graph illustrates the neighborhoods $N_0$ and $N_1$ induced by the \texttt{conn} fact.}
    \label{fig:graph-encoding-example}
\end{figure}

\begin{figure}
    $$
    \begin{array}{rcl}
    z_j &:=& h_j + Drop(\mathlarger{\sum_{N_i}} h'_{GAT_i})\\
    h'_j &:=& FFN(Norm(z_j))\vspace{11pt}\\
    FFN(x_j) &:=& Norm(Lin2(Drop(Lin1(x_j)))))
    \end{array}
    $$
    \caption{
        The recurrence relation of a node $j$'s representation $h_j$. $h'_{GAT_i}$ represents the output of a graph attention layer operating with neighborhood $N_i$ according to \cite{velivckovic2017graph}, $h_j$ the representation of node $j$ at the previous step. $Norm$ refers to batch normalization \cite{ioffe2015batch}, $Drop$ to dropout regularization \cite{hinton2012improving} and $Lin1$ and $Lin2$ to linear layers with an inner dimension of $4N$.
    }
    \label{fig:recurrence}
\end{figure}

\subsection{Synthesizer Model}
\label{sec:graph-transformer}

For an illustration of the synthesizer model's architecture, please see Figure~\ref{fig:architecture}. Given a fact base $\mathcal{F}$ we first apply our embedding scheme as described in \cref{sec:graph-embedding}. We then employ a 2-layer GNN-based encoder network to produce the latent representation of a synthesis input.
Given this representation, a processors network is trained to perform the actual synthesis task in high-dimensional space. Last, we apply a set of decoder networks, to obtain the synthesized values of unknown parameter, given the latent synthesis~output.

%In this context, the synthesis problem for network configurations corresponds to completing partially provided fact bases.

% \paragraph{High-Level Architecture}

% We employ the high-level architecture to obtain the latent synthesis output $y_\mathcal{F}$:
% $$
% \begin{array}{rcl}
%     \mathbf{x_{\mathcal{F}}} &:=& Encoder(Embedding(\mathcal{F}))\\
%     \mathbf{y_{\mathcal{F}}} &:=& Processor(\mathbf{x_{\mathcal{F}}} + \mathbf{z})\\
%     z_i &\sim& \mathcal{N}(0,1)
% \end{array}
% $$
% \todo{z is only added for $i<N/2$}

% $Embedding$ corresponds to the graph-based embedding as discussed in \cref{sec:graph-embedding} and $Encoder$ is a 2-layer graph attention module. $Processor$

\paragraph{Encoding} The encoder GNN operates on the embedded representation of a fact base. It produces the high-dimensional representation of a synthesis input as required for the processor network. We additionally apply noise to the first half of the units of the latent representation via $\mathbf{z}$, as a source of non-determinism. According to our experiments this improves model performance and we hypothesize this is due to the synthesis problem having more than one solution in most cases.

\paragraph{Iterative Processor} The processor network is modelled as an iterative process. It consists of a 6-layer graph attention module which we apply for a total of 4 iterations. In the framework of neural algorithmic reasoning, this iterative computational structure encodes an inductive bias towards an iterative solution to the synthesis problem. Because of this bias, our processor network essentially learns an algorithmic procedure which iteratively synthesizes the values of unknown parameters in a fact base.

\paragraph{Graph Attention Layer} In the GNNs we employ, we rely on a composed variant of the graph attention layer as introduced by \cite{velivckovic2017graph}. We employ multiple graph attention layers in lockstep, one per neighborhood $N_i$ defined by our graph embedding (cf. \cref{sec:graph-embedding}), and combine the intermediate results after each step. Specifically, the recurrence relation of a node $j$'s representation $h_j$ is defined as shown in \cref{fig:recurrence}. These mechanics of combining the results of the different graph attention layers $h'_{GAT_i}$, directly corresponds to how multiple attention heads are combined in the original Transformer architecture \cite{vaswani2017attention}.

\paragraph{Argument Decoder Networks} To synthesize the values of unknown parameters, the model maintains a set of decoder networks. That is, it provides one decoder network per integer argument per fact type in a fact base. When decoding, the network is applied to the latent synthesis output of the corresponding fact node. For example, a synthesizer model which operates on the fact base in \cref{fig:datalog-encoding}, would provide a decoder network $D_{\text{connected}_2}: \mathbb{R}^D \rightarrow \mathbb{R^N}$ to decode values for the third argument of a \texttt{conn} fact. In our experiments, decoder networks are implemented as simple multi-layer perceptron models.

\paragraph{Supervision Signal} During training, we mask all fact arguments that represent to-be-synthesized configuration parameters in our synthesis setting. As a supervision signal we use the masked values as the ground-truth and apply a negative log-likelihood loss function to the output distribution of the corresponding argument decoder networks.

%The synthesizer model learns a conditional distribution of fact bases which are consistent with respect to the protocols' semantics.

%\todo{introduce synthesis as a completion problem of an encoded fact base (a la BERT). Introduce masking, introduce decoding of integer and truth values. Synthesis is learning a conditional distribution of consistent fact bases.}

%Using this method, we obtain the node features $h_c$ per constant, $h_f$ per fact and adjacency information in terms of node neighborhood functions $N_i(h_c)$ and $N_i(h_f)$. Overall, this encoding makes a fact base suitable for processing using standard graph neural networks.

%- Brief description of the Graph Transformer Model
\subsection{Multi-Shot Sampling}
\label{sec:decoding-sampling}

%Multi-Stage Parameter Sampling (sampling methods: topk, high-temp, low-temp)
To sample concrete values from the output distributions over unknown parameters, we apply a multi-shot sampling strategy. That is, we sample values only for a subset of unknown parameters, insert them in our input fact base and run the synthesis model again. We repeat this process until no more unknown parameters remain. This multi-shot sampling strategy allows the model to incorporate the concrete values of previously synthesized parameters in its computation. In our evaluation in \cref{sec:evaluation}, we include a comparison of how this compares to sampling all unknown parameters at once.

%In a fact base with multiple holes, we apply the corresponding decoder networks to obtain a value distribution for each integer hole. However, instead of sampling all integer holes in one


==> diff/git-latexdiff.34107/new/sections/3_bgp_ospf.tex <==
\section{BGP/OSPF Synthesis}
\label{sec:bgp-ospf}

\newcommand{\as}{\ac{AS}~}
\newcommand{\ases}{\acp{AS}~}

\newcommand{\squareann}{{\tiny$\blacksquare\;$}}
\newcommand{\triangleann}{{\small$\blacktriangle\;$}}

\begin{figure*}
    \centering
    \includegraphics[width=0.95\textwidth]{figures/networks-all.pdf}
    \caption{(a) An illustration of a small AS network, including internal peers (blue), external peers (purple), BGP sessions as well as physical links. (b) The propagation of two BGP announcement across the network. (c) The resulting forwarding plane after applying BGP and OSPF.}
    \label{fig:network-fwd-tree}
\end{figure*}

We now discuss an instantiation of our learning-based framework for the case of BGP and OSPF protocols. In \cref{sec:synthesis-setting} we introduce a basic networking model, BGP and OSPF protocols and the synthesis setting. Given this model, \cref{sec:training} describes how to generate a corresponding dataset of input/output samples and train a synthesizer model.
%This shall serve as a prerequisite to the instantiation of our learning-based synthesis framework for the BGP and OSPF protocol in \cref{sec:training}.

\subsection{Synthesis Setting}
\label{sec:synthesis-setting}

\paragraph{Graphical Model} We assume an abstract network model which can be represented as an undirected graph as shown in \cref{fig:network-fwd-tree} (a). We always consider a set of internal routers (A, B, C, D in \cref{fig:network-fwd-tree}) as well as a set of adjacent external routers (E, F  in \cref{fig:network-fwd-tree}). The group of internal routers forms the \emph{\as} under consideration whereas external routers belong to other adjacent \ases. In practice, an \as represents an administrative domain controlled by a single operator. 

\paragraph{Forwarding Plane} For an example of a possible forwarding plane in this abstract model, consider \cref{fig:network-fwd-tree} (c) which illustrates the forwarding plane of traffic destined towards some destination reachable via external peer $E$ or $F$. Each router of the network forwards traffic along some of its outgoing links. In practice, a number of protocols are used to compute the forwarding plane. However, here we focus on OSPF and BGP.

\paragraph{OSPF} The OSPF protocol \cite{moy1994ospf} is a link-state protocol, typically used as an interior gateway protocol~(IGP), i.e., to route traffic within an \ac{AS}. Given link weights per physical link in the network, OSPF simply routes traffic along the shortest path towards the destination.

\paragraph{BGP} The BGP protocol \cite{rekhter1994border} on the other hand is a path-vector protocol used to exchange reachability information mostly on the level of \acp{AS}.
%These are groups of routers typically operated by a single party (e.g. an ISP).
When using BGP, a routing destination announces its existence to other \ases and routers, by sending out a BGP announcement. Receivers of such announcements may then choose to pass them on to other \acp{AS}, redistribute them internally and/or modify them. Instead of communicating along physical links directly, the BGP protocol requires manually configured BGP sessions among routers of the \as and external peers, as indicated by the BGP session edges in \cref{fig:network-fwd-tree}(a).
%\todo{more discussion of eBGP vs iBGP and support for route reflection (more of an implementation detail, maybe only mention in dataset generation where simulation code is discussed)}.

%\paragraph{BGP Decision Procedure}~
%\todo{discuss decision procedure}
In case a router receives more than one announcement for a destination, a designated BGP decision process is applied to determine a single best route. \cref{fig:bgp-decision} shows the ordered list of comparison criteria of this decision process. The different criteria depend different properties of a route announcements, including the IGP cost towards the routing destination. As a consequence, when used together, OSPF as IGP protocol and BGP will interact. %Note also that BGP is an iterative process which needs multiple rounds of propagation to converge.

\paragraph{Example}
%\todo{run through simple BGP+OSPF example of computing the forwarding plane}
To better understand BGP/OSPF routing, consider the simple example given in \cref{fig:network-fwd-tree} (b). Here, our example \as imports BGP announcements \squareann and \triangleann from E and F respectively. Both represent a route to the same destination. As shown, both announcements have a so-called local preference of 2. For simplicity, we ignore other properties such as the AS path length, Origin and MED in this example. The announcements are propagated among BGP neighbors and the best route is selected according to the decision procedure in \cref{fig:bgp-decision}. See \cref{fig:network-fwd-tree} (b) for an illustration of the intermediate states of this propagation process. As both announcements have a local preference of 2, rule 1 of the decision process is not used. Instead, in round 2, node B selects \squareann over \triangleann due to a lower IGP cost of 2 via egress node A as compared to 3 via egress node D (rule 6). Node D selects \triangleann over \squareann, since it learns this route directly from an external peer (rule 5). After Round 3, the BGP propagation process converges to a stable state and we can derive the forwarding plane as shown in \cref{fig:network-fwd-tree} (c).


%, as well as external peers E and F which belong to other \acp{AS}. External peers are routers which are connected via eBGP sessions to routers of the \ac{AS} under consideration. They announce BGP routes to their neighbors, which are propagated within the network

%\paragraph{BGP/OSPF Configuration Synthesis} We phrase the BGP/OSPF configuration synthesis problem on the level of the forwarding plane. This means that users provide a specification which constraints the set of allowed forwarding planes. This includes predicates which enforce forwarding paths, block forwarding paths or assert higher-level properties like traffic isolation and reachability. Given such a specification, we consider network configuration synthesis as the task of configuring OSPF and BGP in a way that produces a forwarding plane which satisfies the provided specification.

\paragraph{BGP/OSPF Configuration Synthesis} According to our general synthesis framework, we consider the BGP/OSPF configuration synthesis problem at the level of the forwarding plane. However, we further also define the set of synthesized parameters: For OSPF we synthesize link weights as explored in a wide range of existing work (e.g. \cite{el2018netcomplete,fortz2000internet}. For BGP, the set of parameters is not defined as clearly: Depending on the requirements of a network operator, one may employ custom BGP import and export policies at every router of a network to implement complex behavior. However, in this instantiation we focus on a simplified setting, where we assume BGP route announcements to only be modified when imported into the \as from an external peer. Previous work has already pointed out that this is a reasonable assumption which holds for the majority of real-world networks \cite{caesar2005bgp,cittadini2010doing, steffen2020probabilistic}.

\begin{figure}
    \small{
    \begin{enumerate}
        \setlength{\itemsep}{0pt}
        \setlength{\parskip}{0pt}
        \item Highest Local preference
        \item Lowest AS path length
        \item Prefer Origin (IGP $>$ EBGP $>$ INCOMPLETE)
        \item Lowest Multi-exit discriminator (MED)
        \item External over internal announcements
        \item Lowest IGP cost to egress
        \item Lowest BGP peer id (tie breaker)
    \end{enumerate}}
    \vspace{-15pt}
    \caption{The BGP decision process \cite{rekhter1994border}. The shown rules are applied in order until a single best BGP announcements remains.}
    \label{fig:bgp-decision}
\end{figure}

\subsection{Dataset Generation and Training}
\label{sec:training}
To train a synthesizer model, we need a large number of fact bases encoding a variety of network topologies, configurations and forwarding specifications. Further, we must provide the model with target values for unknown parameters as a supervision signal. This section discusses how we construct such a dataset for BGP/OSPF synthesis.
%Further, we provide an example of what a corresponding fact base looks like, including a description of the supported specification language.

\paragraph{Dataset Generation} To obtain network configurations and corresponding forwarding specifications we employ a generative process: We first randomly configure BGP and OSPF parameters for some topology. Then we simulate the OSPF and BGP protocol and compute the resulting forwarding plane. Based on this, we extract a forwarding specification which fixes a random subset of forwarding paths, reachability and isolation properties that are satisfied by the forwarding plane.

\paragraph{Topologies} For training, our dataset is based on random topologies with $16$-$24$ routers. We generate the physical layout of these graphs by triangulation of uniformly sampled points in two-dimensional space.

\paragraph{Simulation} To compute the forwarding plane given an OSPF and BGP configuration, we simulate the protocols. For OSPF, we implement shortest path computation to obtain the forwarding plane. For BGP, we implement the full BGP decision process as shown in \cref{fig:bgp-decision}, except for the MED attribute. In addition to the basic networking model discussed in \cref{sec:synthesis-setting}, we implement support for eBGP and iBGP, fully-meshed BGP session layouts as well as layouts relying on route reflection. For more details of these BGP concepts see \cite{bates2000rr}.

%Note that the synthesizer model will reason on the level of the provided training samples. That is, to improve the overall synthesis quality in a real-world setting, it is helpful to implement simulation code which behaves very similar to real-world networks. Another promising approach would be to extract training samples from real-world networks, thereby circumventing the need for simulation, however, we leave this as future work.

%While this can be a considerable effort, it is typically an easier task than to implement the synthesizer directly. The concrete semantics of protocols and their simulation is a well-defined procedure, whereas implementing efficient synthesis tools is still an open problem.

\paragraph{Fact Base Encoding} We encode synthesis input using a small set of facts. For an example of a corresponding fact base see \cref{fig:bgp-ospf-fact-base}. We use the \texttt{router}, \texttt{external} and \texttt{network} facts to mark routers, external peers and routing destinations respectively. Physical links between routers are encoded as \texttt{connected(R1,R2,W)} facts where \texttt{W} denotes the OSPF link weight. Further, we rely on \texttt{ibgp}, \texttt{ebgp}, \texttt{route\_reflector} and \texttt{bgp\_route} facts to represent different types of BGP sessions and imported routes. Using the notion of unknown parameters as discussed in \cref{sec:graph-embedding}, we encode configuration parameters, e.g., properties of imported routes or OSPF link weights.

\paragraph{Specification Language} We support a small specification language with three types of forwarding predicates:

\begin{itemize}
    \setlength{\itemsep}{0pt}
    \setlength{\parskip}{2pt}
    \item \texttt{fwd(R1, Net, R2)} specifies that router \texttt{R1} forwards traffic destined for \texttt{Net} to its neighbor \texttt{R2}.
    \item \texttt{reachable(R1, Net, R2)} specifies that traffic destined for \texttt{Net} that passes through \texttt{R1} also passes through \texttt{R2} before reaching its destination.
    \item \texttt{trafficIsolation(R1, R2, N1, N2)} specifies that it must not hold that $[fwd(R1,R2,N1)]_{\mathcal{B}} \wedge [fwd(R1,R2,N2)]_{\mathcal{B}}$.
\end{itemize}

In the negative case of each predicate, the opposite must hold true for the fact to be satisfied. This specification language can easily be extended by including new specification predicates in the dataset generation process. One must simply provide a method of extracting positive and negative cases of a specification fact from a given forwarding plane. Once included in the training dataset of a synthesizer model, the resulting synthesis system will be able to consider specifications relying on the new type of predicates.

% \todo{info on loss function, optimizer, etc.}
\paragraph{Training} We generate a dataset of $10,240$ input/output samples and instantiate our synthesizer model with a hidden dimension $D$ of $64$. For optimization, we use the Adam optimizer \cite{kingma2014adam} with a learning rate of $10^{-4}$. We stop training after the specification consistency on a validation dataset no longer increases at $\sim2800$ epochs.

\begin{figure}
\begin{minipage}[t]{0.22\textwidth}
\begin{lstlisting}[basicstyle=\ttfamily\tiny]
# topology and configuration
router(c5)
router(c3)
router(c1)
router(c0)
network(c6)
network(c7)

external(c8)
external(c9)
external(c10)
external(c11)
external(c12)
external(c13)

route_reflector(c2)
route_reflector(c4)

connected(c2,c4,?)
connected(c2,c5,?)
connected(c2,c3,?)
connected(c4,c5,?)
connected(c4,c3,?)
connected(c4,c0,?)
connected(c5,c1,?)
connected(c5,c0,?)
connected(c3,c0,?)
connected(c3,c1,?)
connected(c1,c0,?)

ibgp(c2,c4)
ibgp(c2,c5)
ibgp(c2,c0)
ibgp(c2,c1)
ibgp(c4,c3)
ibgp(c4,c4)
\end{lstlisting}
\end{minipage}
\begin{minipage}[t]{0.2\textwidth}
\begin{lstlisting}[basicstyle=\ttfamily\tiny]
ebgp(c2,c12)
ebgp(c5,c9)
ebgp(c5,c10)
ebgp(c5,c13)
ebgp(c0,c8)
ebgp(c0,c11)

bgp_route(c8,c6,?,?,1,?,1,8)
bgp_route(c9,c6,?,?,0,?,1,9)
bgp_route(c10,c6,?,?,0,?,1,10)
bgp_route(c11,c7,?,?,0,?,1,11)
bgp_route(c12,c7,?,?,0,?,1,12)
bgp_route(c13,c7,?,?,2,?,1,13)

# forwarding specification
fwd(c0,c6,c3)
fwd(c3,c6,c2)
fwd(c2,c6,c4)
not fwd(c3,c6,c0)
not fwd(c0,c6,c11)
not fwd(c11,c6,c0)

not trafficIsolation(c1,c0,c7,c6)
not trafficIsolation(c1,c0,c7,c6)
trafficIsolation(c0,c3,c6,c7)
trafficIsolation(c0,c3,c6,c7)

reachable(c5,c6,c10)
reachable(c1,c6,c4)
not reachable(c0,c6,c5)
reachable(c5,c6,c10)
\end{lstlisting}
\end{minipage}
\caption{An example of a fact base encoding a topology, a sketch of a BGP and OSPF configuration and a forwarding specification.}
\label{fig:bgp-ospf-fact-base}
\end{figure} 

==> diff/git-latexdiff.34107/new/sections/4_evaluation.tex <==
\section{Evaluation}
\label{sec:evaluation}

We trained a synthesizer model to perform configuration synthesis for BGP and OSPF. We now assess the performance of the resulting neural synthesizer with respect to two core metrics: (1) the quality of synthesized configurations in terms of their consistency with the provided forwarding specifications (\cref{sec:synthesis-quality}), and (ii) the time a learned synthesizer takes when compared to the state-of-the-art SMT-based synthesizer NetComplete \cite{el2018netcomplete} (\cref{sec:synthesis-vs-smt}).

\paragraph{Dataset} We compare across three datasets: Small, Medium and Large. Each dataset represents 8 real-world topologies, sampled from the Topology Zoo \cite{knight2011internet}, where the number of nodes lies between 0-34, 34-68 and 68-170 respectively. To obtain forwarding specifications for the sampled topologies, we use our generative pipeline as discussed in \cref{sec:training}. In each topology, we do synthesis for 4 different traffic classes (routing destinations) at a time.

\paragraph{Experimental Setup} We run all our experiments on an Ubuntu Linux machine with an Intel(R)~Core(TM)~i9-9900X~@~3.50GHz processor, 64GB of system memory and an NVIDIA GeForce RTX 3080 GPU with 10GB of video~memory.

\subsection{Synthesis Quality}
\label{sec:synthesis-quality}
To assess our learned synthesizer, we examine its behavior with increasingly large topologies and specifications.

\paragraph{Specifications} Using the same generative model as described in \cref{sec:training}, we generate forwarding specifications for the topologies in our three datasets with each specification constructed from $3 \times n$ requirements, one per supported predicate type:  \texttt{fwd} requirements correspond to specifying or blocking a forwarding path using multiple \texttt{fwd} predicates whereas \texttt{reachable} and \texttt{trafficIsolation} requirements each translate to a single specification fact. We compare across increasingly large specifications of $3\times 2$, $3\times 8$ and $3 \times 16$ requirements, respectively.

\paragraph{Methodology} For each pair of topology and specification, we run our synthesizer 5 times and report the network configurations with the highest overall consistency value. For sampling, we rely on our multi-shot sampling strategy where we randomly group the unknown parameters of a configuration into 4 groups (4-shot sampling).

\paragraph{Results} We summarize our results in \cref{fig:eval-consistency}. On average, our synthesis model produces network configurations that are $>91\%$ consistent with the provided forwarding specifications across all datasets and sizes of specifications. When only few requirements are given, the synthesizer model even succeeds in producing fully-consistent configurations. We observe a slightly decreasing consistency with increasingly large topologies.

%\texttt{fwd} facts are satisfied more easily, whereas \texttt{reachable} and \texttt{trafficIsolation} facts are violated more often.

\paragraph{Multi-Shot Sampling} In \cref{fig:eval-consistency-baseline}, we report the average specification consistency using our multi-shot sampling strategy as compared to sampling all unknown parameters at once. As a baseline we have also sampled random configurations from a uniform distribution (per parameter) and compute the corresponding specification consistency. Over the baseline, our synthesizer model shows clear improvement and multi-shot sampling further increases consistency.

\begin{figure*}
    \begin{center}
        \textbf{Specification Consistency}\\
        \footnotesize
        \begin{tabular}{rrcccccccccc}
        \toprule
        \multicolumn{2}{c}{Dataset} & \tiny\texttt{fwd} & \tiny\texttt{reachable}  & \tiny\texttt{trafficIsolation} & Overall & $\emptyset$     No. Full Matches & $\emptyset$ No. $>90\%$ Matches\\
        \midrule
        $3\times 2$ requirements & Small & 0.95 & 0.94 & 1.00 & \textbf{0.95} & 0.62 & 0.62\\
& Medium & 0.96 & 1.00 & 0.94 & \textbf{0.96} & 0.88 & 0.88\\
& Large & 0.94 & 0.94 & 1.00 & \textbf{0.93} & 0.62 & 0.62\\
\midrule
$3\times 8$ requirements & Small & 0.97 & 0.98 & 0.97 & \textbf{0.98} & 0.50 & 1.00\\
& Medium & 0.99 & 0.95 & 1.00 & \textbf{0.98} & 0.50 & 1.00\\
& Large & 0.96 & 0.95 & 0.91 & \textbf{0.94} & 0.38 & 0.88\\
\midrule
$3\times 16$ requirements & Small & 0.97 & 0.89 & 0.95 & \textbf{0.94} & 0.38 & 0.75\\
& Medium & 0.98 & 0.97 & 0.97 & \textbf{0.98} & 0.38 & 1.00\\
& Large & 0.92 & 0.88 & 0.95 & \textbf{0.91} & 0.12 & 0.50\\
    \end{tabular}\end{center}
    \caption{Average specification consistency of the network configurations synthesized by our trained synthesizer model. Per sample we run the synthesizer with a specification of $3\times N$ requirements, where the specifications always include $N$ requirements per supported predicate type (\texttt{fwd}, \texttt{reachable}, \texttt{trafficIsolation}).}
    \label{fig:eval-consistency}
\end{figure*}

\begin{figure}
    \begin{center}
        \footnotesize
        \begin{tabular}{rrcccccccccc}
        &  & \multicolumn{2}{c}{Neural}\\
        & Random & 1-Shot & 4-shot\\
        \toprule
        Small & 0.83 & 0.92 & \textbf{0.94} \\
        Medium & 0.88 & 0.95 & \textbf{0.98} \\
        Large & 0.78 & 0.88 & \textbf{0.91} \\
    \end{tabular}\end{center}
    \caption{Average specification consistency with $3\times 16$ requirements when sampling configurations randomly from a uniform distribution and 1-shot/4-shot sampling using our synthesizer model.}
    \label{fig:eval-consistency-baseline}
\end{figure}

\begin{figure*}[ht]
    \footnotesize
    \begin{center}
        \textbf{BGP Synthesis Time}
        \footnotesize
        \begin{tabular}{rrccccccccc}
        \toprule
        &&\multicolumn{3}{c}{Synthesis Time (s)} & \multicolumn{2}{c}{Accuracy (Neural)} \\
        \multicolumn{2}{l}{\# Requirements} & NetComplete & Neural (CPU) & Speedup &$\emptyset$ Consistency& $\emptyset$ No. Full Matches\\
        \midrule
    2 requirements &Small & 18.073s & 0.641s & \textbf{28.2x} & 0.969 & 0.875\\
        &Medium & 60.864s & 2.748s & \textbf{22.2x} & 0.939 & 0.75\\
        &Large & 1389.485s\tiny{  7/8 TO} & 22.301s & \textbf{62.3x} & 0.989 & 0.875\\
    \midrule
    8 requirements &Small & 247.691s & 1.065s & \textbf{232.5x} & 0.96 & 0.75\\
        &Medium & $>$25m\tiny{  8/8 TO} & 3.47s & \textbf{432.2x} & 0.968 & 0.5\\
        &Large & $>$25m\tiny{  8/8 TO} & 30.961s & \textbf{48.4x} & 0.969 & 0.75\\
    \midrule
    16 requirements &Small & 1416.828s\tiny{  7/8 TO} & 2.528s & \textbf{560.5x} & 0.926 & 0.25\\
        &Medium & $>$25m\tiny{  8/8 TO} & 5.481s & \textbf{273.7x} & 0.947 & 0.25\\
        &Large & $>$25m\tiny{  8/8 TO} & 69.092s & \textbf{21.7x} & 0.959 & 0.25\\
    \end{tabular}\end{center}
    \caption{Comparing consistency and synthesis time of our method (Neural) with the SMT-based state-of-art synthesis tool NetComplete. The notation {\tiny{n/8 TO}} indicates the number of timed out synthesis runs out of 8 (25+ minutes).}
    \label{fig:evaluation-compare-bgp}
\end{figure*}

\begin{figure*}[ht]
    \begin{center}
        \footnotesize
        \textbf{OSPF Synthesis Time}\\
        \footnotesize
        \begin{tabular}{rrccccccccc}
        \toprule
        &&\multicolumn{3}{c}{Synthesis Time (s)} & \multicolumn{2}{c}{Accuracy (Neural)} \\
        \multicolumn{2}{l}{} & NetComplete & Neural (GPU) & Speedup &$\emptyset$ Consistency& $\emptyset$ No. Full Matches\\
        \midrule
    2 requirements &Small & 0.265s & 0.091s & \textbf{2.9x} & 1.000 & 1.00\\
     &Medium & 0.404s & 0.098s & \textbf{4.1x} & 1.000 & 1.00\\
     &Large & 0.944s & 0.14s & \textbf{6.7x} & 1.000 & 1.00\\
    \midrule
    8 requirements &Small & 0.876s & 0.164s & \textbf{5.3x} & 0.982 & 0.75\\
     &Medium & 1.517s & 0.103s & \textbf{14.7x} & 1.000 & 1.00\\
     &Large & 3.505s & 0.316s & \textbf{11.1x} & 0.981 & 0.50\\
    \midrule
    16 requirements &Small & 1.65s & 0.21s & \textbf{7.9x} & 0.991 & 0.625\\
     &Medium & 2.646s & 0.245s & \textbf{10.8x} & 0.989 & 0.50\\
     &Large & $>$566.636s+\tiny{  3/8 TO} & 0.233s & \textbf{2430.4x} & 0.987 & 0.875\\
    \end{tabular}\end{center}
    \caption{Comparing consistency and synthesis time of our method (Neural) with the SMT-based OSPF synthesis tool NetComplete. The notation {\tiny{n/8 TO}} indicates the number of timed out synthesis runs out of 8 (25+ minutes).}
    \label{fig:evaluation-compare-ospf}
\end{figure*}


\subsection{Comparison to SMT-based Synthesis}
\label{sec:synthesis-vs-smt}

%To provide a comparison of our learned BGP/OSPF synthesizer with SMT-based methods,
We now compare the synthesis time of the learned neural synthesizer with those of NetComplte, a state-of-art configuration synthesis tool based on SMT-solvers \cite{el2018netcomplete}.

\paragraph{Specifications} As the type of supported requirements in NetComplete does not fully align with our model, we restrict this comparison to specifications which only include forwarding paths (i.e. \texttt{fwd} predicates). Further, NetComplete does not support cross-protocol synthesis as in our case and instead requires users to specify for each requirement the protocol to use for its implementation. To bridge this gap, we split the generated forwarding requirements into BGP and OSPF paths for a corresponding NetComplete specification.
%\todo{note on NetComplete installing policies at all routers, not only the edges of the AS}

\paragraph{Methodology} We compare both OSPF synthesis and BGP/OSPF-synthesis. We configure our trained synthesizer model to do OSPF synthesis by only predicting link weights. For each pair of topology and specification, we report the total time of running our synthesizer 4 times using 4-shot sampling, whereas for consistency we report the best out of the 4 runs. For NetComplete, we run the synthesizer with a timeout of 25 minutes. In case a NetComplete attempt times out, we report 25 minutes as a lower bound for its runtime.

\paragraph{OSPF Synthesis Time Results} We document the results of comparing OSPF synthesis time in \cref{fig:evaluation-compare-ospf}. Our synthesizer model achieves a speedup of 2-10x over NetComplete. With 16 requirements and dataset Large this speedup even increases to $2000\times$. Further, our model achieves very high consistency with the provided specification, often producing fully-consistent configurations.

\paragraph{BGP/OSPF Synthesis Time Results} In \cref{fig:evaluation-compare-bgp} we show the comparison of BGP/OSPF synthesis time. Our synthesizer model outperforms NetComplete by multiple orders of magnitude. We observe a speedup of $20-560\times$ which appears to increase with the size of topology and specification. Further, the average specification consistency of the synthesized configurations is greater than $92\%$ across all datasets, even for large topologies. In many cases, our synthesizer model produces fully-consistent configurations, especially with small topologies and specifications. In comparison, NetComplete times out on more than half of the synthesis tasks which means that we can only observe a lower bound of speedup in these cases. Note that our synthesizer model is running on a CPU due to memory restrictions with large topologies. However, running it on a GPU results in even greater speedups (up to $1000\times$, cf. \cref{app:sec:bgp-gpu-performance}). 

==> diff/git-latexdiff.34107/new/sections/5_related_work.tex <==
\section{Related Work}
\label{sec:related-work}

\paragraph{Traditional Configuration Synthesis} 
%A range of existing work is concerned with network configuration synthesis. 
Next to methods based on compilation such as Propane/PropaneAT \cite{beckett2017network}, there are a number of configuration synthesis methods based on constraint solving: Examples include ConfigAssure \cite{narain2008declarative}, SyNet \cite{el2017network} and NetComplete \cite{el2018netcomplete}. Due to their hand-coded nature, these methods are highly protocol-specific and can be very slow due to the solvers they employ. Although some of them allow for cross-protocol reasoning, this is not implemented as transparently as in our framework and users must specify per requirement which protocol to use for its implementation. In contrast, our approach has lower precision but allows for fully transparent cross-protocol reasoning, meaning forwarding requirements are not protocol-bound and the synthesizer chooses how to implement them. Further, our learned BGP/OSPF synthesis tool exhibits much lower synthesis times as compared to an SMT-based tool like NetComplete.

% \begin{itemize}
%     \item NetComplete, SyNet
%     \item Propane, PropaneAT
%     \item DeepBGP
% \end{itemize}

\paragraph{GNNs and Networking} DeepBGP \cite{bahnasy2020deepbgp} relies on GNNs and reinforcement learning to do configuration synthesis. However, it is limited to BGP configuration synthesis and is slower than SMT-based synthesis according to the author's evaluation. In contrast, our learning-based framework is cross-protocol, does not rely on reinforcement learning and provides better synthesis performance. Apart from configuration synthesis, GNNs have also been applied to other problems in the networking domain. For example, the authors of RouteNet \cite{rusek2020routenet} use GNNs to predict performance metrics of network configurations. Other work that is concerned with learning improved protocols includes Q-Routing \cite{boyan1994packet} or more modern approaches such as the Graph-Query Neural Network architecture \cite{geyer2018learning}.

\paragraph{Neural Algorithmic Reasoning} 
Neural algorithmic reasoning (NAR) as proposed in \cite{velivckovic2021neural}, describes the idea of replacing traditional algorithms with neural networks to learn improved algorithmic procedures. Exemplary work includes graph-related algorithms \cite{velivckovic2019neural} or solvers for combinatorial optimization problems \cite{cappart2021combinatorial,joshi2020learning,selsam2019guiding}. Our synthesis framework is the first applications of NAR to the networking domain and relies on the NAR-native encode-process-decode architecture. According to the hierarchy of NAR approaches in \cite{cappart2021combinatorial}, our method is an algorithm-level approach, as we do not supervise on intermediate steps. Although, such step-level methods promise better generalization, it is not clear what an intermediate result of a general synthesis procedure would be. However, future work on a step-level approach may further improve synthesis quality.

% \begin{itemize}
%     \item RouteNet
%     \item GraphNET
%     \item Learning and generating distributed routing protocols using graph-based deep learning
%     \item Unveiling the potential of Graph Neural Networks for network modeling and optimization in SDN
% \end{itemize}

==> diff/git-latexdiff.34107/new/sections/6_conclusion.tex <==
\setlength{\parskip}{6pt plus4mm minus4mm}
\section{Conclusion}
\label{sec:conclusion}
We presented a learning-based framework for configuration synthesis based on the idea of neural algorithmic reasoning. To assess the effectiveness of the system, we instantiated it for the case of BGP/OSPF synthesis. In contrast to traditional synthesis methods, our system supports transparent cross-protocol reasoning and learns synthesis rules only from data. Using our system, synthesis is sped up by a factor of up to $500\times$ when compared to SMT-based methods. Further, our evaluation demonstrates that the resulting synthesis tool provides excellent synthesis quality, producing configurations with high specification consistency. Overall, our results illustrate that exploring the direction of learning-based network configuration synthesis is a promising direction, enabling new cross-protocol reasoning capabilities and great performance improvements. Promising future work includes construction of hybrid systems, integrating both neural models and SMT-based approaches to obtain the best of both worlds.

==> diff/git-latexdiff.34107/old/acronyms.tex <==
\DeclareAcronym{AS}{
    short = AS,
    long = autonomous system,
    short-plural = es ,
    long-plural = s
}

==> diff/git-latexdiff.34107/old/sections/0_abstract.tex <==
% Context
Computer networks employ a number of different protocols to enable efficient routing. However, due to the complexity of multiple interacting protocols, it can be hard for network operators to implement high-level routing policies and requirements. Network configuration synthesis promises to address this situation by automatically generating configurations that satisfy a provided specification. However, existing synthesis methods are often limited to single-protocol reasoning, depend on protocol-specific and hand-coded synthesis rules, and are difficult to scale due to the SMT-based methods they employ. In this work we present a rather different, learning-based method for addressing the configuration synthesis challenge, one based on the recently proposed paradigm of neural algorithmic reasoning. Our framework is protocol-agnostic, enables cross-protocol reasoning and does not depend on any hardcoded synthesis rules. To evaluate, we instantiate our framework for the case of BGP/OSPF synthesis. Our experiments show we can synthesize configurations with a very high degree of specification consistency while observing speedups of up to $500\times$ compared to a state-of-the-art SMT-based synthesis tool.


==> diff/git-latexdiff.34107/old/sections/1_intro.tex <==
\section{Introduction}
\label{sec:introduction}

The backbone of the internet consists of many connected computer networks operated by different internet service providers (ISPs) and other large organizations. These networks rely on a number of protocols to enable effective and policy-driven routing of traffic. Based on router-level configurations, the protocols perform a distributed computation to construct a network's forwarding state. However, the relatively low-level router configuration makes it hard for network operators to directly enforce network-wide policies and requirements. This often leads to misconfiguration, which can cause global outages such as the recent hours-long blackout of the entire Facebook platform \cite{janardhan2021} and comparable events \cite{mccarthy_2019}.
%
\paragraph{Configuration Synthesis} This situation has triggered a number of research efforts regarding the synthesis of network configurations \cite{el2018netcomplete,beckett2017network,narain2008declarative}. Configuration synthesis is concerned with the task of automatically generating router-level configurations given a set of high-level requirements. However, this synthesis problem can be very hard to solve, since network configurations typically consist of a considerable number of tunable parameters, where the execution of several interacting protocols yields the overall forwarding state. An effective synthesis tool must thus account for this fact and be able to reason across multiple protocols.

\paragraph{SMT-based Synthesis} Some of the most successful efforts in providing cross-protocol synthesis capabilities are based on satisfiability modulo theory (SMT) solvers \cite{el2018netcomplete,el2017network}. While SMT-based synthesis is a promising method, it comes with a number of limitations:
% \item protocol-specific
% fully hand-coded synthesis rules, a lot of implementation effort, cross-protocol support extra complicated
(1) SMT-based synthesizers are hand-crafted and highly protocol-specific. To implement synthesis, we must first express our networking model, protocol semantics including vendor and device specific behavior in terms of first-order logic constraints. This is a time-intensive and complicated process, requiring lots of expert knowledge.
%  model-dependent: synthesis is reasoning on the level of some assumed model which may not reflect the real world: even if a configuration is synthesized based on some spec, it may behave differently and violate spec in practice
Further, (2) logic-based modelling introduces a disconnect between the synthesis tool and real-world behavior \cite{birkner2021metha}. More specifically, synthesized configurations may satisfy a provided specification within a formal framework, but may not behave the same way in the real world.
% can be very slow
And, (3) SMT-based synthesis can be very slow or fail to complete, especially when reasoning about large network topologies. In practice however, network operators reconfigure their networks on a daily basis \cite{vissicchio2012improving}, which means an effective synthesis tool must be fast.

% \item fully learned, no hand-coded synthesis rules (model-free), very flexible to adapt to more/new protocols
% \item protocol-agnostic, cross-protocol
\paragraph{Neural Algorithmic Reasoning for Synthesis} Recent work on neural algorithmic reasoning (NAR) proposes to replace traditional algorithms with neural networks to learn improved algorithmic procedures \cite{velivckovic2021neural}.
It has been shown to be a powerful and fast algorithmic approximation method for a number of graph-related \cite{velivckovic2019neural} and combinatorial optimization problems \cite{cappart2021combinatorial}. Further, due to its learned nature, NAR allows for learning procedures directly from (real-world) data, without the need for manual feature extraction. Overall, this positions NAR as an attractive method to obtain a fast, fully-learned synthesis procedure, which entirely avoids the need for a formal model or any hand-crafted synthesis rules. Based on this promising outlook, this paper explores how to apply the NAR paradigm to the problem of network configuration synthesis.

To that end, we propose a \textbf{new learning-based framework for configuration synthesis} as an alternative to SMT-based approaches. Our framework is protocol-agnostic, enables cross-protocol reasoning and avoids the need to manually provide synthesis rules. Instead of implementing the synthesizer explicitly, we replace it by an iterative graph neural network which is trained on input/output samples of specifications, topologies and configurations.
%While our approach still requires some protocol-specific implementation efforts, it is limited to implementing the simulation of the involved protocols.
Our method is highly flexible due to its generic nature and can be extended to any protocol. Further, the synthesizer model learns a whole distribution of network configurations. As a consequence, we can directly sample multiple alternative configurations, not possible with standard SMT solvers. We apply our framework to a non-trivial synthesis setting where both the Border Gateway Protocol (BGP) and the Open Shortest Path First (OSPF) protocol are used. We demonstrate that our learned synthesis tool is up to~$500\times$ faster than a state-of-the-art SMT-based synthesizer, while producing configurations which enjoy more than 90\% satisfaction of the given specification.

\paragraph{Main Contributions} Our core contributions are:
\vspace{-5pt}
\begin{itemize}
    \setlength{\itemsep}{5pt}
    \setlength{\parskip}{0pt}
    \item A learning-based framework for network configuration synthesis based on neural algorithmic reasoning.
    \item A neural network architecture for learning synthesizer models which relies on a generic graph-based encoding of network topologies and configurations.
    \item An extensive evaluation of our learning-based synthesizer, in terms of both precision and scalability, on the challenging setting where both BGP and OSPF protocols are involved.
\end{itemize}

\section{Overview}
\label{sec:overview}

\begin{figure}
    \begin{center}
        \includegraphics[width=0.45\textwidth]{figures/synthesizer-overview.pdf}
    \end{center}
    \caption{An overview of our learning-based synthesis framework.}
    \label{fig:learning-based-synthesis}
\end{figure}

We first discuss the core concepts behind our learning-based synthesis framework, illustrated in \cref{fig:learning-based-synthesis}.

\paragraph{Dataset} To train a synthesizer model, we first generate a dataset of input/output samples. For this, we rely on a generative pipeline as shown in the top of \cref{fig:learning-based-synthesis}. First, we sample a random network configuration for some topology using a uniform generative process. Then, we simulate the involved protocols to obtain the corresponding routing behavior. Next, we extract a specification by randomly selecting properties that hold for the simulated routing behavior. This leaves us with a pair of (specification, configuration) added to a dataset of training~samples.

\paragraph{Simulation} Depending on the protocols in use, one implements simulation code to compute the routing behavior induced by a sampled configuration. Although this step is protocol-specific, the overall implementation effort is much lower compared to SMT-based synthesis. Protocols are typically well-defined algorithms which can be simulated, whereas the alternative of implementing a synthesizer often requires expert knowledge about SMT solvers. In practice, our framework may also be adapted to use a real-world network router to compute the behavior of a configuration, thereby capturing the real-world behavior directly.

\paragraph{Neural Synthesizer Model} Given a dataset of pairs each consisting of a configuration and a specification, we now train a graph neural network on this dataset to perform synthesis: given a specification, it tries to predict the configuration. Following the NAR paradigm, we first encode the synthesizer input (specification) in latent space. Then, we apply an iterative processor network which relies on the graph attention mechanism to propagate information \cite{velivckovic2017graph}. Last, we apply a decoder network to extract the synthesized configuration. To remain protocol-agnostic, our model is generic with respect to the input format, using an intermediate representation based on Datalog-like facts.

%More specifically, we employ a slightly modified variant which operates on a graph-based encoding of a specification, topology and configuration parameters.



 \begin{figure*}
     \centering
     \includegraphics[width=0.85\textwidth]{figures/system-overview.pdf}
     \caption{An overview of our synthesis system: (1) First, we use a generic embedding scheme to transform a network topology, protocol configuration sketches and the specification given as Datalog-like facts to a latent input representation. Next, we apply a learned (2) Processor GNN and obtain a latent synthesis output. Last, we apply a (3) Decoder Network to obtain a distribution over possible values per unknown parameter in our configuration.}
     \label{fig:overview-model}
\end{figure*}

\paragraph{Relaxed Specification Consistency} Parts of the configuration synthesis problems are known to be NP-hard \cite{fortz2000internet}. In contrast, our learning-based framework depends on a fixed-size neural network architecture running in polynomial time. Hence, we expect neural synthesis to be less precise than SMT methods and propose the notion of \emph{relaxed~specification~consistency}. That is, to assess the performance of a neural synthesizer, we not only consider if a configuration satisfies a specification, but also the degree up to which it satisfies a specification (e.g., via the relative number of satisfied requirements). This ``soft'' understanding of a specification allows us to evaluate neural synthesis systems which may not always produce fully specification-consistent configurations. Nonetheless, we argue that configurations with less than $100\%$ consistency are still very useful in practice as they provide a good starting point for further manual adjustment by network operators. Note that a similar adjustment process may also be required with SMT-based synthesizers, due to differences between the formal protocol model and the one running on a given real-world router where the configuration is to be deployed.

Next, we discuss the architecture of our neural synthesis framework. In follow-up sections, we instantiate this framework for the case of BGP/OSPF configuration synthesis, and evaluate the resulting instantiation by comparing it to a state-of-the-art SMT-based synthesizer.

% \begin{itemize}
%     \item effort: need to implement simulation code to generate dataset to learn from (typically well-defined in protocol specs, much easier than implementing synthesis directly)
%     \item can be sampled (multiple alternative solutions, not easily possible with SMT-based methods)
%     \item much faster than SMT-based synthesis
% \end{itemize}

% Requirements:
% \begin{itemize}
%     \item protocol-agnostic
%     \item fully learned, no hand-coded synthesis rules
%     \item define: strict specification vs. relaxed specification
% \end{itemize} 

==> diff/git-latexdiff.34107/old/sections/2_model.tex <==
\section{Neural Synthesis Framework}
\label{sec:model}


We now present the architecture of our graph-based neural synthesizer model, illustrated in \cref{fig:overview-model}. First, in \cref{sec:graph-embedding} we introduce our generic graph-based encoding, which allows us to embed network topologies, protocol configuration and the specification into a latent space. Then, in \cref{sec:graph-transformer} we present the architecture of the processor network which we train to perform the synthesis task. Finally, in \cref{sec:decoding-sampling} we discuss how to sample network configurations from the resulting latent synthesis output.

\begin{figure}
    \begin{minipage}[t]{0.21\textwidth}
    \begin{lstlisting}[basicstyle=\ttfamily\small, escapeinside={(*}{*)}]
router(A)
router(B)
(...)

connected(A,B,2)
connected(A,C,?)(*\blackcircled{1}*)
(...)
    \end{lstlisting}
\end{minipage}
\begin{minipage}[t]{0.21\textwidth}
    \begin{lstlisting}[basicstyle=\ttfamily\small, escapeinside={(*}{*)}]
network(N1)
bgp_route(E,N1,2,3,1,0,1)

fwd(A,B,N1)
not fwd(B,A,N1)
(...)
    \end{lstlisting}
\end{minipage}
    \caption{A snippet of a fact base sketch encoding a network's topology, parameters such as link weights (\texttt{connected} facts) and a specification (\texttt{fwd} facts).}
    \label{fig:datalog-encoding}
\end{figure}

\begin{figure}[t]
    \centering
    \includegraphics[width=0.25\textwidth]{figures/synth-architecture.png}
    \caption{The neural synthesizer model architecture.}
    \label{fig:architecture}
\end{figure}

\subsection{Fact Base Embedding}
\label{sec:graph-embedding}
To remain network protocol-agnostic in our model architecture, we implement a generic graph-based encoding of Datalog-like facts, similar to knowledge graphs \cite{rosso2020beyond}. This means that we first encode topologies, configurations and specifications as a set of Datalog-like facts and then employ a generic embedding.
%We chose Datalog facts as the input format of our synthesis approach for its flexibility, wide-spread use in Program Analysis and use in previous work on configuration synthesis \cite{el2017network}.

\paragraph{Fact Base} A set of Datalog-like facts, as depicted in \cref{fig:datalog-encoding}, serves as the input \emph{fact base} $\mathcal{F}$ to our synthesizer model. $\mathcal{F}$ is a set of facts $f(a_0, \dots, a_n)$ where arguments may be constants (e.g. A or B) or integer literals. Further, each fact in a fact base has a corresponding truth value denoted as $[f(a)]_{\mathcal{B}}$. For instance, from the fact base in \cref{fig:datalog-encoding} we can derive $[fwd(A,B,N1)]_{\mathcal{B}} = \text{\texttt{true}}$ and $[fwd(B,A,N1)]_{\mathcal{B}} = \text{\texttt{false}}$.

\paragraph{Consistency} We represent a network's topology, the protocol configuration and parameters as well as the specification, all in a single fact base. Given the semantics of the protocols in use, we can then check whether the specification encoded in a fact base is satisfied by the provided configuration. To quantify, we define the notion of relaxed specification consistency, as discussed earlier, with respect to a fact base: Given a fact base $\mathcal{F}$, a subset of specification facts $S \subset \mathcal{F}$ and protocol semantics $\mathcal{P}$, the \emph{consistency} of a fact base is defined as the relative number of satisfied facts in $S$ with respect to the routing behavior obtained via $\mathcal{P}$. The contents of $S$ depend on the concrete instantiation of the synthesizer model. For an example of possible specification facts, see our instantiation of the synthesizer model for BGP/OSPF in \cref{sec:training}.

\begin{figure*}
    \def\arraystretch{1.5}
    \begin{tabular}{lr}
        %$T_f: T_1 \times \dots \times T_n$ & \textit{(fact type declaration)}\\
        $emb(f) := \mathbf{V_f}$ & \textit{(learned fact type embedding)}\\
        $emb(b) := \mathbf{W_{\text{bool}}}\;onehot(b)$ & \textit{(learned boolean embedding)}\\
        $emb(f,i,v) := \mathbf{W_{f_i}}\;onehot(v)$ & \textit{(learned integer embedding)}\\
        $emb(f,i,?) := \mathbf{V_{hole}}$ & \textit{(learned hole embedding)}\vspace{10pt}\\
        $\mathlarger{
        h_c := \sum_{f(c) \in \mathcal{F}}
        emb(f)
        }$ & \textit{(constant embedding)}\vspace{10pt}\\
        $h_{f(a_0, \dots, a_n)} := emb(f) + emb([f(a_0, \dots, a_n)]_{\mathcal{B}}) + \mathlarger{
        \sum_{(i,v) \in \mathcal{I}(f(a_0, \dots, a_n))}
        emb(f, i, v)
        }$\hspace{-1.2cm} & \textit{(fact embedding)}\\
        $\mathcal{I}(f(a_0, \dots, a_n)) := \{(i,v) \; | \; f(a_0, \dots, a_{i-1}, v, \dots, a_n) \in \mathcal{F} \wedge v:Int \wedge i \in \mathbb{N}$ \}& \textit{(integer arguments)}\vspace{10pt}\\
        $N_i(h_c) := \{h_f \; | \; \exists i \in \mathbb{N} . f(a_0, \dots, a_{i-1}, c, a_{i+1}, \dots, a_n) \in \mathcal{F}\}$& \textit{(i-th neighborhood of constant node)} \\
        $N_i(h_f) := \{h_c \; | \; \exists i \in \mathbb{N} . f(a_0, \dots, a_{i-1}, c, a_{i+1}, \dots, a_n) \in \mathcal{F}\}$& \textit{(i-th neighborhood of fact node)} \\
    \end{tabular}
    \caption{Translating a fact base $\mathcal{F}$ to node features. $f$ denotes a predicate, $v$ integer values, $b$ boolean values as 0 or 1, $i$ argument indices and $[f(a)]_{\mathcal{B}}$ the truth value of a fact. }
    \label{fig:graph-embedding}
\end{figure*}

%discuss embedding as shown in \cref{fig:datalog-encoding}. Note how this makes fact bases a suitable input to standard GNN architectures.

\paragraph{Fact Base Sketching} In a synthesis setting, we are confronted with incomplete fact bases, i.e. the specification and topology is given but the network configuration is to be synthesized. For these cases, we also consider fact bases with unknown parameters inspired by the idea of program sketching in program synthesis \cite{solar2008program}. More specifically, users may replace an unknown integer argument of a fact by a \texttt{?} symbol, indicating a value to be synthesized. Using this mechanic, we can represent the synthesis input as an incomplete fact base which encodes to-be-synthesized values as unknown parameters. As an example, consider \cref{fig:datalog-encoding} \blackcircled{1}, where the link weight between router nodes \texttt{A} and \texttt{C} is represented as an unknown parameter.

\paragraph{Embedding} We employ a structurally-defined embedding scheme to transform a fact base into a graph with node features as required for processing with graph neural networks. Given a fact base $\mathcal{F}$, we apply the rules in \cref{fig:graph-embedding} to obtain node features and adjacency information. Both a fact $f$ and a constant $c$ are represented as distinct nodes with features $h_c$ and $h_f$, respectively. The relationships between facts and constants is encoded as node adjacency as defined by the neighborhood functions $N_i$.

We use multiple neighborhood functions, i.e. multiple types of edges, to encode the argument position of a constant occurring in a fact. Hence, the number of neighborhood functions corresponds to the maximum number of arguments in a single fact, e.g. 3 in \cref{fig:datalog-encoding}. Integer arguments and unary facts are directly accounted for in the respective node or fact embedding. To handle unknown parameters, we replace the corresponding $emb(...)$ term with the learned $\mathbf{V_{hole}}$ embedding.

Considering the embedding function $emb$, the learned parameters of our embedding are $\mathbf{V_f} \in \mathbb{R}^D$ per fact type in~$\mathcal{F}$, $\mathbf{W_{\text{bool}}} \in \mathbb{R}^{D \times 2}$ for boolean values, $\mathbf{W_{f_i}} \in \mathbb{R}^{D \times N}$ per integer argument of fact type $f$ and $\mathbf{V_{hole}} \in \mathbb{R}^D$ to represent unknown parameters. Hyperparameter $D$ represents the dimension of the latent space the synthesizer model operates in and $N$ specifies the number of supported integer values. An example of applying this embedding scheme to a simple fact base is given in \cref{fig:graph-encoding-example}.

\begin{figure}
    \begin{minipage}[t]{0.2\textwidth}
        \centering
        \footnotesize
        \textbf{Fact Base}
        \begin{lstlisting}[basicstyle=\ttfamily\small]
router(A)
router(B)

conn(A, B, 12)
        \end{lstlisting}
    \end{minipage}
    \begin{minipage}[t]{0.15\textwidth}
        \centering
        \textbf{Graph}\\
        \vspace{5pt}
        \includegraphics[width=0.7\textwidth]{figures/graph-encoding.pdf}
    \end{minipage}\\
    \centering\\
    \vspace{10pt}
    \textbf{Node Features}\\
    \vspace{10pt}
    \begin{minipage}[t]{0.5\textwidth}
        $\begin{array}{rcl}
        h_A &:=& emb(router) = \mathbf{V_{\text{router}}}\\
        h_B &:=& emb(router) = \mathbf{V_{\text{router}}}\\
        h_{\text{conn(A,B,12)}} &:=& emb(conn) + emb(conn, 2, 12)\\
        &:=& \mathbf{V_{\text{conn}}} + \mathbf{W_{conn_2}} onehot(12)
    \end{array}$
    \end{minipage}
    \caption{An example of embedding a simple fact base using the embedding scheme of \cref{fig:graph-embedding}. The shown graph illustrates the neighborhoods $N_0$ and $N_1$ induced by the \texttt{conn} fact.}
    \label{fig:graph-encoding-example}
\end{figure}

\begin{figure}
    $$
    \begin{array}{rcl}
    z_j &:=& h_j + Drop(\mathlarger{\sum_{N_i}} h'_{GAT_i})\\
    h'_j &:=& FFN(Norm(z_j))\vspace{11pt}\\
    FFN(x_j) &:=& Norm(Lin2(Drop(Lin1(x_j)))))
    \end{array}
    $$
    \caption{
        The recurrence relation of a node $j$'s representation $h_j$. $h'_{GAT_i}$ represents the output of a graph attention layer operating with neighborhood $N_i$ according to \cite{velivckovic2017graph}, $h_j$ the representation of node $j$ at the previous step. $Norm$ refers to batch normalization \cite{ioffe2015batch}, $Drop$ to dropout regularization \cite{hinton2012improving} and $Lin1$ and $Lin2$ to linear layers with an inner dimension of $4N$.
    }
    \label{fig:recurrence}
\end{figure}

\subsection{Synthesizer Model}
\label{sec:graph-transformer}

For an illustration of the synthesizer model's architecture, please see Figure~\ref{fig:architecture}. Given a fact base $\mathcal{F}$ we first apply our embedding scheme as described in \cref{sec:graph-embedding}. We then employ a 2-layer GNN-based encoder network to produce the latent representation of a synthesis input.
Given this representation, a processors network is trained to perform the actual synthesis task in high-dimensional space. Last, we apply a set of decoder networks, to obtain the synthesized values of unknown parameter, given the latent synthesis~output.

%In this context, the synthesis problem for network configurations corresponds to completing partially provided fact bases.

% \paragraph{High-Level Architecture}

% We employ the high-level architecture to obtain the latent synthesis output $y_\mathcal{F}$:
% $$
% \begin{array}{rcl}
%     \mathbf{x_{\mathcal{F}}} &:=& Encoder(Embedding(\mathcal{F}))\\
%     \mathbf{y_{\mathcal{F}}} &:=& Processor(\mathbf{x_{\mathcal{F}}} + \mathbf{z})\\
%     z_i &\sim& \mathcal{N}(0,1)
% \end{array}
% $$
% \todo{z is only added for $i<N/2$}

% $Embedding$ corresponds to the graph-based embedding as discussed in \cref{sec:graph-embedding} and $Encoder$ is a 2-layer graph attention module. $Processor$

\paragraph{Encoding} The encoder GNN operates on the embedded representation of a fact base. It produces the high-dimensional representation of a synthesis input as required for the processor network. We additionally apply noise to the first half of the units of the latent representation via $\mathbf{z}$, as a source of non-determinism. According to our experiments this improves model performance and we hypothesize this is due to the synthesis problem having more than one solution in most cases.

\paragraph{Iterative Processor} The processor network is modelled as an iterative process. For this, we apply the same 6-layer graph attention module for a total of 4 iterations.
In the framework of neural algorithmic reasoning, this iterative computational structure encodes an inductive bias towards an iterative solution to the synthesis problem. Because of this bias, our processor network essentially learns an algorithmic procedure which iteratively synthesizes the values of unknown parameters in a fact base.

\paragraph{Graph Attention Layer} In the GNNs we employ, we rely on a composed variant of the graph attention layer as introduced by \cite{velivckovic2017graph}. We employ multiple graph attention layers in lockstep, one per neighborhood $N_i$ defined by our graph embedding (cf. \cref{sec:graph-embedding}), and combine the intermediate results after each step. Specifically, the recurrence relation of a node $j$'s representation $h_j$ is defined as shown in \cref{fig:recurrence}. These mechanics of combining the results of the different graph attention layers $h'_{GAT_i}$, directly corresponds to how multiple attention heads are combined in the original Transformer architecture \cite{vaswani2017attention}.

\paragraph{Argument Decoder Networks} To synthesize the values of unknown parameters, the model maintains a set of decoder networks. That is, it provides one decoder network per integer argument per fact type in a fact base. When decoding, the network is applied to the latent synthesis output of the corresponding fact node. For example, a synthesizer model which operates on the fact base in \cref{fig:graph-encoding-example}, would provide a decoder network $D_{\text{conn}_2}: \mathbb{R}^D \rightarrow \mathbb{R^N}$ to decode values for the third argument of a \texttt{conn} fact. In our experiments, decoder networks are implemented as simple multi-layer perceptron models.

%The synthesizer model learns a conditional distribution of fact bases which are consistent with respect to the protocols' semantics.

%\todo{introduce synthesis as a completion problem of an encoded fact base (a la BERT). Introduce masking, introduce decoding of integer and truth values. Synthesis is learning a conditional distribution of consistent fact bases.}

%Using this method, we obtain the node features $h_c$ per constant, $h_f$ per fact and adjacency information in terms of node neighborhood functions $N_i(h_c)$ and $N_i(h_f)$. Overall, this encoding makes a fact base suitable for processing using standard graph neural networks.

%- Brief description of the Graph Transformer Model
\subsection{Multi-Shot Sampling}
\label{sec:decoding-sampling}

%Multi-Stage Parameter Sampling (sampling methods: topk, high-temp, low-temp)
To sample concrete values from the output distributions over unknown parameters, we apply a multi-shot sampling strategy. That is, we sample values only for a subset of unknown parameters, insert them in our input fact base and run the synthesis model again. We repeat this process until no more unknown parameters remain. This multi-shot sampling strategy allows the model to incorporate the concrete values of previously synthesized parameters in its computation. In our evaluation in \cref{sec:evaluation}, we include a comparison of how this compares to sampling all unknown parameters at once.

%In a fact base with multiple holes, we apply the corresponding decoder networks to obtain a value distribution for each integer hole. However, instead of sampling all integer holes in one


==> diff/git-latexdiff.34107/old/sections/3_bgp_ospf.tex <==
\section{BGP/OSPF Synthesis}
\label{sec:bgp-ospf}

\newcommand{\as}{\ac{AS}~}
\newcommand{\ases}{\acp{AS}~}

\newcommand{\squareann}{{\tiny$\blacksquare\;$}}
\newcommand{\triangleann}{{\small$\blacktriangle\;$}}

\begin{figure*}
    \centering
    \includegraphics[width=0.95\textwidth]{figures/networks-all.pdf}
    \caption{(a) An illustration of a small AS network, including internal peers (blue), external peers (purple), BGP sessions as well as physical links. (b) The propagation of two BGP announcement across the network. (c) The resulting forwarding plane after applying BGP and OSPF.}
    \label{fig:network-fwd-tree}
\end{figure*}

We now discuss an instantiation of our learning-based framework for the case of BGP and OSPF protocols. In \cref{sec:synthesis-setting} we introduce a basic networking model, BGP and OSPF protocols and the synthesis setting. Given this model, \cref{sec:training} describes how to generate a corresponding dataset of input/output samples and train a synthesizer model.
%This shall serve as a prerequisite to the instantiation of our learning-based synthesis framework for the BGP and OSPF protocol in \cref{sec:training}.

\subsection{Synthesis Setting}
\label{sec:synthesis-setting}

\paragraph{Graphical Model} We assume an abstract network model which can be represented as an undirected graph as shown in \cref{fig:network-fwd-tree} (a). We always consider a set of internal routers (A, B, C, D in \cref{fig:network-fwd-tree}) as well as a set of adjacent external routers (E, F  in \cref{fig:network-fwd-tree}). The group of internal routers forms the \emph{\as} under consideration whereas external routers belong to other adjacent \ases. In practice, an \as represents an administrative domain controlled by a single operator.

\paragraph{Forwarding Plane} We focus on the \emph{forwarding plane} of a network. This means we are interested in how a router forwards packets given incoming traffic of different traffic classes. For this, each router maintains a routing table which determines which of its outgoing edges is used to forward packets of a certain traffic class. As an example, consider \cref{fig:network-fwd-tree} (c) which illustrates the forwarding plane of some traffic class reachable via external peer $E$ or $F$ in our example network. Each router of the network forwards traffic along some of its outgoing links. In practice, a number of protocols are used to populate a router's routing tables. For the instantiation of our synthesis framework however, we focus on OSPF and BGP.

\paragraph{OSPF} The OSPF protocol \cite{moy1994ospf} is a link-state protocol, typically used as an interior gateway protocol~(IGP), i.e., to route traffic within an \ac{AS}. Given link weights per physical link in the network, OSPF simply routes traffic along the shortest path towards the destination.

\paragraph{BGP} The BGP protocol \cite{rekhter1994border} on the other hand is a path-vector protocol used to exchange reachability information mostly on the level of \acp{AS}.
%These are groups of routers typically operated by a single party (e.g. an ISP).
When using BGP, a routing destination announces its existence to other \ases and routers, by sending out a BGP announcement. Receivers of such announcements may then choose to pass them on to other \acp{AS}, redistribute them internally and/or modify them. Instead of communicating along physical links directly, the BGP protocol requires manually configured BGP sessions among routers of the \as and external peers, as indicated by the BGP session edges in \cref{fig:network-fwd-tree}(a).
%\todo{more discussion of eBGP vs iBGP and support for route reflection (more of an implementation detail, maybe only mention in dataset generation where simulation code is discussed)}.

%\paragraph{BGP Decision Procedure}~
%\todo{discuss decision procedure}
In case a router receives more than one announcement for a destination, a designated BGP decision process is applied to determine a single best route. \cref{fig:bgp-decision} shows the ordered list of comparison criteria of this decision process. The different criteria depend different properties of a route announcements, including the IGP cost towards the routing destination. As a consequence, when used together, OSPF as IGP protocol and BGP will interact. %Note also that BGP is an iterative process which needs multiple rounds of propagation to converge.

\paragraph{Example}
%\todo{run through simple BGP+OSPF example of computing the forwarding plane}
To better understand BGP/OSPF routing, consider the simple example given in \cref{fig:network-fwd-tree} (b). Here, our example \as imports BGP announcements \squareann and \triangleann from E and F respectively. Both represent a route to the same destination. As shown, both announcements have a so-called local preference of 2. For simplicity, we ignore other properties such as the AS path length, Origin and MED in this example. The announcements are propagated among BGP neighbors and the best route is selected according to the decision procedure in \cref{fig:bgp-decision}. See \cref{fig:network-fwd-tree} (b) for an illustration of the intermediate states of this propagation process. As both announcements have a local preference of 2, rule 1 of the decision process is not used. Instead, in round 2, node B selects \squareann over \triangleann due to a lower IGP cost of 2 via egress node A as compared to 3 via egress node D (rule 6). Node D selects \triangleann over \squareann, since it learns this route directly from an external peer (rule 5). After Round 3, the BGP propagation process converges to a stable state and we can derive the forwarding plane as shown in \cref{fig:network-fwd-tree} (c).


%, as well as external peers E and F which belong to other \acp{AS}. External peers are routers which are connected via eBGP sessions to routers of the \ac{AS} under consideration. They announce BGP routes to their neighbors, which are propagated within the network

\paragraph{Problem Statement: Configuration Synthesis} We phrase the BGP/OSPF configuration synthesis problem on the level of the forwarding plane. This means that users provide a specification which constraints the set of allowed forwarding planes. This includes predicates which enforce forwarding paths, block forwarding paths or assert higher-level properties like traffic isolation and reachability. Given such a specification, we consider network configuration synthesis as the task of configuring OSPF and BGP in a way that produces a forwarding plane which satisfies the provided specification.

\paragraph{Search Space} To limit the space of candidate configurations, we define the set of synthesized parameters: For OSPF we synthesize link weights as explored in a wide range of existing work (e.g. \cite{el2018netcomplete,fortz2000internet}. BGP parameters on the other hand are not defined as clearly: Depending on the requirements of a network operator, one may employ custom BGP import and export policies at every router of a network to implement complex behavior. However, in this work we focus on a simplified setting, where we assume BGP route announcements to only be modified when imported into the \as from an external peer. Previous work has already pointed out that this is a reasonable assumption which holds for the majority of real-world networks \cite{caesar2005bgp,cittadini2010doing, steffen2020probabilistic}.

\begin{figure}
    \small{
    \begin{enumerate}
        \setlength{\itemsep}{0pt}
        \setlength{\parskip}{0pt}
        \item Highest Local preference
        \item Lowest AS path length
        \item Prefer Origin (IGP $>$ EBGP $>$ INCOMPLETE)
        \item Lowest Multi-exit discriminator (MED)
        \item External over internal announcements
        \item Lowest IGP cost to egress
        \item Lowest BGP peer id (tie breaker)
    \end{enumerate}}
    \vspace{-15pt}
    \caption{The BGP decision process \cite{rekhter1994border}. The shown rules are applied in order until a single best BGP announcements remains.}
    \label{fig:bgp-decision}
\end{figure}

\subsection{Dataset Generation and Training}
\label{sec:training}
To train a synthesizer model, we need a large number of fact bases encoding a variety of network topologies, configurations and forwarding specifications. Further, we must provide the model with target values for unknown parameters as a supervision signal. This section discusses how we construct such a dataset for BGP/OSPF synthesis.
%Further, we provide an example of what a corresponding fact base looks like, including a description of the supported specification language.

\paragraph{Dataset Generation} To obtain network configurations and corresponding forwarding specifications we employ a generative process: We first randomly configure BGP and OSPF parameters for some topology. Then we simulate the OSPF and BGP protocol and compute the resulting forwarding plane. Based on this, we extract a forwarding specification which fixes a random subset of forwarding paths, reachability and isolation properties that are satisfied by the forwarding plane.

\paragraph{Topologies} For training, our dataset is based on random topologies with $16$-$24$ routers. We generate the physical layout of these graphs by triangulation of uniformly sampled points in two-dimensional space.

\paragraph{Simulation} To compute the forwarding plane given an OSPF and BGP configuration, we simulate the protocols. For OSPF, we implement shortest path computation to obtain the forwarding plane. For BGP, we implement the full BGP decision process as shown in \cref{fig:bgp-decision}, except for the MED attribute. In addition to the basic networking model discussed in \cref{sec:synthesis-setting}, we implement support for eBGP and iBGP, fully-meshed BGP session layouts as well as layouts relying on route reflection. For more details of these BGP concepts see \cite{bates2000rr}.

%Note that the synthesizer model will reason on the level of the provided training samples. That is, to improve the overall synthesis quality in a real-world setting, it is helpful to implement simulation code which behaves very similar to real-world networks. Another promising approach would be to extract training samples from real-world networks, thereby circumventing the need for simulation, however, we leave this as future work.

%While this can be a considerable effort, it is typically an easier task than to implement the synthesizer directly. The concrete semantics of protocols and their simulation is a well-defined procedure, whereas implementing efficient synthesis tools is still an open problem.

\paragraph{Fact Base Encoding} We encode synthesis input using a small set of facts. For an example of a corresponding fact base see \cref{fig:bgp-ospf-fact-base}. We use the \texttt{router}, \texttt{external} and \texttt{network} facts to mark routers, external peers and routing destinations respectively. Physical links between routers are encoded as \texttt{connected(R1,R2,W)} facts where \texttt{W} denotes the OSPF link weight. Further, we rely on \texttt{ibgp}, \texttt{ebgp}, \texttt{route\_reflector} and \texttt{bgp\_route} facts to represent different types of BGP sessions and imported routes. Using the notion of unknown parameters as discussed in \cref{sec:graph-embedding}, we encode configuration parameters, e.g., properties of imported routes or OSPF link weights.

\paragraph{Specification Language} We support a small specification language with three types of forwarding predicates:

\begin{itemize}
    \setlength{\itemsep}{0pt}
    \setlength{\parskip}{2pt}
    \item \texttt{fwd(R1, Net, R2)} specifies that router \texttt{R1} forwards traffic destined for \texttt{Net} to its neighbor \texttt{R2}.
    \item \texttt{reachable(R1, Net, R2)} specifies that traffic destined for \texttt{Net} that passes through \texttt{R1} also passes through \texttt{R2} before reaching its destination.
    \item \texttt{trafficIsolation(R1, R2, N1, N2)} specifies that it must not hold that $[fwd(R1,R2,N1)]_{\mathcal{B}} \wedge [fwd(R1,R2,N2)]_{\mathcal{B}}$.
\end{itemize}

In the negative case of each predicate, the opposite must hold true for the fact to be satisfied. This specification language can easily be extended by including new specification predicates in the dataset generation process. One must simply provide a method of extracting positive and negative cases of a specification fact from a given forwarding plane. Once included in the training dataset of a synthesizer model, the resulting synthesis system will be able to consider specifications relying on the new type of predicates.

% \todo{info on loss function, optimizer, etc.}
\paragraph{Training} We generate a dataset of $10,240$ input/output samples and instantiate our synthesizer model with a hidden dimension $D$ of $64$. For optimization, we use the Adam optimizer \cite{kingma2014adam} with a learning rate of $10^{-4}$, applying negative log-likelihood loss to the decoder networks' outputs. We stop training after the specification consistency on a validation dataset no longer increases at around $\sim2800$ epochs.

\begin{figure}
\begin{minipage}[t]{0.22\textwidth}
\begin{lstlisting}[basicstyle=\ttfamily\tiny]
# topology and configuration
router(c5)
router(c3)
router(c1)
router(c0)
network(c6)
network(c7)

external(c8)
external(c9)
external(c10)
external(c11)
external(c12)
external(c13)

route_reflector(c2)
route_reflector(c4)

connected(c2,c4,?)
connected(c2,c5,?)
connected(c2,c3,?)
connected(c4,c5,?)
connected(c4,c3,?)
connected(c4,c0,?)
connected(c5,c1,?)
connected(c5,c0,?)
connected(c3,c0,?)
connected(c3,c1,?)
connected(c1,c0,?)

ibgp(c2,c4)
ibgp(c2,c5)
ibgp(c2,c0)
ibgp(c2,c1)
ibgp(c4,c3)
ibgp(c4,c4)
\end{lstlisting}
\end{minipage}
\begin{minipage}[t]{0.2\textwidth}
\begin{lstlisting}[basicstyle=\ttfamily\tiny]
ebgp(c2,c12)
ebgp(c5,c9)
ebgp(c5,c10)
ebgp(c5,c13)
ebgp(c0,c8)
ebgp(c0,c11)

bgp_route(c8,c6,?,?,1,?,1,8)
bgp_route(c9,c6,?,?,0,?,1,9)
bgp_route(c10,c6,?,?,0,?,1,10)
bgp_route(c11,c7,?,?,0,?,1,11)
bgp_route(c12,c7,?,?,0,?,1,12)
bgp_route(c13,c7,?,?,2,?,1,13)

# forwarding specification
fwd(c0,c6,c3)
fwd(c3,c6,c2)
fwd(c2,c6,c4)
not fwd(c3,c6,c0)
not fwd(c0,c6,c11)
not fwd(c11,c6,c0)

not trafficIsolation(c1,c0,c7,c6)
not trafficIsolation(c1,c0,c7,c6)
trafficIsolation(c0,c3,c6,c7)
trafficIsolation(c0,c3,c6,c7)

reachable(c5,c6,c10)
reachable(c1,c6,c4)
not reachable(c0,c6,c5)
reachable(c5,c6,c10)
\end{lstlisting}
\end{minipage}
\caption{An example of a fact base encoding a topology, a sketch of a BGP and OSPF configuration and a forwarding specification.}
\label{fig:bgp-ospf-fact-base}
\end{figure} 

==> diff/git-latexdiff.34107/old/sections/4_evaluation.tex <==
\section{Evaluation}
\label{sec:evaluation}

We trained a synthesizer model to perform configuration synthesis for BGP and OSPF. We now assess the performance of the resulting neural synthesizer with respect to two core metrics: (1) the quality of synthesized configurations in terms of their consistency with the provided forwarding specifications (\cref{sec:synthesis-quality}), and (ii) the time a learned synthesizer takes when compared to the state-of-the-art SMT-based synthesizer NetComplete \cite{el2018netcomplete} (\cref{sec:synthesis-vs-smt}).

\paragraph{Dataset} We compare across three datasets: Small, Medium and Large. Each dataset represents 8 real-world topologies, sampled from the Topology Zoo \cite{knight2011internet}, where the number of nodes lies between 0-34, 34-68 and 68-170 respectively. To obtain forwarding specifications for the sampled topologies, we use our generative pipeline as discussed in \cref{sec:training}. In each topology, we do synthesis for 4 different traffic classes (routing destinations) at a time.

\paragraph{Experimental Setup} We run all our experiments on an Ubuntu Linux machine with an Intel(R)~Core(TM)~i9-9900X~@~3.50GHz processor, 64GB of system memory and an NVIDIA GeForce RTX 3080 GPU with 10GB of video~memory.

\subsection{Synthesis Quality}
\label{sec:synthesis-quality}
To assess our learned synthesizer, we examine its behavior with increasingly large topologies and specifications.

\paragraph{Specifications} Using the same generative model as described in \cref{sec:training}, we generate forwarding specifications for the topologies in our three datasets with each specification constructed from $3 \times n$ requirements, one per supported predicate type:  \texttt{fwd} requirements correspond to specifying or blocking a forwarding path using multiple \texttt{fwd} predicates whereas \texttt{reachable} and \texttt{trafficIsolation} requirements each translate to a single specification fact. We compare across increasingly large specifications of $3\times 2$, $3\times 8$ and $3 \times 16$ requirements, respectively.

\paragraph{Methodology} For each pair of topology and specification, we run our synthesizer 5 times and report the network configurations with the highest overall consistency value. For sampling, we rely on our multi-shot sampling strategy where we randomly group the unknown parameters of a configuration into 4 groups (4-shot sampling).

\paragraph{Results} We summarize our results in \cref{fig:eval-consistency}. On average, our synthesis model produces network configurations that are $>91\%$ consistent with the provided forwarding specifications across all datasets and sizes of specifications. When only few requirements are given, the synthesizer model even succeeds in producing fully-consistent configurations. We observe a slightly decreasing consistency with increasingly large topologies.

%\texttt{fwd} facts are satisfied more easily, whereas \texttt{reachable} and \texttt{trafficIsolation} facts are violated more often.

\paragraph{Multi-Shot Sampling} In \cref{fig:eval-consistency-baseline}, we report the average specification consistency using our multi-shot sampling strategy as compared to sampling all unknown parameters at once. As a baseline we have also sampled random configurations from a uniform distribution (per parameter) and compute the corresponding specification consistency. Over the baseline, our synthesizer model shows clear improvement and multi-shot sampling further increases consistency.

\begin{figure*}
    \begin{center}
        \textbf{Specification Consistency}\\
        \footnotesize
        \begin{tabular}{rrcccccccccc}
        \toprule
        \multicolumn{2}{c}{Dataset} & \tiny\texttt{fwd} & \tiny\texttt{reachable}  & \tiny\texttt{trafficIsolation} & Overall & $\emptyset$     No. Full Matches & $\emptyset$ No. $>90\%$ Matches\\
        \midrule
        $3\times 2$ requirements & Small & 0.95 & 0.94 & 1.00 & \textbf{0.95} & 0.62 & 0.62\\
& Medium & 0.96 & 1.00 & 0.94 & \textbf{0.96} & 0.88 & 0.88\\
& Large & 0.94 & 0.94 & 1.00 & \textbf{0.93} & 0.62 & 0.62\\
\midrule
$3\times 8$ requirements & Small & 0.97 & 0.98 & 0.97 & \textbf{0.98} & 0.50 & 1.00\\
& Medium & 0.99 & 0.95 & 1.00 & \textbf{0.98} & 0.50 & 1.00\\
& Large & 0.96 & 0.95 & 0.91 & \textbf{0.94} & 0.38 & 0.88\\
\midrule
$3\times 16$ requirements & Small & 0.97 & 0.89 & 0.95 & \textbf{0.94} & 0.38 & 0.75\\
& Medium & 0.98 & 0.97 & 0.97 & \textbf{0.98} & 0.38 & 1.00\\
& Large & 0.92 & 0.88 & 0.95 & \textbf{0.91} & 0.12 & 0.50\\
    \end{tabular}\end{center}
    \caption{Average specification consistency of the network configurations synthesized by our trained synthesizer model. Per sample we run the synthesizer with a specification of $3\times N$ requirements, where the specifications always include $N$ requirements per supported predicate type (\texttt{fwd}, \texttt{reachable}, \texttt{trafficIsolation}).}
    \label{fig:eval-consistency}
\end{figure*}

\begin{figure}
    \begin{center}
        \footnotesize
        \begin{tabular}{rrcccccccccc}
        &  & \multicolumn{2}{c}{Neural}\\
        & Random & 1-Shot & 4-shot\\
        \toprule
        Small & 0.83 & 0.92 & \textbf{0.94} \\
        Medium & 0.88 & 0.95 & \textbf{0.98} \\
        Large & 0.78 & 0.88 & \textbf{0.91} \\
    \end{tabular}\end{center}
    \caption{Average specification consistency with $3\times 16$ requirements when sampling configurations randomly from a uniform distribution and 1-shot/4-shot sampling using our synthesizer model.}
    \label{fig:eval-consistency-baseline}
\end{figure}

\begin{figure*}[ht]
    \footnotesize
    \begin{center}
        \textbf{BGP Synthesis Time}
        \footnotesize
        \begin{tabular}{rrccccccccc}
        \toprule
        &&\multicolumn{3}{c}{Synthesis Time (s)} & \multicolumn{2}{c}{Accuracy (Neural)} \\
        \multicolumn{2}{l}{\# Requirements} & NetComplete & Neural (CPU) & Speedup &$\emptyset$ Consistency& $\emptyset$ No. Full Matches\\
        \midrule
    2 requirements &Small & 18.073s & 0.641s & \textbf{28.2x} & 0.969 & 0.875\\
        &Medium & 60.864s & 2.748s & \textbf{22.2x} & 0.939 & 0.75\\
        &Large & 1389.485s\tiny{  7/8 TO} & 22.301s & \textbf{62.3x} & 0.989 & 0.875\\
    \midrule
    8 requirements &Small & 247.691s & 1.065s & \textbf{232.5x} & 0.96 & 0.75\\
        &Medium & $>$25m\tiny{  8/8 TO} & 3.47s & \textbf{432.2x} & 0.968 & 0.5\\
        &Large & $>$25m\tiny{  8/8 TO} & 30.961s & \textbf{48.4x} & 0.969 & 0.75\\
    \midrule
    16 requirements &Small & 1416.828s\tiny{  7/8 TO} & 2.528s & \textbf{560.5x} & 0.926 & 0.25\\
        &Medium & $>$25m\tiny{  8/8 TO} & 5.481s & \textbf{273.7x} & 0.947 & 0.25\\
        &Large & $>$25m\tiny{  8/8 TO} & 69.092s & \textbf{21.7x} & 0.959 & 0.25\\
    \end{tabular}\end{center}
    \caption{Comparing consistency and synthesis time of our method (Neural) with the SMT-based state-of-art synthesis tool NetComplete. The notation {\tiny{n/8 TO}} indicates the number of timed out synthesis runs out of 8 (25+ minutes).}
    \label{fig:evaluation-compare-bgp}
\end{figure*}

\begin{figure*}[ht]
    \begin{center}
        \footnotesize
        \textbf{OSPF Synthesis Time}\\
        \footnotesize
        \begin{tabular}{rrccccccccc}
        \toprule
        &&\multicolumn{3}{c}{Synthesis Time (s)} & \multicolumn{2}{c}{Accuracy (Neural)} \\
        \multicolumn{2}{l}{} & NetComplete & Neural (GPU) & Speedup &$\emptyset$ Consistency& $\emptyset$ No. Full Matches\\
        \midrule
    2 requirements &Small & 0.265s & 0.091s & \textbf{2.9x} & 1.000 & 1.00\\
     &Medium & 0.404s & 0.098s & \textbf{4.1x} & 1.000 & 1.00\\
     &Large & 0.944s & 0.14s & \textbf{6.7x} & 1.000 & 1.00\\
    \midrule
    8 requirements &Small & 0.876s & 0.164s & \textbf{5.3x} & 0.982 & 0.75\\
     &Medium & 1.517s & 0.103s & \textbf{14.7x} & 1.000 & 1.00\\
     &Large & 3.505s & 0.316s & \textbf{11.1x} & 0.981 & 0.50\\
    \midrule
    16 requirements &Small & 1.65s & 0.21s & \textbf{7.9x} & 0.991 & 0.625\\
     &Medium & 2.646s & 0.245s & \textbf{10.8x} & 0.989 & 0.50\\
     &Large & $>$566.636s+\tiny{  3/8 TO} & 0.233s & \textbf{2430.4x} & 0.987 & 0.875\\
    \end{tabular}\end{center}
    \caption{Comparing consistency and synthesis time of our method (Neural) with the SMT-based OSPF synthesis tool NetComplete. The notation {\tiny{n/8 TO}} indicates the number of timed out synthesis runs out of 8 (25+ minutes).}
    \label{fig:evaluation-compare-ospf}
\end{figure*}


\subsection{Comparison to SMT-based Synthesis}
\label{sec:synthesis-vs-smt}

%To provide a comparison of our learned BGP/OSPF synthesizer with SMT-based methods,
We now compare the synthesis time of the learned neural synthesizer with those of NetComplte, a state-of-art configuration synthesis tool based on SMT-solvers \cite{el2018netcomplete}.

\paragraph{Specifications} As the type of supported requirements in NetComplete does not fully align with our model, we restrict this comparison to specifications which only include forwarding paths (i.e. \texttt{fwd} predicates). Further, NetComplete does not support cross-protocol synthesis as in our case and instead requires users to specify for each requirement the protocol to use for its implementation. To bridge this gap, we split the generated forwarding requirements into BGP and OSPF paths for a corresponding NetComplete specification.
%\todo{note on NetComplete installing policies at all routers, not only the edges of the AS}

\paragraph{Methodology} We compare both OSPF synthesis and BGP/OSPF-synthesis. We configure our trained synthesizer model to do OSPF synthesis by only predicting link weights. For each pair of topology and specification, we report the total time of running our synthesizer 4 times using 4-shot sampling, whereas for consistency we report the best out of the 4 runs. For NetComplete, we run the synthesizer with a timeout of 25 minutes. In case a NetComplete attempt times out, we report 25 minutes as a lower bound for its runtime.

\paragraph{OSPF Synthesis Time Results} We document the results of comparing OSPF synthesis time in \cref{fig:evaluation-compare-ospf}. Our synthesizer model achieves a speedup of 2-10x over NetComplete. With 16 requirements and dataset Large this speedup even increases to $2000\times$. Further, our model achieves very high consistency with the provided specification, often producing fully-consistent configurations.

\paragraph{BGP/OSPF Synthesis Time Results} In \cref{fig:evaluation-compare-bgp} we show the comparison of BGP/OSPF synthesis time. Our synthesizer model outperforms NetComplete by multiple orders of magnitude. We observe a speedup of $20-560\times$ which appears to increase with the size of topology and specification. Further, the average specification consistency of the synthesized configurations is greater than $92\%$ across all datasets, even for large topologies. In many cases, our synthesizer model produces fully-consistent configurations, especially with small topologies and specifications. In comparison, NetComplete times out on more than half of the synthesis tasks which means that we can only observe a lower bound of speedup in these cases. Note that our synthesizer model is running on a CPU due to memory restrictions with large topologies. However, running it on a GPU results in even greater speedups (up to $1000\times$, cf. \cref{app:sec:bgp-gpu-performance}). 

==> diff/git-latexdiff.34107/old/sections/5_related_work.tex <==
\section{Related Work}
\label{sec:related-work}

\paragraph{Traditional Configuration Synthesis} 
%A range of existing work is concerned with network configuration synthesis. 
Next to methods based on compilation such as Propane/PropaneAT \cite{beckett2017network}, there are a number of configuration synthesis methods based on constraint solving: Examples include ConfigAssure \cite{narain2008declarative}, SyNet \cite{el2017network} and NetComplete \cite{el2018netcomplete}. Due to their hand-coded nature, these methods are highly protocol-specific and can be very slow due to the solvers they employ. Although some of them allow for cross-protocol reasoning, this is not implemented as transparently as in our framework and users must specify per requirement which protocol to use for its implementation. In contrast, our approach has lower precision but allows for fully transparent cross-protocol reasoning, meaning forwarding requirements are not protocol-bound and the synthesizer chooses how to implement them. Further, our learned BGP/OSPF synthesis tool exhibits much lower synthesis times as compared to an SMT-based tool like NetComplete.

% \begin{itemize}
%     \item NetComplete, SyNet
%     \item Propane, PropaneAT
%     \item DeepBGP
% \end{itemize}

\paragraph{GNNs and Networking} DeepBGP \cite{bahnasy2020deepbgp} relies on GNNs and reinforcement learning to do configuration synthesis. However, it is limited to BGP configuration synthesis and is slower than SMT-based synthesis according to the author's evaluation. In contrast, our learning-based framework is cross-protocol, does not rely on reinforcement learning and provides better synthesis performance. Apart from configuration synthesis, GNNs have also been applied to other problems in the networking domain. For example, the authors of RouteNet \cite{rusek2020routenet} use GNNs to predict performance metrics of network configurations. Other work that is concerned with learning improved protocols includes Q-Routing \cite{boyan1994packet} or more modern approaches such as the Graph-Query Neural Network architecture \cite{geyer2018learning}.

\paragraph{Neural Algorithmic Reasoning} 
Neural algorithmic reasoning (NAR) as proposed in \cite{velivckovic2021neural}, describes the idea of replacing traditional algorithms with neural networks to learn improved algorithmic procedures. Exemplary work includes graph-related algorithms \cite{velivckovic2019neural} or solvers for combinatorial optimization problems \cite{cappart2021combinatorial,joshi2020learning,selsam2019guiding}. Our synthesis framework is the first applications of NAR to the networking domain and relies on the NAR-native encode-process-decode architecture. According to the hierarchy of NAR approaches in \cite{cappart2021combinatorial}, our method is an algorithm-level approach, as we do not supervise on intermediate steps. Although, such step-level methods promise better generalization, it is not clear what an intermediate result of a general synthesis procedure would be. However, future work on a step-level approach may further improve synthesis quality.

% \begin{itemize}
%     \item RouteNet
%     \item GraphNET
%     \item Learning and generating distributed routing protocols using graph-based deep learning
%     \item Unveiling the potential of Graph Neural Networks for network modeling and optimization in SDN
% \end{itemize}

==> diff/git-latexdiff.34107/old/sections/6_conclusion.tex <==
\setlength{\parskip}{6pt plus4mm minus4mm}
\section{Conclusion}
\label{sec:conclusion}
We presented a learning-based framework for configuration synthesis based on the idea of neural algorithmic reasoning. To assess the effectiveness of the system, we instantiated it for the case of BGP/OSPF synthesis. In contrast to traditional synthesis methods, our system supports transparent cross-protocol reasoning and learns synthesis rules only from data. Using our system, synthesis is sped up by a factor of up to $500\times$ when compared to SMT-based methods. Further, our evaluation demonstrates that the resulting synthesis tool provides excellent synthesis quality, producing configurations with high specification consistency. Overall, our results illustrate that exploring the direction of learning-based network configuration synthesis is a promising direction, enabling new cross-protocol reasoning capabilities and great performance improvements. Promising future work includes construction of hybrid systems, integrating both neural models and SMT-based approaches to obtain the best of both worlds.

==> diff/git-latexdiff.34367/new/acronyms.tex <==
\DeclareAcronym{AS}{
    short = AS,
    long = autonomous system,
    short-plural = es ,
    long-plural = s
}

==> diff/git-latexdiff.34367/new/sections/0_abstract.tex <==
% Context
Computer networks employ a number of different protocols to enable efficient routing. However, due to the complexity of multiple interacting protocols, it can be hard for network operators to implement high-level routing policies and requirements. Network configuration synthesis promises to address this situation by automatically generating configurations that satisfy a provided specification. However, existing synthesis methods are often limited to single-protocol reasoning, depend on protocol-specific and hand-coded synthesis rules, and are difficult to scale due to the SMT-based methods they employ. In this work we present a rather different, learning-based method for addressing the configuration synthesis challenge, one based on the recently proposed paradigm of neural algorithmic reasoning. Our framework is protocol-agnostic, enables cross-protocol reasoning and does not depend on any hardcoded synthesis rules. To evaluate, we instantiate our framework for the case of BGP/OSPF synthesis. Our experiments show we can synthesize configurations with a very high degree of specification consistency while observing speedups of up to $500\times$ compared to a state-of-the-art SMT-based synthesis tool.


==> diff/git-latexdiff.34367/new/sections/1_intro.tex <==
\section{Introduction}
\label{sec:introduction}

The backbone of the internet consists of many connected computer networks operated by different internet service providers (ISPs) and other large organizations. These networks rely on a number of protocols to enable effective and policy-driven routing of traffic. Based on router-level configurations, the protocols perform a distributed computation to construct a network's forwarding state. However, the relatively low-level router configuration makes it hard for network operators to directly enforce network-wide policies and requirements. This often leads to misconfiguration, which can cause global outages such as the recent hours-long blackout of the entire Facebook platform \cite{janardhan2021} and comparable events \cite{mccarthy_2019}.
%
\paragraph{Configuration Synthesis} This situation has triggered a number of research efforts regarding the synthesis of network configurations \cite{el2018netcomplete,beckett2017network,narain2008declarative}. Configuration synthesis is concerned with the task of automatically generating router-level configurations given a set of high-level requirements. However, this synthesis problem can be very hard to solve, since network configurations typically consist of a considerable number of tunable parameters, where the execution of several interacting protocols yields the overall forwarding state. An effective synthesis tool must thus account for this fact and be able to reason across multiple protocols.

\paragraph{SMT-based Synthesis} Some of the most successful efforts in providing cross-protocol synthesis capabilities are based on satisfiability modulo theory (SMT) solvers \cite{el2018netcomplete,el2017network}. While SMT-based synthesis is a promising method, it comes with a number of limitations:
% \item protocol-specific
% fully hand-coded synthesis rules, a lot of implementation effort, cross-protocol support extra complicated
(1) SMT-based synthesizers are hand-crafted and highly protocol-specific. To implement synthesis, we must first express our networking model, protocol semantics including vendor and device specific behavior in terms of first-order logic constraints. This is a time-intensive and complicated process, requiring lots of expert knowledge.
%  model-dependent: synthesis is reasoning on the level of some assumed model which may not reflect the real world: even if a configuration is synthesized based on some spec, it may behave differently and violate spec in practice
Further, (2) logic-based modelling introduces a disconnect between the synthesis tool and real-world behavior \cite{birkner2021metha}. More specifically, synthesized configurations may satisfy a provided specification within a formal framework, but may not behave the same way in the real world.
% can be very slow
And, (3) SMT-based synthesis can be very slow or fail to complete, especially when reasoning about large network topologies. In practice however, network operators reconfigure their networks on a daily basis \cite{vissicchio2012improving}, which means an effective synthesis tool must be fast.

% \item fully learned, no hand-coded synthesis rules (model-free), very flexible to adapt to more/new protocols
% \item protocol-agnostic, cross-protocol
\paragraph{Neural Algorithmic Reasoning for Synthesis} Recent work on neural algorithmic reasoning (NAR) proposes to replace traditional algorithms with neural networks to learn improved algorithmic procedures \cite{velivckovic2021neural}.
It has been shown to be a powerful and fast algorithmic approximation method for a number of graph-related \cite{velivckovic2019neural} and combinatorial optimization problems \cite{cappart2021combinatorial}. Further, due to its learned nature, NAR allows for learning procedures directly from (real-world) data, without the need for manual feature extraction. Overall, this positions NAR as an attractive method to obtain a fast, fully-learned synthesis procedure, which entirely avoids the need for a formal model or any hand-crafted synthesis rules. Based on this promising outlook, this paper explores how to apply the NAR paradigm to the problem of network configuration synthesis.

To that end, we propose a \textbf{new learning-based framework for configuration synthesis} as an alternative to SMT-based approaches. Our framework is protocol-agnostic, enables cross-protocol reasoning and avoids the need to manually provide synthesis rules. We build upon the idea of NAR, and train a graph-based processor neural network to learn a synthesis procedure in latent space. A key challenge in a multi-protocol setting is the diversity of different protocols and configuration parameters. To this end, we implement a generic embedding scheme based on Datalog-like facts and program sketching \cite{solar2008program}, which allows us to easily adapt our framework to new protocols. Further, our synthesis model produces a whole distribution of network configurations. As a consequence, we can directly sample multiple alternative synthesis outputs, which is not possible with standard SMT solvers. We apply our framework to a non-trivial synthesis setting where both the Border Gateway Protocol (BGP) and the Open Shortest Path First (OSPF) protocol are used. We demonstrate that our learned synthesis tool is up to~$500\times$ faster than a state-of-the-art SMT-based synthesizer, while producing configurations which on average enjoy more than 91\% satisfaction of the provided specification.

\paragraph{Main Contributions} Our core contributions are:
\vspace{-5pt}
\begin{itemize}
    \setlength{\itemsep}{5pt}
    \setlength{\parskip}{0pt}
    \item A learning-based framework for network configuration synthesis based on neural algorithmic reasoning.
    \item A neural network architecture for learning synthesizer models which relies on a generic graph-based encoding of network topologies and configurations.
    \item An extensive evaluation of our learning-based synthesizer, in terms of both precision and scalability, on the challenging setting where both the BGP and OSPF protocols are involved.
\end{itemize}

\section{Framework Overview}
\label{sec:overview}

\begin{figure}
    \begin{center}
        \includegraphics[width=0.45\textwidth]{figures/synthesizer-overview.pdf}
    \end{center}
    \caption{An overview of our learning-based synthesis framework.}
    \label{fig:learning-based-synthesis}
\end{figure}

%As an example, consider \cref{fig:network-fwd-tree} (c) which illustrates the forwarding plane of some traffic class reachable via external peer $E$ or $F$ in our example network. Each router of the network forwards traffic along some of its outgoing links. In practice, a number of protocols are used to populate a router's routing tables. For the instantiation of our synthesis framework however, we focus on OSPF and BGP.

In the following, we discuss the fundamentals and core steps of our learning-based framework as illustrated in \cref{fig:learning-based-synthesis}.

\paragraph{Network Configuration} In this work, we consider the configuration synthesis problem at the level of the so-called \emph{forwarding plane} of a network. This means we look at how each router forwards traffic, given a packet with a certain destination. The forwarding plane is determined by a distributed computation whose exact semantics depend on the different routing protocols in use. To adapt the forwarding behavior, network operators change configuration parameters at the router-level (e.g. link weights), such that running the protocols results in the desired forwarding plane. Given this context, we define the problem of configuration synthesis as follows.

\paragraph{Configuration Synthesis} The configuration synthesis problem corresponds to automatically generating these router-level configurations, such that a set of given requirements about the forwarding plane is satisfied. Typical requirements include reachability, traffic isolation and other forwarding properties. 

\paragraph{Dataset} To train a synthesizer model, we first generate a dataset of input/output samples for the synthesis problem. For this, we rely on a generative pipeline as shown in the top of \cref{fig:learning-based-synthesis}. First, we sample a random network configuration for some topology using a uniform generative process. Then, we simulate the involved protocols to obtain the corresponding forwarding plane. Next, we extract a specification by randomly selecting properties that hold for the computed forwarding plane. This leaves us with a specification and topology as input and corresponding configuration as the output to a synthesis problem.

\paragraph{Simulation} Depending on the protocols in use, one implements simulation code to compute the forwarding plane induced by a sampled configuration. Although this step is protocol-specific, the overall implementation effort is much lower compared to SMT-based synthesis. Protocols are typically well-defined algorithms which can be simulated, whereas the alternative of implementing a synthesizer often requires expert knowledge about SMT solvers. In practice, our framework may also be adapted to use a real-world network router to compute the behavior of a configuration, thereby capturing the real-world behavior directly.

\paragraph{Neural Synthesizer Model} Based on the generated dataset, we train a graph neural network (GNN) to perform synthesis. For this, the network's input consists of a topology, a specification and a configuration sketch where to-be-synthesized parameters are omitted. Following the NAR paradigm, we first encode this synthesizer input in latent space. Then, we apply an iterative processor network which relies on the graph attention mechanism to propagate information \cite{velivckovic2017graph}. Last, we apply a decoder network to predict the values of omitted configuration parameters, thereby synthesizing a corresponding configuration. To remain protocol-agnostic, our model is generic with respect to the input format, using an intermediate representation based on Datalog-like facts.
%
\paragraph{Relaxed Specification Consistency} Since parts of the configuration synthesis problems are known to be NP-hard \cite{fortz2000internet}, any precise synthesis method will run into scalability issues, just like SMT-based methods. However, practical synthesis must be fast and scalable to accommodate the size of real-world networks and the frequency at which configurations need to be updated \cite{vissicchio2012improving}. In our learning-based framework, we therefore employ a fixed-size neural network architecture which always runs in polynomial time. While this indeed enables fast synthesis times, we cannot expect our neural system to be as precise as SMT methods. Therefore, to assess the synthesis capabilities of our learning-based system, we rely on the notion of \emph{relaxed~specification~consistency}. More specifically, we do not just check whether a configuration satisfies a specification or not, but also measure the degree up to which a synthesized configuration satisfies a specification (e.g. via the number of satisfied requirements). 

This "soft" understanding of a specification allows us to evaluate neural synthesis systems which may not always produce fully consistent configurations. Further, we argue that configurations with less than $100\%$ consistency are still very useful in practice, as they provide a good starting point for additional adjustments by network operators. Future work may improve the precision of neural synthesis by exploiting partial synthesis methods \cite{el2018netcomplete} to obtain fully consistent solutions, given a partially consistent configuration. However, note also that even exact SMT-based synthesizers may not always produce fully consistent solutions, due to differences between the formal protocol model and the one running on a given real-world router where the configuration is to be deployed \cite{birkner2021metha}.

\paragraph{Instantiation} Our learning-based synthesis framework is generic with respect to the routing protocols in use. This means, it can be instantiated to many different synthesis settings. To do this, users merely provide a drop-in replacement for the simulation component as shown in \cref{fig:learning-based-synthesis}, while other components such as the neural model architecture itself can be directly re-used.

%More specifically, we employ a slightly modified variant which operates on a graph-based encoding of a specification, topology and configuration parameters.

%  \begin{figure*}
%      \centering
%      \includegraphics[width=0.85\textwidth]{figures/system-overview.pdf}
%      \caption{An overview of our synthesis system: (1) First, we use a generic embedding scheme to transform a network topology, protocol configuration sketches and the specification given as Datalog-like facts to a latent input representation. Next, we apply a learned (2) Processor GNN and obtain a latent synthesis output. Last, we apply a (3) Decoder Network to obtain a distribution over possible values per unknown parameter in our configuration.}
%      \label{fig:overview-model}
% \end{figure*}
%

In this paper, we first discuss the architecture of our neural synthesis model. In follow-up sections, we instantiate our framework  for the case of BGP/OSPF configuration synthesis, and evaluate the resulting instantiation by comparing it to a state-of-the-art SMT-based synthesizer.

% \begin{itemize}
%     \item effort: need to implement simulation code to generate dataset to learn from (typically well-defined in protocol specs, much easier than implementing synthesis directly)
%     \item can be sampled (multiple alternative solutions, not easily possible with SMT-based methods)
%     \item much faster than SMT-based synthesis
% \end{itemize}

% Requirements:
% \begin{itemize}
%     \item protocol-agnostic
%     \item fully learned, no hand-coded synthesis rules
%     \item define: strict specification vs. relaxed specification
% \end{itemize} 

==> diff/git-latexdiff.34367/new/sections/2_model.tex <==
\section{Neural Synthesis Model}
\label{sec:model}


We now present the architecture of our graph-based neural synthesizer model, illustrated in \cref{fig:overview-model}. First, in \cref{sec:graph-embedding} we introduce our generic graph-based encoding, which allows us to embed network topologies, protocol configuration and the specification into a latent space. Then, in \cref{sec:graph-transformer} we present the architecture of the processor network which we train to perform the synthesis task. Finally, in \cref{sec:decoding-sampling} we discuss how to sample network configurations from the resulting latent synthesis output.

\begin{figure}
    \begin{minipage}[t]{0.21\textwidth}
    \begin{lstlisting}[basicstyle=\ttfamily\small, escapeinside={(*}{*)}]
router(A)
router(B)
(...)

connected(A,B,2)
connected(A,C,?)(*\blackcircled{1}*)
(...)
    \end{lstlisting}
\end{minipage}
\begin{minipage}[t]{0.21\textwidth}
    \begin{lstlisting}[basicstyle=\ttfamily\small, escapeinside={(*}{*)}]
network(N1)
bgp_route(E,N1,2,3,1,0,1)

fwd(A,B,N1)
not fwd(B,A,N1)
(...)
    \end{lstlisting}
\end{minipage}
    \caption{A snippet of a fact base sketch encoding a network's topology, parameters such as link weights (\texttt{connected} facts) and a specification (\texttt{fwd} facts).}
    \label{fig:datalog-encoding}
\end{figure}

\begin{figure}[t]
    \centering
    \includegraphics[width=0.25\textwidth]{figures/synth-architecture.png}
    \caption{The neural synthesizer model architecture.}
    \label{fig:architecture}
\end{figure}

\subsection{Fact Base Embedding}
\label{sec:graph-embedding}
To remain network protocol-agnostic in our model architecture, we implement a generic graph-based encoding of Datalog-like facts, similar to knowledge graphs \cite{rosso2020beyond}. This means that we first encode topologies, configurations and specifications as a set of Datalog-like facts and then employ a generic embedding.
%We chose Datalog facts as the input format of our synthesis approach for its flexibility, wide-spread use in Program Analysis and use in previous work on configuration synthesis \cite{el2017network}.

\paragraph{Fact Base} A set of Datalog-like facts, as depicted in \cref{fig:datalog-encoding}, serves as the input \emph{fact base} $\mathcal{F}$ to our synthesizer model. $\mathcal{F}$ is a set of facts $f(a_0, \dots, a_n)$ where arguments may be constants (e.g. A or B) or integer literals. Further, each fact in a fact base has a corresponding truth value denoted as $[f(a)]_{\mathcal{B}}$. For instance, from the fact base in \cref{fig:datalog-encoding} we can derive $[fwd(A,B,N1)]_{\mathcal{B}} = \text{\texttt{true}}$ and $[fwd(B,A,N1)]_{\mathcal{B}} = \text{\texttt{false}}$.

\paragraph{Consistency} We represent a network's topology, the protocol configuration and parameters as well as the specification, all in a single fact base. Given the semantics of the protocols in use, we can then check whether the specification encoded in a fact base is satisfied by the provided configuration. To quantify, we define the notion of relaxed specification consistency, as discussed earlier, with respect to a fact base: Given a fact base $\mathcal{F}$, a subset of specification facts $S \subset \mathcal{F}$ and protocol semantics $\mathcal{P}$, the \emph{consistency} of a fact base is defined as the relative number of satisfied facts in $S$ with respect to the forwarding plane obtained via $\mathcal{P}$. The contents of $S$ depend on the concrete instantiation of the synthesizer model. For an example of possible specification facts, see our instantiation of the synthesizer model for BGP/OSPF in \cref{sec:training}.

\begin{figure*}
    \footnotesize
    \def\arraystretch{1.4}
    \begin{tabular}{lr}
        %$T_f: T_1 \times \dots \times T_n$ & \textit{(fact type declaration)}\\
        $emb(f) := \mathbf{V_f}$ & \textit{(learned fact type embedding)}\\
        $emb(b) := \mathbf{W_{\text{bool}}}\;onehot(b)$ & \textit{(learned boolean embedding)}\\
        $emb(f,i,v) := \mathbf{W_{f_i}}\;onehot(v)$ & \textit{(learned integer embedding)}\\
        $emb(f,i,?) := \mathbf{V_{hole}}$ & \textit{(learned hole embedding)}\vspace{2pt}\\
        $\mathlarger{
        h_c := \sum_{f(c) \in \mathcal{F}}
        emb(f)
        }$ & \textit{(constant embedding)}\vspace{2pt}\\
        $h_{f(a_0, \dots, a_n)} := emb(f) + emb([f(a_0, \dots, a_n)]_{\mathcal{B}}) + \mathlarger{
        \sum_{(i,v) \in \mathcal{I}(f(a_0, \dots, a_n))}
        emb(f, i, v)
        }$\hspace{-1.2cm} & \textit{(fact embedding)}\\
        $\mathcal{I}(f(a_0, \dots, a_n)) := \{(i,v) \; | \; f(a_0, \dots, a_{i-1}, v, \dots, a_n) \in \mathcal{F} \wedge v:Int \wedge i \in \mathbb{N}$ \}& \textit{(integer arguments)}\vspace{2pt}\\
        $N_i(h_c) := \{h_f \; | \; \exists i \in \mathbb{N} . f(a_0, \dots, a_{i-1}, c, a_{i+1}, \dots, a_n) \in \mathcal{F}\}$& \textit{(i-th neighborhood of constant node)} \\
        $N_i(h_f) := \{h_c \; | \; \exists i \in \mathbb{N} . f(a_0, \dots, a_{i-1}, c, a_{i+1}, \dots, a_n) \in \mathcal{F}\}$& \textit{(i-th neighborhood of fact node)} \\
    \end{tabular}
    \caption{Translating a fact base $\mathcal{F}$ to node features. $f$ denotes a predicate, $v$ integer values, $b$ boolean values as 0 or 1, $i$ argument indices and $[f(a)]_{\mathcal{B}}$ the truth value of a fact. }
    \label{fig:graph-embedding}
\end{figure*}

%discuss embedding as shown in \cref{fig:datalog-encoding}. Note how this makes fact bases a suitable input to standard GNN architectures.

\paragraph{Fact Base Sketching} In a synthesis setting, we are confronted with incomplete fact bases, i.e. the specification and topology is given but the network configuration is to be synthesized. For these cases, we also consider fact bases with unknown parameters inspired by the idea of program sketching in program synthesis \cite{solar2008program}. More specifically, users may replace an unknown integer argument of a fact by a \texttt{?} symbol, indicating a value to be synthesized. Using this mechanic, we can represent the synthesis input as an incomplete fact base which encodes to-be-synthesized values as unknown parameters. As an example, consider \cref{fig:datalog-encoding} \blackcircled{1}, where the link weight between router nodes \texttt{A} and \texttt{C} is represented as an unknown parameter.

\paragraph{Embedding} We employ a structurally-defined embedding scheme to transform a fact base into a graph with node features as required for processing with graph neural networks. Given a fact base $\mathcal{F}$, we apply the rules in \cref{fig:graph-embedding} to obtain node features and adjacency information. Both a fact $f$ and a constant $c$ are represented as distinct nodes with features $h_c$ and $h_f$, respectively. The relationships between facts and constants is encoded as node adjacency as defined by the neighborhood functions $N_i$.

We use multiple neighborhood functions, i.e. multiple types of edges, to encode the argument position of a constant occurring in a fact. Hence, the number of neighborhood functions corresponds to the maximum number of arguments in a single fact, e.g. 3 in \cref{fig:datalog-encoding}. Integer arguments and unary facts are directly accounted for in the respective node or fact embedding. To handle unknown parameters, we replace the corresponding $emb(...)$ term with the learned $\mathbf{V_{hole}}$ embedding.

Considering the embedding function $emb$, the learned parameters of our embedding are $\mathbf{V_f} \in \mathbb{R}^D$ per fact type in~$\mathcal{F}$, $\mathbf{W_{\text{bool}}} \in \mathbb{R}^{D \times 2}$ for boolean values, $\mathbf{W_{f_i}} \in \mathbb{R}^{D \times N}$ per integer argument of fact type $f$ and $\mathbf{V_{hole}} \in \mathbb{R}^D$ to represent unknown parameters. Hyperparameter $D$ represents the dimension of the latent space the synthesizer model operates in and $N$ specifies the number of supported integer values. An example of applying this embedding scheme to a simple fact base is given in \cref{fig:graph-encoding-example}.

\begin{figure}
    \begin{minipage}[t]{0.2\textwidth}
        \centering
        \footnotesize
        \textbf{Fact Base}
        \begin{lstlisting}[basicstyle=\ttfamily\small]
router(A)
router(B)

conn(A, B, 12)
        \end{lstlisting}
    \end{minipage}
    \begin{minipage}[t]{0.15\textwidth}
        \centering
        \textbf{Graph}\\
        \vspace{5pt}
        \includegraphics[width=0.7\textwidth]{figures/graph-encoding.pdf}
    \end{minipage}\\
    \centering\\
    \vspace{10pt}
    \textbf{Node Features}\\
    \vspace{10pt}
    \begin{minipage}[t]{0.5\textwidth}
        $\begin{array}{rcl}
        h_A &:=& emb(router) = \mathbf{V_{\text{router}}}\\
        h_B &:=& emb(router) = \mathbf{V_{\text{router}}}\\
        h_{\text{conn(A,B,12)}} &:=& emb(conn) + emb(conn, 2, 12)\\
        &:=& \mathbf{V_{\text{conn}}} + \mathbf{W_{conn_2}} onehot(12)
    \end{array}$
    \end{minipage}
    \caption{An example of embedding a simple fact base using the embedding scheme of \cref{fig:graph-embedding}. The shown graph illustrates the neighborhoods $N_0$ and $N_1$ induced by the \texttt{conn} fact.}
    \label{fig:graph-encoding-example}
\end{figure}

\begin{figure}
    $$
    \begin{array}{rcl}
    z_j &:=& h_j + Drop(\mathlarger{\sum_{N_i}} h'_{GAT_i})\\
    h'_j &:=& FFN(Norm(z_j))\vspace{11pt}\\
    FFN(x_j) &:=& Norm(Lin2(Drop(Lin1(x_j)))))
    \end{array}
    $$
    \caption{
        The recurrence relation of a node $j$'s representation $h_j$. $h'_{GAT_i}$ represents the output of a graph attention layer operating with neighborhood $N_i$ according to \cite{velivckovic2017graph}, $h_j$ the representation of node $j$ at the previous step. $Norm$ refers to batch normalization \cite{ioffe2015batch}, $Drop$ to dropout regularization \cite{hinton2012improving} and $Lin1$ and $Lin2$ to linear layers with an inner dimension of $4N$.
    }
    \label{fig:recurrence}
\end{figure}

\subsection{Synthesizer Model}
\label{sec:graph-transformer}

For an illustration of the synthesizer model's architecture, please see Figure~\ref{fig:architecture}. Given a fact base $\mathcal{F}$ we first apply our embedding scheme as described in \cref{sec:graph-embedding}. We then employ a 2-layer GNN-based encoder network to produce the latent representation of a synthesis input.
Given this representation, a processors network is trained to perform the actual synthesis task in high-dimensional space. Last, we apply a set of decoder networks, to obtain the synthesized values of unknown parameter, given the latent synthesis~output.

%In this context, the synthesis problem for network configurations corresponds to completing partially provided fact bases.

% \paragraph{High-Level Architecture}

% We employ the high-level architecture to obtain the latent synthesis output $y_\mathcal{F}$:
% $$
% \begin{array}{rcl}
%     \mathbf{x_{\mathcal{F}}} &:=& Encoder(Embedding(\mathcal{F}))\\
%     \mathbf{y_{\mathcal{F}}} &:=& Processor(\mathbf{x_{\mathcal{F}}} + \mathbf{z})\\
%     z_i &\sim& \mathcal{N}(0,1)
% \end{array}
% $$
% \todo{z is only added for $i<N/2$}

% $Embedding$ corresponds to the graph-based embedding as discussed in \cref{sec:graph-embedding} and $Encoder$ is a 2-layer graph attention module. $Processor$

\paragraph{Encoding} The encoder GNN operates on the embedded representation of a fact base. It produces the high-dimensional representation of a synthesis input as required for the processor network. We additionally apply noise to the first half of the units of the latent representation via $\mathbf{z}$, as a source of non-determinism. According to our experiments this improves model performance and we hypothesize this is due to the synthesis problem having more than one solution in most cases.

\paragraph{Iterative Processor} The processor network is modelled as an iterative process. It consists of a 6-layer graph attention module which we apply for a total of 4 iterations. In the framework of neural algorithmic reasoning, this iterative computational structure encodes an inductive bias towards an iterative solution to the synthesis problem. Because of this bias, our processor network essentially learns an algorithmic procedure which iteratively synthesizes the values of unknown parameters in a fact base.

\paragraph{Graph Attention Layer} In the GNNs we employ, we rely on a composed variant of the graph attention layer as introduced by \cite{velivckovic2017graph}. We employ multiple graph attention layers in lockstep, one per neighborhood $N_i$ defined by our graph embedding (cf. \cref{sec:graph-embedding}), and combine the intermediate results after each step. Specifically, the recurrence relation of a node $j$'s representation $h_j$ is defined as shown in \cref{fig:recurrence}. These mechanics of combining the results of the different graph attention layers $h'_{GAT_i}$, directly corresponds to how multiple attention heads are combined in the original Transformer architecture \cite{vaswani2017attention}.

\paragraph{Argument Decoder Networks} To synthesize the values of unknown parameters, the model maintains a set of decoder networks. That is, it provides one decoder network per integer argument per fact type in a fact base. When decoding, the network is applied to the latent synthesis output of the corresponding fact node. For example, a synthesizer model which operates on the fact base in \cref{fig:datalog-encoding}, would provide a decoder network $D_{\text{connected}_2}: \mathbb{R}^D \rightarrow \mathbb{R^N}$ to decode values for the third argument of a \texttt{conn} fact. In our experiments, decoder networks are implemented as simple multi-layer perceptron models.

\paragraph{Supervision Signal} During training, we mask all fact arguments that represent to-be-synthesized configuration parameters in our synthesis setting. As a supervision signal we use the masked values as the ground-truth and apply a negative log-likelihood loss function to the output distribution of the corresponding argument decoder networks.

%The synthesizer model learns a conditional distribution of fact bases which are consistent with respect to the protocols' semantics.

%\todo{introduce synthesis as a completion problem of an encoded fact base (a la BERT). Introduce masking, introduce decoding of integer and truth values. Synthesis is learning a conditional distribution of consistent fact bases.}

%Using this method, we obtain the node features $h_c$ per constant, $h_f$ per fact and adjacency information in terms of node neighborhood functions $N_i(h_c)$ and $N_i(h_f)$. Overall, this encoding makes a fact base suitable for processing using standard graph neural networks.

%- Brief description of the Graph Transformer Model
\subsection{Multi-Shot Sampling}
\label{sec:decoding-sampling}

%Multi-Stage Parameter Sampling (sampling methods: topk, high-temp, low-temp)
To sample concrete values from the output distributions over unknown parameters, we apply a multi-shot sampling strategy. That is, we sample values only for a subset of unknown parameters, insert them in our input fact base and run the synthesis model again. We repeat this process until no more unknown parameters remain. This multi-shot sampling strategy allows the model to incorporate the concrete values of previously synthesized parameters in its computation. In our evaluation in \cref{sec:evaluation}, we include a comparison of how this compares to sampling all unknown parameters at once.

%In a fact base with multiple holes, we apply the corresponding decoder networks to obtain a value distribution for each integer hole. However, instead of sampling all integer holes in one


==> diff/git-latexdiff.34367/new/sections/3_bgp_ospf.tex <==
\section{BGP/OSPF Synthesis}
\label{sec:bgp-ospf}

\newcommand{\as}{\ac{AS}~}
\newcommand{\ases}{\acp{AS}~}

\newcommand{\squareann}{{\tiny$\blacksquare\;$}}
\newcommand{\triangleann}{{\small$\blacktriangle\;$}}

\begin{figure*}
    \centering
    \includegraphics[width=0.95\textwidth]{figures/networks-all.pdf}
    \caption{(a) An illustration of a small AS network, including internal peers (blue), external peers (purple), BGP sessions as well as physical links. (b) The propagation of two BGP announcement across the network. (c) The resulting forwarding plane after applying BGP and OSPF.}
    \label{fig:network-fwd-tree}
\end{figure*}

We now discuss an instantiation of our learning-based framework for the case of BGP and OSPF protocols. In \cref{sec:synthesis-setting} we introduce a basic networking model, BGP and OSPF protocols and the synthesis setting. Given this model, \cref{sec:training} describes how to generate a corresponding dataset of input/output samples and train a synthesizer model.
%This shall serve as a prerequisite to the instantiation of our learning-based synthesis framework for the BGP and OSPF protocol in \cref{sec:training}.

\subsection{Synthesis Setting}
\label{sec:synthesis-setting}

\paragraph{Graphical Model} We assume an abstract network model which can be represented as an undirected graph as shown in \cref{fig:network-fwd-tree} (a). We always consider a set of internal routers (A, B, C, D in \cref{fig:network-fwd-tree}) as well as a set of adjacent external routers (E, F  in \cref{fig:network-fwd-tree}). The group of internal routers forms the \emph{\as} under consideration whereas external routers belong to other adjacent \ases. In practice, an \as represents an administrative domain controlled by a single operator. 

\paragraph{Forwarding Plane} For an example of a possible forwarding plane in this abstract model, consider \cref{fig:network-fwd-tree} (c) which illustrates the forwarding plane of traffic destined towards some destination reachable via external peer $E$ or $F$. Each router of the network forwards traffic along some of its outgoing links. In practice, a number of protocols are used to compute the forwarding plane. However, here we focus on OSPF and BGP.

\paragraph{OSPF} The OSPF protocol \cite{moy1994ospf} is a link-state protocol, typically used as an interior gateway protocol~(IGP), i.e., to route traffic within an \ac{AS}. Given link weights per physical link in the network, OSPF simply routes traffic along the shortest path towards the destination.

\paragraph{BGP} The BGP protocol \cite{rekhter1994border} on the other hand is a path-vector protocol used to exchange reachability information mostly on the level of \acp{AS}.
%These are groups of routers typically operated by a single party (e.g. an ISP).
When using BGP, a routing destination announces its existence to other \ases and routers, by sending out a BGP announcement. Receivers of such announcements may then choose to pass them on to other \acp{AS}, redistribute them internally and/or modify them. Instead of communicating along physical links directly, the BGP protocol requires manually configured BGP sessions among routers of the \as and external peers, as indicated by the BGP session edges in \cref{fig:network-fwd-tree}(a).
%\todo{more discussion of eBGP vs iBGP and support for route reflection (more of an implementation detail, maybe only mention in dataset generation where simulation code is discussed)}.

%\paragraph{BGP Decision Procedure}~
%\todo{discuss decision procedure}
In case a router receives more than one announcement for a destination, a designated BGP decision process is applied to determine a single best route. \cref{fig:bgp-decision} shows the ordered list of comparison criteria of this decision process. The different criteria depend different properties of a route announcements, including the IGP cost towards the routing destination. As a consequence, when used together, OSPF as IGP protocol and BGP will interact. %Note also that BGP is an iterative process which needs multiple rounds of propagation to converge.

\paragraph{Example}
%\todo{run through simple BGP+OSPF example of computing the forwarding plane}
To better understand BGP/OSPF routing, consider the simple example given in \cref{fig:network-fwd-tree} (b). Here, our example \as imports BGP announcements \squareann and \triangleann from E and F respectively. Both represent a route to the same destination. As shown, both announcements have a so-called local preference of 2. For simplicity, we ignore other properties such as the AS path length, Origin and MED in this example. The announcements are propagated among BGP neighbors and the best route is selected according to the decision procedure in \cref{fig:bgp-decision}. See \cref{fig:network-fwd-tree} (b) for an illustration of the intermediate states of this propagation process. As both announcements have a local preference of 2, rule 1 of the decision process is not used. Instead, in round 2, node B selects \squareann over \triangleann due to a lower IGP cost of 2 via egress node A as compared to 3 via egress node D (rule 6). Node D selects \triangleann over \squareann, since it learns this route directly from an external peer (rule 5). After Round 3, the BGP propagation process converges to a stable state and we can derive the forwarding plane as shown in \cref{fig:network-fwd-tree} (c).


%, as well as external peers E and F which belong to other \acp{AS}. External peers are routers which are connected via eBGP sessions to routers of the \ac{AS} under consideration. They announce BGP routes to their neighbors, which are propagated within the network

%\paragraph{BGP/OSPF Configuration Synthesis} We phrase the BGP/OSPF configuration synthesis problem on the level of the forwarding plane. This means that users provide a specification which constraints the set of allowed forwarding planes. This includes predicates which enforce forwarding paths, block forwarding paths or assert higher-level properties like traffic isolation and reachability. Given such a specification, we consider network configuration synthesis as the task of configuring OSPF and BGP in a way that produces a forwarding plane which satisfies the provided specification.

\paragraph{BGP/OSPF Configuration Synthesis} According to our general synthesis framework, we consider the BGP/OSPF configuration synthesis problem at the level of the forwarding plane. However, we further also define the set of synthesized parameters: For OSPF we synthesize link weights as explored in a wide range of existing work (e.g. \cite{el2018netcomplete,fortz2000internet}. For BGP, the set of parameters is not defined as clearly: Depending on the requirements of a network operator, one may employ custom BGP import and export policies at every router of a network to implement complex behavior. However, in this instantiation we focus on a simplified setting, where we assume BGP route announcements to only be modified when imported into the \as from an external peer. Previous work has already pointed out that this is a reasonable assumption which holds for the majority of real-world networks \cite{caesar2005bgp,cittadini2010doing, steffen2020probabilistic}.

\begin{figure}
    \small{
    \begin{enumerate}
        \setlength{\itemsep}{0pt}
        \setlength{\parskip}{0pt}
        \item Highest Local preference
        \item Lowest AS path length
        \item Prefer Origin (IGP $>$ EBGP $>$ INCOMPLETE)
        \item Lowest Multi-exit discriminator (MED)
        \item External over internal announcements
        \item Lowest IGP cost to egress
        \item Lowest BGP peer id (tie breaker)
    \end{enumerate}}
    \vspace{-15pt}
    \caption{The BGP decision process \cite{rekhter1994border}. The shown rules are applied in order until a single best BGP announcements remains.}
    \label{fig:bgp-decision}
\end{figure}

\subsection{Dataset Generation and Training}
\label{sec:training}
To train a synthesizer model, we need a large number of fact bases encoding a variety of network topologies, configurations and forwarding specifications. Further, we must provide the model with target values for unknown parameters as a supervision signal. This section discusses how we construct such a dataset for BGP/OSPF synthesis.
%Further, we provide an example of what a corresponding fact base looks like, including a description of the supported specification language.

\paragraph{Dataset Generation} To obtain network configurations and corresponding forwarding specifications we employ a generative process: We first randomly configure BGP and OSPF parameters for some topology. Then we simulate the OSPF and BGP protocol and compute the resulting forwarding plane. Based on this, we extract a forwarding specification which fixes a random subset of forwarding paths, reachability and isolation properties that are satisfied by the forwarding plane.

\paragraph{Topologies} For training, our dataset is based on random topologies with $16$-$24$ routers. We generate the physical layout of these graphs by triangulation of uniformly sampled points in two-dimensional space.

\paragraph{Simulation} To compute the forwarding plane given an OSPF and BGP configuration, we simulate the protocols. For OSPF, we implement shortest path computation to obtain the forwarding plane. For BGP, we implement the full BGP decision process as shown in \cref{fig:bgp-decision}, except for the MED attribute. In addition to the basic networking model discussed in \cref{sec:synthesis-setting}, we implement support for eBGP and iBGP, fully-meshed BGP session layouts as well as layouts relying on route reflection. For more details of these BGP concepts see \cite{bates2000rr}.

%Note that the synthesizer model will reason on the level of the provided training samples. That is, to improve the overall synthesis quality in a real-world setting, it is helpful to implement simulation code which behaves very similar to real-world networks. Another promising approach would be to extract training samples from real-world networks, thereby circumventing the need for simulation, however, we leave this as future work.

%While this can be a considerable effort, it is typically an easier task than to implement the synthesizer directly. The concrete semantics of protocols and their simulation is a well-defined procedure, whereas implementing efficient synthesis tools is still an open problem.

\paragraph{Fact Base Encoding} We encode synthesis input using a small set of facts. For an example of a corresponding fact base see \cref{fig:bgp-ospf-fact-base}. We use the \texttt{router}, \texttt{external} and \texttt{network} facts to mark routers, external peers and routing destinations respectively. Physical links between routers are encoded as \texttt{connected(R1,R2,W)} facts where \texttt{W} denotes the OSPF link weight. Further, we rely on \texttt{ibgp}, \texttt{ebgp}, \texttt{route\_reflector} and \texttt{bgp\_route} facts to represent different types of BGP sessions and imported routes. Using the notion of unknown parameters as discussed in \cref{sec:graph-embedding}, we encode configuration parameters, e.g., properties of imported routes or OSPF link weights.

\paragraph{Specification Language} We support a small specification language with three types of forwarding predicates:

\begin{itemize}
    \setlength{\itemsep}{0pt}
    \setlength{\parskip}{2pt}
    \item \texttt{fwd(R1, Net, R2)} specifies that router \texttt{R1} forwards traffic destined for \texttt{Net} to its neighbor \texttt{R2}.
    \item \texttt{reachable(R1, Net, R2)} specifies that traffic destined for \texttt{Net} that passes through \texttt{R1} also passes through \texttt{R2} before reaching its destination.
    \item \texttt{trafficIsolation(R1, R2, N1, N2)} specifies that it must not hold that $[fwd(R1,R2,N1)]_{\mathcal{B}} \wedge [fwd(R1,R2,N2)]_{\mathcal{B}}$.
\end{itemize}

In the negative case of each predicate, the opposite must hold true for the fact to be satisfied. This specification language can easily be extended by including new specification predicates in the dataset generation process. One must simply provide a method of extracting positive and negative cases of a specification fact from a given forwarding plane. Once included in the training dataset of a synthesizer model, the resulting synthesis system will be able to consider specifications relying on the new type of predicates.

% \todo{info on loss function, optimizer, etc.}
\paragraph{Training} We generate a dataset of $10,240$ input/output samples and instantiate our synthesizer model with a hidden dimension $D$ of $64$. For optimization, we use the Adam optimizer \cite{kingma2014adam} with a learning rate of $10^{-4}$. We stop training after the specification consistency on a validation dataset no longer increases at $\sim2800$ epochs.

\begin{figure}
\begin{minipage}[t]{0.22\textwidth}
\begin{lstlisting}[basicstyle=\ttfamily\tiny]
# topology and configuration
router(c5)
router(c3)
router(c1)
router(c0)
network(c6)
network(c7)

external(c8)
external(c9)
external(c10)
external(c11)
external(c12)
external(c13)

route_reflector(c2)
route_reflector(c4)

connected(c2,c4,?)
connected(c2,c5,?)
connected(c2,c3,?)
connected(c4,c5,?)
connected(c4,c3,?)
connected(c4,c0,?)
connected(c5,c1,?)
connected(c5,c0,?)
connected(c3,c0,?)
connected(c3,c1,?)
connected(c1,c0,?)

ibgp(c2,c4)
ibgp(c2,c5)
ibgp(c2,c0)
ibgp(c2,c1)
ibgp(c4,c3)
ibgp(c4,c4)
\end{lstlisting}
\end{minipage}
\begin{minipage}[t]{0.2\textwidth}
\begin{lstlisting}[basicstyle=\ttfamily\tiny]
ebgp(c2,c12)
ebgp(c5,c9)
ebgp(c5,c10)
ebgp(c5,c13)
ebgp(c0,c8)
ebgp(c0,c11)

bgp_route(c8,c6,?,?,1,?,1,8)
bgp_route(c9,c6,?,?,0,?,1,9)
bgp_route(c10,c6,?,?,0,?,1,10)
bgp_route(c11,c7,?,?,0,?,1,11)
bgp_route(c12,c7,?,?,0,?,1,12)
bgp_route(c13,c7,?,?,2,?,1,13)

# forwarding specification
fwd(c0,c6,c3)
fwd(c3,c6,c2)
fwd(c2,c6,c4)
not fwd(c3,c6,c0)
not fwd(c0,c6,c11)
not fwd(c11,c6,c0)

not trafficIsolation(c1,c0,c7,c6)
not trafficIsolation(c1,c0,c7,c6)
trafficIsolation(c0,c3,c6,c7)
trafficIsolation(c0,c3,c6,c7)

reachable(c5,c6,c10)
reachable(c1,c6,c4)
not reachable(c0,c6,c5)
reachable(c5,c6,c10)
\end{lstlisting}
\end{minipage}
\caption{An example of a fact base encoding a topology, a sketch of a BGP and OSPF configuration and a forwarding specification.}
\label{fig:bgp-ospf-fact-base}
\end{figure} 

==> diff/git-latexdiff.34367/new/sections/4_evaluation.tex <==
\section{Evaluation}
\label{sec:evaluation}

We trained a synthesizer model to perform configuration synthesis for BGP and OSPF. We now assess the performance of the resulting neural synthesizer with respect to two core metrics: (1) the quality of synthesized configurations in terms of their consistency with the provided forwarding specifications (\cref{sec:synthesis-quality}), and (ii) the time a learned synthesizer takes when compared to the state-of-the-art SMT-based synthesizer NetComplete \cite{el2018netcomplete} (\cref{sec:synthesis-vs-smt}).

\paragraph{Dataset} We compare across three datasets: Small, Medium and Large. Each dataset represents 8 real-world topologies, sampled from the Topology Zoo \cite{knight2011internet}, where the number of nodes lies between 0-34, 34-68 and 68-170 respectively. To obtain forwarding specifications for the sampled topologies, we use our generative pipeline as discussed in \cref{sec:training}. In each topology, we do synthesis for 4 different traffic classes (routing destinations) at a time.

\paragraph{Experimental Setup} We run all our experiments on an Ubuntu Linux machine with an Intel(R)~Core(TM)~i9-9900X~@~3.50GHz processor, 64GB of system memory and an NVIDIA GeForce RTX 3080 GPU with 10GB of video~memory.

\subsection{Synthesis Quality}
\label{sec:synthesis-quality}
To assess our learned synthesizer, we examine its behavior with increasingly large topologies and specifications.

\paragraph{Specifications} Using the same generative model as described in \cref{sec:training}, we generate forwarding specifications for the topologies in our three datasets with each specification constructed from $3 \times n$ requirements, one per supported predicate type:  \texttt{fwd} requirements correspond to specifying or blocking a forwarding path using multiple \texttt{fwd} predicates whereas \texttt{reachable} and \texttt{trafficIsolation} requirements each translate to a single specification fact. We compare across increasingly large specifications of $3\times 2$, $3\times 8$ and $3 \times 16$ requirements, respectively.

\paragraph{Methodology} For each pair of topology and specification, we run our synthesizer 5 times and report the network configurations with the highest overall consistency value. For sampling, we rely on our multi-shot sampling strategy where we randomly group the unknown parameters of a configuration into 4 groups (4-shot sampling).

\paragraph{Results} We summarize our results in \cref{fig:eval-consistency}. On average, our synthesis model produces network configurations that are $>91\%$ consistent with the provided forwarding specifications across all datasets and sizes of specifications. When only few requirements are given, the synthesizer model even succeeds in producing fully-consistent configurations. We observe a slightly decreasing consistency with increasingly large topologies.

%\texttt{fwd} facts are satisfied more easily, whereas \texttt{reachable} and \texttt{trafficIsolation} facts are violated more often.

\paragraph{Multi-Shot Sampling} In \cref{fig:eval-consistency-baseline}, we report the average specification consistency using our multi-shot sampling strategy as compared to sampling all unknown parameters at once. As a baseline we have also sampled random configurations from a uniform distribution (per parameter) and compute the corresponding specification consistency. Over the baseline, our synthesizer model shows clear improvement and multi-shot sampling further increases consistency.

\begin{figure*}
    \begin{center}
        \textbf{Specification Consistency}\\
        \footnotesize
        \begin{tabular}{rrcccccccccc}
        \toprule
        \multicolumn{2}{c}{Dataset} & \tiny\texttt{fwd} & \tiny\texttt{reachable}  & \tiny\texttt{trafficIsolation} & Overall & $\emptyset$     No. Full Matches & $\emptyset$ No. $>90\%$ Matches\\
        \midrule
        $3\times 2$ requirements & Small & 0.95 & 0.94 & 1.00 & \textbf{0.95} & 0.62 & 0.62\\
& Medium & 0.96 & 1.00 & 0.94 & \textbf{0.96} & 0.88 & 0.88\\
& Large & 0.94 & 0.94 & 1.00 & \textbf{0.93} & 0.62 & 0.62\\
\midrule
$3\times 8$ requirements & Small & 0.97 & 0.98 & 0.97 & \textbf{0.98} & 0.50 & 1.00\\
& Medium & 0.99 & 0.95 & 1.00 & \textbf{0.98} & 0.50 & 1.00\\
& Large & 0.96 & 0.95 & 0.91 & \textbf{0.94} & 0.38 & 0.88\\
\midrule
$3\times 16$ requirements & Small & 0.97 & 0.89 & 0.95 & \textbf{0.94} & 0.38 & 0.75\\
& Medium & 0.98 & 0.97 & 0.97 & \textbf{0.98} & 0.38 & 1.00\\
& Large & 0.92 & 0.88 & 0.95 & \textbf{0.91} & 0.12 & 0.50\\
    \end{tabular}\end{center}
    \caption{Average specification consistency of the network configurations synthesized by our trained synthesizer model. Per sample we run the synthesizer with a specification of $3\times N$ requirements, where the specifications always include $N$ requirements per supported predicate type (\texttt{fwd}, \texttt{reachable}, \texttt{trafficIsolation}).}
    \label{fig:eval-consistency}
\end{figure*}

\begin{figure}
    \begin{center}
        \footnotesize
        \begin{tabular}{rrcccccccccc}
        &  & \multicolumn{2}{c}{Neural}\\
        & Random & 1-Shot & 4-shot\\
        \toprule
        Small & 0.83 & 0.92 & \textbf{0.94} \\
        Medium & 0.88 & 0.95 & \textbf{0.98} \\
        Large & 0.78 & 0.88 & \textbf{0.91} \\
    \end{tabular}\end{center}
    \caption{Average specification consistency with $3\times 16$ requirements when sampling configurations randomly from a uniform distribution and 1-shot/4-shot sampling using our synthesizer model.}
    \label{fig:eval-consistency-baseline}
\end{figure}

\begin{figure*}[ht]
    \footnotesize
    \begin{center}
        \textbf{BGP Synthesis Time}
        \footnotesize
        \begin{tabular}{rrccccccccc}
        \toprule
        &&\multicolumn{3}{c}{Synthesis Time (s)} & \multicolumn{2}{c}{Accuracy (Neural)} \\
        \multicolumn{2}{l}{\# Requirements} & NetComplete & Neural (CPU) & Speedup &$\emptyset$ Consistency& $\emptyset$ No. Full Matches\\
        \midrule
    2 requirements &Small & 18.073s & 0.641s & \textbf{28.2x} & 0.969 & 0.875\\
        &Medium & 60.864s & 2.748s & \textbf{22.2x} & 0.939 & 0.75\\
        &Large & 1389.485s\tiny{  7/8 TO} & 22.301s & \textbf{62.3x} & 0.989 & 0.875\\
    \midrule
    8 requirements &Small & 247.691s & 1.065s & \textbf{232.5x} & 0.96 & 0.75\\
        &Medium & $>$25m\tiny{  8/8 TO} & 3.47s & \textbf{432.2x} & 0.968 & 0.5\\
        &Large & $>$25m\tiny{  8/8 TO} & 30.961s & \textbf{48.4x} & 0.969 & 0.75\\
    \midrule
    16 requirements &Small & 1416.828s\tiny{  7/8 TO} & 2.528s & \textbf{560.5x} & 0.926 & 0.25\\
        &Medium & $>$25m\tiny{  8/8 TO} & 5.481s & \textbf{273.7x} & 0.947 & 0.25\\
        &Large & $>$25m\tiny{  8/8 TO} & 69.092s & \textbf{21.7x} & 0.959 & 0.25\\
    \end{tabular}\end{center}
    \caption{Comparing consistency and synthesis time of our method (Neural) with the SMT-based state-of-art synthesis tool NetComplete. The notation {\tiny{n/8 TO}} indicates the number of timed out synthesis runs out of 8 (25+ minutes).}
    \label{fig:evaluation-compare-bgp}
\end{figure*}

\begin{figure*}[ht]
    \begin{center}
        \footnotesize
        \textbf{OSPF Synthesis Time}\\
        \footnotesize
        \begin{tabular}{rrccccccccc}
        \toprule
        &&\multicolumn{3}{c}{Synthesis Time (s)} & \multicolumn{2}{c}{Accuracy (Neural)} \\
        \multicolumn{2}{l}{} & NetComplete & Neural (GPU) & Speedup &$\emptyset$ Consistency& $\emptyset$ No. Full Matches\\
        \midrule
    2 requirements &Small & 0.265s & 0.091s & \textbf{2.9x} & 1.000 & 1.00\\
     &Medium & 0.404s & 0.098s & \textbf{4.1x} & 1.000 & 1.00\\
     &Large & 0.944s & 0.14s & \textbf{6.7x} & 1.000 & 1.00\\
    \midrule
    8 requirements &Small & 0.876s & 0.164s & \textbf{5.3x} & 0.982 & 0.75\\
     &Medium & 1.517s & 0.103s & \textbf{14.7x} & 1.000 & 1.00\\
     &Large & 3.505s & 0.316s & \textbf{11.1x} & 0.981 & 0.50\\
    \midrule
    16 requirements &Small & 1.65s & 0.21s & \textbf{7.9x} & 0.991 & 0.625\\
     &Medium & 2.646s & 0.245s & \textbf{10.8x} & 0.989 & 0.50\\
     &Large & $>$566.636s+\tiny{  3/8 TO} & 0.233s & \textbf{2430.4x} & 0.987 & 0.875\\
    \end{tabular}\end{center}
    \caption{Comparing consistency and synthesis time of our method (Neural) with the SMT-based OSPF synthesis tool NetComplete. The notation {\tiny{n/8 TO}} indicates the number of timed out synthesis runs out of 8 (25+ minutes).}
    \label{fig:evaluation-compare-ospf}
\end{figure*}


\subsection{Comparison to SMT-based Synthesis}
\label{sec:synthesis-vs-smt}

%To provide a comparison of our learned BGP/OSPF synthesizer with SMT-based methods,
We now compare the synthesis time of the learned neural synthesizer with those of NetComplte, a state-of-art configuration synthesis tool based on SMT-solvers \cite{el2018netcomplete}.

\paragraph{Specifications} As the type of supported requirements in NetComplete does not fully align with our model, we restrict this comparison to specifications which only include forwarding paths (i.e. \texttt{fwd} predicates). Further, NetComplete does not support cross-protocol synthesis as in our case and instead requires users to specify for each requirement the protocol to use for its implementation. To bridge this gap, we split the generated forwarding requirements into BGP and OSPF paths for a corresponding NetComplete specification.
%\todo{note on NetComplete installing policies at all routers, not only the edges of the AS}

\paragraph{Methodology} We compare both OSPF synthesis and BGP/OSPF-synthesis. We configure our trained synthesizer model to do OSPF synthesis by only predicting link weights. For each pair of topology and specification, we report the total time of running our synthesizer 4 times using 4-shot sampling, whereas for consistency we report the best out of the 4 runs. For NetComplete, we run the synthesizer with a timeout of 25 minutes. In case a NetComplete attempt times out, we report 25 minutes as a lower bound for its runtime.

\paragraph{OSPF Synthesis Time Results} We document the results of comparing OSPF synthesis time in \cref{fig:evaluation-compare-ospf}. Our synthesizer model achieves a speedup of 2-10x over NetComplete. With 16 requirements and dataset Large this speedup even increases to $2000\times$. Further, our model achieves very high consistency with the provided specification, often producing fully-consistent configurations.

\paragraph{BGP/OSPF Synthesis Time Results} In \cref{fig:evaluation-compare-bgp} we show the comparison of BGP/OSPF synthesis time. Our synthesizer model outperforms NetComplete by multiple orders of magnitude. We observe a speedup of $20-560\times$ which appears to increase with the size of topology and specification. Further, the average specification consistency of the synthesized configurations is greater than $92\%$ across all datasets, even for large topologies. In many cases, our synthesizer model produces fully-consistent configurations, especially with small topologies and specifications. In comparison, NetComplete times out on more than half of the synthesis tasks which means that we can only observe a lower bound of speedup in these cases. Note that our synthesizer model is running on a CPU due to memory restrictions with large topologies. However, running it on a GPU results in even greater speedups (up to $1000\times$, cf. \cref{app:sec:bgp-gpu-performance}). 

==> diff/git-latexdiff.34367/new/sections/5_related_work.tex <==
\section{Related Work}
\label{sec:related-work}

\paragraph{Traditional Configuration Synthesis} 
%A range of existing work is concerned with network configuration synthesis. 
Next to methods based on compilation such as Propane/PropaneAT \cite{beckett2017network}, there are a number of configuration synthesis methods based on constraint solving: Examples include ConfigAssure \cite{narain2008declarative}, SyNet \cite{el2017network} and NetComplete \cite{el2018netcomplete}. Due to their hand-coded nature, these methods are highly protocol-specific and can be very slow due to the solvers they employ. Although some of them allow for cross-protocol reasoning, this is not implemented as transparently as in our framework and users must specify per requirement which protocol to use for its implementation. In contrast, our approach has lower precision but allows for fully transparent cross-protocol reasoning, meaning forwarding requirements are not protocol-bound and the synthesizer chooses how to implement them. Further, our learned BGP/OSPF synthesis tool exhibits much lower synthesis times as compared to an SMT-based tool like NetComplete.

% \begin{itemize}
%     \item NetComplete, SyNet
%     \item Propane, PropaneAT
%     \item DeepBGP
% \end{itemize}

\paragraph{GNNs and Networking} DeepBGP \cite{bahnasy2020deepbgp} relies on GNNs and reinforcement learning to do configuration synthesis. However, it is limited to BGP configuration synthesis and is slower than SMT-based synthesis according to the author's evaluation. In contrast, our learning-based framework is cross-protocol, does not rely on reinforcement learning and provides better synthesis performance. Apart from configuration synthesis, GNNs have also been applied to other problems in the networking domain. For example, the authors of RouteNet \cite{rusek2020routenet} use GNNs to predict performance metrics of network configurations. Other work that is concerned with learning improved protocols includes Q-Routing \cite{boyan1994packet} or more modern approaches such as the Graph-Query Neural Network architecture \cite{geyer2018learning}.

\paragraph{Neural Algorithmic Reasoning} 
Neural algorithmic reasoning (NAR) as proposed in \cite{velivckovic2021neural}, describes the idea of replacing traditional algorithms with neural networks to learn improved algorithmic procedures. Exemplary work includes graph-related algorithms \cite{velivckovic2019neural} or solvers for combinatorial optimization problems \cite{cappart2021combinatorial,joshi2020learning,selsam2019guiding}. Our synthesis framework is the first applications of NAR to the networking domain and relies on the NAR-native encode-process-decode architecture. According to the hierarchy of NAR approaches in \cite{cappart2021combinatorial}, our method is an algorithm-level approach, as we do not supervise on intermediate steps. Although, such step-level methods promise better generalization, it is not clear what an intermediate result of a general synthesis procedure would be. However, future work on a step-level approach may further improve synthesis quality.

% \begin{itemize}
%     \item RouteNet
%     \item GraphNET
%     \item Learning and generating distributed routing protocols using graph-based deep learning
%     \item Unveiling the potential of Graph Neural Networks for network modeling and optimization in SDN
% \end{itemize}

==> diff/git-latexdiff.34367/new/sections/6_conclusion.tex <==
\setlength{\parskip}{6pt plus4mm minus4mm}
\section{Conclusion}
\label{sec:conclusion}
We presented a learning-based framework for configuration synthesis based on the idea of neural algorithmic reasoning. To assess the effectiveness of the system, we instantiated it for the case of BGP/OSPF synthesis. In contrast to traditional synthesis methods, our system supports transparent cross-protocol reasoning and learns synthesis rules only from data. Using our system, synthesis is sped up by a factor of up to $500\times$ when compared to SMT-based methods. Further, our evaluation demonstrates that the resulting synthesis tool provides excellent synthesis quality, producing configurations with high specification consistency. Overall, our results illustrate that exploring the direction of learning-based network configuration synthesis is a promising direction, enabling new cross-protocol reasoning capabilities and great performance improvements. Promising future work includes construction of hybrid systems, integrating both neural models and SMT-based approaches to obtain the best of both worlds.

==> diff/git-latexdiff.34367/old/acronyms.tex <==
\DeclareAcronym{AS}{
    short = AS,
    long = autonomous system,
    short-plural = es ,
    long-plural = s
}

==> diff/git-latexdiff.34367/old/sections/0_abstract.tex <==
% Context
Computer networks employ a number of different protocols to enable efficient routing. However, due to the complexity of multiple interacting protocols, it can be hard for network operators to implement high-level routing policies and requirements. Network configuration synthesis promises to address this situation by automatically generating configurations that satisfy a provided specification. However, existing synthesis methods are often limited to single-protocol reasoning, depend on protocol-specific and hand-coded synthesis rules, and are difficult to scale due to the SMT-based methods they employ. In this work we present a rather different, learning-based method for addressing the configuration synthesis challenge, one based on the recently proposed paradigm of neural algorithmic reasoning. Our framework is protocol-agnostic, enables cross-protocol reasoning and does not depend on any hardcoded synthesis rules. To evaluate, we instantiate our framework for the case of BGP/OSPF synthesis. Our experiments show we can synthesize configurations with a very high degree of specification consistency while observing speedups of up to $500\times$ compared to a state-of-the-art SMT-based synthesis tool.


==> diff/git-latexdiff.34367/old/sections/1_intro.tex <==
\section{Introduction}
\label{sec:introduction}

The backbone of the internet consists of many connected computer networks operated by different internet service providers (ISPs) and other large organizations. These networks rely on a number of protocols to enable effective and policy-driven routing of traffic. Based on router-level configurations, the protocols perform a distributed computation to construct a network's forwarding state. However, the relatively low-level router configuration makes it hard for network operators to directly enforce network-wide policies and requirements. This often leads to misconfiguration, which can cause global outages such as the recent hours-long blackout of the entire Facebook platform \cite{janardhan2021} and comparable events \cite{mccarthy_2019}.
%
\paragraph{Configuration Synthesis} This situation has triggered a number of research efforts regarding the synthesis of network configurations \cite{el2018netcomplete,beckett2017network,narain2008declarative}. Configuration synthesis is concerned with the task of automatically generating router-level configurations given a set of high-level requirements. However, this synthesis problem can be very hard to solve, since network configurations typically consist of a considerable number of tunable parameters, where the execution of several interacting protocols yields the overall forwarding state. An effective synthesis tool must thus account for this fact and be able to reason across multiple protocols.

\paragraph{SMT-based Synthesis} Some of the most successful efforts in providing cross-protocol synthesis capabilities are based on satisfiability modulo theory (SMT) solvers \cite{el2018netcomplete,el2017network}. While SMT-based synthesis is a promising method, it comes with a number of limitations:
% \item protocol-specific
% fully hand-coded synthesis rules, a lot of implementation effort, cross-protocol support extra complicated
(1) SMT-based synthesizers are hand-crafted and highly protocol-specific. To implement synthesis, we must first express our networking model, protocol semantics including vendor and device specific behavior in terms of first-order logic constraints. This is a time-intensive and complicated process, requiring lots of expert knowledge.
%  model-dependent: synthesis is reasoning on the level of some assumed model which may not reflect the real world: even if a configuration is synthesized based on some spec, it may behave differently and violate spec in practice
Further, (2) logic-based modelling introduces a disconnect between the synthesis tool and real-world behavior \cite{birkner2021metha}. More specifically, synthesized configurations may satisfy a provided specification within a formal framework, but may not behave the same way in the real world.
% can be very slow
And, (3) SMT-based synthesis can be very slow or fail to complete, especially when reasoning about large network topologies. In practice however, network operators reconfigure their networks on a daily basis \cite{vissicchio2012improving}, which means an effective synthesis tool must be fast.

% \item fully learned, no hand-coded synthesis rules (model-free), very flexible to adapt to more/new protocols
% \item protocol-agnostic, cross-protocol
\paragraph{Neural Algorithmic Reasoning for Synthesis} Recent work on neural algorithmic reasoning (NAR) proposes to replace traditional algorithms with neural networks to learn improved algorithmic procedures \cite{velivckovic2021neural}.
It has been shown to be a powerful and fast algorithmic approximation method for a number of graph-related \cite{velivckovic2019neural} and combinatorial optimization problems \cite{cappart2021combinatorial}. Further, due to its learned nature, NAR allows for learning procedures directly from (real-world) data, without the need for manual feature extraction. Overall, this positions NAR as an attractive method to obtain a fast, fully-learned synthesis procedure, which entirely avoids the need for a formal model or any hand-crafted synthesis rules. Based on this promising outlook, this paper explores how to apply the NAR paradigm to the problem of network configuration synthesis.

To that end, we propose a \textbf{new learning-based framework for configuration synthesis} as an alternative to SMT-based approaches. Our framework is protocol-agnostic, enables cross-protocol reasoning and avoids the need to manually provide synthesis rules. Instead of implementing the synthesizer explicitly, we replace it by an iterative graph neural network which is trained on input/output samples of specifications, topologies and configurations.
%While our approach still requires some protocol-specific implementation efforts, it is limited to implementing the simulation of the involved protocols.
Our method is highly flexible due to its generic nature and can be extended to any protocol. Further, the synthesizer model learns a whole distribution of network configurations. As a consequence, we can directly sample multiple alternative configurations, not possible with standard SMT solvers. We apply our framework to a non-trivial synthesis setting where both the Border Gateway Protocol (BGP) and the Open Shortest Path First (OSPF) protocol are used. We demonstrate that our learned synthesis tool is up to~$500\times$ faster than a state-of-the-art SMT-based synthesizer, while producing configurations which enjoy more than 90\% satisfaction of the given specification.

\paragraph{Main Contributions} Our core contributions are:
\vspace{-5pt}
\begin{itemize}
    \setlength{\itemsep}{5pt}
    \setlength{\parskip}{0pt}
    \item A learning-based framework for network configuration synthesis based on neural algorithmic reasoning.
    \item A neural network architecture for learning synthesizer models which relies on a generic graph-based encoding of network topologies and configurations.
    \item An extensive evaluation of our learning-based synthesizer, in terms of both precision and scalability, on the challenging setting where both BGP and OSPF protocols are involved.
\end{itemize}

\section{Overview}
\label{sec:overview}

\begin{figure}
    \begin{center}
        \includegraphics[width=0.45\textwidth]{figures/synthesizer-overview.pdf}
    \end{center}
    \caption{An overview of our learning-based synthesis framework.}
    \label{fig:learning-based-synthesis}
\end{figure}

We first discuss the core concepts behind our learning-based synthesis framework, illustrated in \cref{fig:learning-based-synthesis}.

\paragraph{Dataset} To train a synthesizer model, we first generate a dataset of input/output samples. For this, we rely on a generative pipeline as shown in the top of \cref{fig:learning-based-synthesis}. First, we sample a random network configuration for some topology using a uniform generative process. Then, we simulate the involved protocols to obtain the corresponding routing behavior. Next, we extract a specification by randomly selecting properties that hold for the simulated routing behavior. This leaves us with a pair of (specification, configuration) added to a dataset of training~samples.

\paragraph{Simulation} Depending on the protocols in use, one implements simulation code to compute the routing behavior induced by a sampled configuration. Although this step is protocol-specific, the overall implementation effort is much lower compared to SMT-based synthesis. Protocols are typically well-defined algorithms which can be simulated, whereas the alternative of implementing a synthesizer often requires expert knowledge about SMT solvers. In practice, our framework may also be adapted to use a real-world network router to compute the behavior of a configuration, thereby capturing the real-world behavior directly.

\paragraph{Neural Synthesizer Model} Given a dataset of pairs each consisting of a configuration and a specification, we now train a graph neural network on this dataset to perform synthesis: given a specification, it tries to predict the configuration. Following the NAR paradigm, we first encode the synthesizer input (specification) in latent space. Then, we apply an iterative processor network which relies on the graph attention mechanism to propagate information \cite{velivckovic2017graph}. Last, we apply a decoder network to extract the synthesized configuration. To remain protocol-agnostic, our model is generic with respect to the input format, using an intermediate representation based on Datalog-like facts.

%More specifically, we employ a slightly modified variant which operates on a graph-based encoding of a specification, topology and configuration parameters.



 \begin{figure*}
     \centering
     \includegraphics[width=0.85\textwidth]{figures/system-overview.pdf}
     \caption{An overview of our synthesis system: (1) First, we use a generic embedding scheme to transform a network topology, protocol configuration sketches and the specification given as Datalog-like facts to a latent input representation. Next, we apply a learned (2) Processor GNN and obtain a latent synthesis output. Last, we apply a (3) Decoder Network to obtain a distribution over possible values per unknown parameter in our configuration.}
     \label{fig:overview-model}
\end{figure*}

\paragraph{Relaxed Specification Consistency} Parts of the configuration synthesis problems are known to be NP-hard \cite{fortz2000internet}. In contrast, our learning-based framework depends on a fixed-size neural network architecture running in polynomial time. Hence, we expect neural synthesis to be less precise than SMT methods and propose the notion of \emph{relaxed~specification~consistency}. That is, to assess the performance of a neural synthesizer, we not only consider if a configuration satisfies a specification, but also the degree up to which it satisfies a specification (e.g., via the relative number of satisfied requirements). This ``soft'' understanding of a specification allows us to evaluate neural synthesis systems which may not always produce fully specification-consistent configurations. Nonetheless, we argue that configurations with less than $100\%$ consistency are still very useful in practice as they provide a good starting point for further manual adjustment by network operators. Note that a similar adjustment process may also be required with SMT-based synthesizers, due to differences between the formal protocol model and the one running on a given real-world router where the configuration is to be deployed.

Next, we discuss the architecture of our neural synthesis framework. In follow-up sections, we instantiate this framework for the case of BGP/OSPF configuration synthesis, and evaluate the resulting instantiation by comparing it to a state-of-the-art SMT-based synthesizer.

% \begin{itemize}
%     \item effort: need to implement simulation code to generate dataset to learn from (typically well-defined in protocol specs, much easier than implementing synthesis directly)
%     \item can be sampled (multiple alternative solutions, not easily possible with SMT-based methods)
%     \item much faster than SMT-based synthesis
% \end{itemize}

% Requirements:
% \begin{itemize}
%     \item protocol-agnostic
%     \item fully learned, no hand-coded synthesis rules
%     \item define: strict specification vs. relaxed specification
% \end{itemize} 

==> diff/git-latexdiff.34367/old/sections/2_model.tex <==
\section{Neural Synthesis Framework}
\label{sec:model}


We now present the architecture of our graph-based neural synthesizer model, illustrated in \cref{fig:overview-model}. First, in \cref{sec:graph-embedding} we introduce our generic graph-based encoding, which allows us to embed network topologies, protocol configuration and the specification into a latent space. Then, in \cref{sec:graph-transformer} we present the architecture of the processor network which we train to perform the synthesis task. Finally, in \cref{sec:decoding-sampling} we discuss how to sample network configurations from the resulting latent synthesis output.

\begin{figure}
    \begin{minipage}[t]{0.21\textwidth}
    \begin{lstlisting}[basicstyle=\ttfamily\small, escapeinside={(*}{*)}]
router(A)
router(B)
(...)

connected(A,B,2)
connected(A,C,?)(*\blackcircled{1}*)
(...)
    \end{lstlisting}
\end{minipage}
\begin{minipage}[t]{0.21\textwidth}
    \begin{lstlisting}[basicstyle=\ttfamily\small, escapeinside={(*}{*)}]
network(N1)
bgp_route(E,N1,2,3,1,0,1)

fwd(A,B,N1)
not fwd(B,A,N1)
(...)
    \end{lstlisting}
\end{minipage}
    \caption{A snippet of a fact base sketch encoding a network's topology, parameters such as link weights (\texttt{connected} facts) and a specification (\texttt{fwd} facts).}
    \label{fig:datalog-encoding}
\end{figure}

\begin{figure}[t]
    \centering
    \includegraphics[width=0.25\textwidth]{figures/synth-architecture.png}
    \caption{The neural synthesizer model architecture.}
    \label{fig:architecture}
\end{figure}

\subsection{Fact Base Embedding}
\label{sec:graph-embedding}
To remain network protocol-agnostic in our model architecture, we implement a generic graph-based encoding of Datalog-like facts, similar to knowledge graphs \cite{rosso2020beyond}. This means that we first encode topologies, configurations and specifications as a set of Datalog-like facts and then employ a generic embedding.
%We chose Datalog facts as the input format of our synthesis approach for its flexibility, wide-spread use in Program Analysis and use in previous work on configuration synthesis \cite{el2017network}.

\paragraph{Fact Base} A set of Datalog-like facts, as depicted in \cref{fig:datalog-encoding}, serves as the input \emph{fact base} $\mathcal{F}$ to our synthesizer model. $\mathcal{F}$ is a set of facts $f(a_0, \dots, a_n)$ where arguments may be constants (e.g. A or B) or integer literals. Further, each fact in a fact base has a corresponding truth value denoted as $[f(a)]_{\mathcal{B}}$. For instance, from the fact base in \cref{fig:datalog-encoding} we can derive $[fwd(A,B,N1)]_{\mathcal{B}} = \text{\texttt{true}}$ and $[fwd(B,A,N1)]_{\mathcal{B}} = \text{\texttt{false}}$.

\paragraph{Consistency} We represent a network's topology, the protocol configuration and parameters as well as the specification, all in a single fact base. Given the semantics of the protocols in use, we can then check whether the specification encoded in a fact base is satisfied by the provided configuration. To quantify, we define the notion of relaxed specification consistency, as discussed earlier, with respect to a fact base: Given a fact base $\mathcal{F}$, a subset of specification facts $S \subset \mathcal{F}$ and protocol semantics $\mathcal{P}$, the \emph{consistency} of a fact base is defined as the relative number of satisfied facts in $S$ with respect to the routing behavior obtained via $\mathcal{P}$. The contents of $S$ depend on the concrete instantiation of the synthesizer model. For an example of possible specification facts, see our instantiation of the synthesizer model for BGP/OSPF in \cref{sec:training}.

\begin{figure*}
    \def\arraystretch{1.5}
    \begin{tabular}{lr}
        %$T_f: T_1 \times \dots \times T_n$ & \textit{(fact type declaration)}\\
        $emb(f) := \mathbf{V_f}$ & \textit{(learned fact type embedding)}\\
        $emb(b) := \mathbf{W_{\text{bool}}}\;onehot(b)$ & \textit{(learned boolean embedding)}\\
        $emb(f,i,v) := \mathbf{W_{f_i}}\;onehot(v)$ & \textit{(learned integer embedding)}\\
        $emb(f,i,?) := \mathbf{V_{hole}}$ & \textit{(learned hole embedding)}\vspace{10pt}\\
        $\mathlarger{
        h_c := \sum_{f(c) \in \mathcal{F}}
        emb(f)
        }$ & \textit{(constant embedding)}\vspace{10pt}\\
        $h_{f(a_0, \dots, a_n)} := emb(f) + emb([f(a_0, \dots, a_n)]_{\mathcal{B}}) + \mathlarger{
        \sum_{(i,v) \in \mathcal{I}(f(a_0, \dots, a_n))}
        emb(f, i, v)
        }$\hspace{-1.2cm} & \textit{(fact embedding)}\\
        $\mathcal{I}(f(a_0, \dots, a_n)) := \{(i,v) \; | \; f(a_0, \dots, a_{i-1}, v, \dots, a_n) \in \mathcal{F} \wedge v:Int \wedge i \in \mathbb{N}$ \}& \textit{(integer arguments)}\vspace{10pt}\\
        $N_i(h_c) := \{h_f \; | \; \exists i \in \mathbb{N} . f(a_0, \dots, a_{i-1}, c, a_{i+1}, \dots, a_n) \in \mathcal{F}\}$& \textit{(i-th neighborhood of constant node)} \\
        $N_i(h_f) := \{h_c \; | \; \exists i \in \mathbb{N} . f(a_0, \dots, a_{i-1}, c, a_{i+1}, \dots, a_n) \in \mathcal{F}\}$& \textit{(i-th neighborhood of fact node)} \\
    \end{tabular}
    \caption{Translating a fact base $\mathcal{F}$ to node features. $f$ denotes a predicate, $v$ integer values, $b$ boolean values as 0 or 1, $i$ argument indices and $[f(a)]_{\mathcal{B}}$ the truth value of a fact. }
    \label{fig:graph-embedding}
\end{figure*}

%discuss embedding as shown in \cref{fig:datalog-encoding}. Note how this makes fact bases a suitable input to standard GNN architectures.

\paragraph{Fact Base Sketching} In a synthesis setting, we are confronted with incomplete fact bases, i.e. the specification and topology is given but the network configuration is to be synthesized. For these cases, we also consider fact bases with unknown parameters inspired by the idea of program sketching in program synthesis \cite{solar2008program}. More specifically, users may replace an unknown integer argument of a fact by a \texttt{?} symbol, indicating a value to be synthesized. Using this mechanic, we can represent the synthesis input as an incomplete fact base which encodes to-be-synthesized values as unknown parameters. As an example, consider \cref{fig:datalog-encoding} \blackcircled{1}, where the link weight between router nodes \texttt{A} and \texttt{C} is represented as an unknown parameter.

\paragraph{Embedding} We employ a structurally-defined embedding scheme to transform a fact base into a graph with node features as required for processing with graph neural networks. Given a fact base $\mathcal{F}$, we apply the rules in \cref{fig:graph-embedding} to obtain node features and adjacency information. Both a fact $f$ and a constant $c$ are represented as distinct nodes with features $h_c$ and $h_f$, respectively. The relationships between facts and constants is encoded as node adjacency as defined by the neighborhood functions $N_i$.

We use multiple neighborhood functions, i.e. multiple types of edges, to encode the argument position of a constant occurring in a fact. Hence, the number of neighborhood functions corresponds to the maximum number of arguments in a single fact, e.g. 3 in \cref{fig:datalog-encoding}. Integer arguments and unary facts are directly accounted for in the respective node or fact embedding. To handle unknown parameters, we replace the corresponding $emb(...)$ term with the learned $\mathbf{V_{hole}}$ embedding.

Considering the embedding function $emb$, the learned parameters of our embedding are $\mathbf{V_f} \in \mathbb{R}^D$ per fact type in~$\mathcal{F}$, $\mathbf{W_{\text{bool}}} \in \mathbb{R}^{D \times 2}$ for boolean values, $\mathbf{W_{f_i}} \in \mathbb{R}^{D \times N}$ per integer argument of fact type $f$ and $\mathbf{V_{hole}} \in \mathbb{R}^D$ to represent unknown parameters. Hyperparameter $D$ represents the dimension of the latent space the synthesizer model operates in and $N$ specifies the number of supported integer values. An example of applying this embedding scheme to a simple fact base is given in \cref{fig:graph-encoding-example}.

\begin{figure}
    \begin{minipage}[t]{0.2\textwidth}
        \centering
        \footnotesize
        \textbf{Fact Base}
        \begin{lstlisting}[basicstyle=\ttfamily\small]
router(A)
router(B)

conn(A, B, 12)
        \end{lstlisting}
    \end{minipage}
    \begin{minipage}[t]{0.15\textwidth}
        \centering
        \textbf{Graph}\\
        \vspace{5pt}
        \includegraphics[width=0.7\textwidth]{figures/graph-encoding.pdf}
    \end{minipage}\\
    \centering\\
    \vspace{10pt}
    \textbf{Node Features}\\
    \vspace{10pt}
    \begin{minipage}[t]{0.5\textwidth}
        $\begin{array}{rcl}
        h_A &:=& emb(router) = \mathbf{V_{\text{router}}}\\
        h_B &:=& emb(router) = \mathbf{V_{\text{router}}}\\
        h_{\text{conn(A,B,12)}} &:=& emb(conn) + emb(conn, 2, 12)\\
        &:=& \mathbf{V_{\text{conn}}} + \mathbf{W_{conn_2}} onehot(12)
    \end{array}$
    \end{minipage}
    \caption{An example of embedding a simple fact base using the embedding scheme of \cref{fig:graph-embedding}. The shown graph illustrates the neighborhoods $N_0$ and $N_1$ induced by the \texttt{conn} fact.}
    \label{fig:graph-encoding-example}
\end{figure}

\begin{figure}
    $$
    \begin{array}{rcl}
    z_j &:=& h_j + Drop(\mathlarger{\sum_{N_i}} h'_{GAT_i})\\
    h'_j &:=& FFN(Norm(z_j))\vspace{11pt}\\
    FFN(x_j) &:=& Norm(Lin2(Drop(Lin1(x_j)))))
    \end{array}
    $$
    \caption{
        The recurrence relation of a node $j$'s representation $h_j$. $h'_{GAT_i}$ represents the output of a graph attention layer operating with neighborhood $N_i$ according to \cite{velivckovic2017graph}, $h_j$ the representation of node $j$ at the previous step. $Norm$ refers to batch normalization \cite{ioffe2015batch}, $Drop$ to dropout regularization \cite{hinton2012improving} and $Lin1$ and $Lin2$ to linear layers with an inner dimension of $4N$.
    }
    \label{fig:recurrence}
\end{figure}

\subsection{Synthesizer Model}
\label{sec:graph-transformer}

For an illustration of the synthesizer model's architecture, please see Figure~\ref{fig:architecture}. Given a fact base $\mathcal{F}$ we first apply our embedding scheme as described in \cref{sec:graph-embedding}. We then employ a 2-layer GNN-based encoder network to produce the latent representation of a synthesis input.
Given this representation, a processors network is trained to perform the actual synthesis task in high-dimensional space. Last, we apply a set of decoder networks, to obtain the synthesized values of unknown parameter, given the latent synthesis~output.

%In this context, the synthesis problem for network configurations corresponds to completing partially provided fact bases.

% \paragraph{High-Level Architecture}

% We employ the high-level architecture to obtain the latent synthesis output $y_\mathcal{F}$:
% $$
% \begin{array}{rcl}
%     \mathbf{x_{\mathcal{F}}} &:=& Encoder(Embedding(\mathcal{F}))\\
%     \mathbf{y_{\mathcal{F}}} &:=& Processor(\mathbf{x_{\mathcal{F}}} + \mathbf{z})\\
%     z_i &\sim& \mathcal{N}(0,1)
% \end{array}
% $$
% \todo{z is only added for $i<N/2$}

% $Embedding$ corresponds to the graph-based embedding as discussed in \cref{sec:graph-embedding} and $Encoder$ is a 2-layer graph attention module. $Processor$

\paragraph{Encoding} The encoder GNN operates on the embedded representation of a fact base. It produces the high-dimensional representation of a synthesis input as required for the processor network. We additionally apply noise to the first half of the units of the latent representation via $\mathbf{z}$, as a source of non-determinism. According to our experiments this improves model performance and we hypothesize this is due to the synthesis problem having more than one solution in most cases.

\paragraph{Iterative Processor} The processor network is modelled as an iterative process. For this, we apply the same 6-layer graph attention module for a total of 4 iterations.
In the framework of neural algorithmic reasoning, this iterative computational structure encodes an inductive bias towards an iterative solution to the synthesis problem. Because of this bias, our processor network essentially learns an algorithmic procedure which iteratively synthesizes the values of unknown parameters in a fact base.

\paragraph{Graph Attention Layer} In the GNNs we employ, we rely on a composed variant of the graph attention layer as introduced by \cite{velivckovic2017graph}. We employ multiple graph attention layers in lockstep, one per neighborhood $N_i$ defined by our graph embedding (cf. \cref{sec:graph-embedding}), and combine the intermediate results after each step. Specifically, the recurrence relation of a node $j$'s representation $h_j$ is defined as shown in \cref{fig:recurrence}. These mechanics of combining the results of the different graph attention layers $h'_{GAT_i}$, directly corresponds to how multiple attention heads are combined in the original Transformer architecture \cite{vaswani2017attention}.

\paragraph{Argument Decoder Networks} To synthesize the values of unknown parameters, the model maintains a set of decoder networks. That is, it provides one decoder network per integer argument per fact type in a fact base. When decoding, the network is applied to the latent synthesis output of the corresponding fact node. For example, a synthesizer model which operates on the fact base in \cref{fig:graph-encoding-example}, would provide a decoder network $D_{\text{conn}_2}: \mathbb{R}^D \rightarrow \mathbb{R^N}$ to decode values for the third argument of a \texttt{conn} fact. In our experiments, decoder networks are implemented as simple multi-layer perceptron models.

%The synthesizer model learns a conditional distribution of fact bases which are consistent with respect to the protocols' semantics.

%\todo{introduce synthesis as a completion problem of an encoded fact base (a la BERT). Introduce masking, introduce decoding of integer and truth values. Synthesis is learning a conditional distribution of consistent fact bases.}

%Using this method, we obtain the node features $h_c$ per constant, $h_f$ per fact and adjacency information in terms of node neighborhood functions $N_i(h_c)$ and $N_i(h_f)$. Overall, this encoding makes a fact base suitable for processing using standard graph neural networks.

%- Brief description of the Graph Transformer Model
\subsection{Multi-Shot Sampling}
\label{sec:decoding-sampling}

%Multi-Stage Parameter Sampling (sampling methods: topk, high-temp, low-temp)
To sample concrete values from the output distributions over unknown parameters, we apply a multi-shot sampling strategy. That is, we sample values only for a subset of unknown parameters, insert them in our input fact base and run the synthesis model again. We repeat this process until no more unknown parameters remain. This multi-shot sampling strategy allows the model to incorporate the concrete values of previously synthesized parameters in its computation. In our evaluation in \cref{sec:evaluation}, we include a comparison of how this compares to sampling all unknown parameters at once.

%In a fact base with multiple holes, we apply the corresponding decoder networks to obtain a value distribution for each integer hole. However, instead of sampling all integer holes in one


==> diff/git-latexdiff.34367/old/sections/3_bgp_ospf.tex <==
\section{BGP/OSPF Synthesis}
\label{sec:bgp-ospf}

\newcommand{\as}{\ac{AS}~}
\newcommand{\ases}{\acp{AS}~}

\newcommand{\squareann}{{\tiny$\blacksquare\;$}}
\newcommand{\triangleann}{{\small$\blacktriangle\;$}}

\begin{figure*}
    \centering
    \includegraphics[width=0.95\textwidth]{figures/networks-all.pdf}
    \caption{(a) An illustration of a small AS network, including internal peers (blue), external peers (purple), BGP sessions as well as physical links. (b) The propagation of two BGP announcement across the network. (c) The resulting forwarding plane after applying BGP and OSPF.}
    \label{fig:network-fwd-tree}
\end{figure*}

We now discuss an instantiation of our learning-based framework for the case of BGP and OSPF protocols. In \cref{sec:synthesis-setting} we introduce a basic networking model, BGP and OSPF protocols and the synthesis setting. Given this model, \cref{sec:training} describes how to generate a corresponding dataset of input/output samples and train a synthesizer model.
%This shall serve as a prerequisite to the instantiation of our learning-based synthesis framework for the BGP and OSPF protocol in \cref{sec:training}.

\subsection{Synthesis Setting}
\label{sec:synthesis-setting}

\paragraph{Graphical Model} We assume an abstract network model which can be represented as an undirected graph as shown in \cref{fig:network-fwd-tree} (a). We always consider a set of internal routers (A, B, C, D in \cref{fig:network-fwd-tree}) as well as a set of adjacent external routers (E, F  in \cref{fig:network-fwd-tree}). The group of internal routers forms the \emph{\as} under consideration whereas external routers belong to other adjacent \ases. In practice, an \as represents an administrative domain controlled by a single operator.

\paragraph{Forwarding Plane} We focus on the \emph{forwarding plane} of a network. This means we are interested in how a router forwards packets given incoming traffic of different traffic classes. For this, each router maintains a routing table which determines which of its outgoing edges is used to forward packets of a certain traffic class. As an example, consider \cref{fig:network-fwd-tree} (c) which illustrates the forwarding plane of some traffic class reachable via external peer $E$ or $F$ in our example network. Each router of the network forwards traffic along some of its outgoing links. In practice, a number of protocols are used to populate a router's routing tables. For the instantiation of our synthesis framework however, we focus on OSPF and BGP.

\paragraph{OSPF} The OSPF protocol \cite{moy1994ospf} is a link-state protocol, typically used as an interior gateway protocol~(IGP), i.e., to route traffic within an \ac{AS}. Given link weights per physical link in the network, OSPF simply routes traffic along the shortest path towards the destination.

\paragraph{BGP} The BGP protocol \cite{rekhter1994border} on the other hand is a path-vector protocol used to exchange reachability information mostly on the level of \acp{AS}.
%These are groups of routers typically operated by a single party (e.g. an ISP).
When using BGP, a routing destination announces its existence to other \ases and routers, by sending out a BGP announcement. Receivers of such announcements may then choose to pass them on to other \acp{AS}, redistribute them internally and/or modify them. Instead of communicating along physical links directly, the BGP protocol requires manually configured BGP sessions among routers of the \as and external peers, as indicated by the BGP session edges in \cref{fig:network-fwd-tree}(a).
%\todo{more discussion of eBGP vs iBGP and support for route reflection (more of an implementation detail, maybe only mention in dataset generation where simulation code is discussed)}.

%\paragraph{BGP Decision Procedure}~
%\todo{discuss decision procedure}
In case a router receives more than one announcement for a destination, a designated BGP decision process is applied to determine a single best route. \cref{fig:bgp-decision} shows the ordered list of comparison criteria of this decision process. The different criteria depend different properties of a route announcements, including the IGP cost towards the routing destination. As a consequence, when used together, OSPF as IGP protocol and BGP will interact. %Note also that BGP is an iterative process which needs multiple rounds of propagation to converge.

\paragraph{Example}
%\todo{run through simple BGP+OSPF example of computing the forwarding plane}
To better understand BGP/OSPF routing, consider the simple example given in \cref{fig:network-fwd-tree} (b). Here, our example \as imports BGP announcements \squareann and \triangleann from E and F respectively. Both represent a route to the same destination. As shown, both announcements have a so-called local preference of 2. For simplicity, we ignore other properties such as the AS path length, Origin and MED in this example. The announcements are propagated among BGP neighbors and the best route is selected according to the decision procedure in \cref{fig:bgp-decision}. See \cref{fig:network-fwd-tree} (b) for an illustration of the intermediate states of this propagation process. As both announcements have a local preference of 2, rule 1 of the decision process is not used. Instead, in round 2, node B selects \squareann over \triangleann due to a lower IGP cost of 2 via egress node A as compared to 3 via egress node D (rule 6). Node D selects \triangleann over \squareann, since it learns this route directly from an external peer (rule 5). After Round 3, the BGP propagation process converges to a stable state and we can derive the forwarding plane as shown in \cref{fig:network-fwd-tree} (c).


%, as well as external peers E and F which belong to other \acp{AS}. External peers are routers which are connected via eBGP sessions to routers of the \ac{AS} under consideration. They announce BGP routes to their neighbors, which are propagated within the network

\paragraph{Problem Statement: Configuration Synthesis} We phrase the BGP/OSPF configuration synthesis problem on the level of the forwarding plane. This means that users provide a specification which constraints the set of allowed forwarding planes. This includes predicates which enforce forwarding paths, block forwarding paths or assert higher-level properties like traffic isolation and reachability. Given such a specification, we consider network configuration synthesis as the task of configuring OSPF and BGP in a way that produces a forwarding plane which satisfies the provided specification.

\paragraph{Search Space} To limit the space of candidate configurations, we define the set of synthesized parameters: For OSPF we synthesize link weights as explored in a wide range of existing work (e.g. \cite{el2018netcomplete,fortz2000internet}. BGP parameters on the other hand are not defined as clearly: Depending on the requirements of a network operator, one may employ custom BGP import and export policies at every router of a network to implement complex behavior. However, in this work we focus on a simplified setting, where we assume BGP route announcements to only be modified when imported into the \as from an external peer. Previous work has already pointed out that this is a reasonable assumption which holds for the majority of real-world networks \cite{caesar2005bgp,cittadini2010doing, steffen2020probabilistic}.

\begin{figure}
    \small{
    \begin{enumerate}
        \setlength{\itemsep}{0pt}
        \setlength{\parskip}{0pt}
        \item Highest Local preference
        \item Lowest AS path length
        \item Prefer Origin (IGP $>$ EBGP $>$ INCOMPLETE)
        \item Lowest Multi-exit discriminator (MED)
        \item External over internal announcements
        \item Lowest IGP cost to egress
        \item Lowest BGP peer id (tie breaker)
    \end{enumerate}}
    \vspace{-15pt}
    \caption{The BGP decision process \cite{rekhter1994border}. The shown rules are applied in order until a single best BGP announcements remains.}
    \label{fig:bgp-decision}
\end{figure}

\subsection{Dataset Generation and Training}
\label{sec:training}
To train a synthesizer model, we need a large number of fact bases encoding a variety of network topologies, configurations and forwarding specifications. Further, we must provide the model with target values for unknown parameters as a supervision signal. This section discusses how we construct such a dataset for BGP/OSPF synthesis.
%Further, we provide an example of what a corresponding fact base looks like, including a description of the supported specification language.

\paragraph{Dataset Generation} To obtain network configurations and corresponding forwarding specifications we employ a generative process: We first randomly configure BGP and OSPF parameters for some topology. Then we simulate the OSPF and BGP protocol and compute the resulting forwarding plane. Based on this, we extract a forwarding specification which fixes a random subset of forwarding paths, reachability and isolation properties that are satisfied by the forwarding plane.

\paragraph{Topologies} For training, our dataset is based on random topologies with $16$-$24$ routers. We generate the physical layout of these graphs by triangulation of uniformly sampled points in two-dimensional space.

\paragraph{Simulation} To compute the forwarding plane given an OSPF and BGP configuration, we simulate the protocols. For OSPF, we implement shortest path computation to obtain the forwarding plane. For BGP, we implement the full BGP decision process as shown in \cref{fig:bgp-decision}, except for the MED attribute. In addition to the basic networking model discussed in \cref{sec:synthesis-setting}, we implement support for eBGP and iBGP, fully-meshed BGP session layouts as well as layouts relying on route reflection. For more details of these BGP concepts see \cite{bates2000rr}.

%Note that the synthesizer model will reason on the level of the provided training samples. That is, to improve the overall synthesis quality in a real-world setting, it is helpful to implement simulation code which behaves very similar to real-world networks. Another promising approach would be to extract training samples from real-world networks, thereby circumventing the need for simulation, however, we leave this as future work.

%While this can be a considerable effort, it is typically an easier task than to implement the synthesizer directly. The concrete semantics of protocols and their simulation is a well-defined procedure, whereas implementing efficient synthesis tools is still an open problem.

\paragraph{Fact Base Encoding} We encode synthesis input using a small set of facts. For an example of a corresponding fact base see \cref{fig:bgp-ospf-fact-base}. We use the \texttt{router}, \texttt{external} and \texttt{network} facts to mark routers, external peers and routing destinations respectively. Physical links between routers are encoded as \texttt{connected(R1,R2,W)} facts where \texttt{W} denotes the OSPF link weight. Further, we rely on \texttt{ibgp}, \texttt{ebgp}, \texttt{route\_reflector} and \texttt{bgp\_route} facts to represent different types of BGP sessions and imported routes. Using the notion of unknown parameters as discussed in \cref{sec:graph-embedding}, we encode configuration parameters, e.g., properties of imported routes or OSPF link weights.

\paragraph{Specification Language} We support a small specification language with three types of forwarding predicates:

\begin{itemize}
    \setlength{\itemsep}{0pt}
    \setlength{\parskip}{2pt}
    \item \texttt{fwd(R1, Net, R2)} specifies that router \texttt{R1} forwards traffic destined for \texttt{Net} to its neighbor \texttt{R2}.
    \item \texttt{reachable(R1, Net, R2)} specifies that traffic destined for \texttt{Net} that passes through \texttt{R1} also passes through \texttt{R2} before reaching its destination.
    \item \texttt{trafficIsolation(R1, R2, N1, N2)} specifies that it must not hold that $[fwd(R1,R2,N1)]_{\mathcal{B}} \wedge [fwd(R1,R2,N2)]_{\mathcal{B}}$.
\end{itemize}

In the negative case of each predicate, the opposite must hold true for the fact to be satisfied. This specification language can easily be extended by including new specification predicates in the dataset generation process. One must simply provide a method of extracting positive and negative cases of a specification fact from a given forwarding plane. Once included in the training dataset of a synthesizer model, the resulting synthesis system will be able to consider specifications relying on the new type of predicates.

% \todo{info on loss function, optimizer, etc.}
\paragraph{Training} We generate a dataset of $10,240$ input/output samples and instantiate our synthesizer model with a hidden dimension $D$ of $64$. For optimization, we use the Adam optimizer \cite{kingma2014adam} with a learning rate of $10^{-4}$, applying negative log-likelihood loss to the decoder networks' outputs. We stop training after the specification consistency on a validation dataset no longer increases at around $\sim2800$ epochs.

\begin{figure}
\begin{minipage}[t]{0.22\textwidth}
\begin{lstlisting}[basicstyle=\ttfamily\tiny]
# topology and configuration
router(c5)
router(c3)
router(c1)
router(c0)
network(c6)
network(c7)

external(c8)
external(c9)
external(c10)
external(c11)
external(c12)
external(c13)

route_reflector(c2)
route_reflector(c4)

connected(c2,c4,?)
connected(c2,c5,?)
connected(c2,c3,?)
connected(c4,c5,?)
connected(c4,c3,?)
connected(c4,c0,?)
connected(c5,c1,?)
connected(c5,c0,?)
connected(c3,c0,?)
connected(c3,c1,?)
connected(c1,c0,?)

ibgp(c2,c4)
ibgp(c2,c5)
ibgp(c2,c0)
ibgp(c2,c1)
ibgp(c4,c3)
ibgp(c4,c4)
\end{lstlisting}
\end{minipage}
\begin{minipage}[t]{0.2\textwidth}
\begin{lstlisting}[basicstyle=\ttfamily\tiny]
ebgp(c2,c12)
ebgp(c5,c9)
ebgp(c5,c10)
ebgp(c5,c13)
ebgp(c0,c8)
ebgp(c0,c11)

bgp_route(c8,c6,?,?,1,?,1,8)
bgp_route(c9,c6,?,?,0,?,1,9)
bgp_route(c10,c6,?,?,0,?,1,10)
bgp_route(c11,c7,?,?,0,?,1,11)
bgp_route(c12,c7,?,?,0,?,1,12)
bgp_route(c13,c7,?,?,2,?,1,13)

# forwarding specification
fwd(c0,c6,c3)
fwd(c3,c6,c2)
fwd(c2,c6,c4)
not fwd(c3,c6,c0)
not fwd(c0,c6,c11)
not fwd(c11,c6,c0)

not trafficIsolation(c1,c0,c7,c6)
not trafficIsolation(c1,c0,c7,c6)
trafficIsolation(c0,c3,c6,c7)
trafficIsolation(c0,c3,c6,c7)

reachable(c5,c6,c10)
reachable(c1,c6,c4)
not reachable(c0,c6,c5)
reachable(c5,c6,c10)
\end{lstlisting}
\end{minipage}
\caption{An example of a fact base encoding a topology, a sketch of a BGP and OSPF configuration and a forwarding specification.}
\label{fig:bgp-ospf-fact-base}
\end{figure} 

==> diff/git-latexdiff.34367/old/sections/4_evaluation.tex <==
\section{Evaluation}
\label{sec:evaluation}

We trained a synthesizer model to perform configuration synthesis for BGP and OSPF. We now assess the performance of the resulting neural synthesizer with respect to two core metrics: (1) the quality of synthesized configurations in terms of their consistency with the provided forwarding specifications (\cref{sec:synthesis-quality}), and (ii) the time a learned synthesizer takes when compared to the state-of-the-art SMT-based synthesizer NetComplete \cite{el2018netcomplete} (\cref{sec:synthesis-vs-smt}).

\paragraph{Dataset} We compare across three datasets: Small, Medium and Large. Each dataset represents 8 real-world topologies, sampled from the Topology Zoo \cite{knight2011internet}, where the number of nodes lies between 0-34, 34-68 and 68-170 respectively. To obtain forwarding specifications for the sampled topologies, we use our generative pipeline as discussed in \cref{sec:training}. In each topology, we do synthesis for 4 different traffic classes (routing destinations) at a time.

\paragraph{Experimental Setup} We run all our experiments on an Ubuntu Linux machine with an Intel(R)~Core(TM)~i9-9900X~@~3.50GHz processor, 64GB of system memory and an NVIDIA GeForce RTX 3080 GPU with 10GB of video~memory.

\subsection{Synthesis Quality}
\label{sec:synthesis-quality}
To assess our learned synthesizer, we examine its behavior with increasingly large topologies and specifications.

\paragraph{Specifications} Using the same generative model as described in \cref{sec:training}, we generate forwarding specifications for the topologies in our three datasets with each specification constructed from $3 \times n$ requirements, one per supported predicate type:  \texttt{fwd} requirements correspond to specifying or blocking a forwarding path using multiple \texttt{fwd} predicates whereas \texttt{reachable} and \texttt{trafficIsolation} requirements each translate to a single specification fact. We compare across increasingly large specifications of $3\times 2$, $3\times 8$ and $3 \times 16$ requirements, respectively.

\paragraph{Methodology} For each pair of topology and specification, we run our synthesizer 5 times and report the network configurations with the highest overall consistency value. For sampling, we rely on our multi-shot sampling strategy where we randomly group the unknown parameters of a configuration into 4 groups (4-shot sampling).

\paragraph{Results} We summarize our results in \cref{fig:eval-consistency}. On average, our synthesis model produces network configurations that are $>91\%$ consistent with the provided forwarding specifications across all datasets and sizes of specifications. When only few requirements are given, the synthesizer model even succeeds in producing fully-consistent configurations. We observe a slightly decreasing consistency with increasingly large topologies.

%\texttt{fwd} facts are satisfied more easily, whereas \texttt{reachable} and \texttt{trafficIsolation} facts are violated more often.

\paragraph{Multi-Shot Sampling} In \cref{fig:eval-consistency-baseline}, we report the average specification consistency using our multi-shot sampling strategy as compared to sampling all unknown parameters at once. As a baseline we have also sampled random configurations from a uniform distribution (per parameter) and compute the corresponding specification consistency. Over the baseline, our synthesizer model shows clear improvement and multi-shot sampling further increases consistency.

\begin{figure*}
    \begin{center}
        \textbf{Specification Consistency}\\
        \footnotesize
        \begin{tabular}{rrcccccccccc}
        \toprule
        \multicolumn{2}{c}{Dataset} & \tiny\texttt{fwd} & \tiny\texttt{reachable}  & \tiny\texttt{trafficIsolation} & Overall & $\emptyset$     No. Full Matches & $\emptyset$ No. $>90\%$ Matches\\
        \midrule
        $3\times 2$ requirements & Small & 0.95 & 0.94 & 1.00 & \textbf{0.95} & 0.62 & 0.62\\
& Medium & 0.96 & 1.00 & 0.94 & \textbf{0.96} & 0.88 & 0.88\\
& Large & 0.94 & 0.94 & 1.00 & \textbf{0.93} & 0.62 & 0.62\\
\midrule
$3\times 8$ requirements & Small & 0.97 & 0.98 & 0.97 & \textbf{0.98} & 0.50 & 1.00\\
& Medium & 0.99 & 0.95 & 1.00 & \textbf{0.98} & 0.50 & 1.00\\
& Large & 0.96 & 0.95 & 0.91 & \textbf{0.94} & 0.38 & 0.88\\
\midrule
$3\times 16$ requirements & Small & 0.97 & 0.89 & 0.95 & \textbf{0.94} & 0.38 & 0.75\\
& Medium & 0.98 & 0.97 & 0.97 & \textbf{0.98} & 0.38 & 1.00\\
& Large & 0.92 & 0.88 & 0.95 & \textbf{0.91} & 0.12 & 0.50\\
    \end{tabular}\end{center}
    \caption{Average specification consistency of the network configurations synthesized by our trained synthesizer model. Per sample we run the synthesizer with a specification of $3\times N$ requirements, where the specifications always include $N$ requirements per supported predicate type (\texttt{fwd}, \texttt{reachable}, \texttt{trafficIsolation}).}
    \label{fig:eval-consistency}
\end{figure*}

\begin{figure}
    \begin{center}
        \footnotesize
        \begin{tabular}{rrcccccccccc}
        &  & \multicolumn{2}{c}{Neural}\\
        & Random & 1-Shot & 4-shot\\
        \toprule
        Small & 0.83 & 0.92 & \textbf{0.94} \\
        Medium & 0.88 & 0.95 & \textbf{0.98} \\
        Large & 0.78 & 0.88 & \textbf{0.91} \\
    \end{tabular}\end{center}
    \caption{Average specification consistency with $3\times 16$ requirements when sampling configurations randomly from a uniform distribution and 1-shot/4-shot sampling using our synthesizer model.}
    \label{fig:eval-consistency-baseline}
\end{figure}

\begin{figure*}[ht]
    \footnotesize
    \begin{center}
        \textbf{BGP Synthesis Time}
        \footnotesize
        \begin{tabular}{rrccccccccc}
        \toprule
        &&\multicolumn{3}{c}{Synthesis Time (s)} & \multicolumn{2}{c}{Accuracy (Neural)} \\
        \multicolumn{2}{l}{\# Requirements} & NetComplete & Neural (CPU) & Speedup &$\emptyset$ Consistency& $\emptyset$ No. Full Matches\\
        \midrule
    2 requirements &Small & 18.073s & 0.641s & \textbf{28.2x} & 0.969 & 0.875\\
        &Medium & 60.864s & 2.748s & \textbf{22.2x} & 0.939 & 0.75\\
        &Large & 1389.485s\tiny{  7/8 TO} & 22.301s & \textbf{62.3x} & 0.989 & 0.875\\
    \midrule
    8 requirements &Small & 247.691s & 1.065s & \textbf{232.5x} & 0.96 & 0.75\\
        &Medium & $>$25m\tiny{  8/8 TO} & 3.47s & \textbf{432.2x} & 0.968 & 0.5\\
        &Large & $>$25m\tiny{  8/8 TO} & 30.961s & \textbf{48.4x} & 0.969 & 0.75\\
    \midrule
    16 requirements &Small & 1416.828s\tiny{  7/8 TO} & 2.528s & \textbf{560.5x} & 0.926 & 0.25\\
        &Medium & $>$25m\tiny{  8/8 TO} & 5.481s & \textbf{273.7x} & 0.947 & 0.25\\
        &Large & $>$25m\tiny{  8/8 TO} & 69.092s & \textbf{21.7x} & 0.959 & 0.25\\
    \end{tabular}\end{center}
    \caption{Comparing consistency and synthesis time of our method (Neural) with the SMT-based state-of-art synthesis tool NetComplete. The notation {\tiny{n/8 TO}} indicates the number of timed out synthesis runs out of 8 (25+ minutes).}
    \label{fig:evaluation-compare-bgp}
\end{figure*}

\begin{figure*}[ht]
    \begin{center}
        \footnotesize
        \textbf{OSPF Synthesis Time}\\
        \footnotesize
        \begin{tabular}{rrccccccccc}
        \toprule
        &&\multicolumn{3}{c}{Synthesis Time (s)} & \multicolumn{2}{c}{Accuracy (Neural)} \\
        \multicolumn{2}{l}{} & NetComplete & Neural (GPU) & Speedup &$\emptyset$ Consistency& $\emptyset$ No. Full Matches\\
        \midrule
    2 requirements &Small & 0.265s & 0.091s & \textbf{2.9x} & 1.000 & 1.00\\
     &Medium & 0.404s & 0.098s & \textbf{4.1x} & 1.000 & 1.00\\
     &Large & 0.944s & 0.14s & \textbf{6.7x} & 1.000 & 1.00\\
    \midrule
    8 requirements &Small & 0.876s & 0.164s & \textbf{5.3x} & 0.982 & 0.75\\
     &Medium & 1.517s & 0.103s & \textbf{14.7x} & 1.000 & 1.00\\
     &Large & 3.505s & 0.316s & \textbf{11.1x} & 0.981 & 0.50\\
    \midrule
    16 requirements &Small & 1.65s & 0.21s & \textbf{7.9x} & 0.991 & 0.625\\
     &Medium & 2.646s & 0.245s & \textbf{10.8x} & 0.989 & 0.50\\
     &Large & $>$566.636s+\tiny{  3/8 TO} & 0.233s & \textbf{2430.4x} & 0.987 & 0.875\\
    \end{tabular}\end{center}
    \caption{Comparing consistency and synthesis time of our method (Neural) with the SMT-based OSPF synthesis tool NetComplete. The notation {\tiny{n/8 TO}} indicates the number of timed out synthesis runs out of 8 (25+ minutes).}
    \label{fig:evaluation-compare-ospf}
\end{figure*}


\subsection{Comparison to SMT-based Synthesis}
\label{sec:synthesis-vs-smt}

%To provide a comparison of our learned BGP/OSPF synthesizer with SMT-based methods,
We now compare the synthesis time of the learned neural synthesizer with those of NetComplte, a state-of-art configuration synthesis tool based on SMT-solvers \cite{el2018netcomplete}.

\paragraph{Specifications} As the type of supported requirements in NetComplete does not fully align with our model, we restrict this comparison to specifications which only include forwarding paths (i.e. \texttt{fwd} predicates). Further, NetComplete does not support cross-protocol synthesis as in our case and instead requires users to specify for each requirement the protocol to use for its implementation. To bridge this gap, we split the generated forwarding requirements into BGP and OSPF paths for a corresponding NetComplete specification.
%\todo{note on NetComplete installing policies at all routers, not only the edges of the AS}

\paragraph{Methodology} We compare both OSPF synthesis and BGP/OSPF-synthesis. We configure our trained synthesizer model to do OSPF synthesis by only predicting link weights. For each pair of topology and specification, we report the total time of running our synthesizer 4 times using 4-shot sampling, whereas for consistency we report the best out of the 4 runs. For NetComplete, we run the synthesizer with a timeout of 25 minutes. In case a NetComplete attempt times out, we report 25 minutes as a lower bound for its runtime.

\paragraph{OSPF Synthesis Time Results} We document the results of comparing OSPF synthesis time in \cref{fig:evaluation-compare-ospf}. Our synthesizer model achieves a speedup of 2-10x over NetComplete. With 16 requirements and dataset Large this speedup even increases to $2000\times$. Further, our model achieves very high consistency with the provided specification, often producing fully-consistent configurations.

\paragraph{BGP/OSPF Synthesis Time Results} In \cref{fig:evaluation-compare-bgp} we show the comparison of BGP/OSPF synthesis time. Our synthesizer model outperforms NetComplete by multiple orders of magnitude. We observe a speedup of $20-560\times$ which appears to increase with the size of topology and specification. Further, the average specification consistency of the synthesized configurations is greater than $92\%$ across all datasets, even for large topologies. In many cases, our synthesizer model produces fully-consistent configurations, especially with small topologies and specifications. In comparison, NetComplete times out on more than half of the synthesis tasks which means that we can only observe a lower bound of speedup in these cases. Note that our synthesizer model is running on a CPU due to memory restrictions with large topologies. However, running it on a GPU results in even greater speedups (up to $1000\times$, cf. \cref{app:sec:bgp-gpu-performance}). 

==> diff/git-latexdiff.34367/old/sections/5_related_work.tex <==
\section{Related Work}
\label{sec:related-work}

\paragraph{Traditional Configuration Synthesis} 
%A range of existing work is concerned with network configuration synthesis. 
Next to methods based on compilation such as Propane/PropaneAT \cite{beckett2017network}, there are a number of configuration synthesis methods based on constraint solving: Examples include ConfigAssure \cite{narain2008declarative}, SyNet \cite{el2017network} and NetComplete \cite{el2018netcomplete}. Due to their hand-coded nature, these methods are highly protocol-specific and can be very slow due to the solvers they employ. Although some of them allow for cross-protocol reasoning, this is not implemented as transparently as in our framework and users must specify per requirement which protocol to use for its implementation. In contrast, our approach has lower precision but allows for fully transparent cross-protocol reasoning, meaning forwarding requirements are not protocol-bound and the synthesizer chooses how to implement them. Further, our learned BGP/OSPF synthesis tool exhibits much lower synthesis times as compared to an SMT-based tool like NetComplete.

% \begin{itemize}
%     \item NetComplete, SyNet
%     \item Propane, PropaneAT
%     \item DeepBGP
% \end{itemize}

\paragraph{GNNs and Networking} DeepBGP \cite{bahnasy2020deepbgp} relies on GNNs and reinforcement learning to do configuration synthesis. However, it is limited to BGP configuration synthesis and is slower than SMT-based synthesis according to the author's evaluation. In contrast, our learning-based framework is cross-protocol, does not rely on reinforcement learning and provides better synthesis performance. Apart from configuration synthesis, GNNs have also been applied to other problems in the networking domain. For example, the authors of RouteNet \cite{rusek2020routenet} use GNNs to predict performance metrics of network configurations. Other work that is concerned with learning improved protocols includes Q-Routing \cite{boyan1994packet} or more modern approaches such as the Graph-Query Neural Network architecture \cite{geyer2018learning}.

\paragraph{Neural Algorithmic Reasoning} 
Neural algorithmic reasoning (NAR) as proposed in \cite{velivckovic2021neural}, describes the idea of replacing traditional algorithms with neural networks to learn improved algorithmic procedures. Exemplary work includes graph-related algorithms \cite{velivckovic2019neural} or solvers for combinatorial optimization problems \cite{cappart2021combinatorial,joshi2020learning,selsam2019guiding}. Our synthesis framework is the first applications of NAR to the networking domain and relies on the NAR-native encode-process-decode architecture. According to the hierarchy of NAR approaches in \cite{cappart2021combinatorial}, our method is an algorithm-level approach, as we do not supervise on intermediate steps. Although, such step-level methods promise better generalization, it is not clear what an intermediate result of a general synthesis procedure would be. However, future work on a step-level approach may further improve synthesis quality.

% \begin{itemize}
%     \item RouteNet
%     \item GraphNET
%     \item Learning and generating distributed routing protocols using graph-based deep learning
%     \item Unveiling the potential of Graph Neural Networks for network modeling and optimization in SDN
% \end{itemize}

==> diff/git-latexdiff.34367/old/sections/6_conclusion.tex <==
\setlength{\parskip}{6pt plus4mm minus4mm}
\section{Conclusion}
\label{sec:conclusion}
We presented a learning-based framework for configuration synthesis based on the idea of neural algorithmic reasoning. To assess the effectiveness of the system, we instantiated it for the case of BGP/OSPF synthesis. In contrast to traditional synthesis methods, our system supports transparent cross-protocol reasoning and learns synthesis rules only from data. Using our system, synthesis is sped up by a factor of up to $500\times$ when compared to SMT-based methods. Further, our evaluation demonstrates that the resulting synthesis tool provides excellent synthesis quality, producing configurations with high specification consistency. Overall, our results illustrate that exploring the direction of learning-based network configuration synthesis is a promising direction, enabling new cross-protocol reasoning capabilities and great performance improvements. Promising future work includes construction of hybrid systems, integrating both neural models and SMT-based approaches to obtain the best of both worlds.

==> diff/git-latexdiff.34588/new/acronyms.tex <==
\DeclareAcronym{AS}{
    short = AS,
    long = autonomous system,
    short-plural = es ,
    long-plural = s
}

==> diff/git-latexdiff.34588/new/sections/0_abstract.tex <==
% Context
Computer networks employ a number of different protocols to enable efficient routing. However, due to the complexity of multiple interacting protocols, it can be hard for network operators to implement high-level routing policies and requirements. Network configuration synthesis promises to address this situation by automatically generating configurations that satisfy a provided specification. However, existing synthesis methods are often limited to single-protocol reasoning, depend on protocol-specific and hand-coded synthesis rules, and are difficult to scale due to the SMT-based methods they employ. In this work we present a rather different, learning-based method for addressing the configuration synthesis challenge, one based on the recently proposed paradigm of neural algorithmic reasoning. Our framework is protocol-agnostic, enables cross-protocol reasoning and does not depend on any hardcoded synthesis rules. To evaluate, we instantiate our framework for the case of BGP/OSPF synthesis. Our experiments show we can synthesize configurations with a very high degree of specification consistency while observing speedups of up to $500\times$ compared to a state-of-the-art SMT-based synthesis tool.


==> diff/git-latexdiff.34588/new/sections/1_intro.tex <==
\section{Introduction}
\label{sec:introduction}

The backbone of the internet consists of many connected computer networks operated by different internet service providers (ISPs) and other large organizations. These networks rely on a number of protocols to enable effective and policy-driven routing of traffic. Based on router-level configurations, the protocols perform a distributed computation to construct a network's forwarding state. However, the relatively low-level router configuration makes it hard for network operators to directly enforce network-wide policies and requirements. This often leads to misconfiguration, which can cause global outages such as the recent hours-long blackout of the entire Facebook platform \cite{janardhan2021} and comparable events \cite{mccarthy_2019}.
%
\paragraph{Configuration Synthesis} This situation has triggered a number of research efforts regarding the synthesis of network configurations \cite{el2018netcomplete,beckett2017network,narain2008declarative}. Configuration synthesis is concerned with the task of automatically generating router-level configurations given a set of high-level requirements. However, this synthesis problem can be very hard to solve, since network configurations typically consist of a considerable number of tunable parameters, where the execution of several interacting protocols yields the overall forwarding state. An effective synthesis tool must thus account for this fact and be able to reason across multiple protocols.

\paragraph{SMT-based Synthesis} Some of the most successful efforts in providing cross-protocol synthesis capabilities are based on satisfiability modulo theory (SMT) solvers \cite{el2018netcomplete,el2017network}. While SMT-based synthesis is a promising method, it comes with a number of limitations:
% \item protocol-specific
% fully hand-coded synthesis rules, a lot of implementation effort, cross-protocol support extra complicated
(1) SMT-based synthesizers are hand-crafted and highly protocol-specific. To implement synthesis, we must first express our networking model, protocol semantics including vendor and device specific behavior in terms of first-order logic constraints. This is a time-intensive and complicated process, requiring lots of expert knowledge.
%  model-dependent: synthesis is reasoning on the level of some assumed model which may not reflect the real world: even if a configuration is synthesized based on some spec, it may behave differently and violate spec in practice
Further, (2) logic-based modelling introduces a disconnect between the synthesis tool and real-world behavior \cite{birkner2021metha}. More specifically, synthesized configurations may satisfy a provided specification within a formal framework, but may not behave the same way in the real world.
% can be very slow
And, (3) SMT-based synthesis can be very slow or fail to complete, especially when reasoning about large network topologies. In practice however, network operators reconfigure their networks on a daily basis \cite{vissicchio2012improving}, which means an effective synthesis tool must be fast.

% \item fully learned, no hand-coded synthesis rules (model-free), very flexible to adapt to more/new protocols
% \item protocol-agnostic, cross-protocol
\paragraph{Neural Algorithmic Reasoning for Synthesis} Recent work on neural algorithmic reasoning (NAR) proposes to replace traditional algorithms with neural networks to learn improved algorithmic procedures \cite{velivckovic2021neural}.
It has been shown to be a powerful and fast algorithmic approximation method for a number of graph-related \cite{velivckovic2019neural} and combinatorial optimization problems \cite{cappart2021combinatorial}. Further, due to its learned nature, NAR allows for learning procedures directly from (real-world) data, without the need for manual feature extraction. Overall, this positions NAR as an attractive method to obtain a fast, fully-learned synthesis procedure, which entirely avoids the need for a formal model or any hand-crafted synthesis rules. Based on this promising outlook, this paper explores how to apply the NAR paradigm to the problem of network configuration synthesis.

To that end, we propose a \textbf{new learning-based framework for configuration synthesis} as an alternative to SMT-based approaches. Our framework is protocol-agnostic, enables cross-protocol reasoning and avoids the need to manually provide synthesis rules. We build upon the idea of NAR, and train a graph-based processor neural network to learn a synthesis procedure in latent space. A key challenge in a multi-protocol setting is the diversity of different protocols and configuration parameters. To this end, we implement a generic embedding scheme based on Datalog-like facts and program sketching \cite{solar2008program}, which allows us to easily adapt our framework to new protocols. Further, our synthesis model produces a whole distribution of network configurations. As a consequence, we can directly sample multiple alternative synthesis outputs, which is not possible with standard SMT solvers. We apply our framework to a non-trivial synthesis setting where both the Border Gateway Protocol (BGP) and the Open Shortest Path First (OSPF) protocol are used. We demonstrate that our learned synthesis tool is up to~$500\times$ faster than a state-of-the-art SMT-based synthesizer, while producing configurations which on average enjoy more than 91\% satisfaction of the provided specification.

\paragraph{Main Contributions} Our core contributions are:
\vspace{-5pt}
\begin{itemize}
    \setlength{\itemsep}{5pt}
    \setlength{\parskip}{0pt}
    \item A learning-based framework for network configuration synthesis based on neural algorithmic reasoning.
    \item A neural network architecture for learning synthesizer models which relies on a generic graph-based encoding of network topologies and configurations.
    \item An extensive evaluation of our learning-based synthesizer, in terms of both precision and scalability, on the challenging setting where both the BGP and OSPF protocols are involved.
\end{itemize}

\section{Framework Overview}
\label{sec:overview}

\begin{figure}
    \begin{center}
        \includegraphics[width=0.45\textwidth]{figures/synthesizer-overview.pdf}
    \end{center}
    \caption{An overview of our learning-based synthesis framework.}
    \label{fig:learning-based-synthesis}
\end{figure}

%As an example, consider \cref{fig:network-fwd-tree} (c) which illustrates the forwarding plane of some traffic class reachable via external peer $E$ or $F$ in our example network. Each router of the network forwards traffic along some of its outgoing links. In practice, a number of protocols are used to populate a router's routing tables. For the instantiation of our synthesis framework however, we focus on OSPF and BGP.

In the following, we discuss the fundamentals and core steps of our learning-based framework as illustrated in \cref{fig:learning-based-synthesis}.

\paragraph{Network Configuration} In this work, we consider the configuration synthesis problem at the level of the so-called \emph{forwarding plane} of a network. This means we look at how each router forwards traffic, given a packet with a certain destination. The forwarding plane is determined by a distributed computation whose exact semantics depend on the different routing protocols in use. To adapt the forwarding behavior, network operators change configuration parameters at the router-level (e.g. link weights), such that running the protocols results in the desired forwarding plane. Given this context, we define the problem of configuration synthesis as follows.

\paragraph{Configuration Synthesis} The configuration synthesis problem corresponds to automatically generating these router-level configurations, such that a set of given requirements about the forwarding plane is satisfied. Typical requirements include reachability, traffic isolation and other forwarding properties. 

\paragraph{Dataset} To train a synthesizer model, we first generate a dataset of input/output samples for the synthesis problem. For this, we rely on a generative pipeline as shown in the top of \cref{fig:learning-based-synthesis}. First, we sample a random network configuration for some topology using a uniform generative process. Then, we simulate the involved protocols to obtain the corresponding forwarding plane. Next, we extract a specification by randomly selecting properties that hold for the computed forwarding plane. This leaves us with a specification and topology as input and corresponding configuration as the output to a synthesis problem.

\paragraph{Simulation} Depending on the protocols in use, one implements simulation code to compute the forwarding plane induced by a sampled configuration. Although this step is protocol-specific, the overall implementation effort is much lower compared to SMT-based synthesis. Protocols are typically well-defined algorithms which can be simulated, whereas the alternative of implementing a synthesizer often requires expert knowledge about SMT solvers. In practice, our framework may also be adapted to use a real-world network router to compute the behavior of a configuration, thereby capturing the real-world behavior directly.

\paragraph{Neural Synthesizer Model} Based on the generated dataset, we train a graph neural network (GNN) to perform synthesis. For this, the network's input consists of a topology, a specification and a configuration sketch where to-be-synthesized parameters are omitted. Following the NAR paradigm, we first encode this synthesizer input in latent space. Then, we apply an iterative processor network which relies on the graph attention mechanism to propagate information \cite{velivckovic2017graph}. Last, we apply a decoder network to predict the values of omitted configuration parameters, thereby synthesizing a corresponding configuration. To remain protocol-agnostic, our model is generic with respect to the input format, using an intermediate representation based on Datalog-like facts.
%
\paragraph{Relaxed Specification Consistency} Since parts of the configuration synthesis problems are known to be NP-hard \cite{fortz2000internet}, any precise synthesis method will run into scalability issues, just like SMT-based methods. However, practical synthesis must be fast and scalable to accommodate the size of real-world networks and the frequency at which configurations need to be updated \cite{vissicchio2012improving}. In our learning-based framework, we therefore employ a fixed-size neural network architecture which always runs in polynomial time. While this indeed enables fast synthesis times, we cannot expect our neural system to be as precise as SMT methods. Therefore, to assess the synthesis capabilities of our learning-based system, we rely on the notion of \emph{relaxed~specification~consistency}. More specifically, we do not just check whether a configuration satisfies a specification or not, but also measure the degree up to which a synthesized configuration satisfies a specification (e.g. via the number of satisfied requirements). 

This "soft" understanding of a specification allows us to evaluate neural synthesis systems which may not always produce fully consistent configurations. Further, we argue that configurations with less than $100\%$ consistency are still very useful in practice, as they provide a good starting point for additional adjustments by network operators. Future work may improve the precision of neural synthesis by exploiting partial synthesis methods \cite{el2018netcomplete} to obtain fully consistent solutions, given a partially consistent configuration. However, note also that even exact SMT-based synthesizers may not always produce fully consistent solutions, due to differences between the formal protocol model and the one running on a given real-world router where the configuration is to be deployed \cite{birkner2021metha}.

\paragraph{Instantiation} Our learning-based synthesis framework is generic with respect to the routing protocols in use. This means, it can be instantiated to many different synthesis settings. To do this, users merely provide a drop-in replacement for the simulation component as shown in \cref{fig:learning-based-synthesis}, while other components such as the neural model architecture itself can be directly re-used.

%More specifically, we employ a slightly modified variant which operates on a graph-based encoding of a specification, topology and configuration parameters.

%  \begin{figure*}
%      \centering
%      \includegraphics[width=0.85\textwidth]{figures/system-overview.pdf}
%      \caption{An overview of our synthesis system: (1) First, we use a generic embedding scheme to transform a network topology, protocol configuration sketches and the specification given as Datalog-like facts to a latent input representation. Next, we apply a learned (2) Processor GNN and obtain a latent synthesis output. Last, we apply a (3) Decoder Network to obtain a distribution over possible values per unknown parameter in our configuration.}
%      \label{fig:overview-model}
% \end{figure*}
%

In this paper, we first discuss the architecture of our neural synthesis model. In follow-up sections, we instantiate our framework  for the case of BGP/OSPF configuration synthesis, and evaluate the resulting instantiation by comparing it to a state-of-the-art SMT-based synthesizer.

% \begin{itemize}
%     \item effort: need to implement simulation code to generate dataset to learn from (typically well-defined in protocol specs, much easier than implementing synthesis directly)
%     \item can be sampled (multiple alternative solutions, not easily possible with SMT-based methods)
%     \item much faster than SMT-based synthesis
% \end{itemize}

% Requirements:
% \begin{itemize}
%     \item protocol-agnostic
%     \item fully learned, no hand-coded synthesis rules
%     \item define: strict specification vs. relaxed specification
% \end{itemize} 

==> diff/git-latexdiff.34588/new/sections/2_model.tex <==
\section{Neural Synthesis Model}
\label{sec:model}


We now present the architecture of our graph-based neural synthesizer model, illustrated in \cref{fig:overview-model}. First, in \cref{sec:graph-embedding} we introduce our generic graph-based encoding, which allows us to embed network topologies, protocol configuration and the specification into a latent space. Then, in \cref{sec:graph-transformer} we present the architecture of the processor network which we train to perform the synthesis task. Finally, in \cref{sec:decoding-sampling} we discuss how to sample network configurations from the resulting latent synthesis output.

\begin{figure}
    \begin{minipage}[t]{0.21\textwidth}
    \begin{lstlisting}[basicstyle=\ttfamily\small, escapeinside={(*}{*)}]
router(A)
router(B)
(...)

connected(A,B,2)
connected(A,C,?)(*\blackcircled{1}*)
(...)
    \end{lstlisting}
\end{minipage}
\begin{minipage}[t]{0.21\textwidth}
    \begin{lstlisting}[basicstyle=\ttfamily\small, escapeinside={(*}{*)}]
network(N1)
bgp_route(E,N1,2,3,1,0,1)

fwd(A,B,N1)
not fwd(B,A,N1)
(...)
    \end{lstlisting}
\end{minipage}
    \caption{A snippet of a fact base sketch encoding a network's topology, parameters such as link weights (\texttt{connected} facts) and a specification (\texttt{fwd} facts).}
    \label{fig:datalog-encoding}
\end{figure}

\begin{figure}[t]
    \centering
    \includegraphics[width=0.25\textwidth]{figures/synth-architecture.png}
    \caption{The neural synthesizer model architecture.}
    \label{fig:architecture}
\end{figure}

\subsection{Fact Base Embedding}
\label{sec:graph-embedding}
To remain network protocol-agnostic in our model architecture, we implement a generic graph-based encoding of Datalog-like facts, similar to knowledge graphs \cite{rosso2020beyond}. This means that we first encode topologies, configurations and specifications as a set of Datalog-like facts and then employ a generic embedding.
%We chose Datalog facts as the input format of our synthesis approach for its flexibility, wide-spread use in Program Analysis and use in previous work on configuration synthesis \cite{el2017network}.

\paragraph{Fact Base} A set of Datalog-like facts, as depicted in \cref{fig:datalog-encoding}, serves as the input \emph{fact base} $\mathcal{F}$ to our synthesizer model. $\mathcal{F}$ is a set of facts $f(a_0, \dots, a_n)$ where arguments may be constants (e.g. A or B) or integer literals. Further, each fact in a fact base has a corresponding truth value denoted as $[f(a)]_{\mathcal{B}}$. For instance, from the fact base in \cref{fig:datalog-encoding} we can derive $[fwd(A,B,N1)]_{\mathcal{B}} = \text{\texttt{true}}$ and $[fwd(B,A,N1)]_{\mathcal{B}} = \text{\texttt{false}}$.

\paragraph{Consistency} We represent a network's topology, the protocol configuration and parameters as well as the specification, all in a single fact base. Given the semantics of the protocols in use, we can then check whether the specification encoded in a fact base is satisfied by the provided configuration. To quantify, we define the notion of relaxed specification consistency, as discussed earlier, with respect to a fact base: Given a fact base $\mathcal{F}$, a subset of specification facts $S \subset \mathcal{F}$ and protocol semantics $\mathcal{P}$, the \emph{consistency} of a fact base is defined as the relative number of satisfied facts in $S$ with respect to the forwarding plane obtained via $\mathcal{P}$. The contents of $S$ depend on the concrete instantiation of the synthesizer model. For an example of possible specification facts, see our instantiation of the synthesizer model for BGP/OSPF in \cref{sec:training}.

\begin{figure*}
    \footnotesize
    \def\arraystretch{1.4}
    \begin{tabular}{lr}
        %$T_f: T_1 \times \dots \times T_n$ & \textit{(fact type declaration)}\\
        $emb(f) := \mathbf{V_f}$ & \textit{(learned fact type embedding)}\\
        $emb(b) := \mathbf{W_{\text{bool}}}\;onehot(b)$ & \textit{(learned boolean embedding)}\\
        $emb(f,i,v) := \mathbf{W_{f_i}}\;onehot(v)$ & \textit{(learned integer embedding)}\\
        $emb(f,i,?) := \mathbf{V_{hole}}$ & \textit{(learned hole embedding)}\vspace{2pt}\\
        $\mathlarger{
        h_c := \sum_{f(c) \in \mathcal{F}}
        emb(f)
        }$ & \textit{(constant embedding)}\vspace{2pt}\\
        $h_{f(a_0, \dots, a_n)} := emb(f) + emb([f(a_0, \dots, a_n)]_{\mathcal{B}}) + \mathlarger{
        \sum_{(i,v) \in \mathcal{I}(f(a_0, \dots, a_n))}
        emb(f, i, v)
        }$\hspace{-1.2cm} & \textit{(fact embedding)}\\
        $\mathcal{I}(f(a_0, \dots, a_n)) := \{(i,v) \; | \; f(a_0, \dots, a_{i-1}, v, \dots, a_n) \in \mathcal{F} \wedge v:Int \wedge i \in \mathbb{N}$ \}& \textit{(integer arguments)}\vspace{2pt}\\
        $N_i(h_c) := \{h_f \; | \; \exists i \in \mathbb{N} . f(a_0, \dots, a_{i-1}, c, a_{i+1}, \dots, a_n) \in \mathcal{F}\}$& \textit{(i-th neighborhood of constant node)} \\
        $N_i(h_f) := \{h_c \; | \; \exists i \in \mathbb{N} . f(a_0, \dots, a_{i-1}, c, a_{i+1}, \dots, a_n) \in \mathcal{F}\}$& \textit{(i-th neighborhood of fact node)} \\
    \end{tabular}
    \caption{Translating a fact base $\mathcal{F}$ to node features. $f$ denotes a predicate, $v$ integer values, $b$ boolean values as 0 or 1, $i$ argument indices and $[f(a)]_{\mathcal{B}}$ the truth value of a fact. }
    \label{fig:graph-embedding}
\end{figure*}

%discuss embedding as shown in \cref{fig:datalog-encoding}. Note how this makes fact bases a suitable input to standard GNN architectures.

\paragraph{Fact Base Sketching} In a synthesis setting, we are confronted with incomplete fact bases, i.e. the specification and topology is given but the network configuration is to be synthesized. For these cases, we also consider fact bases with unknown parameters inspired by the idea of program sketching in program synthesis \cite{solar2008program}. More specifically, users may replace an unknown integer argument of a fact by a \texttt{?} symbol, indicating a value to be synthesized. Using this mechanic, we can represent the synthesis input as an incomplete fact base which encodes to-be-synthesized values as unknown parameters. As an example, consider \cref{fig:datalog-encoding} \blackcircled{1}, where the link weight between router nodes \texttt{A} and \texttt{C} is represented as an unknown parameter.

\paragraph{Embedding} We employ a structurally-defined embedding scheme to transform a fact base into a graph with node features as required for processing with graph neural networks. Given a fact base $\mathcal{F}$, we apply the rules in \cref{fig:graph-embedding} to obtain node features and adjacency information. Both a fact $f$ and a constant $c$ are represented as distinct nodes with features $h_c$ and $h_f$, respectively. The relationships between facts and constants is encoded as node adjacency as defined by the neighborhood functions $N_i$.

We use multiple neighborhood functions, i.e. multiple types of edges, to encode the argument position of a constant occurring in a fact. Hence, the number of neighborhood functions corresponds to the maximum number of arguments in a single fact, e.g. 3 in \cref{fig:datalog-encoding}. Integer arguments and unary facts are directly accounted for in the respective node or fact embedding. To handle unknown parameters, we replace the corresponding $emb(...)$ term with the learned $\mathbf{V_{hole}}$ embedding.

Considering the embedding function $emb$, the learned parameters of our embedding are $\mathbf{V_f} \in \mathbb{R}^D$ per fact type in~$\mathcal{F}$, $\mathbf{W_{\text{bool}}} \in \mathbb{R}^{D \times 2}$ for boolean values, $\mathbf{W_{f_i}} \in \mathbb{R}^{D \times N}$ per integer argument of fact type $f$ and $\mathbf{V_{hole}} \in \mathbb{R}^D$ to represent unknown parameters. Hyperparameter $D$ represents the dimension of the latent space the synthesizer model operates in and $N$ specifies the number of supported integer values. An example of applying this embedding scheme to a simple fact base is given in \cref{fig:graph-encoding-example}.

\begin{figure}
    \begin{minipage}[t]{0.2\textwidth}
        \centering
        \footnotesize
        \textbf{Fact Base}
        \begin{lstlisting}[basicstyle=\ttfamily\small]
router(A)
router(B)

conn(A, B, 12)
        \end{lstlisting}
    \end{minipage}
    \begin{minipage}[t]{0.15\textwidth}
        \centering
        \textbf{Graph}\\
        \vspace{5pt}
        \includegraphics[width=0.7\textwidth]{figures/graph-encoding.pdf}
    \end{minipage}\\
    \centering\\
    \vspace{10pt}
    \textbf{Node Features}\\
    \vspace{10pt}
    \begin{minipage}[t]{0.5\textwidth}
        $\begin{array}{rcl}
        h_A &:=& emb(router) = \mathbf{V_{\text{router}}}\\
        h_B &:=& emb(router) = \mathbf{V_{\text{router}}}\\
        h_{\text{conn(A,B,12)}} &:=& emb(conn) + emb(conn, 2, 12)\\
        &:=& \mathbf{V_{\text{conn}}} + \mathbf{W_{conn_2}} onehot(12)
    \end{array}$
    \end{minipage}
    \caption{An example of embedding a simple fact base using the embedding scheme of \cref{fig:graph-embedding}. The shown graph illustrates the neighborhoods $N_0$ and $N_1$ induced by the \texttt{conn} fact.}
    \label{fig:graph-encoding-example}
\end{figure}

\begin{figure}
    $$
    \begin{array}{rcl}
    z_j &:=& h_j + Drop(\mathlarger{\sum_{N_i}} h'_{GAT_i})\\
    h'_j &:=& FFN(Norm(z_j))\vspace{11pt}\\
    FFN(x_j) &:=& Norm(Lin2(Drop(Lin1(x_j)))))
    \end{array}
    $$
    \caption{
        The recurrence relation of a node $j$'s representation $h_j$. $h'_{GAT_i}$ represents the output of a graph attention layer operating with neighborhood $N_i$ according to \cite{velivckovic2017graph}, $h_j$ the representation of node $j$ at the previous step. $Norm$ refers to batch normalization \cite{ioffe2015batch}, $Drop$ to dropout regularization \cite{hinton2012improving} and $Lin1$ and $Lin2$ to linear layers with an inner dimension of $4N$.
    }
    \label{fig:recurrence}
\end{figure}

\subsection{Synthesizer Model}
\label{sec:graph-transformer}

For an illustration of the synthesizer model's architecture, please see Figure~\ref{fig:architecture}. Given a fact base $\mathcal{F}$ we first apply our embedding scheme as described in \cref{sec:graph-embedding}. We then employ a 2-layer GNN-based encoder network to produce the latent representation of a synthesis input.
Given this representation, a processors network is trained to perform the actual synthesis task in high-dimensional space. Last, we apply a set of decoder networks, to obtain the synthesized values of unknown parameter, given the latent synthesis~output.

%In this context, the synthesis problem for network configurations corresponds to completing partially provided fact bases.

% \paragraph{High-Level Architecture}

% We employ the high-level architecture to obtain the latent synthesis output $y_\mathcal{F}$:
% $$
% \begin{array}{rcl}
%     \mathbf{x_{\mathcal{F}}} &:=& Encoder(Embedding(\mathcal{F}))\\
%     \mathbf{y_{\mathcal{F}}} &:=& Processor(\mathbf{x_{\mathcal{F}}} + \mathbf{z})\\
%     z_i &\sim& \mathcal{N}(0,1)
% \end{array}
% $$
% \todo{z is only added for $i<N/2$}

% $Embedding$ corresponds to the graph-based embedding as discussed in \cref{sec:graph-embedding} and $Encoder$ is a 2-layer graph attention module. $Processor$

\paragraph{Encoding} The encoder GNN operates on the embedded representation of a fact base. It produces the high-dimensional representation of a synthesis input as required for the processor network. We additionally apply noise to the first half of the units of the latent representation via $\mathbf{z}$, as a source of non-determinism. According to our experiments this improves model performance and we hypothesize this is due to the synthesis problem having more than one solution in most cases.

\paragraph{Iterative Processor} The processor network is modelled as an iterative process. It consists of a 6-layer graph attention module which we apply for a total of 4 iterations. In the framework of neural algorithmic reasoning, this iterative computational structure encodes an inductive bias towards an iterative solution to the synthesis problem. Because of this bias, our processor network essentially learns an algorithmic procedure which iteratively synthesizes the values of unknown parameters in a fact base.

\paragraph{Graph Attention Layer} In the GNNs we employ, we rely on a composed variant of the graph attention layer as introduced by \cite{velivckovic2017graph}. We employ multiple graph attention layers in lockstep, one per neighborhood $N_i$ defined by our graph embedding (cf. \cref{sec:graph-embedding}), and combine the intermediate results after each step. Specifically, the recurrence relation of a node $j$'s representation $h_j$ is defined as shown in \cref{fig:recurrence}. These mechanics of combining the results of the different graph attention layers $h'_{GAT_i}$, directly corresponds to how multiple attention heads are combined in the original Transformer architecture \cite{vaswani2017attention}.

\paragraph{Argument Decoder Networks} To synthesize the values of unknown parameters, the model maintains a set of decoder networks. That is, it provides one decoder network per integer argument per fact type in a fact base. When decoding, the network is applied to the latent synthesis output of the corresponding fact node. For example, a synthesizer model which operates on the fact base in \cref{fig:datalog-encoding}, would provide a decoder network $D_{\text{connected}_2}: \mathbb{R}^D \rightarrow \mathbb{R^N}$ to decode values for the third argument of a \texttt{conn} fact. In our experiments, decoder networks are implemented as simple multi-layer perceptron models.

\paragraph{Supervision Signal} During training, we mask all fact arguments that represent to-be-synthesized configuration parameters in our synthesis setting. As a supervision signal we use the masked values as the ground-truth and apply a negative log-likelihood loss function to the output distribution of the corresponding argument decoder networks.

%The synthesizer model learns a conditional distribution of fact bases which are consistent with respect to the protocols' semantics.

%\todo{introduce synthesis as a completion problem of an encoded fact base (a la BERT). Introduce masking, introduce decoding of integer and truth values. Synthesis is learning a conditional distribution of consistent fact bases.}

%Using this method, we obtain the node features $h_c$ per constant, $h_f$ per fact and adjacency information in terms of node neighborhood functions $N_i(h_c)$ and $N_i(h_f)$. Overall, this encoding makes a fact base suitable for processing using standard graph neural networks.

%- Brief description of the Graph Transformer Model
\subsection{Multi-Shot Sampling}
\label{sec:decoding-sampling}

%Multi-Stage Parameter Sampling (sampling methods: topk, high-temp, low-temp)
To sample concrete values from the output distributions over unknown parameters, we apply a multi-shot sampling strategy. That is, we sample values only for a subset of unknown parameters, insert them in our input fact base and run the synthesis model again. We repeat this process until no more unknown parameters remain. This multi-shot sampling strategy allows the model to incorporate the concrete values of previously synthesized parameters in its computation. In our evaluation in \cref{sec:evaluation}, we include a comparison of how this compares to sampling all unknown parameters at once.

%In a fact base with multiple holes, we apply the corresponding decoder networks to obtain a value distribution for each integer hole. However, instead of sampling all integer holes in one


==> diff/git-latexdiff.34588/new/sections/3_bgp_ospf.tex <==
\section{BGP/OSPF Synthesis}
\label{sec:bgp-ospf}

\newcommand{\as}{\ac{AS}~}
\newcommand{\ases}{\acp{AS}~}

\newcommand{\squareann}{{\tiny$\blacksquare\;$}}
\newcommand{\triangleann}{{\small$\blacktriangle\;$}}

\begin{figure*}
    \centering
    \includegraphics[width=0.95\textwidth]{figures/networks-all.pdf}
    \caption{(a) An illustration of a small AS network, including internal peers (blue), external peers (purple), BGP sessions as well as physical links. (b) The propagation of two BGP announcement across the network. (c) The resulting forwarding plane after applying BGP and OSPF.}
    \label{fig:network-fwd-tree}
\end{figure*}

We now discuss an instantiation of our learning-based framework for the case of BGP and OSPF protocols. In \cref{sec:synthesis-setting} we introduce a basic networking model, BGP and OSPF protocols and the synthesis setting. Given this model, \cref{sec:training} describes how to generate a corresponding dataset of input/output samples and train a synthesizer model.
%This shall serve as a prerequisite to the instantiation of our learning-based synthesis framework for the BGP and OSPF protocol in \cref{sec:training}.

\subsection{Synthesis Setting}
\label{sec:synthesis-setting}

\paragraph{Graphical Model} We assume an abstract network model which can be represented as an undirected graph as shown in \cref{fig:network-fwd-tree} (a). We always consider a set of internal routers (A, B, C, D in \cref{fig:network-fwd-tree}) as well as a set of adjacent external routers (E, F  in \cref{fig:network-fwd-tree}). The group of internal routers forms the \emph{\as} under consideration whereas external routers belong to other adjacent \ases. In practice, an \as represents an administrative domain controlled by a single operator. 

\paragraph{Forwarding Plane} For an example of a possible forwarding plane in this abstract model, consider \cref{fig:network-fwd-tree} (c) which illustrates the forwarding plane of traffic destined towards some destination reachable via external peer $E$ or $F$. Each router of the network forwards traffic along some of its outgoing links. In practice, a number of protocols are used to compute the forwarding plane. However, here we focus on OSPF and BGP.

\paragraph{OSPF} The OSPF protocol \cite{moy1994ospf} is a link-state protocol, typically used as an interior gateway protocol~(IGP), i.e., to route traffic within an \ac{AS}. Given link weights per physical link in the network, OSPF simply routes traffic along the shortest path towards the destination.

\paragraph{BGP} The BGP protocol \cite{rekhter1994border} on the other hand is a path-vector protocol used to exchange reachability information mostly on the level of \acp{AS}.
%These are groups of routers typically operated by a single party (e.g. an ISP).
When using BGP, a routing destination announces its existence to other \ases and routers, by sending out a BGP announcement. Receivers of such announcements may then choose to pass them on to other \acp{AS}, redistribute them internally and/or modify them. Instead of communicating along physical links directly, the BGP protocol requires manually configured BGP sessions among routers of the \as and external peers, as indicated by the BGP session edges in \cref{fig:network-fwd-tree}(a).
%\todo{more discussion of eBGP vs iBGP and support for route reflection (more of an implementation detail, maybe only mention in dataset generation where simulation code is discussed)}.

%\paragraph{BGP Decision Procedure}~
%\todo{discuss decision procedure}
In case a router receives more than one announcement for a destination, a designated BGP decision process is applied to determine a single best route. \cref{fig:bgp-decision} shows the ordered list of comparison criteria of this decision process. The different criteria depend different properties of a route announcements, including the IGP cost towards the routing destination. As a consequence, when used together, OSPF as IGP protocol and BGP will interact. %Note also that BGP is an iterative process which needs multiple rounds of propagation to converge.

\paragraph{Example}
%\todo{run through simple BGP+OSPF example of computing the forwarding plane}
To better understand BGP/OSPF routing, consider the simple example given in \cref{fig:network-fwd-tree} (b). Here, our example \as imports BGP announcements \squareann and \triangleann from E and F respectively. Both represent a route to the same destination. As shown, both announcements have a so-called local preference of 2. For simplicity, we ignore other properties such as the AS path length, Origin and MED in this example. The announcements are propagated among BGP neighbors and the best route is selected according to the decision procedure in \cref{fig:bgp-decision}. See \cref{fig:network-fwd-tree} (b) for an illustration of the intermediate states of this propagation process. As both announcements have a local preference of 2, rule 1 of the decision process is not used. Instead, in round 2, node B selects \squareann over \triangleann due to a lower IGP cost of 2 via egress node A as compared to 3 via egress node D (rule 6). Node D selects \triangleann over \squareann, since it learns this route directly from an external peer (rule 5). After Round 3, the BGP propagation process converges to a stable state and we can derive the forwarding plane as shown in \cref{fig:network-fwd-tree} (c).


%, as well as external peers E and F which belong to other \acp{AS}. External peers are routers which are connected via eBGP sessions to routers of the \ac{AS} under consideration. They announce BGP routes to their neighbors, which are propagated within the network

%\paragraph{BGP/OSPF Configuration Synthesis} We phrase the BGP/OSPF configuration synthesis problem on the level of the forwarding plane. This means that users provide a specification which constraints the set of allowed forwarding planes. This includes predicates which enforce forwarding paths, block forwarding paths or assert higher-level properties like traffic isolation and reachability. Given such a specification, we consider network configuration synthesis as the task of configuring OSPF and BGP in a way that produces a forwarding plane which satisfies the provided specification.

\paragraph{BGP/OSPF Configuration Synthesis} According to our general synthesis framework, we consider the BGP/OSPF configuration synthesis problem at the level of the forwarding plane. However, we further also define the set of synthesized parameters: For OSPF we synthesize link weights as explored in a wide range of existing work (e.g. \cite{el2018netcomplete,fortz2000internet}. For BGP, the set of parameters is not defined as clearly: Depending on the requirements of a network operator, one may employ custom BGP import and export policies at every router of a network to implement complex behavior. However, in this instantiation we focus on a simplified setting, where we assume BGP route announcements to only be modified when imported into the \as from an external peer. Previous work has already pointed out that this is a reasonable assumption which holds for the majority of real-world networks \cite{caesar2005bgp,cittadini2010doing, steffen2020probabilistic}.

\begin{figure}
    \small{
    \begin{enumerate}
        \setlength{\itemsep}{0pt}
        \setlength{\parskip}{0pt}
        \item Highest Local preference
        \item Lowest AS path length
        \item Prefer Origin (IGP $>$ EBGP $>$ INCOMPLETE)
        \item Lowest Multi-exit discriminator (MED)
        \item External over internal announcements
        \item Lowest IGP cost to egress
        \item Lowest BGP peer id (tie breaker)
    \end{enumerate}}
    \vspace{-15pt}
    \caption{The BGP decision process \cite{rekhter1994border}. The shown rules are applied in order until a single best BGP announcements remains.}
    \label{fig:bgp-decision}
\end{figure}

\subsection{Dataset Generation and Training}
\label{sec:training}
To train a synthesizer model, we need a large number of fact bases encoding a variety of network topologies, configurations and forwarding specifications. Further, we must provide the model with target values for unknown parameters as a supervision signal. This section discusses how we construct such a dataset for BGP/OSPF synthesis.
%Further, we provide an example of what a corresponding fact base looks like, including a description of the supported specification language.

\paragraph{Dataset Generation} To obtain network configurations and corresponding forwarding specifications we employ a generative process: We first randomly configure BGP and OSPF parameters for some topology. Then we simulate the OSPF and BGP protocol and compute the resulting forwarding plane. Based on this, we extract a forwarding specification which fixes a random subset of forwarding paths, reachability and isolation properties that are satisfied by the forwarding plane.

\paragraph{Topologies} For training, our dataset is based on random topologies with $16$-$24$ routers. We generate the physical layout of these graphs by triangulation of uniformly sampled points in two-dimensional space.

\paragraph{Simulation} To compute the forwarding plane given an OSPF and BGP configuration, we simulate the protocols. For OSPF, we implement shortest path computation to obtain the forwarding plane. For BGP, we implement the full BGP decision process as shown in \cref{fig:bgp-decision}, except for the MED attribute. In addition to the basic networking model discussed in \cref{sec:synthesis-setting}, we implement support for eBGP and iBGP, fully-meshed BGP session layouts as well as layouts relying on route reflection. For more details of these BGP concepts see \cite{bates2000rr}.

%Note that the synthesizer model will reason on the level of the provided training samples. That is, to improve the overall synthesis quality in a real-world setting, it is helpful to implement simulation code which behaves very similar to real-world networks. Another promising approach would be to extract training samples from real-world networks, thereby circumventing the need for simulation, however, we leave this as future work.

%While this can be a considerable effort, it is typically an easier task than to implement the synthesizer directly. The concrete semantics of protocols and their simulation is a well-defined procedure, whereas implementing efficient synthesis tools is still an open problem.

\paragraph{Fact Base Encoding} We encode synthesis input using a small set of facts. For an example of a corresponding fact base see \cref{fig:bgp-ospf-fact-base}. We use the \texttt{router}, \texttt{external} and \texttt{network} facts to mark routers, external peers and routing destinations respectively. Physical links between routers are encoded as \texttt{connected(R1,R2,W)} facts where \texttt{W} denotes the OSPF link weight. Further, we rely on \texttt{ibgp}, \texttt{ebgp}, \texttt{route\_reflector} and \texttt{bgp\_route} facts to represent different types of BGP sessions and imported routes. Using the notion of unknown parameters as discussed in \cref{sec:graph-embedding}, we encode configuration parameters, e.g., properties of imported routes or OSPF link weights.

\paragraph{Specification Language} We support a small specification language with three types of forwarding predicates:

\begin{itemize}
    \setlength{\itemsep}{0pt}
    \setlength{\parskip}{2pt}
    \item \texttt{fwd(R1, Net, R2)} specifies that router \texttt{R1} forwards traffic destined for \texttt{Net} to its neighbor \texttt{R2}.
    \item \texttt{reachable(R1, Net, R2)} specifies that traffic destined for \texttt{Net} that passes through \texttt{R1} also passes through \texttt{R2} before reaching its destination.
    \item \texttt{trafficIsolation(R1, R2, N1, N2)} specifies that it must not hold that $[fwd(R1,R2,N1)]_{\mathcal{B}} \wedge [fwd(R1,R2,N2)]_{\mathcal{B}}$.
\end{itemize}

In the negative case of each predicate, the opposite must hold true for the fact to be satisfied. This specification language can easily be extended by including new specification predicates in the dataset generation process. One must simply provide a method of extracting positive and negative cases of a specification fact from a given forwarding plane. Once included in the training dataset of a synthesizer model, the resulting synthesis system will be able to consider specifications relying on the new type of predicates.

% \todo{info on loss function, optimizer, etc.}
\paragraph{Training} We generate a dataset of $10,240$ input/output samples and instantiate our synthesizer model with a hidden dimension $D$ of $64$. For optimization, we use the Adam optimizer \cite{kingma2014adam} with a learning rate of $10^{-4}$. We stop training after the specification consistency on a validation dataset no longer increases at $\sim2800$ epochs.

\begin{figure}
\begin{minipage}[t]{0.22\textwidth}
\begin{lstlisting}[basicstyle=\ttfamily\tiny]
# topology and configuration
router(c5)
router(c3)
router(c1)
router(c0)
network(c6)
network(c7)

external(c8)
external(c9)
external(c10)
external(c11)
external(c12)
external(c13)

route_reflector(c2)
route_reflector(c4)

connected(c2,c4,?)
connected(c2,c5,?)
connected(c2,c3,?)
connected(c4,c5,?)
connected(c4,c3,?)
connected(c4,c0,?)
connected(c5,c1,?)
connected(c5,c0,?)
connected(c3,c0,?)
connected(c3,c1,?)
connected(c1,c0,?)

ibgp(c2,c4)
ibgp(c2,c5)
ibgp(c2,c0)
ibgp(c2,c1)
ibgp(c4,c3)
ibgp(c4,c4)
\end{lstlisting}
\end{minipage}
\begin{minipage}[t]{0.2\textwidth}
\begin{lstlisting}[basicstyle=\ttfamily\tiny]
ebgp(c2,c12)
ebgp(c5,c9)
ebgp(c5,c10)
ebgp(c5,c13)
ebgp(c0,c8)
ebgp(c0,c11)

bgp_route(c8,c6,?,?,1,?,1,8)
bgp_route(c9,c6,?,?,0,?,1,9)
bgp_route(c10,c6,?,?,0,?,1,10)
bgp_route(c11,c7,?,?,0,?,1,11)
bgp_route(c12,c7,?,?,0,?,1,12)
bgp_route(c13,c7,?,?,2,?,1,13)

# forwarding specification
fwd(c0,c6,c3)
fwd(c3,c6,c2)
fwd(c2,c6,c4)
not fwd(c3,c6,c0)
not fwd(c0,c6,c11)
not fwd(c11,c6,c0)

not trafficIsolation(c1,c0,c7,c6)
not trafficIsolation(c1,c0,c7,c6)
trafficIsolation(c0,c3,c6,c7)
trafficIsolation(c0,c3,c6,c7)

reachable(c5,c6,c10)
reachable(c1,c6,c4)
not reachable(c0,c6,c5)
reachable(c5,c6,c10)
\end{lstlisting}
\end{minipage}
\caption{An example of a fact base encoding a topology, a sketch of a BGP and OSPF configuration and a forwarding specification.}
\label{fig:bgp-ospf-fact-base}
\end{figure} 

==> diff/git-latexdiff.34588/new/sections/4_evaluation.tex <==
\section{Evaluation}
\label{sec:evaluation}

We trained a synthesizer model to perform configuration synthesis for BGP and OSPF. We now assess the performance of the resulting neural synthesizer with respect to two core metrics: (1) the quality of synthesized configurations in terms of their consistency with the provided forwarding specifications (\cref{sec:synthesis-quality}), and (ii) the time a learned synthesizer takes when compared to the state-of-the-art SMT-based synthesizer NetComplete \cite{el2018netcomplete} (\cref{sec:synthesis-vs-smt}).

\paragraph{Dataset} We compare across three datasets: Small, Medium and Large. Each dataset represents 8 real-world topologies, sampled from the Topology Zoo \cite{knight2011internet}, where the number of nodes lies between 0-34, 34-68 and 68-170 respectively. To obtain forwarding specifications for the sampled topologies, we use our generative pipeline as discussed in \cref{sec:training}. In each topology, we do synthesis for 4 different traffic classes (routing destinations) at a time.

\paragraph{Experimental Setup} We run all our experiments on an Ubuntu Linux machine with an Intel(R)~Core(TM)~i9-9900X~@~3.50GHz processor, 64GB of system memory and an NVIDIA GeForce RTX 3080 GPU with 10GB of video~memory.

\subsection{Synthesis Quality}
\label{sec:synthesis-quality}
To assess our learned synthesizer, we examine its behavior with increasingly large topologies and specifications.

\paragraph{Specifications} Using the same generative model as described in \cref{sec:training}, we generate forwarding specifications for the topologies in our three datasets with each specification constructed from $3 \times n$ requirements, one per supported predicate type:  \texttt{fwd} requirements correspond to specifying or blocking a forwarding path using multiple \texttt{fwd} predicates whereas \texttt{reachable} and \texttt{trafficIsolation} requirements each translate to a single specification fact. We compare across increasingly large specifications of $3\times 2$, $3\times 8$ and $3 \times 16$ requirements, respectively.

\paragraph{Methodology} For each pair of topology and specification, we run our synthesizer 5 times and report the network configurations with the highest overall consistency value. For sampling, we rely on our multi-shot sampling strategy where we randomly group the unknown parameters of a configuration into 4 groups (4-shot sampling).

\paragraph{Results} We summarize our results in \cref{fig:eval-consistency}. On average, our synthesis model produces network configurations that are $>91\%$ consistent with the provided forwarding specifications across all datasets and sizes of specifications. When only few requirements are given, the synthesizer model even succeeds in producing fully-consistent configurations. We observe a slightly decreasing consistency with increasingly large topologies.

%\texttt{fwd} facts are satisfied more easily, whereas \texttt{reachable} and \texttt{trafficIsolation} facts are violated more often.

\paragraph{Multi-Shot Sampling} In \cref{fig:eval-consistency-baseline}, we report the average specification consistency using our multi-shot sampling strategy as compared to sampling all unknown parameters at once. As a baseline we have also sampled random configurations from a uniform distribution (per parameter) and compute the corresponding specification consistency. Over the baseline, our synthesizer model shows clear improvement and multi-shot sampling further increases consistency.

\begin{figure*}
    \begin{center}
        \textbf{Specification Consistency}\\
        \footnotesize
        \begin{tabular}{rrcccccccccc}
        \toprule
        \multicolumn{2}{c}{Dataset} & \tiny\texttt{fwd} & \tiny\texttt{reachable}  & \tiny\texttt{trafficIsolation} & Overall & $\emptyset$     No. Full Matches & $\emptyset$ No. $>90\%$ Matches\\
        \midrule
        $3\times 2$ requirements & Small & 0.95 & 0.94 & 1.00 & \textbf{0.95} & 0.62 & 0.62\\
& Medium & 0.96 & 1.00 & 0.94 & \textbf{0.96} & 0.88 & 0.88\\
& Large & 0.94 & 0.94 & 1.00 & \textbf{0.93} & 0.62 & 0.62\\
\midrule
$3\times 8$ requirements & Small & 0.97 & 0.98 & 0.97 & \textbf{0.98} & 0.50 & 1.00\\
& Medium & 0.99 & 0.95 & 1.00 & \textbf{0.98} & 0.50 & 1.00\\
& Large & 0.96 & 0.95 & 0.91 & \textbf{0.94} & 0.38 & 0.88\\
\midrule
$3\times 16$ requirements & Small & 0.97 & 0.89 & 0.95 & \textbf{0.94} & 0.38 & 0.75\\
& Medium & 0.98 & 0.97 & 0.97 & \textbf{0.98} & 0.38 & 1.00\\
& Large & 0.92 & 0.88 & 0.95 & \textbf{0.91} & 0.12 & 0.50\\
    \end{tabular}\end{center}
    \caption{Average specification consistency of the network configurations synthesized by our trained synthesizer model. Per sample we run the synthesizer with a specification of $3\times N$ requirements, where the specifications always include $N$ requirements per supported predicate type (\texttt{fwd}, \texttt{reachable}, \texttt{trafficIsolation}).}
    \label{fig:eval-consistency}
\end{figure*}

\begin{figure}
    \begin{center}
        \footnotesize
        \begin{tabular}{rrcccccccccc}
        &  & \multicolumn{2}{c}{Neural}\\
        & Random & 1-Shot & 4-shot\\
        \toprule
        Small & 0.83 & 0.92 & \textbf{0.94} \\
        Medium & 0.88 & 0.95 & \textbf{0.98} \\
        Large & 0.78 & 0.88 & \textbf{0.91} \\
    \end{tabular}\end{center}
    \caption{Average specification consistency with $3\times 16$ requirements when sampling configurations randomly from a uniform distribution and 1-shot/4-shot sampling using our synthesizer model.}
    \label{fig:eval-consistency-baseline}
\end{figure}

\begin{figure*}[ht]
    \footnotesize
    \begin{center}
        \textbf{BGP Synthesis Time}
        \footnotesize
        \begin{tabular}{rrccccccccc}
        \toprule
        &&\multicolumn{3}{c}{Synthesis Time (s)} & \multicolumn{2}{c}{Accuracy (Neural)} \\
        \multicolumn{2}{l}{\# Requirements} & NetComplete & Neural (CPU) & Speedup &$\emptyset$ Consistency& $\emptyset$ No. Full Matches\\
        \midrule
    2 requirements &Small & 18.073s & 0.641s & \textbf{28.2x} & 0.969 & 0.875\\
        &Medium & 60.864s & 2.748s & \textbf{22.2x} & 0.939 & 0.75\\
        &Large & 1389.485s\tiny{  7/8 TO} & 22.301s & \textbf{62.3x} & 0.989 & 0.875\\
    \midrule
    8 requirements &Small & 247.691s & 1.065s & \textbf{232.5x} & 0.96 & 0.75\\
        &Medium & $>$25m\tiny{  8/8 TO} & 3.47s & \textbf{432.2x} & 0.968 & 0.5\\
        &Large & $>$25m\tiny{  8/8 TO} & 30.961s & \textbf{48.4x} & 0.969 & 0.75\\
    \midrule
    16 requirements &Small & 1416.828s\tiny{  7/8 TO} & 2.528s & \textbf{560.5x} & 0.926 & 0.25\\
        &Medium & $>$25m\tiny{  8/8 TO} & 5.481s & \textbf{273.7x} & 0.947 & 0.25\\
        &Large & $>$25m\tiny{  8/8 TO} & 69.092s & \textbf{21.7x} & 0.959 & 0.25\\
    \end{tabular}\end{center}
    \caption{Comparing consistency and synthesis time of our method (Neural) with the SMT-based state-of-art synthesis tool NetComplete. The notation {\tiny{n/8 TO}} indicates the number of timed out synthesis runs out of 8 (25+ minutes).}
    \label{fig:evaluation-compare-bgp}
\end{figure*}

\begin{figure*}[ht]
    \begin{center}
        \footnotesize
        \textbf{OSPF Synthesis Time}\\
        \footnotesize
        \begin{tabular}{rrccccccccc}
        \toprule
        &&\multicolumn{3}{c}{Synthesis Time (s)} & \multicolumn{2}{c}{Accuracy (Neural)} \\
        \multicolumn{2}{l}{} & NetComplete & Neural (GPU) & Speedup &$\emptyset$ Consistency& $\emptyset$ No. Full Matches\\
        \midrule
    2 requirements &Small & 0.265s & 0.091s & \textbf{2.9x} & 1.000 & 1.00\\
     &Medium & 0.404s & 0.098s & \textbf{4.1x} & 1.000 & 1.00\\
     &Large & 0.944s & 0.14s & \textbf{6.7x} & 1.000 & 1.00\\
    \midrule
    8 requirements &Small & 0.876s & 0.164s & \textbf{5.3x} & 0.982 & 0.75\\
     &Medium & 1.517s & 0.103s & \textbf{14.7x} & 1.000 & 1.00\\
     &Large & 3.505s & 0.316s & \textbf{11.1x} & 0.981 & 0.50\\
    \midrule
    16 requirements &Small & 1.65s & 0.21s & \textbf{7.9x} & 0.991 & 0.625\\
     &Medium & 2.646s & 0.245s & \textbf{10.8x} & 0.989 & 0.50\\
     &Large & $>$566.636s+\tiny{  3/8 TO} & 0.233s & \textbf{2430.4x} & 0.987 & 0.875\\
    \end{tabular}\end{center}
    \caption{Comparing consistency and synthesis time of our method (Neural) with the SMT-based OSPF synthesis tool NetComplete. The notation {\tiny{n/8 TO}} indicates the number of timed out synthesis runs out of 8 (25+ minutes).}
    \label{fig:evaluation-compare-ospf}
\end{figure*}


\subsection{Comparison to SMT-based Synthesis}
\label{sec:synthesis-vs-smt}

%To provide a comparison of our learned BGP/OSPF synthesizer with SMT-based methods,
We now compare the synthesis time of the learned neural synthesizer with those of NetComplte, a state-of-art configuration synthesis tool based on SMT-solvers \cite{el2018netcomplete}.

\paragraph{Specifications} As the type of supported requirements in NetComplete does not fully align with our model, we restrict this comparison to specifications which only include forwarding paths (i.e. \texttt{fwd} predicates). Further, NetComplete does not support cross-protocol synthesis as in our case and instead requires users to specify for each requirement the protocol to use for its implementation. To bridge this gap, we split the generated forwarding requirements into BGP and OSPF paths for a corresponding NetComplete specification.
%\todo{note on NetComplete installing policies at all routers, not only the edges of the AS}

\paragraph{Methodology} We compare both OSPF synthesis and BGP/OSPF-synthesis. We configure our trained synthesizer model to do OSPF synthesis by only predicting link weights. For each pair of topology and specification, we report the total time of running our synthesizer 4 times using 4-shot sampling, whereas for consistency we report the best out of the 4 runs. For NetComplete, we run the synthesizer with a timeout of 25 minutes. In case a NetComplete attempt times out, we report 25 minutes as a lower bound for its runtime.

\paragraph{OSPF Synthesis Time Results} We document the results of comparing OSPF synthesis time in \cref{fig:evaluation-compare-ospf}. Our synthesizer model achieves a speedup of 2-10x over NetComplete. With 16 requirements and dataset Large this speedup even increases to $2000\times$. Further, our model achieves very high consistency with the provided specification, often producing fully-consistent configurations.

\paragraph{BGP/OSPF Synthesis Time Results} In \cref{fig:evaluation-compare-bgp} we show the comparison of BGP/OSPF synthesis time. Our synthesizer model outperforms NetComplete by multiple orders of magnitude. We observe a speedup of $20-560\times$ which appears to increase with the size of topology and specification. Further, the average specification consistency of the synthesized configurations is greater than $92\%$ across all datasets, even for large topologies. In many cases, our synthesizer model produces fully-consistent configurations, especially with small topologies and specifications. In comparison, NetComplete times out on more than half of the synthesis tasks which means that we can only observe a lower bound of speedup in these cases. Note that our synthesizer model is running on a CPU due to memory restrictions with large topologies. However, running it on a GPU results in even greater speedups (up to $1000\times$, cf. \cref{app:sec:bgp-gpu-performance}). 

==> diff/git-latexdiff.34588/new/sections/5_related_work.tex <==
\section{Related Work}
\label{sec:related-work}

\paragraph{Traditional Configuration Synthesis} 
%A range of existing work is concerned with network configuration synthesis. 
Next to methods based on compilation such as Propane/PropaneAT \cite{beckett2017network}, there are a number of configuration synthesis methods based on constraint solving: Examples include ConfigAssure \cite{narain2008declarative}, SyNet \cite{el2017network} and NetComplete \cite{el2018netcomplete}. Due to their hand-coded nature, these methods are highly protocol-specific and can be very slow due to the solvers they employ. Although some of them allow for cross-protocol reasoning, this is not implemented as transparently as in our framework and users must specify per requirement which protocol to use for its implementation. In contrast, our approach has lower precision but allows for fully transparent cross-protocol reasoning, meaning forwarding requirements are not protocol-bound and the synthesizer chooses how to implement them. Further, our learned BGP/OSPF synthesis tool exhibits much lower synthesis times as compared to an SMT-based tool like NetComplete.

% \begin{itemize}
%     \item NetComplete, SyNet
%     \item Propane, PropaneAT
%     \item DeepBGP
% \end{itemize}

\paragraph{GNNs and Networking} DeepBGP \cite{bahnasy2020deepbgp} relies on GNNs and reinforcement learning to do configuration synthesis. However, it is limited to BGP configuration synthesis and is slower than SMT-based synthesis according to the author's evaluation. In contrast, our learning-based framework is cross-protocol, does not rely on reinforcement learning and provides better synthesis performance. Apart from configuration synthesis, GNNs have also been applied to other problems in the networking domain. For example, the authors of RouteNet \cite{rusek2020routenet} use GNNs to predict performance metrics of network configurations. Other work that is concerned with learning improved protocols includes Q-Routing \cite{boyan1994packet} or more modern approaches such as the Graph-Query Neural Network architecture \cite{geyer2018learning}.

\paragraph{Neural Algorithmic Reasoning} 
Neural algorithmic reasoning (NAR) as proposed in \cite{velivckovic2021neural}, describes the idea of replacing traditional algorithms with neural networks to learn improved algorithmic procedures. Exemplary work includes graph-related algorithms \cite{velivckovic2019neural} or solvers for combinatorial optimization problems \cite{cappart2021combinatorial,joshi2020learning,selsam2019guiding}. Our synthesis framework is the first applications of NAR to the networking domain and relies on the NAR-native encode-process-decode architecture. According to the hierarchy of NAR approaches in \cite{cappart2021combinatorial}, our method is an algorithm-level approach, as we do not supervise on intermediate steps. Although, such step-level methods promise better generalization, it is not clear what an intermediate result of a general synthesis procedure would be. However, future work on a step-level approach may further improve synthesis quality.

% \begin{itemize}
%     \item RouteNet
%     \item GraphNET
%     \item Learning and generating distributed routing protocols using graph-based deep learning
%     \item Unveiling the potential of Graph Neural Networks for network modeling and optimization in SDN
% \end{itemize}

==> diff/git-latexdiff.34588/new/sections/6_conclusion.tex <==
\setlength{\parskip}{6pt plus4mm minus4mm}
\section{Conclusion}
\label{sec:conclusion}
We presented a learning-based framework for configuration synthesis based on the idea of neural algorithmic reasoning. To assess the effectiveness of the system, we instantiated it for the case of BGP/OSPF synthesis. In contrast to traditional synthesis methods, our system supports transparent cross-protocol reasoning and learns synthesis rules only from data. Using our system, synthesis is sped up by a factor of up to $500\times$ when compared to SMT-based methods. Further, our evaluation demonstrates that the resulting synthesis tool provides excellent synthesis quality, producing configurations with high specification consistency. Overall, our results illustrate that exploring the direction of learning-based network configuration synthesis is a promising direction, enabling new cross-protocol reasoning capabilities and great performance improvements. Promising future work includes construction of hybrid systems, integrating both neural models and SMT-based approaches to obtain the best of both worlds.

==> diff/git-latexdiff.34588/old/acronyms.tex <==
\DeclareAcronym{AS}{
    short = AS,
    long = autonomous system,
    short-plural = es ,
    long-plural = s
}

==> diff/git-latexdiff.34588/old/sections/0_abstract.tex <==
% Context
Computer networks employ a number of different protocols to enable efficient routing. However, due to the complexity of multiple interacting protocols, it can be hard for network operators to implement high-level routing policies and requirements. Network configuration synthesis promises to address this situation by automatically generating configurations that satisfy a provided specification. However, existing synthesis methods are often limited to single-protocol reasoning, depend on protocol-specific and hand-coded synthesis rules, and are difficult to scale due to the SMT-based methods they employ. In this work we present a rather different, learning-based method for addressing the configuration synthesis challenge, one based on the recently proposed paradigm of neural algorithmic reasoning. Our framework is protocol-agnostic, enables cross-protocol reasoning and does not depend on any hardcoded synthesis rules. To evaluate, we instantiate our framework for the case of BGP/OSPF synthesis. Our experiments show we can synthesize configurations with a very high degree of specification consistency while observing speedups of up to $500\times$ compared to a state-of-the-art SMT-based synthesis tool.


==> diff/git-latexdiff.34588/old/sections/1_intro.tex <==
\section{Introduction}
\label{sec:introduction}

The backbone of the internet consists of many connected computer networks operated by different internet service providers (ISPs) and other large organizations. These networks rely on a number of protocols to enable effective and policy-driven routing of traffic. Based on router-level configurations, the protocols perform a distributed computation to construct a network's forwarding state. However, the relatively low-level router configuration makes it hard for network operators to directly enforce network-wide policies and requirements. This often leads to misconfiguration, which can cause global outages such as the recent hours-long blackout of the entire Facebook platform \cite{janardhan2021} and comparable events \cite{mccarthy_2019}.
%
\paragraph{Configuration Synthesis} This situation has triggered a number of research efforts regarding the synthesis of network configurations \cite{el2018netcomplete,beckett2017network,narain2008declarative}. Configuration synthesis is concerned with the task of automatically generating router-level configurations given a set of high-level requirements. However, this synthesis problem can be very hard to solve, since network configurations typically consist of a considerable number of tunable parameters, where the execution of several interacting protocols yields the overall forwarding state. An effective synthesis tool must thus account for this fact and be able to reason across multiple protocols.

\paragraph{SMT-based Synthesis} Some of the most successful efforts in providing cross-protocol synthesis capabilities are based on satisfiability modulo theory (SMT) solvers \cite{el2018netcomplete,el2017network}. While SMT-based synthesis is a promising method, it comes with a number of limitations:
% \item protocol-specific
% fully hand-coded synthesis rules, a lot of implementation effort, cross-protocol support extra complicated
(1) SMT-based synthesizers are hand-crafted and highly protocol-specific. To implement synthesis, we must first express our networking model, protocol semantics including vendor and device specific behavior in terms of first-order logic constraints. This is a time-intensive and complicated process, requiring lots of expert knowledge.
%  model-dependent: synthesis is reasoning on the level of some assumed model which may not reflect the real world: even if a configuration is synthesized based on some spec, it may behave differently and violate spec in practice
Further, (2) logic-based modelling introduces a disconnect between the synthesis tool and real-world behavior \cite{birkner2021metha}. More specifically, synthesized configurations may satisfy a provided specification within a formal framework, but may not behave the same way in the real world.
% can be very slow
And, (3) SMT-based synthesis can be very slow or fail to complete, especially when reasoning about large network topologies. In practice however, network operators reconfigure their networks on a daily basis \cite{vissicchio2012improving}, which means an effective synthesis tool must be fast.

% \item fully learned, no hand-coded synthesis rules (model-free), very flexible to adapt to more/new protocols
% \item protocol-agnostic, cross-protocol
\paragraph{Neural Algorithmic Reasoning for Synthesis} Recent work on neural algorithmic reasoning (NAR) proposes to replace traditional algorithms with neural networks to learn improved algorithmic procedures \cite{velivckovic2021neural}.
It has been shown to be a powerful and fast algorithmic approximation method for a number of graph-related \cite{velivckovic2019neural} and combinatorial optimization problems \cite{cappart2021combinatorial}. Further, due to its learned nature, NAR allows for learning procedures directly from (real-world) data, without the need for manual feature extraction. Overall, this positions NAR as an attractive method to obtain a fast, fully-learned synthesis procedure, which entirely avoids the need for a formal model or any hand-crafted synthesis rules. Based on this promising outlook, this paper explores how to apply the NAR paradigm to the problem of network configuration synthesis.

To that end, we propose a \textbf{new learning-based framework for configuration synthesis} as an alternative to SMT-based approaches. Our framework is protocol-agnostic, enables cross-protocol reasoning and avoids the need to manually provide synthesis rules. Instead of implementing the synthesizer explicitly, we replace it by an iterative graph neural network which is trained on input/output samples of specifications, topologies and configurations.
%While our approach still requires some protocol-specific implementation efforts, it is limited to implementing the simulation of the involved protocols.
Our method is highly flexible due to its generic nature and can be extended to any protocol. Further, the synthesizer model learns a whole distribution of network configurations. As a consequence, we can directly sample multiple alternative configurations, not possible with standard SMT solvers. We apply our framework to a non-trivial synthesis setting where both the Border Gateway Protocol (BGP) and the Open Shortest Path First (OSPF) protocol are used. We demonstrate that our learned synthesis tool is up to~$500\times$ faster than a state-of-the-art SMT-based synthesizer, while producing configurations which enjoy more than 90\% satisfaction of the given specification.

\paragraph{Main Contributions} Our core contributions are:
\vspace{-5pt}
\begin{itemize}
    \setlength{\itemsep}{5pt}
    \setlength{\parskip}{0pt}
    \item A learning-based framework for network configuration synthesis based on neural algorithmic reasoning.
    \item A neural network architecture for learning synthesizer models which relies on a generic graph-based encoding of network topologies and configurations.
    \item An extensive evaluation of our learning-based synthesizer, in terms of both precision and scalability, on the challenging setting where both BGP and OSPF protocols are involved.
\end{itemize}

\section{Overview}
\label{sec:overview}

\begin{figure}
    \begin{center}
        \includegraphics[width=0.45\textwidth]{figures/synthesizer-overview.pdf}
    \end{center}
    \caption{An overview of our learning-based synthesis framework.}
    \label{fig:learning-based-synthesis}
\end{figure}

We first discuss the core concepts behind our learning-based synthesis framework, illustrated in \cref{fig:learning-based-synthesis}.

\paragraph{Dataset} To train a synthesizer model, we first generate a dataset of input/output samples. For this, we rely on a generative pipeline as shown in the top of \cref{fig:learning-based-synthesis}. First, we sample a random network configuration for some topology using a uniform generative process. Then, we simulate the involved protocols to obtain the corresponding routing behavior. Next, we extract a specification by randomly selecting properties that hold for the simulated routing behavior. This leaves us with a pair of (specification, configuration) added to a dataset of training~samples.

\paragraph{Simulation} Depending on the protocols in use, one implements simulation code to compute the routing behavior induced by a sampled configuration. Although this step is protocol-specific, the overall implementation effort is much lower compared to SMT-based synthesis. Protocols are typically well-defined algorithms which can be simulated, whereas the alternative of implementing a synthesizer often requires expert knowledge about SMT solvers. In practice, our framework may also be adapted to use a real-world network router to compute the behavior of a configuration, thereby capturing the real-world behavior directly.

\paragraph{Neural Synthesizer Model} Given a dataset of pairs each consisting of a configuration and a specification, we now train a graph neural network on this dataset to perform synthesis: given a specification, it tries to predict the configuration. Following the NAR paradigm, we first encode the synthesizer input (specification) in latent space. Then, we apply an iterative processor network which relies on the graph attention mechanism to propagate information \cite{velivckovic2017graph}. Last, we apply a decoder network to extract the synthesized configuration. To remain protocol-agnostic, our model is generic with respect to the input format, using an intermediate representation based on Datalog-like facts.

%More specifically, we employ a slightly modified variant which operates on a graph-based encoding of a specification, topology and configuration parameters.



 \begin{figure*}
     \centering
     \includegraphics[width=0.85\textwidth]{figures/system-overview.pdf}
     \caption{An overview of our synthesis system: (1) First, we use a generic embedding scheme to transform a network topology, protocol configuration sketches and the specification given as Datalog-like facts to a latent input representation. Next, we apply a learned (2) Processor GNN and obtain a latent synthesis output. Last, we apply a (3) Decoder Network to obtain a distribution over possible values per unknown parameter in our configuration.}
     \label{fig:overview-model}
\end{figure*}

\paragraph{Relaxed Specification Consistency} Parts of the configuration synthesis problems are known to be NP-hard \cite{fortz2000internet}. In contrast, our learning-based framework depends on a fixed-size neural network architecture running in polynomial time. Hence, we expect neural synthesis to be less precise than SMT methods and propose the notion of \emph{relaxed~specification~consistency}. That is, to assess the performance of a neural synthesizer, we not only consider if a configuration satisfies a specification, but also the degree up to which it satisfies a specification (e.g., via the relative number of satisfied requirements). This ``soft'' understanding of a specification allows us to evaluate neural synthesis systems which may not always produce fully specification-consistent configurations. Nonetheless, we argue that configurations with less than $100\%$ consistency are still very useful in practice as they provide a good starting point for further manual adjustment by network operators. Note that a similar adjustment process may also be required with SMT-based synthesizers, due to differences between the formal protocol model and the one running on a given real-world router where the configuration is to be deployed.

Next, we discuss the architecture of our neural synthesis framework. In follow-up sections, we instantiate this framework for the case of BGP/OSPF configuration synthesis, and evaluate the resulting instantiation by comparing it to a state-of-the-art SMT-based synthesizer.

% \begin{itemize}
%     \item effort: need to implement simulation code to generate dataset to learn from (typically well-defined in protocol specs, much easier than implementing synthesis directly)
%     \item can be sampled (multiple alternative solutions, not easily possible with SMT-based methods)
%     \item much faster than SMT-based synthesis
% \end{itemize}

% Requirements:
% \begin{itemize}
%     \item protocol-agnostic
%     \item fully learned, no hand-coded synthesis rules
%     \item define: strict specification vs. relaxed specification
% \end{itemize} 

==> diff/git-latexdiff.34588/old/sections/2_model.tex <==
\section{Neural Synthesis Framework}
\label{sec:model}


We now present the architecture of our graph-based neural synthesizer model, illustrated in \cref{fig:overview-model}. First, in \cref{sec:graph-embedding} we introduce our generic graph-based encoding, which allows us to embed network topologies, protocol configuration and the specification into a latent space. Then, in \cref{sec:graph-transformer} we present the architecture of the processor network which we train to perform the synthesis task. Finally, in \cref{sec:decoding-sampling} we discuss how to sample network configurations from the resulting latent synthesis output.

\begin{figure}
    \begin{minipage}[t]{0.21\textwidth}
    \begin{lstlisting}[basicstyle=\ttfamily\small, escapeinside={(*}{*)}]
router(A)
router(B)
(...)

connected(A,B,2)
connected(A,C,?)(*\blackcircled{1}*)
(...)
    \end{lstlisting}
\end{minipage}
\begin{minipage}[t]{0.21\textwidth}
    \begin{lstlisting}[basicstyle=\ttfamily\small, escapeinside={(*}{*)}]
network(N1)
bgp_route(E,N1,2,3,1,0,1)

fwd(A,B,N1)
not fwd(B,A,N1)
(...)
    \end{lstlisting}
\end{minipage}
    \caption{A snippet of a fact base sketch encoding a network's topology, parameters such as link weights (\texttt{connected} facts) and a specification (\texttt{fwd} facts).}
    \label{fig:datalog-encoding}
\end{figure}

\begin{figure}[t]
    \centering
    \includegraphics[width=0.25\textwidth]{figures/synth-architecture.png}
    \caption{The neural synthesizer model architecture.}
    \label{fig:architecture}
\end{figure}

\subsection{Fact Base Embedding}
\label{sec:graph-embedding}
To remain network protocol-agnostic in our model architecture, we implement a generic graph-based encoding of Datalog-like facts, similar to knowledge graphs \cite{rosso2020beyond}. This means that we first encode topologies, configurations and specifications as a set of Datalog-like facts and then employ a generic embedding.
%We chose Datalog facts as the input format of our synthesis approach for its flexibility, wide-spread use in Program Analysis and use in previous work on configuration synthesis \cite{el2017network}.

\paragraph{Fact Base} A set of Datalog-like facts, as depicted in \cref{fig:datalog-encoding}, serves as the input \emph{fact base} $\mathcal{F}$ to our synthesizer model. $\mathcal{F}$ is a set of facts $f(a_0, \dots, a_n)$ where arguments may be constants (e.g. A or B) or integer literals. Further, each fact in a fact base has a corresponding truth value denoted as $[f(a)]_{\mathcal{B}}$. For instance, from the fact base in \cref{fig:datalog-encoding} we can derive $[fwd(A,B,N1)]_{\mathcal{B}} = \text{\texttt{true}}$ and $[fwd(B,A,N1)]_{\mathcal{B}} = \text{\texttt{false}}$.

\paragraph{Consistency} We represent a network's topology, the protocol configuration and parameters as well as the specification, all in a single fact base. Given the semantics of the protocols in use, we can then check whether the specification encoded in a fact base is satisfied by the provided configuration. To quantify, we define the notion of relaxed specification consistency, as discussed earlier, with respect to a fact base: Given a fact base $\mathcal{F}$, a subset of specification facts $S \subset \mathcal{F}$ and protocol semantics $\mathcal{P}$, the \emph{consistency} of a fact base is defined as the relative number of satisfied facts in $S$ with respect to the routing behavior obtained via $\mathcal{P}$. The contents of $S$ depend on the concrete instantiation of the synthesizer model. For an example of possible specification facts, see our instantiation of the synthesizer model for BGP/OSPF in \cref{sec:training}.

\begin{figure*}
    \def\arraystretch{1.5}
    \begin{tabular}{lr}
        %$T_f: T_1 \times \dots \times T_n$ & \textit{(fact type declaration)}\\
        $emb(f) := \mathbf{V_f}$ & \textit{(learned fact type embedding)}\\
        $emb(b) := \mathbf{W_{\text{bool}}}\;onehot(b)$ & \textit{(learned boolean embedding)}\\
        $emb(f,i,v) := \mathbf{W_{f_i}}\;onehot(v)$ & \textit{(learned integer embedding)}\\
        $emb(f,i,?) := \mathbf{V_{hole}}$ & \textit{(learned hole embedding)}\vspace{10pt}\\
        $\mathlarger{
        h_c := \sum_{f(c) \in \mathcal{F}}
        emb(f)
        }$ & \textit{(constant embedding)}\vspace{10pt}\\
        $h_{f(a_0, \dots, a_n)} := emb(f) + emb([f(a_0, \dots, a_n)]_{\mathcal{B}}) + \mathlarger{
        \sum_{(i,v) \in \mathcal{I}(f(a_0, \dots, a_n))}
        emb(f, i, v)
        }$\hspace{-1.2cm} & \textit{(fact embedding)}\\
        $\mathcal{I}(f(a_0, \dots, a_n)) := \{(i,v) \; | \; f(a_0, \dots, a_{i-1}, v, \dots, a_n) \in \mathcal{F} \wedge v:Int \wedge i \in \mathbb{N}$ \}& \textit{(integer arguments)}\vspace{10pt}\\
        $N_i(h_c) := \{h_f \; | \; \exists i \in \mathbb{N} . f(a_0, \dots, a_{i-1}, c, a_{i+1}, \dots, a_n) \in \mathcal{F}\}$& \textit{(i-th neighborhood of constant node)} \\
        $N_i(h_f) := \{h_c \; | \; \exists i \in \mathbb{N} . f(a_0, \dots, a_{i-1}, c, a_{i+1}, \dots, a_n) \in \mathcal{F}\}$& \textit{(i-th neighborhood of fact node)} \\
    \end{tabular}
    \caption{Translating a fact base $\mathcal{F}$ to node features. $f$ denotes a predicate, $v$ integer values, $b$ boolean values as 0 or 1, $i$ argument indices and $[f(a)]_{\mathcal{B}}$ the truth value of a fact. }
    \label{fig:graph-embedding}
\end{figure*}

%discuss embedding as shown in \cref{fig:datalog-encoding}. Note how this makes fact bases a suitable input to standard GNN architectures.

\paragraph{Fact Base Sketching} In a synthesis setting, we are confronted with incomplete fact bases, i.e. the specification and topology is given but the network configuration is to be synthesized. For these cases, we also consider fact bases with unknown parameters inspired by the idea of program sketching in program synthesis \cite{solar2008program}. More specifically, users may replace an unknown integer argument of a fact by a \texttt{?} symbol, indicating a value to be synthesized. Using this mechanic, we can represent the synthesis input as an incomplete fact base which encodes to-be-synthesized values as unknown parameters. As an example, consider \cref{fig:datalog-encoding} \blackcircled{1}, where the link weight between router nodes \texttt{A} and \texttt{C} is represented as an unknown parameter.

\paragraph{Embedding} We employ a structurally-defined embedding scheme to transform a fact base into a graph with node features as required for processing with graph neural networks. Given a fact base $\mathcal{F}$, we apply the rules in \cref{fig:graph-embedding} to obtain node features and adjacency information. Both a fact $f$ and a constant $c$ are represented as distinct nodes with features $h_c$ and $h_f$, respectively. The relationships between facts and constants is encoded as node adjacency as defined by the neighborhood functions $N_i$.

We use multiple neighborhood functions, i.e. multiple types of edges, to encode the argument position of a constant occurring in a fact. Hence, the number of neighborhood functions corresponds to the maximum number of arguments in a single fact, e.g. 3 in \cref{fig:datalog-encoding}. Integer arguments and unary facts are directly accounted for in the respective node or fact embedding. To handle unknown parameters, we replace the corresponding $emb(...)$ term with the learned $\mathbf{V_{hole}}$ embedding.

Considering the embedding function $emb$, the learned parameters of our embedding are $\mathbf{V_f} \in \mathbb{R}^D$ per fact type in~$\mathcal{F}$, $\mathbf{W_{\text{bool}}} \in \mathbb{R}^{D \times 2}$ for boolean values, $\mathbf{W_{f_i}} \in \mathbb{R}^{D \times N}$ per integer argument of fact type $f$ and $\mathbf{V_{hole}} \in \mathbb{R}^D$ to represent unknown parameters. Hyperparameter $D$ represents the dimension of the latent space the synthesizer model operates in and $N$ specifies the number of supported integer values. An example of applying this embedding scheme to a simple fact base is given in \cref{fig:graph-encoding-example}.

\begin{figure}
    \begin{minipage}[t]{0.2\textwidth}
        \centering
        \footnotesize
        \textbf{Fact Base}
        \begin{lstlisting}[basicstyle=\ttfamily\small]
router(A)
router(B)

conn(A, B, 12)
        \end{lstlisting}
    \end{minipage}
    \begin{minipage}[t]{0.15\textwidth}
        \centering
        \textbf{Graph}\\
        \vspace{5pt}
        \includegraphics[width=0.7\textwidth]{figures/graph-encoding.pdf}
    \end{minipage}\\
    \centering\\
    \vspace{10pt}
    \textbf{Node Features}\\
    \vspace{10pt}
    \begin{minipage}[t]{0.5\textwidth}
        $\begin{array}{rcl}
        h_A &:=& emb(router) = \mathbf{V_{\text{router}}}\\
        h_B &:=& emb(router) = \mathbf{V_{\text{router}}}\\
        h_{\text{conn(A,B,12)}} &:=& emb(conn) + emb(conn, 2, 12)\\
        &:=& \mathbf{V_{\text{conn}}} + \mathbf{W_{conn_2}} onehot(12)
    \end{array}$
    \end{minipage}
    \caption{An example of embedding a simple fact base using the embedding scheme of \cref{fig:graph-embedding}. The shown graph illustrates the neighborhoods $N_0$ and $N_1$ induced by the \texttt{conn} fact.}
    \label{fig:graph-encoding-example}
\end{figure}

\begin{figure}
    $$
    \begin{array}{rcl}
    z_j &:=& h_j + Drop(\mathlarger{\sum_{N_i}} h'_{GAT_i})\\
    h'_j &:=& FFN(Norm(z_j))\vspace{11pt}\\
    FFN(x_j) &:=& Norm(Lin2(Drop(Lin1(x_j)))))
    \end{array}
    $$
    \caption{
        The recurrence relation of a node $j$'s representation $h_j$. $h'_{GAT_i}$ represents the output of a graph attention layer operating with neighborhood $N_i$ according to \cite{velivckovic2017graph}, $h_j$ the representation of node $j$ at the previous step. $Norm$ refers to batch normalization \cite{ioffe2015batch}, $Drop$ to dropout regularization \cite{hinton2012improving} and $Lin1$ and $Lin2$ to linear layers with an inner dimension of $4N$.
    }
    \label{fig:recurrence}
\end{figure}

\subsection{Synthesizer Model}
\label{sec:graph-transformer}

For an illustration of the synthesizer model's architecture, please see Figure~\ref{fig:architecture}. Given a fact base $\mathcal{F}$ we first apply our embedding scheme as described in \cref{sec:graph-embedding}. We then employ a 2-layer GNN-based encoder network to produce the latent representation of a synthesis input.
Given this representation, a processors network is trained to perform the actual synthesis task in high-dimensional space. Last, we apply a set of decoder networks, to obtain the synthesized values of unknown parameter, given the latent synthesis~output.

%In this context, the synthesis problem for network configurations corresponds to completing partially provided fact bases.

% \paragraph{High-Level Architecture}

% We employ the high-level architecture to obtain the latent synthesis output $y_\mathcal{F}$:
% $$
% \begin{array}{rcl}
%     \mathbf{x_{\mathcal{F}}} &:=& Encoder(Embedding(\mathcal{F}))\\
%     \mathbf{y_{\mathcal{F}}} &:=& Processor(\mathbf{x_{\mathcal{F}}} + \mathbf{z})\\
%     z_i &\sim& \mathcal{N}(0,1)
% \end{array}
% $$
% \todo{z is only added for $i<N/2$}

% $Embedding$ corresponds to the graph-based embedding as discussed in \cref{sec:graph-embedding} and $Encoder$ is a 2-layer graph attention module. $Processor$

\paragraph{Encoding} The encoder GNN operates on the embedded representation of a fact base. It produces the high-dimensional representation of a synthesis input as required for the processor network. We additionally apply noise to the first half of the units of the latent representation via $\mathbf{z}$, as a source of non-determinism. According to our experiments this improves model performance and we hypothesize this is due to the synthesis problem having more than one solution in most cases.

\paragraph{Iterative Processor} The processor network is modelled as an iterative process. For this, we apply the same 6-layer graph attention module for a total of 4 iterations.
In the framework of neural algorithmic reasoning, this iterative computational structure encodes an inductive bias towards an iterative solution to the synthesis problem. Because of this bias, our processor network essentially learns an algorithmic procedure which iteratively synthesizes the values of unknown parameters in a fact base.

\paragraph{Graph Attention Layer} In the GNNs we employ, we rely on a composed variant of the graph attention layer as introduced by \cite{velivckovic2017graph}. We employ multiple graph attention layers in lockstep, one per neighborhood $N_i$ defined by our graph embedding (cf. \cref{sec:graph-embedding}), and combine the intermediate results after each step. Specifically, the recurrence relation of a node $j$'s representation $h_j$ is defined as shown in \cref{fig:recurrence}. These mechanics of combining the results of the different graph attention layers $h'_{GAT_i}$, directly corresponds to how multiple attention heads are combined in the original Transformer architecture \cite{vaswani2017attention}.

\paragraph{Argument Decoder Networks} To synthesize the values of unknown parameters, the model maintains a set of decoder networks. That is, it provides one decoder network per integer argument per fact type in a fact base. When decoding, the network is applied to the latent synthesis output of the corresponding fact node. For example, a synthesizer model which operates on the fact base in \cref{fig:graph-encoding-example}, would provide a decoder network $D_{\text{conn}_2}: \mathbb{R}^D \rightarrow \mathbb{R^N}$ to decode values for the third argument of a \texttt{conn} fact. In our experiments, decoder networks are implemented as simple multi-layer perceptron models.

%The synthesizer model learns a conditional distribution of fact bases which are consistent with respect to the protocols' semantics.

%\todo{introduce synthesis as a completion problem of an encoded fact base (a la BERT). Introduce masking, introduce decoding of integer and truth values. Synthesis is learning a conditional distribution of consistent fact bases.}

%Using this method, we obtain the node features $h_c$ per constant, $h_f$ per fact and adjacency information in terms of node neighborhood functions $N_i(h_c)$ and $N_i(h_f)$. Overall, this encoding makes a fact base suitable for processing using standard graph neural networks.

%- Brief description of the Graph Transformer Model
\subsection{Multi-Shot Sampling}
\label{sec:decoding-sampling}

%Multi-Stage Parameter Sampling (sampling methods: topk, high-temp, low-temp)
To sample concrete values from the output distributions over unknown parameters, we apply a multi-shot sampling strategy. That is, we sample values only for a subset of unknown parameters, insert them in our input fact base and run the synthesis model again. We repeat this process until no more unknown parameters remain. This multi-shot sampling strategy allows the model to incorporate the concrete values of previously synthesized parameters in its computation. In our evaluation in \cref{sec:evaluation}, we include a comparison of how this compares to sampling all unknown parameters at once.

%In a fact base with multiple holes, we apply the corresponding decoder networks to obtain a value distribution for each integer hole. However, instead of sampling all integer holes in one


==> diff/git-latexdiff.34588/old/sections/3_bgp_ospf.tex <==
\section{BGP/OSPF Synthesis}
\label{sec:bgp-ospf}

\newcommand{\as}{\ac{AS}~}
\newcommand{\ases}{\acp{AS}~}

\newcommand{\squareann}{{\tiny$\blacksquare\;$}}
\newcommand{\triangleann}{{\small$\blacktriangle\;$}}

\begin{figure*}
    \centering
    \includegraphics[width=0.95\textwidth]{figures/networks-all.pdf}
    \caption{(a) An illustration of a small AS network, including internal peers (blue), external peers (purple), BGP sessions as well as physical links. (b) The propagation of two BGP announcement across the network. (c) The resulting forwarding plane after applying BGP and OSPF.}
    \label{fig:network-fwd-tree}
\end{figure*}

We now discuss an instantiation of our learning-based framework for the case of BGP and OSPF protocols. In \cref{sec:synthesis-setting} we introduce a basic networking model, BGP and OSPF protocols and the synthesis setting. Given this model, \cref{sec:training} describes how to generate a corresponding dataset of input/output samples and train a synthesizer model.
%This shall serve as a prerequisite to the instantiation of our learning-based synthesis framework for the BGP and OSPF protocol in \cref{sec:training}.

\subsection{Synthesis Setting}
\label{sec:synthesis-setting}

\paragraph{Graphical Model} We assume an abstract network model which can be represented as an undirected graph as shown in \cref{fig:network-fwd-tree} (a). We always consider a set of internal routers (A, B, C, D in \cref{fig:network-fwd-tree}) as well as a set of adjacent external routers (E, F  in \cref{fig:network-fwd-tree}). The group of internal routers forms the \emph{\as} under consideration whereas external routers belong to other adjacent \ases. In practice, an \as represents an administrative domain controlled by a single operator.

\paragraph{Forwarding Plane} We focus on the \emph{forwarding plane} of a network. This means we are interested in how a router forwards packets given incoming traffic of different traffic classes. For this, each router maintains a routing table which determines which of its outgoing edges is used to forward packets of a certain traffic class. As an example, consider \cref{fig:network-fwd-tree} (c) which illustrates the forwarding plane of some traffic class reachable via external peer $E$ or $F$ in our example network. Each router of the network forwards traffic along some of its outgoing links. In practice, a number of protocols are used to populate a router's routing tables. For the instantiation of our synthesis framework however, we focus on OSPF and BGP.

\paragraph{OSPF} The OSPF protocol \cite{moy1994ospf} is a link-state protocol, typically used as an interior gateway protocol~(IGP), i.e., to route traffic within an \ac{AS}. Given link weights per physical link in the network, OSPF simply routes traffic along the shortest path towards the destination.

\paragraph{BGP} The BGP protocol \cite{rekhter1994border} on the other hand is a path-vector protocol used to exchange reachability information mostly on the level of \acp{AS}.
%These are groups of routers typically operated by a single party (e.g. an ISP).
When using BGP, a routing destination announces its existence to other \ases and routers, by sending out a BGP announcement. Receivers of such announcements may then choose to pass them on to other \acp{AS}, redistribute them internally and/or modify them. Instead of communicating along physical links directly, the BGP protocol requires manually configured BGP sessions among routers of the \as and external peers, as indicated by the BGP session edges in \cref{fig:network-fwd-tree}(a).
%\todo{more discussion of eBGP vs iBGP and support for route reflection (more of an implementation detail, maybe only mention in dataset generation where simulation code is discussed)}.

%\paragraph{BGP Decision Procedure}~
%\todo{discuss decision procedure}
In case a router receives more than one announcement for a destination, a designated BGP decision process is applied to determine a single best route. \cref{fig:bgp-decision} shows the ordered list of comparison criteria of this decision process. The different criteria depend different properties of a route announcements, including the IGP cost towards the routing destination. As a consequence, when used together, OSPF as IGP protocol and BGP will interact. %Note also that BGP is an iterative process which needs multiple rounds of propagation to converge.

\paragraph{Example}
%\todo{run through simple BGP+OSPF example of computing the forwarding plane}
To better understand BGP/OSPF routing, consider the simple example given in \cref{fig:network-fwd-tree} (b). Here, our example \as imports BGP announcements \squareann and \triangleann from E and F respectively. Both represent a route to the same destination. As shown, both announcements have a so-called local preference of 2. For simplicity, we ignore other properties such as the AS path length, Origin and MED in this example. The announcements are propagated among BGP neighbors and the best route is selected according to the decision procedure in \cref{fig:bgp-decision}. See \cref{fig:network-fwd-tree} (b) for an illustration of the intermediate states of this propagation process. As both announcements have a local preference of 2, rule 1 of the decision process is not used. Instead, in round 2, node B selects \squareann over \triangleann due to a lower IGP cost of 2 via egress node A as compared to 3 via egress node D (rule 6). Node D selects \triangleann over \squareann, since it learns this route directly from an external peer (rule 5). After Round 3, the BGP propagation process converges to a stable state and we can derive the forwarding plane as shown in \cref{fig:network-fwd-tree} (c).


%, as well as external peers E and F which belong to other \acp{AS}. External peers are routers which are connected via eBGP sessions to routers of the \ac{AS} under consideration. They announce BGP routes to their neighbors, which are propagated within the network

\paragraph{Problem Statement: Configuration Synthesis} We phrase the BGP/OSPF configuration synthesis problem on the level of the forwarding plane. This means that users provide a specification which constraints the set of allowed forwarding planes. This includes predicates which enforce forwarding paths, block forwarding paths or assert higher-level properties like traffic isolation and reachability. Given such a specification, we consider network configuration synthesis as the task of configuring OSPF and BGP in a way that produces a forwarding plane which satisfies the provided specification.

\paragraph{Search Space} To limit the space of candidate configurations, we define the set of synthesized parameters: For OSPF we synthesize link weights as explored in a wide range of existing work (e.g. \cite{el2018netcomplete,fortz2000internet}. BGP parameters on the other hand are not defined as clearly: Depending on the requirements of a network operator, one may employ custom BGP import and export policies at every router of a network to implement complex behavior. However, in this work we focus on a simplified setting, where we assume BGP route announcements to only be modified when imported into the \as from an external peer. Previous work has already pointed out that this is a reasonable assumption which holds for the majority of real-world networks \cite{caesar2005bgp,cittadini2010doing, steffen2020probabilistic}.

\begin{figure}
    \small{
    \begin{enumerate}
        \setlength{\itemsep}{0pt}
        \setlength{\parskip}{0pt}
        \item Highest Local preference
        \item Lowest AS path length
        \item Prefer Origin (IGP $>$ EBGP $>$ INCOMPLETE)
        \item Lowest Multi-exit discriminator (MED)
        \item External over internal announcements
        \item Lowest IGP cost to egress
        \item Lowest BGP peer id (tie breaker)
    \end{enumerate}}
    \vspace{-15pt}
    \caption{The BGP decision process \cite{rekhter1994border}. The shown rules are applied in order until a single best BGP announcements remains.}
    \label{fig:bgp-decision}
\end{figure}

\subsection{Dataset Generation and Training}
\label{sec:training}
To train a synthesizer model, we need a large number of fact bases encoding a variety of network topologies, configurations and forwarding specifications. Further, we must provide the model with target values for unknown parameters as a supervision signal. This section discusses how we construct such a dataset for BGP/OSPF synthesis.
%Further, we provide an example of what a corresponding fact base looks like, including a description of the supported specification language.

\paragraph{Dataset Generation} To obtain network configurations and corresponding forwarding specifications we employ a generative process: We first randomly configure BGP and OSPF parameters for some topology. Then we simulate the OSPF and BGP protocol and compute the resulting forwarding plane. Based on this, we extract a forwarding specification which fixes a random subset of forwarding paths, reachability and isolation properties that are satisfied by the forwarding plane.

\paragraph{Topologies} For training, our dataset is based on random topologies with $16$-$24$ routers. We generate the physical layout of these graphs by triangulation of uniformly sampled points in two-dimensional space.

\paragraph{Simulation} To compute the forwarding plane given an OSPF and BGP configuration, we simulate the protocols. For OSPF, we implement shortest path computation to obtain the forwarding plane. For BGP, we implement the full BGP decision process as shown in \cref{fig:bgp-decision}, except for the MED attribute. In addition to the basic networking model discussed in \cref{sec:synthesis-setting}, we implement support for eBGP and iBGP, fully-meshed BGP session layouts as well as layouts relying on route reflection. For more details of these BGP concepts see \cite{bates2000rr}.

%Note that the synthesizer model will reason on the level of the provided training samples. That is, to improve the overall synthesis quality in a real-world setting, it is helpful to implement simulation code which behaves very similar to real-world networks. Another promising approach would be to extract training samples from real-world networks, thereby circumventing the need for simulation, however, we leave this as future work.

%While this can be a considerable effort, it is typically an easier task than to implement the synthesizer directly. The concrete semantics of protocols and their simulation is a well-defined procedure, whereas implementing efficient synthesis tools is still an open problem.

\paragraph{Fact Base Encoding} We encode synthesis input using a small set of facts. For an example of a corresponding fact base see \cref{fig:bgp-ospf-fact-base}. We use the \texttt{router}, \texttt{external} and \texttt{network} facts to mark routers, external peers and routing destinations respectively. Physical links between routers are encoded as \texttt{connected(R1,R2,W)} facts where \texttt{W} denotes the OSPF link weight. Further, we rely on \texttt{ibgp}, \texttt{ebgp}, \texttt{route\_reflector} and \texttt{bgp\_route} facts to represent different types of BGP sessions and imported routes. Using the notion of unknown parameters as discussed in \cref{sec:graph-embedding}, we encode configuration parameters, e.g., properties of imported routes or OSPF link weights.

\paragraph{Specification Language} We support a small specification language with three types of forwarding predicates:

\begin{itemize}
    \setlength{\itemsep}{0pt}
    \setlength{\parskip}{2pt}
    \item \texttt{fwd(R1, Net, R2)} specifies that router \texttt{R1} forwards traffic destined for \texttt{Net} to its neighbor \texttt{R2}.
    \item \texttt{reachable(R1, Net, R2)} specifies that traffic destined for \texttt{Net} that passes through \texttt{R1} also passes through \texttt{R2} before reaching its destination.
    \item \texttt{trafficIsolation(R1, R2, N1, N2)} specifies that it must not hold that $[fwd(R1,R2,N1)]_{\mathcal{B}} \wedge [fwd(R1,R2,N2)]_{\mathcal{B}}$.
\end{itemize}

In the negative case of each predicate, the opposite must hold true for the fact to be satisfied. This specification language can easily be extended by including new specification predicates in the dataset generation process. One must simply provide a method of extracting positive and negative cases of a specification fact from a given forwarding plane. Once included in the training dataset of a synthesizer model, the resulting synthesis system will be able to consider specifications relying on the new type of predicates.

% \todo{info on loss function, optimizer, etc.}
\paragraph{Training} We generate a dataset of $10,240$ input/output samples and instantiate our synthesizer model with a hidden dimension $D$ of $64$. For optimization, we use the Adam optimizer \cite{kingma2014adam} with a learning rate of $10^{-4}$, applying negative log-likelihood loss to the decoder networks' outputs. We stop training after the specification consistency on a validation dataset no longer increases at around $\sim2800$ epochs.

\begin{figure}
\begin{minipage}[t]{0.22\textwidth}
\begin{lstlisting}[basicstyle=\ttfamily\tiny]
# topology and configuration
router(c5)
router(c3)
router(c1)
router(c0)
network(c6)
network(c7)

external(c8)
external(c9)
external(c10)
external(c11)
external(c12)
external(c13)

route_reflector(c2)
route_reflector(c4)

connected(c2,c4,?)
connected(c2,c5,?)
connected(c2,c3,?)
connected(c4,c5,?)
connected(c4,c3,?)
connected(c4,c0,?)
connected(c5,c1,?)
connected(c5,c0,?)
connected(c3,c0,?)
connected(c3,c1,?)
connected(c1,c0,?)

ibgp(c2,c4)
ibgp(c2,c5)
ibgp(c2,c0)
ibgp(c2,c1)
ibgp(c4,c3)
ibgp(c4,c4)
\end{lstlisting}
\end{minipage}
\begin{minipage}[t]{0.2\textwidth}
\begin{lstlisting}[basicstyle=\ttfamily\tiny]
ebgp(c2,c12)
ebgp(c5,c9)
ebgp(c5,c10)
ebgp(c5,c13)
ebgp(c0,c8)
ebgp(c0,c11)

bgp_route(c8,c6,?,?,1,?,1,8)
bgp_route(c9,c6,?,?,0,?,1,9)
bgp_route(c10,c6,?,?,0,?,1,10)
bgp_route(c11,c7,?,?,0,?,1,11)
bgp_route(c12,c7,?,?,0,?,1,12)
bgp_route(c13,c7,?,?,2,?,1,13)

# forwarding specification
fwd(c0,c6,c3)
fwd(c3,c6,c2)
fwd(c2,c6,c4)
not fwd(c3,c6,c0)
not fwd(c0,c6,c11)
not fwd(c11,c6,c0)

not trafficIsolation(c1,c0,c7,c6)
not trafficIsolation(c1,c0,c7,c6)
trafficIsolation(c0,c3,c6,c7)
trafficIsolation(c0,c3,c6,c7)

reachable(c5,c6,c10)
reachable(c1,c6,c4)
not reachable(c0,c6,c5)
reachable(c5,c6,c10)
\end{lstlisting}
\end{minipage}
\caption{An example of a fact base encoding a topology, a sketch of a BGP and OSPF configuration and a forwarding specification.}
\label{fig:bgp-ospf-fact-base}
\end{figure} 

==> diff/git-latexdiff.34588/old/sections/4_evaluation.tex <==
\section{Evaluation}
\label{sec:evaluation}

We trained a synthesizer model to perform configuration synthesis for BGP and OSPF. We now assess the performance of the resulting neural synthesizer with respect to two core metrics: (1) the quality of synthesized configurations in terms of their consistency with the provided forwarding specifications (\cref{sec:synthesis-quality}), and (ii) the time a learned synthesizer takes when compared to the state-of-the-art SMT-based synthesizer NetComplete \cite{el2018netcomplete} (\cref{sec:synthesis-vs-smt}).

\paragraph{Dataset} We compare across three datasets: Small, Medium and Large. Each dataset represents 8 real-world topologies, sampled from the Topology Zoo \cite{knight2011internet}, where the number of nodes lies between 0-34, 34-68 and 68-170 respectively. To obtain forwarding specifications for the sampled topologies, we use our generative pipeline as discussed in \cref{sec:training}. In each topology, we do synthesis for 4 different traffic classes (routing destinations) at a time.

\paragraph{Experimental Setup} We run all our experiments on an Ubuntu Linux machine with an Intel(R)~Core(TM)~i9-9900X~@~3.50GHz processor, 64GB of system memory and an NVIDIA GeForce RTX 3080 GPU with 10GB of video~memory.

\subsection{Synthesis Quality}
\label{sec:synthesis-quality}
To assess our learned synthesizer, we examine its behavior with increasingly large topologies and specifications.

\paragraph{Specifications} Using the same generative model as described in \cref{sec:training}, we generate forwarding specifications for the topologies in our three datasets with each specification constructed from $3 \times n$ requirements, one per supported predicate type:  \texttt{fwd} requirements correspond to specifying or blocking a forwarding path using multiple \texttt{fwd} predicates whereas \texttt{reachable} and \texttt{trafficIsolation} requirements each translate to a single specification fact. We compare across increasingly large specifications of $3\times 2$, $3\times 8$ and $3 \times 16$ requirements, respectively.

\paragraph{Methodology} For each pair of topology and specification, we run our synthesizer 5 times and report the network configurations with the highest overall consistency value. For sampling, we rely on our multi-shot sampling strategy where we randomly group the unknown parameters of a configuration into 4 groups (4-shot sampling).

\paragraph{Results} We summarize our results in \cref{fig:eval-consistency}. On average, our synthesis model produces network configurations that are $>91\%$ consistent with the provided forwarding specifications across all datasets and sizes of specifications. When only few requirements are given, the synthesizer model even succeeds in producing fully-consistent configurations. We observe a slightly decreasing consistency with increasingly large topologies.

%\texttt{fwd} facts are satisfied more easily, whereas \texttt{reachable} and \texttt{trafficIsolation} facts are violated more often.

\paragraph{Multi-Shot Sampling} In \cref{fig:eval-consistency-baseline}, we report the average specification consistency using our multi-shot sampling strategy as compared to sampling all unknown parameters at once. As a baseline we have also sampled random configurations from a uniform distribution (per parameter) and compute the corresponding specification consistency. Over the baseline, our synthesizer model shows clear improvement and multi-shot sampling further increases consistency.

\begin{figure*}
    \begin{center}
        \textbf{Specification Consistency}\\
        \footnotesize
        \begin{tabular}{rrcccccccccc}
        \toprule
        \multicolumn{2}{c}{Dataset} & \tiny\texttt{fwd} & \tiny\texttt{reachable}  & \tiny\texttt{trafficIsolation} & Overall & $\emptyset$     No. Full Matches & $\emptyset$ No. $>90\%$ Matches\\
        \midrule
        $3\times 2$ requirements & Small & 0.95 & 0.94 & 1.00 & \textbf{0.95} & 0.62 & 0.62\\
& Medium & 0.96 & 1.00 & 0.94 & \textbf{0.96} & 0.88 & 0.88\\
& Large & 0.94 & 0.94 & 1.00 & \textbf{0.93} & 0.62 & 0.62\\
\midrule
$3\times 8$ requirements & Small & 0.97 & 0.98 & 0.97 & \textbf{0.98} & 0.50 & 1.00\\
& Medium & 0.99 & 0.95 & 1.00 & \textbf{0.98} & 0.50 & 1.00\\
& Large & 0.96 & 0.95 & 0.91 & \textbf{0.94} & 0.38 & 0.88\\
\midrule
$3\times 16$ requirements & Small & 0.97 & 0.89 & 0.95 & \textbf{0.94} & 0.38 & 0.75\\
& Medium & 0.98 & 0.97 & 0.97 & \textbf{0.98} & 0.38 & 1.00\\
& Large & 0.92 & 0.88 & 0.95 & \textbf{0.91} & 0.12 & 0.50\\
    \end{tabular}\end{center}
    \caption{Average specification consistency of the network configurations synthesized by our trained synthesizer model. Per sample we run the synthesizer with a specification of $3\times N$ requirements, where the specifications always include $N$ requirements per supported predicate type (\texttt{fwd}, \texttt{reachable}, \texttt{trafficIsolation}).}
    \label{fig:eval-consistency}
\end{figure*}

\begin{figure}
    \begin{center}
        \footnotesize
        \begin{tabular}{rrcccccccccc}
        &  & \multicolumn{2}{c}{Neural}\\
        & Random & 1-Shot & 4-shot\\
        \toprule
        Small & 0.83 & 0.92 & \textbf{0.94} \\
        Medium & 0.88 & 0.95 & \textbf{0.98} \\
        Large & 0.78 & 0.88 & \textbf{0.91} \\
    \end{tabular}\end{center}
    \caption{Average specification consistency with $3\times 16$ requirements when sampling configurations randomly from a uniform distribution and 1-shot/4-shot sampling using our synthesizer model.}
    \label{fig:eval-consistency-baseline}
\end{figure}

\begin{figure*}[ht]
    \footnotesize
    \begin{center}
        \textbf{BGP Synthesis Time}
        \footnotesize
        \begin{tabular}{rrccccccccc}
        \toprule
        &&\multicolumn{3}{c}{Synthesis Time (s)} & \multicolumn{2}{c}{Accuracy (Neural)} \\
        \multicolumn{2}{l}{\# Requirements} & NetComplete & Neural (CPU) & Speedup &$\emptyset$ Consistency& $\emptyset$ No. Full Matches\\
        \midrule
    2 requirements &Small & 18.073s & 0.641s & \textbf{28.2x} & 0.969 & 0.875\\
        &Medium & 60.864s & 2.748s & \textbf{22.2x} & 0.939 & 0.75\\
        &Large & 1389.485s\tiny{  7/8 TO} & 22.301s & \textbf{62.3x} & 0.989 & 0.875\\
    \midrule
    8 requirements &Small & 247.691s & 1.065s & \textbf{232.5x} & 0.96 & 0.75\\
        &Medium & $>$25m\tiny{  8/8 TO} & 3.47s & \textbf{432.2x} & 0.968 & 0.5\\
        &Large & $>$25m\tiny{  8/8 TO} & 30.961s & \textbf{48.4x} & 0.969 & 0.75\\
    \midrule
    16 requirements &Small & 1416.828s\tiny{  7/8 TO} & 2.528s & \textbf{560.5x} & 0.926 & 0.25\\
        &Medium & $>$25m\tiny{  8/8 TO} & 5.481s & \textbf{273.7x} & 0.947 & 0.25\\
        &Large & $>$25m\tiny{  8/8 TO} & 69.092s & \textbf{21.7x} & 0.959 & 0.25\\
    \end{tabular}\end{center}
    \caption{Comparing consistency and synthesis time of our method (Neural) with the SMT-based state-of-art synthesis tool NetComplete. The notation {\tiny{n/8 TO}} indicates the number of timed out synthesis runs out of 8 (25+ minutes).}
    \label{fig:evaluation-compare-bgp}
\end{figure*}

\begin{figure*}[ht]
    \begin{center}
        \footnotesize
        \textbf{OSPF Synthesis Time}\\
        \footnotesize
        \begin{tabular}{rrccccccccc}
        \toprule
        &&\multicolumn{3}{c}{Synthesis Time (s)} & \multicolumn{2}{c}{Accuracy (Neural)} \\
        \multicolumn{2}{l}{} & NetComplete & Neural (GPU) & Speedup &$\emptyset$ Consistency& $\emptyset$ No. Full Matches\\
        \midrule
    2 requirements &Small & 0.265s & 0.091s & \textbf{2.9x} & 1.000 & 1.00\\
     &Medium & 0.404s & 0.098s & \textbf{4.1x} & 1.000 & 1.00\\
     &Large & 0.944s & 0.14s & \textbf{6.7x} & 1.000 & 1.00\\
    \midrule
    8 requirements &Small & 0.876s & 0.164s & \textbf{5.3x} & 0.982 & 0.75\\
     &Medium & 1.517s & 0.103s & \textbf{14.7x} & 1.000 & 1.00\\
     &Large & 3.505s & 0.316s & \textbf{11.1x} & 0.981 & 0.50\\
    \midrule
    16 requirements &Small & 1.65s & 0.21s & \textbf{7.9x} & 0.991 & 0.625\\
     &Medium & 2.646s & 0.245s & \textbf{10.8x} & 0.989 & 0.50\\
     &Large & $>$566.636s+\tiny{  3/8 TO} & 0.233s & \textbf{2430.4x} & 0.987 & 0.875\\
    \end{tabular}\end{center}
    \caption{Comparing consistency and synthesis time of our method (Neural) with the SMT-based OSPF synthesis tool NetComplete. The notation {\tiny{n/8 TO}} indicates the number of timed out synthesis runs out of 8 (25+ minutes).}
    \label{fig:evaluation-compare-ospf}
\end{figure*}


\subsection{Comparison to SMT-based Synthesis}
\label{sec:synthesis-vs-smt}

%To provide a comparison of our learned BGP/OSPF synthesizer with SMT-based methods,
We now compare the synthesis time of the learned neural synthesizer with those of NetComplte, a state-of-art configuration synthesis tool based on SMT-solvers \cite{el2018netcomplete}.

\paragraph{Specifications} As the type of supported requirements in NetComplete does not fully align with our model, we restrict this comparison to specifications which only include forwarding paths (i.e. \texttt{fwd} predicates). Further, NetComplete does not support cross-protocol synthesis as in our case and instead requires users to specify for each requirement the protocol to use for its implementation. To bridge this gap, we split the generated forwarding requirements into BGP and OSPF paths for a corresponding NetComplete specification.
%\todo{note on NetComplete installing policies at all routers, not only the edges of the AS}

\paragraph{Methodology} We compare both OSPF synthesis and BGP/OSPF-synthesis. We configure our trained synthesizer model to do OSPF synthesis by only predicting link weights. For each pair of topology and specification, we report the total time of running our synthesizer 4 times using 4-shot sampling, whereas for consistency we report the best out of the 4 runs. For NetComplete, we run the synthesizer with a timeout of 25 minutes. In case a NetComplete attempt times out, we report 25 minutes as a lower bound for its runtime.

\paragraph{OSPF Synthesis Time Results} We document the results of comparing OSPF synthesis time in \cref{fig:evaluation-compare-ospf}. Our synthesizer model achieves a speedup of 2-10x over NetComplete. With 16 requirements and dataset Large this speedup even increases to $2000\times$. Further, our model achieves very high consistency with the provided specification, often producing fully-consistent configurations.

\paragraph{BGP/OSPF Synthesis Time Results} In \cref{fig:evaluation-compare-bgp} we show the comparison of BGP/OSPF synthesis time. Our synthesizer model outperforms NetComplete by multiple orders of magnitude. We observe a speedup of $20-560\times$ which appears to increase with the size of topology and specification. Further, the average specification consistency of the synthesized configurations is greater than $92\%$ across all datasets, even for large topologies. In many cases, our synthesizer model produces fully-consistent configurations, especially with small topologies and specifications. In comparison, NetComplete times out on more than half of the synthesis tasks which means that we can only observe a lower bound of speedup in these cases. Note that our synthesizer model is running on a CPU due to memory restrictions with large topologies. However, running it on a GPU results in even greater speedups (up to $1000\times$, cf. \cref{app:sec:bgp-gpu-performance}). 

==> diff/git-latexdiff.34588/old/sections/5_related_work.tex <==
\section{Related Work}
\label{sec:related-work}

\paragraph{Traditional Configuration Synthesis} 
%A range of existing work is concerned with network configuration synthesis. 
Next to methods based on compilation such as Propane/PropaneAT \cite{beckett2017network}, there are a number of configuration synthesis methods based on constraint solving: Examples include ConfigAssure \cite{narain2008declarative}, SyNet \cite{el2017network} and NetComplete \cite{el2018netcomplete}. Due to their hand-coded nature, these methods are highly protocol-specific and can be very slow due to the solvers they employ. Although some of them allow for cross-protocol reasoning, this is not implemented as transparently as in our framework and users must specify per requirement which protocol to use for its implementation. In contrast, our approach has lower precision but allows for fully transparent cross-protocol reasoning, meaning forwarding requirements are not protocol-bound and the synthesizer chooses how to implement them. Further, our learned BGP/OSPF synthesis tool exhibits much lower synthesis times as compared to an SMT-based tool like NetComplete.

% \begin{itemize}
%     \item NetComplete, SyNet
%     \item Propane, PropaneAT
%     \item DeepBGP
% \end{itemize}

\paragraph{GNNs and Networking} DeepBGP \cite{bahnasy2020deepbgp} relies on GNNs and reinforcement learning to do configuration synthesis. However, it is limited to BGP configuration synthesis and is slower than SMT-based synthesis according to the author's evaluation. In contrast, our learning-based framework is cross-protocol, does not rely on reinforcement learning and provides better synthesis performance. Apart from configuration synthesis, GNNs have also been applied to other problems in the networking domain. For example, the authors of RouteNet \cite{rusek2020routenet} use GNNs to predict performance metrics of network configurations. Other work that is concerned with learning improved protocols includes Q-Routing \cite{boyan1994packet} or more modern approaches such as the Graph-Query Neural Network architecture \cite{geyer2018learning}.

\paragraph{Neural Algorithmic Reasoning} 
Neural algorithmic reasoning (NAR) as proposed in \cite{velivckovic2021neural}, describes the idea of replacing traditional algorithms with neural networks to learn improved algorithmic procedures. Exemplary work includes graph-related algorithms \cite{velivckovic2019neural} or solvers for combinatorial optimization problems \cite{cappart2021combinatorial,joshi2020learning,selsam2019guiding}. Our synthesis framework is the first applications of NAR to the networking domain and relies on the NAR-native encode-process-decode architecture. According to the hierarchy of NAR approaches in \cite{cappart2021combinatorial}, our method is an algorithm-level approach, as we do not supervise on intermediate steps. Although, such step-level methods promise better generalization, it is not clear what an intermediate result of a general synthesis procedure would be. However, future work on a step-level approach may further improve synthesis quality.

% \begin{itemize}
%     \item RouteNet
%     \item GraphNET
%     \item Learning and generating distributed routing protocols using graph-based deep learning
%     \item Unveiling the potential of Graph Neural Networks for network modeling and optimization in SDN
% \end{itemize}

==> diff/git-latexdiff.34588/old/sections/6_conclusion.tex <==
\setlength{\parskip}{6pt plus4mm minus4mm}
\section{Conclusion}
\label{sec:conclusion}
We presented a learning-based framework for configuration synthesis based on the idea of neural algorithmic reasoning. To assess the effectiveness of the system, we instantiated it for the case of BGP/OSPF synthesis. In contrast to traditional synthesis methods, our system supports transparent cross-protocol reasoning and learns synthesis rules only from data. Using our system, synthesis is sped up by a factor of up to $500\times$ when compared to SMT-based methods. Further, our evaluation demonstrates that the resulting synthesis tool provides excellent synthesis quality, producing configurations with high specification consistency. Overall, our results illustrate that exploring the direction of learning-based network configuration synthesis is a promising direction, enabling new cross-protocol reasoning capabilities and great performance improvements. Promising future work includes construction of hybrid systems, integrating both neural models and SMT-based approaches to obtain the best of both worlds.

==> diff/git-latexdiff.34965/new/acronyms.tex <==
\DeclareAcronym{AS}{
    short = AS,
    long = autonomous system,
    short-plural = es ,
    long-plural = s
}

==> diff/git-latexdiff.34965/new/sections/0_abstract.tex <==
% Context
Computer networks employ a number of different protocols to enable efficient routing. However, due to the complexity of multiple interacting protocols, it can be hard for network operators to implement high-level routing policies and requirements. Network configuration synthesis promises to address this situation by automatically generating configurations that satisfy a provided specification. However, existing synthesis methods are often limited to single-protocol reasoning, depend on protocol-specific and hand-coded synthesis rules, and are difficult to scale due to the SMT-based methods they employ. In this work we present a rather different, learning-based method for addressing the configuration synthesis challenge, one based on the recently proposed paradigm of neural algorithmic reasoning. Our framework is protocol-agnostic, enables cross-protocol reasoning and does not depend on any hardcoded synthesis rules. To evaluate, we instantiate our framework for the case of BGP/OSPF synthesis. Our experiments show we can synthesize configurations with a very high degree of specification consistency while observing speedups of up to $500\times$ compared to a state-of-the-art SMT-based synthesis tool.


==> diff/git-latexdiff.34965/new/sections/1_intro.tex <==
\section{Introduction}
\label{sec:introduction}

The backbone of the internet consists of many connected computer networks operated by different internet service providers (ISPs) and other large organizations. These networks rely on a number of protocols to enable effective and policy-driven routing of traffic. Based on router-level configurations, the protocols perform a distributed computation to construct a network's forwarding state. However, the relatively low-level router configuration makes it hard for network operators to directly enforce network-wide policies and requirements. This often leads to misconfiguration, which can cause global outages such as the recent hours-long blackout of the entire Facebook platform \cite{janardhan2021} and comparable events \cite{mccarthy_2019}.
%
\paragraph{Configuration Synthesis} This situation has triggered a number of research efforts regarding the synthesis of network configurations \cite{el2018netcomplete,beckett2017network,narain2008declarative}. Configuration synthesis is concerned with the task of automatically generating router-level configurations given a set of high-level requirements. However, this synthesis problem can be very hard to solve, since network configurations typically consist of a considerable number of tunable parameters, where the execution of several interacting protocols yields the overall forwarding state. An effective synthesis tool must thus account for this fact and be able to reason across multiple protocols.

\paragraph{SMT-based Synthesis} Some of the most successful efforts in providing cross-protocol synthesis capabilities are based on satisfiability modulo theory (SMT) solvers \cite{el2018netcomplete,el2017network}. While SMT-based synthesis is a promising method, it comes with a number of limitations:
% \item protocol-specific
% fully hand-coded synthesis rules, a lot of implementation effort, cross-protocol support extra complicated
(1) SMT-based synthesizers are hand-crafted and highly protocol-specific. To implement synthesis, we must first express our networking model, protocol semantics including vendor and device specific behavior in terms of first-order logic constraints. This is a time-intensive and complicated process, requiring lots of expert knowledge.
%  model-dependent: synthesis is reasoning on the level of some assumed model which may not reflect the real world: even if a configuration is synthesized based on some spec, it may behave differently and violate spec in practice
Further, (2) logic-based modelling introduces a disconnect between the synthesis tool and real-world behavior \cite{birkner2021metha}. More specifically, synthesized configurations may satisfy a provided specification within a formal framework, but may not behave the same way in the real world.
% can be very slow
And, (3) SMT-based synthesis can be very slow or fail to complete, especially when reasoning about large network topologies. In practice however, network operators reconfigure their networks on a daily basis \cite{vissicchio2012improving}, which means an effective synthesis tool must be fast.

% \item fully learned, no hand-coded synthesis rules (model-free), very flexible to adapt to more/new protocols
% \item protocol-agnostic, cross-protocol
\paragraph{Neural Algorithmic Reasoning for Synthesis} Recent work on neural algorithmic reasoning (NAR) proposes to replace traditional algorithms with neural networks to learn improved algorithmic procedures \cite{velivckovic2021neural}.
It has been shown to be a powerful and fast algorithmic approximation method for a number of graph-related \cite{velivckovic2019neural} and combinatorial optimization problems \cite{cappart2021combinatorial}. Further, due to its learned nature, NAR allows for learning procedures directly from (real-world) data, without the need for manual feature extraction. Overall, this positions NAR as an attractive method to obtain a fast, fully-learned synthesis procedure, which entirely avoids the need for a formal model or any hand-crafted synthesis rules. Based on this promising outlook, this paper explores how to apply the NAR paradigm to the problem of network configuration synthesis.

To that end, we propose a \textbf{new learning-based framework for configuration synthesis} as an alternative to SMT-based approaches. Our framework is protocol-agnostic, enables cross-protocol reasoning and avoids the need to manually provide synthesis rules. We build upon the idea of NAR, and train a graph-based processor neural network to learn a synthesis procedure in latent space. A key challenge in a multi-protocol setting is the diversity of different protocols and configuration parameters. To this end, we implement a generic embedding scheme based on Datalog-like facts and program sketching \cite{solar2008program}, which allows us to easily adapt our framework to new protocols. Further, our synthesis model produces a whole distribution of network configurations. As a consequence, we can directly sample multiple alternative synthesis outputs, which is not possible with standard SMT solvers. We apply our framework to a non-trivial synthesis setting where both the Border Gateway Protocol (BGP) and the Open Shortest Path First (OSPF) protocol are used. We demonstrate that our learned synthesis tool is up to~$500\times$ faster than a state-of-the-art SMT-based synthesizer, while producing configurations which on average enjoy more than 91\% satisfaction of the provided specification.

\paragraph{Main Contributions} Our core contributions are:
\vspace{-5pt}
\begin{itemize}
    \setlength{\itemsep}{5pt}
    \setlength{\parskip}{0pt}
    \item A learning-based framework for network configuration synthesis based on neural algorithmic reasoning.
    \item A neural network architecture for learning synthesizer models which relies on a generic graph-based encoding of network topologies and configurations.
    \item An extensive evaluation of our learning-based synthesizer, in terms of both precision and scalability, on the challenging setting where both the BGP and OSPF protocols are involved.
\end{itemize}

\section{Framework Overview}
\label{sec:overview}

\begin{figure}
    \begin{center}
        \includegraphics[width=0.45\textwidth]{figures/synthesizer-overview.pdf}
    \end{center}
    \caption{An overview of our learning-based synthesis framework.}
    \label{fig:learning-based-synthesis}
\end{figure}

%As an example, consider \cref{fig:network-fwd-tree} (c) which illustrates the forwarding plane of some traffic class reachable via external peer $E$ or $F$ in our example network. Each router of the network forwards traffic along some of its outgoing links. In practice, a number of protocols are used to populate a router's routing tables. For the instantiation of our synthesis framework however, we focus on OSPF and BGP.

In the following, we discuss the fundamentals and core steps of our learning-based framework as illustrated in \cref{fig:learning-based-synthesis}.

\paragraph{Network Configuration} In this work, we consider the configuration synthesis problem at the level of the so-called \emph{forwarding plane} of a network. This means we look at how each router forwards traffic, given a packet with a certain destination. The forwarding plane is determined by a distributed computation whose exact semantics depend on the different routing protocols in use. To adapt the forwarding behavior, network operators change configuration parameters at the router-level (e.g. link weights), such that running the protocols results in the desired forwarding plane. Given this context, we define the problem of configuration synthesis as follows.

\paragraph{Configuration Synthesis} The configuration synthesis problem corresponds to automatically generating these router-level configurations, such that a set of given requirements about the forwarding plane is satisfied. Typical requirements include reachability, traffic isolation and other forwarding properties. 

\paragraph{Dataset} To train a synthesizer model, we first generate a dataset of input/output samples for the synthesis problem. For this, we rely on a generative pipeline as shown in the top of \cref{fig:learning-based-synthesis}. First, we sample a random network configuration for some topology using a uniform generative process. Then, we simulate the involved protocols to obtain the corresponding forwarding plane. Next, we extract a specification by randomly selecting properties that hold for the computed forwarding plane. This leaves us with a specification and topology as input and corresponding configuration as the output to a synthesis problem.

\paragraph{Simulation} Depending on the protocols in use, one implements simulation code to compute the forwarding plane induced by a sampled configuration. Although this step is protocol-specific, the overall implementation effort is much lower compared to SMT-based synthesis. Protocols are typically well-defined algorithms which can be simulated, whereas the alternative of implementing a synthesizer often requires expert knowledge about SMT solvers. In practice, our framework may also be adapted to use a real-world network router to compute the behavior of a configuration, thereby capturing the real-world behavior directly.

\paragraph{Neural Synthesizer Model} Based on the generated dataset, we train a graph neural network (GNN) to perform synthesis. For this, the network's input consists of a topology, a specification and a configuration sketch where to-be-synthesized parameters are omitted. Following the NAR paradigm, we first encode this synthesizer input in latent space. Then, we apply an iterative processor network which relies on the graph attention mechanism to propagate information \cite{velivckovic2017graph}. Last, we apply a decoder network to predict the values of omitted configuration parameters, thereby synthesizing a corresponding configuration. To remain protocol-agnostic, our model is generic with respect to the input format, using an intermediate representation based on Datalog-like facts.
%
\paragraph{Relaxed Specification Consistency} Since parts of the configuration synthesis problems are known to be NP-hard \cite{fortz2000internet}, any precise synthesis method will run into scalability issues, just like SMT-based methods. However, practical synthesis must be fast and scalable to accommodate the size of real-world networks and the frequency at which configurations need to be updated \cite{vissicchio2012improving}. In our learning-based framework, we therefore employ a fixed-size neural network architecture which always runs in polynomial time. While this indeed enables fast synthesis times, we cannot expect our neural system to be as precise as SMT methods. Therefore, to assess the synthesis capabilities of our learning-based system, we rely on the notion of \emph{relaxed~specification~consistency}. More specifically, we do not just check whether a configuration satisfies a specification or not, but also measure the degree up to which a synthesized configuration satisfies a specification (e.g. via the number of satisfied requirements). 

This "soft" understanding of a specification allows us to evaluate neural synthesis systems which may not always produce fully consistent configurations. Further, we argue that configurations with less than $100\%$ consistency are still very useful in practice, as they provide a good starting point for additional adjustments by network operators. Future work may improve the precision of neural synthesis by exploiting partial synthesis methods \cite{el2018netcomplete} to obtain fully consistent solutions, given a partially consistent configuration. However, note also that even exact SMT-based synthesizers may not always produce fully consistent solutions, due to differences between the formal protocol model and the one running on a given real-world router where the configuration is to be deployed \cite{birkner2021metha}.

\paragraph{Instantiation} Our learning-based synthesis framework is generic with respect to the routing protocols in use. This means, it can be instantiated to many different synthesis settings. To do this, users merely provide a drop-in replacement for the simulation component as shown in \cref{fig:learning-based-synthesis}, while other components such as the neural model architecture itself can be directly re-used.

%More specifically, we employ a slightly modified variant which operates on a graph-based encoding of a specification, topology and configuration parameters.

%  \begin{figure*}
%      \centering
%      \includegraphics[width=0.85\textwidth]{figures/system-overview.pdf}
%      \caption{An overview of our synthesis system: (1) First, we use a generic embedding scheme to transform a network topology, protocol configuration sketches and the specification given as Datalog-like facts to a latent input representation. Next, we apply a learned (2) Processor GNN and obtain a latent synthesis output. Last, we apply a (3) Decoder Network to obtain a distribution over possible values per unknown parameter in our configuration.}
%      \label{fig:overview-model}
% \end{figure*}
%

In this paper, we first discuss the architecture of our neural synthesis model. In follow-up sections, we instantiate our framework  for the case of BGP/OSPF configuration synthesis, and evaluate the resulting instantiation by comparing it to a state-of-the-art SMT-based synthesizer.

% \begin{itemize}
%     \item effort: need to implement simulation code to generate dataset to learn from (typically well-defined in protocol specs, much easier than implementing synthesis directly)
%     \item can be sampled (multiple alternative solutions, not easily possible with SMT-based methods)
%     \item much faster than SMT-based synthesis
% \end{itemize}

% Requirements:
% \begin{itemize}
%     \item protocol-agnostic
%     \item fully learned, no hand-coded synthesis rules
%     \item define: strict specification vs. relaxed specification
% \end{itemize} 

==> diff/git-latexdiff.34965/new/sections/2_model.tex <==
\section{Neural Synthesis Model}
\label{sec:model}


We now present the architecture of our graph-based neural synthesizer model, illustrated in \cref{fig:overview-model}. First, in \cref{sec:graph-embedding} we introduce our generic graph-based encoding, which allows us to embed network topologies, protocol configuration and the specification into a latent space. Then, in \cref{sec:graph-transformer} we present the architecture of the processor network which we train to perform the synthesis task. Finally, in \cref{sec:decoding-sampling} we discuss how to sample network configurations from the resulting latent synthesis output.

\begin{figure}
    \begin{minipage}[t]{0.21\textwidth}
    \begin{lstlisting}[basicstyle=\ttfamily\small, escapeinside={(*}{*)}]
router(A)
router(B)
(...)

connected(A,B,2)
connected(A,C,?)(*\blackcircled{1}*)
(...)
    \end{lstlisting}
\end{minipage}
\begin{minipage}[t]{0.21\textwidth}
    \begin{lstlisting}[basicstyle=\ttfamily\small, escapeinside={(*}{*)}]
network(N1)
bgp_route(E,N1,2,3,1,0,1)

fwd(A,B,N1)
not fwd(B,A,N1)
(...)
    \end{lstlisting}
\end{minipage}
    \caption{A snippet of a fact base sketch encoding a network's topology, parameters such as link weights (\texttt{connected} facts) and a specification (\texttt{fwd} facts).}
    \label{fig:datalog-encoding}
\end{figure}

\begin{figure}[t]
    \centering
    \includegraphics[width=0.25\textwidth]{figures/synth-architecture.png}
    \caption{The neural synthesizer model architecture.}
    \label{fig:architecture}
\end{figure}

\subsection{Fact Base Embedding}
\label{sec:graph-embedding}
To remain network protocol-agnostic in our model architecture, we implement a generic graph-based encoding of Datalog-like facts, similar to knowledge graphs \cite{rosso2020beyond}. This means that we first encode topologies, configurations and specifications as a set of Datalog-like facts and then employ a generic embedding.
%We chose Datalog facts as the input format of our synthesis approach for its flexibility, wide-spread use in Program Analysis and use in previous work on configuration synthesis \cite{el2017network}.

\paragraph{Fact Base} A set of Datalog-like facts, as depicted in \cref{fig:datalog-encoding}, serves as the input \emph{fact base} $\mathcal{F}$ to our synthesizer model. $\mathcal{F}$ is a set of facts $f(a_0, \dots, a_n)$ where arguments may be constants (e.g. A or B) or integer literals. Further, each fact in a fact base has a corresponding truth value denoted as $[f(a)]_{\mathcal{B}}$. For instance, from the fact base in \cref{fig:datalog-encoding} we can derive $[fwd(A,B,N1)]_{\mathcal{B}} = \text{\texttt{true}}$ and $[fwd(B,A,N1)]_{\mathcal{B}} = \text{\texttt{false}}$.

\paragraph{Consistency} We represent a network's topology, the protocol configuration and parameters as well as the specification, all in a single fact base. Given the semantics of the protocols in use, we can then check whether the specification encoded in a fact base is satisfied by the provided configuration. To quantify, we define the notion of relaxed specification consistency, as discussed earlier, with respect to a fact base: Given a fact base $\mathcal{F}$, a subset of specification facts $S \subset \mathcal{F}$ and protocol semantics $\mathcal{P}$, the \emph{consistency} of a fact base is defined as the relative number of satisfied facts in $S$ with respect to the forwarding plane obtained via $\mathcal{P}$. The contents of $S$ depend on the concrete instantiation of the synthesizer model. For an example of possible specification facts, see our instantiation of the synthesizer model for BGP/OSPF in \cref{sec:training}.

\begin{figure*}
    \footnotesize
    \def\arraystretch{1.4}
    \begin{tabular}{lr}
        %$T_f: T_1 \times \dots \times T_n$ & \textit{(fact type declaration)}\\
        $emb(f) := \mathbf{V_f}$ & \textit{(learned fact type embedding)}\\
        $emb(b) := \mathbf{W_{\text{bool}}}\;onehot(b)$ & \textit{(learned boolean embedding)}\\
        $emb(f,i,v) := \mathbf{W_{f_i}}\;onehot(v)$ & \textit{(learned integer embedding)}\\
        $emb(f,i,?) := \mathbf{V_{hole}}$ & \textit{(learned hole embedding)}\vspace{2pt}\\
        $\mathlarger{
        h_c := \sum_{f(c) \in \mathcal{F}}
        emb(f)
        }$ & \textit{(constant embedding)}\vspace{2pt}\\
        $h_{f(a_0, \dots, a_n)} := emb(f) + emb([f(a_0, \dots, a_n)]_{\mathcal{B}}) + \mathlarger{
        \sum_{(i,v) \in \mathcal{I}(f(a_0, \dots, a_n))}
        emb(f, i, v)
        }$\hspace{-1.2cm} & \textit{(fact embedding)}\\
        $\mathcal{I}(f(a_0, \dots, a_n)) := \{(i,v) \; | \; f(a_0, \dots, a_{i-1}, v, \dots, a_n) \in \mathcal{F} \wedge v:Int \wedge i \in \mathbb{N}$ \}& \textit{(integer arguments)}\vspace{2pt}\\
        $N_i(h_c) := \{h_f \; | \; \exists i \in \mathbb{N} . f(a_0, \dots, a_{i-1}, c, a_{i+1}, \dots, a_n) \in \mathcal{F}\}$& \textit{(i-th neighborhood of constant node)} \\
        $N_i(h_f) := \{h_c \; | \; \exists i \in \mathbb{N} . f(a_0, \dots, a_{i-1}, c, a_{i+1}, \dots, a_n) \in \mathcal{F}\}$& \textit{(i-th neighborhood of fact node)} \\
    \end{tabular}
    \caption{Translating a fact base $\mathcal{F}$ to node features. $f$ denotes a predicate, $v$ integer values, $b$ boolean values as 0 or 1, $i$ argument indices and $[f(a)]_{\mathcal{B}}$ the truth value of a fact. }
    \label{fig:graph-embedding}
\end{figure*}

%discuss embedding as shown in \cref{fig:datalog-encoding}. Note how this makes fact bases a suitable input to standard GNN architectures.

\paragraph{Fact Base Sketching} In a synthesis setting, we are confronted with incomplete fact bases, i.e. the specification and topology is given but the network configuration is to be synthesized. For these cases, we also consider fact bases with unknown parameters inspired by the idea of program sketching in program synthesis \cite{solar2008program}. More specifically, users may replace an unknown integer argument of a fact by a \texttt{?} symbol, indicating a value to be synthesized. Using this mechanic, we can represent the synthesis input as an incomplete fact base which encodes to-be-synthesized values as unknown parameters. As an example, consider \cref{fig:datalog-encoding} \blackcircled{1}, where the link weight between router nodes \texttt{A} and \texttt{C} is represented as an unknown parameter.

\paragraph{Embedding} We employ a structurally-defined embedding scheme to transform a fact base into a graph with node features as required for processing with graph neural networks. Given a fact base $\mathcal{F}$, we apply the rules in \cref{fig:graph-embedding} to obtain node features and adjacency information. Both a fact $f$ and a constant $c$ are represented as distinct nodes with features $h_c$ and $h_f$, respectively. The relationships between facts and constants is encoded as node adjacency as defined by the neighborhood functions $N_i$.

We use multiple neighborhood functions, i.e. multiple types of edges, to encode the argument position of a constant occurring in a fact. Hence, the number of neighborhood functions corresponds to the maximum number of arguments in a single fact, e.g. 3 in \cref{fig:datalog-encoding}. Integer arguments and unary facts are directly accounted for in the respective node or fact embedding. To handle unknown parameters, we replace the corresponding $emb(...)$ term with the learned $\mathbf{V_{hole}}$ embedding.

Considering the embedding function $emb$, the learned parameters of our embedding are $\mathbf{V_f} \in \mathbb{R}^D$ per fact type in~$\mathcal{F}$, $\mathbf{W_{\text{bool}}} \in \mathbb{R}^{D \times 2}$ for boolean values, $\mathbf{W_{f_i}} \in \mathbb{R}^{D \times N}$ per integer argument of fact type $f$ and $\mathbf{V_{hole}} \in \mathbb{R}^D$ to represent unknown parameters. Hyperparameter $D$ represents the dimension of the latent space the synthesizer model operates in and $N$ specifies the number of supported integer values. An example of applying this embedding scheme to a simple fact base is given in \cref{fig:graph-encoding-example}.

\begin{figure}
    \begin{minipage}[t]{0.2\textwidth}
        \centering
        \footnotesize
        \textbf{Fact Base}
        \begin{lstlisting}[basicstyle=\ttfamily\small]
router(A)
router(B)

conn(A, B, 12)
        \end{lstlisting}
    \end{minipage}
    \begin{minipage}[t]{0.15\textwidth}
        \centering
        \textbf{Graph}\\
        \vspace{5pt}
        \includegraphics[width=0.7\textwidth]{figures/graph-encoding.pdf}
    \end{minipage}\\
    \centering\\
    \vspace{10pt}
    \textbf{Node Features}\\
    \vspace{10pt}
    \begin{minipage}[t]{0.5\textwidth}
        $\begin{array}{rcl}
        h_A &:=& emb(router) = \mathbf{V_{\text{router}}}\\
        h_B &:=& emb(router) = \mathbf{V_{\text{router}}}\\
        h_{\text{conn(A,B,12)}} &:=& emb(conn) + emb(conn, 2, 12)\\
        &:=& \mathbf{V_{\text{conn}}} + \mathbf{W_{conn_2}} onehot(12)
    \end{array}$
    \end{minipage}
    \caption{An example of embedding a simple fact base using the embedding scheme of \cref{fig:graph-embedding}. The shown graph illustrates the neighborhoods $N_0$ and $N_1$ induced by the \texttt{conn} fact.}
    \label{fig:graph-encoding-example}
\end{figure}

\begin{figure}
    $$
    \begin{array}{rcl}
    z_j &:=& h_j + Drop(\mathlarger{\sum_{N_i}} h'_{GAT_i})\\
    h'_j &:=& FFN(Norm(z_j))\vspace{11pt}\\
    FFN(x_j) &:=& Norm(Lin2(Drop(Lin1(x_j)))))
    \end{array}
    $$
    \caption{
        The recurrence relation of a node $j$'s representation $h_j$. $h'_{GAT_i}$ represents the output of a graph attention layer operating with neighborhood $N_i$ according to \cite{velivckovic2017graph}, $h_j$ the representation of node $j$ at the previous step. $Norm$ refers to batch normalization \cite{ioffe2015batch}, $Drop$ to dropout regularization \cite{hinton2012improving} and $Lin1$ and $Lin2$ to linear layers with an inner dimension of $4N$.
    }
    \label{fig:recurrence}
\end{figure}

\subsection{Synthesizer Model}
\label{sec:graph-transformer}

For an illustration of the synthesizer model's architecture, please see Figure~\ref{fig:architecture}. Given a fact base $\mathcal{F}$ we first apply our embedding scheme as described in \cref{sec:graph-embedding}. We then employ a 2-layer GNN-based encoder network to produce the latent representation of a synthesis input.
Given this representation, a processors network is trained to perform the actual synthesis task in high-dimensional space. Last, we apply a set of decoder networks, to obtain the synthesized values of unknown parameter, given the latent synthesis~output.

%In this context, the synthesis problem for network configurations corresponds to completing partially provided fact bases.

% \paragraph{High-Level Architecture}

% We employ the high-level architecture to obtain the latent synthesis output $y_\mathcal{F}$:
% $$
% \begin{array}{rcl}
%     \mathbf{x_{\mathcal{F}}} &:=& Encoder(Embedding(\mathcal{F}))\\
%     \mathbf{y_{\mathcal{F}}} &:=& Processor(\mathbf{x_{\mathcal{F}}} + \mathbf{z})\\
%     z_i &\sim& \mathcal{N}(0,1)
% \end{array}
% $$
% \todo{z is only added for $i<N/2$}

% $Embedding$ corresponds to the graph-based embedding as discussed in \cref{sec:graph-embedding} and $Encoder$ is a 2-layer graph attention module. $Processor$

\paragraph{Encoding} The encoder GNN operates on the embedded representation of a fact base. It produces the high-dimensional representation of a synthesis input as required for the processor network. We additionally apply noise to the first half of the units of the latent representation via $\mathbf{z}$, as a source of non-determinism. According to our experiments this improves model performance and we hypothesize this is due to the synthesis problem having more than one solution in most cases.

\paragraph{Iterative Processor} The processor network is modelled as an iterative process. It consists of a 6-layer graph attention module which we apply for a total of 4 iterations. In the framework of neural algorithmic reasoning, this iterative computational structure encodes an inductive bias towards an iterative solution to the synthesis problem. Because of this bias, our processor network essentially learns an algorithmic procedure which iteratively synthesizes the values of unknown parameters in a fact base.

\paragraph{Graph Attention Layer} In the GNNs we employ, we rely on a composed variant of the graph attention layer as introduced by \cite{velivckovic2017graph}. We employ multiple graph attention layers in lockstep, one per neighborhood $N_i$ defined by our graph embedding (cf. \cref{sec:graph-embedding}), and combine the intermediate results after each step. Specifically, the recurrence relation of a node $j$'s representation $h_j$ is defined as shown in \cref{fig:recurrence}. These mechanics of combining the results of the different graph attention layers $h'_{GAT_i}$, directly corresponds to how multiple attention heads are combined in the original Transformer architecture \cite{vaswani2017attention}.

\paragraph{Argument Decoder Networks} To synthesize the values of unknown parameters, the model maintains a set of decoder networks. That is, it provides one decoder network per integer argument per fact type in a fact base. When decoding, the network is applied to the latent synthesis output of the corresponding fact node. For example, a synthesizer model which operates on the fact base in \cref{fig:datalog-encoding}, would provide a decoder network $D_{\text{connected}_2}: \mathbb{R}^D \rightarrow \mathbb{R^N}$ to decode values for the third argument of a \texttt{conn} fact. In our experiments, decoder networks are implemented as simple multi-layer perceptron models.

\paragraph{Supervision Signal} During training, we mask all fact arguments that represent to-be-synthesized configuration parameters in our synthesis setting. As a supervision signal we use the masked values as the ground-truth and apply a negative log-likelihood loss function to the output distribution of the corresponding argument decoder networks.

%The synthesizer model learns a conditional distribution of fact bases which are consistent with respect to the protocols' semantics.

%\todo{introduce synthesis as a completion problem of an encoded fact base (a la BERT). Introduce masking, introduce decoding of integer and truth values. Synthesis is learning a conditional distribution of consistent fact bases.}

%Using this method, we obtain the node features $h_c$ per constant, $h_f$ per fact and adjacency information in terms of node neighborhood functions $N_i(h_c)$ and $N_i(h_f)$. Overall, this encoding makes a fact base suitable for processing using standard graph neural networks.

%- Brief description of the Graph Transformer Model
\subsection{Multi-Shot Sampling}
\label{sec:decoding-sampling}

%Multi-Stage Parameter Sampling (sampling methods: topk, high-temp, low-temp)
To sample concrete values from the output distributions over unknown parameters, we apply a multi-shot sampling strategy. That is, we sample values only for a subset of unknown parameters, insert them in our input fact base and run the synthesis model again. We repeat this process until no more unknown parameters remain. This multi-shot sampling strategy allows the model to incorporate the concrete values of previously synthesized parameters in its computation. In our evaluation in \cref{sec:evaluation}, we include a comparison of how this compares to sampling all unknown parameters at once.

%In a fact base with multiple holes, we apply the corresponding decoder networks to obtain a value distribution for each integer hole. However, instead of sampling all integer holes in one


==> diff/git-latexdiff.34965/new/sections/3_bgp_ospf.tex <==
\section{BGP/OSPF Synthesis}
\label{sec:bgp-ospf}

\newcommand{\as}{\ac{AS}~}
\newcommand{\ases}{\acp{AS}~}

\newcommand{\squareann}{{\tiny$\blacksquare\;$}}
\newcommand{\triangleann}{{\small$\blacktriangle\;$}}

\begin{figure*}
    \centering
    \includegraphics[width=0.95\textwidth]{figures/networks-all.pdf}
    \caption{(a) An illustration of a small AS network, including internal peers (blue), external peers (purple), BGP sessions as well as physical links. (b) The propagation of two BGP announcement across the network. (c) The resulting forwarding plane after applying BGP and OSPF.}
    \label{fig:network-fwd-tree}
\end{figure*}

We now discuss an instantiation of our learning-based framework for the case of BGP and OSPF protocols. In \cref{sec:synthesis-setting} we introduce a basic networking model, BGP and OSPF protocols and the synthesis setting. Given this model, \cref{sec:training} describes how to generate a corresponding dataset of input/output samples and train a synthesizer model.
%This shall serve as a prerequisite to the instantiation of our learning-based synthesis framework for the BGP and OSPF protocol in \cref{sec:training}.

\subsection{Synthesis Setting}
\label{sec:synthesis-setting}

\paragraph{Graphical Model} We assume an abstract network model which can be represented as an undirected graph as shown in \cref{fig:network-fwd-tree} (a). We always consider a set of internal routers (A, B, C, D in \cref{fig:network-fwd-tree}) as well as a set of adjacent external routers (E, F  in \cref{fig:network-fwd-tree}). The group of internal routers forms the \emph{\as} under consideration whereas external routers belong to other adjacent \ases. In practice, an \as represents an administrative domain controlled by a single operator. 

\paragraph{Forwarding Plane} For an example of a possible forwarding plane in this abstract model, consider \cref{fig:network-fwd-tree} (c) which illustrates the forwarding plane of traffic destined towards some destination reachable via external peer $E$ or $F$. Each router of the network forwards traffic along some of its outgoing links. In practice, a number of protocols are used to compute the forwarding plane. However, here we focus on OSPF and BGP.

\paragraph{OSPF} The OSPF protocol \cite{moy1994ospf} is a link-state protocol, typically used as an interior gateway protocol~(IGP), i.e., to route traffic within an \ac{AS}. Given link weights per physical link in the network, OSPF simply routes traffic along the shortest path towards the destination.

\paragraph{BGP} The BGP protocol \cite{rekhter1994border} on the other hand is a path-vector protocol used to exchange reachability information mostly on the level of \acp{AS}.
%These are groups of routers typically operated by a single party (e.g. an ISP).
When using BGP, a routing destination announces its existence to other \ases and routers, by sending out a BGP announcement. Receivers of such announcements may then choose to pass them on to other \acp{AS}, redistribute them internally and/or modify them. Instead of communicating along physical links directly, the BGP protocol requires manually configured BGP sessions among routers of the \as and external peers, as indicated by the BGP session edges in \cref{fig:network-fwd-tree}(a).
%\todo{more discussion of eBGP vs iBGP and support for route reflection (more of an implementation detail, maybe only mention in dataset generation where simulation code is discussed)}.

%\paragraph{BGP Decision Procedure}~
%\todo{discuss decision procedure}
In case a router receives more than one announcement for a destination, a designated BGP decision process is applied to determine a single best route. \cref{fig:bgp-decision} shows the ordered list of comparison criteria of this decision process. The different criteria depend different properties of a route announcements, including the IGP cost towards the routing destination. As a consequence, when used together, OSPF as IGP protocol and BGP will interact. %Note also that BGP is an iterative process which needs multiple rounds of propagation to converge.

\paragraph{Example}
%\todo{run through simple BGP+OSPF example of computing the forwarding plane}
To better understand BGP/OSPF routing, consider the simple example given in \cref{fig:network-fwd-tree} (b). Here, our example \as imports BGP announcements \squareann and \triangleann from E and F respectively. Both represent a route to the same destination. As shown, both announcements have a so-called local preference of 2. For simplicity, we ignore other properties such as the AS path length, Origin and MED in this example. The announcements are propagated among BGP neighbors and the best route is selected according to the decision procedure in \cref{fig:bgp-decision}. See \cref{fig:network-fwd-tree} (b) for an illustration of the intermediate states of this propagation process. As both announcements have a local preference of 2, rule 1 of the decision process is not used. Instead, in round 2, node B selects \squareann over \triangleann due to a lower IGP cost of 2 via egress node A as compared to 3 via egress node D (rule 6). Node D selects \triangleann over \squareann, since it learns this route directly from an external peer (rule 5). After Round 3, the BGP propagation process converges to a stable state and we can derive the forwarding plane as shown in \cref{fig:network-fwd-tree} (c).


%, as well as external peers E and F which belong to other \acp{AS}. External peers are routers which are connected via eBGP sessions to routers of the \ac{AS} under consideration. They announce BGP routes to their neighbors, which are propagated within the network

%\paragraph{BGP/OSPF Configuration Synthesis} We phrase the BGP/OSPF configuration synthesis problem on the level of the forwarding plane. This means that users provide a specification which constraints the set of allowed forwarding planes. This includes predicates which enforce forwarding paths, block forwarding paths or assert higher-level properties like traffic isolation and reachability. Given such a specification, we consider network configuration synthesis as the task of configuring OSPF and BGP in a way that produces a forwarding plane which satisfies the provided specification.

\paragraph{BGP/OSPF Configuration Synthesis} According to our general synthesis framework, we consider the BGP/OSPF configuration synthesis problem at the level of the forwarding plane. However, we further also define the set of synthesized parameters: For OSPF we synthesize link weights as explored in a wide range of existing work (e.g. \cite{el2018netcomplete,fortz2000internet}. For BGP, the set of parameters is not defined as clearly: Depending on the requirements of a network operator, one may employ custom BGP import and export policies at every router of a network to implement complex behavior. However, in this instantiation we focus on a simplified setting, where we assume BGP route announcements to only be modified when imported into the \as from an external peer. Previous work has already pointed out that this is a reasonable assumption which holds for the majority of real-world networks \cite{caesar2005bgp,cittadini2010doing, steffen2020probabilistic}.

\begin{figure}
    \small{
    \begin{enumerate}
        \setlength{\itemsep}{0pt}
        \setlength{\parskip}{0pt}
        \item Highest Local preference
        \item Lowest AS path length
        \item Prefer Origin (IGP $>$ EBGP $>$ INCOMPLETE)
        \item Lowest Multi-exit discriminator (MED)
        \item External over internal announcements
        \item Lowest IGP cost to egress
        \item Lowest BGP peer id (tie breaker)
    \end{enumerate}}
    \vspace{-15pt}
    \caption{The BGP decision process \cite{rekhter1994border}. The shown rules are applied in order until a single best BGP announcements remains.}
    \label{fig:bgp-decision}
\end{figure}

\subsection{Dataset Generation and Training}
\label{sec:training}
To train a synthesizer model, we need a large number of fact bases encoding a variety of network topologies, configurations and forwarding specifications. Further, we must provide the model with target values for unknown parameters as a supervision signal. This section discusses how we construct such a dataset for BGP/OSPF synthesis.
%Further, we provide an example of what a corresponding fact base looks like, including a description of the supported specification language.

\paragraph{Dataset Generation} To obtain network configurations and corresponding forwarding specifications we employ a generative process: We first randomly configure BGP and OSPF parameters for some topology. Then we simulate the OSPF and BGP protocol and compute the resulting forwarding plane. Based on this, we extract a forwarding specification which fixes a random subset of forwarding paths, reachability and isolation properties that are satisfied by the forwarding plane.

\paragraph{Topologies} For training, our dataset is based on random topologies with $16$-$24$ routers. We generate the physical layout of these graphs by triangulation of uniformly sampled points in two-dimensional space.

\paragraph{Simulation} To compute the forwarding plane given an OSPF and BGP configuration, we simulate the protocols. For OSPF, we implement shortest path computation to obtain the forwarding plane. For BGP, we implement the full BGP decision process as shown in \cref{fig:bgp-decision}, except for the MED attribute. In addition to the basic networking model discussed in \cref{sec:synthesis-setting}, we implement support for eBGP and iBGP, fully-meshed BGP session layouts as well as layouts relying on route reflection. For more details of these BGP concepts see \cite{bates2000rr}.

%Note that the synthesizer model will reason on the level of the provided training samples. That is, to improve the overall synthesis quality in a real-world setting, it is helpful to implement simulation code which behaves very similar to real-world networks. Another promising approach would be to extract training samples from real-world networks, thereby circumventing the need for simulation, however, we leave this as future work.

%While this can be a considerable effort, it is typically an easier task than to implement the synthesizer directly. The concrete semantics of protocols and their simulation is a well-defined procedure, whereas implementing efficient synthesis tools is still an open problem.

\paragraph{Fact Base Encoding} We encode synthesis input using a small set of facts. For an example of a corresponding fact base see \cref{fig:bgp-ospf-fact-base}. We use the \texttt{router}, \texttt{external} and \texttt{network} facts to mark routers, external peers and routing destinations respectively. Physical links between routers are encoded as \texttt{connected(R1,R2,W)} facts where \texttt{W} denotes the OSPF link weight. Further, we rely on \texttt{ibgp}, \texttt{ebgp}, \texttt{route\_reflector} and \texttt{bgp\_route} facts to represent different types of BGP sessions and imported routes. Using the notion of unknown parameters as discussed in \cref{sec:graph-embedding}, we encode configuration parameters, e.g., properties of imported routes or OSPF link weights.

\paragraph{Specification Language} We support a small specification language with three types of forwarding predicates:

\begin{itemize}
    \setlength{\itemsep}{0pt}
    \setlength{\parskip}{2pt}
    \item \texttt{fwd(R1, Net, R2)} specifies that router \texttt{R1} forwards traffic destined for \texttt{Net} to its neighbor \texttt{R2}.
    \item \texttt{reachable(R1, Net, R2)} specifies that traffic destined for \texttt{Net} that passes through \texttt{R1} also passes through \texttt{R2} before reaching its destination.
    \item \texttt{trafficIsolation(R1, R2, N1, N2)} specifies that it must not hold that $[fwd(R1,R2,N1)]_{\mathcal{B}} \wedge [fwd(R1,R2,N2)]_{\mathcal{B}}$.
\end{itemize}

In the negative case of each predicate, the opposite must hold true for the fact to be satisfied. This specification language can easily be extended by including new specification predicates in the dataset generation process. One must simply provide a method of extracting positive and negative cases of a specification fact from a given forwarding plane. Once included in the training dataset of a synthesizer model, the resulting synthesis system will be able to consider specifications relying on the new type of predicates.

% \todo{info on loss function, optimizer, etc.}
\paragraph{Training} We generate a dataset of $10,240$ input/output samples and instantiate our synthesizer model with a hidden dimension $D$ of $64$. For optimization, we use the Adam optimizer \cite{kingma2014adam} with a learning rate of $10^{-4}$. We stop training after the specification consistency on a validation dataset no longer increases at $\sim2800$ epochs.

\begin{figure}
\begin{minipage}[t]{0.22\textwidth}
\begin{lstlisting}[basicstyle=\ttfamily\tiny]
# topology and configuration
router(c5)
router(c3)
router(c1)
router(c0)
network(c6)
network(c7)

external(c8)
external(c9)
external(c10)
external(c11)
external(c12)
external(c13)

route_reflector(c2)
route_reflector(c4)

connected(c2,c4,?)
connected(c2,c5,?)
connected(c2,c3,?)
connected(c4,c5,?)
connected(c4,c3,?)
connected(c4,c0,?)
connected(c5,c1,?)
connected(c5,c0,?)
connected(c3,c0,?)
connected(c3,c1,?)
connected(c1,c0,?)

ibgp(c2,c4)
ibgp(c2,c5)
ibgp(c2,c0)
ibgp(c2,c1)
ibgp(c4,c3)
ibgp(c4,c4)
\end{lstlisting}
\end{minipage}
\begin{minipage}[t]{0.2\textwidth}
\begin{lstlisting}[basicstyle=\ttfamily\tiny]
ebgp(c2,c12)
ebgp(c5,c9)
ebgp(c5,c10)
ebgp(c5,c13)
ebgp(c0,c8)
ebgp(c0,c11)

bgp_route(c8,c6,?,?,1,?,1,8)
bgp_route(c9,c6,?,?,0,?,1,9)
bgp_route(c10,c6,?,?,0,?,1,10)
bgp_route(c11,c7,?,?,0,?,1,11)
bgp_route(c12,c7,?,?,0,?,1,12)
bgp_route(c13,c7,?,?,2,?,1,13)

# forwarding specification
fwd(c0,c6,c3)
fwd(c3,c6,c2)
fwd(c2,c6,c4)
not fwd(c3,c6,c0)
not fwd(c0,c6,c11)
not fwd(c11,c6,c0)

not trafficIsolation(c1,c0,c7,c6)
not trafficIsolation(c1,c0,c7,c6)
trafficIsolation(c0,c3,c6,c7)
trafficIsolation(c0,c3,c6,c7)

reachable(c5,c6,c10)
reachable(c1,c6,c4)
not reachable(c0,c6,c5)
reachable(c5,c6,c10)
\end{lstlisting}
\end{minipage}
\caption{An example of a fact base encoding a topology, a sketch of a BGP and OSPF configuration and a forwarding specification.}
\label{fig:bgp-ospf-fact-base}
\end{figure} 

==> diff/git-latexdiff.34965/new/sections/4_evaluation.tex <==
\section{Evaluation}
\label{sec:evaluation}

We trained a synthesizer model to perform configuration synthesis for BGP and OSPF. We now assess the performance of the resulting neural synthesizer with respect to two core metrics: (1) the quality of synthesized configurations in terms of their consistency with the provided forwarding specifications (\cref{sec:synthesis-quality}), and (ii) the time a learned synthesizer takes when compared to the state-of-the-art SMT-based synthesizer NetComplete \cite{el2018netcomplete} (\cref{sec:synthesis-vs-smt}).

\paragraph{Dataset} We compare across three datasets: Small, Medium and Large. Each dataset represents 8 real-world topologies, sampled from the Topology Zoo \cite{knight2011internet}, where the number of nodes lies between 0-34, 34-68 and 68-170 respectively. To obtain forwarding specifications for the sampled topologies, we use our generative pipeline as discussed in \cref{sec:training}. In each topology, we do synthesis for 4 different traffic classes (routing destinations) at a time.

\paragraph{Experimental Setup} We run all our experiments on an Ubuntu Linux machine with an Intel(R)~Core(TM)~i9-9900X~@~3.50GHz processor, 64GB of system memory and an NVIDIA GeForce RTX 3080 GPU with 10GB of video~memory.

\subsection{Synthesis Quality}
\label{sec:synthesis-quality}
To assess our learned synthesizer, we examine its behavior with increasingly large topologies and specifications.

\paragraph{Specifications} Using the same generative model as described in \cref{sec:training}, we generate forwarding specifications for the topologies in our three datasets with each specification constructed from $3 \times n$ requirements, one per supported predicate type:  \texttt{fwd} requirements correspond to specifying or blocking a forwarding path using multiple \texttt{fwd} predicates whereas \texttt{reachable} and \texttt{trafficIsolation} requirements each translate to a single specification fact. We compare across increasingly large specifications of $3\times 2$, $3\times 8$ and $3 \times 16$ requirements, respectively.

\paragraph{Methodology} For each pair of topology and specification, we run our synthesizer 5 times and report the network configurations with the highest overall consistency value. For sampling, we rely on our multi-shot sampling strategy where we randomly group the unknown parameters of a configuration into 4 groups (4-shot sampling).

\paragraph{Results} We summarize our results in \cref{fig:eval-consistency}. On average, our synthesis model produces network configurations that are $>91\%$ consistent with the provided forwarding specifications across all datasets and sizes of specifications. When only few requirements are given, the synthesizer model even succeeds in producing fully-consistent configurations. We observe a slightly decreasing consistency with increasingly large topologies.

%\texttt{fwd} facts are satisfied more easily, whereas \texttt{reachable} and \texttt{trafficIsolation} facts are violated more often.

\paragraph{Multi-Shot Sampling} In \cref{fig:eval-consistency-baseline}, we report the average specification consistency using our multi-shot sampling strategy as compared to sampling all unknown parameters at once. As a baseline we have also sampled random configurations from a uniform distribution (per parameter) and compute the corresponding specification consistency. Over the baseline, our synthesizer model shows clear improvement and multi-shot sampling further increases consistency.

\begin{figure*}
    \begin{center}
        \textbf{Specification Consistency}\\
        \footnotesize
        \begin{tabular}{rrcccccccccc}
        \toprule
        \multicolumn{2}{c}{Dataset} & \tiny\texttt{fwd} & \tiny\texttt{reachable}  & \tiny\texttt{trafficIsolation} & Overall & $\emptyset$     No. Full Matches & $\emptyset$ No. $>90\%$ Matches\\
        \midrule
        $3\times 2$ requirements & Small & 0.95 & 0.94 & 1.00 & \textbf{0.95} & 0.62 & 0.62\\
& Medium & 0.96 & 1.00 & 0.94 & \textbf{0.96} & 0.88 & 0.88\\
& Large & 0.94 & 0.94 & 1.00 & \textbf{0.93} & 0.62 & 0.62\\
\midrule
$3\times 8$ requirements & Small & 0.97 & 0.98 & 0.97 & \textbf{0.98} & 0.50 & 1.00\\
& Medium & 0.99 & 0.95 & 1.00 & \textbf{0.98} & 0.50 & 1.00\\
& Large & 0.96 & 0.95 & 0.91 & \textbf{0.94} & 0.38 & 0.88\\
\midrule
$3\times 16$ requirements & Small & 0.97 & 0.89 & 0.95 & \textbf{0.94} & 0.38 & 0.75\\
& Medium & 0.98 & 0.97 & 0.97 & \textbf{0.98} & 0.38 & 1.00\\
& Large & 0.92 & 0.88 & 0.95 & \textbf{0.91} & 0.12 & 0.50\\
    \end{tabular}\end{center}
    \caption{Average specification consistency of the network configurations synthesized by our trained synthesizer model. Per sample we run the synthesizer with a specification of $3\times N$ requirements, where the specifications always include $N$ requirements per supported predicate type (\texttt{fwd}, \texttt{reachable}, \texttt{trafficIsolation}).}
    \label{fig:eval-consistency}
\end{figure*}

\begin{figure}
    \begin{center}
        \footnotesize
        \begin{tabular}{rrcccccccccc}
        &  & \multicolumn{2}{c}{Neural}\\
        & Random & 1-Shot & 4-shot\\
        \toprule
        Small & 0.83 & 0.92 & \textbf{0.94} \\
        Medium & 0.88 & 0.95 & \textbf{0.98} \\
        Large & 0.78 & 0.88 & \textbf{0.91} \\
    \end{tabular}\end{center}
    \caption{Average specification consistency with $3\times 16$ requirements when sampling configurations randomly from a uniform distribution and 1-shot/4-shot sampling using our synthesizer model.}
    \label{fig:eval-consistency-baseline}
\end{figure}

\begin{figure*}[ht]
    \footnotesize
    \begin{center}
        \textbf{BGP Synthesis Time}
        \footnotesize
        \begin{tabular}{rrccccccccc}
        \toprule
        &&\multicolumn{3}{c}{Synthesis Time (s)} & \multicolumn{2}{c}{Accuracy (Neural)} \\
        \multicolumn{2}{l}{\# Requirements} & NetComplete & Neural (CPU) & Speedup &$\emptyset$ Consistency& $\emptyset$ No. Full Matches\\
        \midrule
    2 requirements &Small & 18.073s & 0.641s & \textbf{28.2x} & 0.969 & 0.875\\
        &Medium & 60.864s & 2.748s & \textbf{22.2x} & 0.939 & 0.75\\
        &Large & 1389.485s\tiny{  7/8 TO} & 22.301s & \textbf{62.3x} & 0.989 & 0.875\\
    \midrule
    8 requirements &Small & 247.691s & 1.065s & \textbf{232.5x} & 0.96 & 0.75\\
        &Medium & $>$25m\tiny{  8/8 TO} & 3.47s & \textbf{432.2x} & 0.968 & 0.5\\
        &Large & $>$25m\tiny{  8/8 TO} & 30.961s & \textbf{48.4x} & 0.969 & 0.75\\
    \midrule
    16 requirements &Small & 1416.828s\tiny{  7/8 TO} & 2.528s & \textbf{560.5x} & 0.926 & 0.25\\
        &Medium & $>$25m\tiny{  8/8 TO} & 5.481s & \textbf{273.7x} & 0.947 & 0.25\\
        &Large & $>$25m\tiny{  8/8 TO} & 69.092s & \textbf{21.7x} & 0.959 & 0.25\\
    \end{tabular}\end{center}
    \caption{Comparing consistency and synthesis time of our method (Neural) with the SMT-based state-of-art synthesis tool NetComplete. The notation {\tiny{n/8 TO}} indicates the number of timed out synthesis runs out of 8 (25+ minutes).}
    \label{fig:evaluation-compare-bgp}
\end{figure*}

\begin{figure*}[ht]
    \begin{center}
        \footnotesize
        \textbf{OSPF Synthesis Time}\\
        \footnotesize
        \begin{tabular}{rrccccccccc}
        \toprule
        &&\multicolumn{3}{c}{Synthesis Time (s)} & \multicolumn{2}{c}{Accuracy (Neural)} \\
        \multicolumn{2}{l}{} & NetComplete & Neural (GPU) & Speedup &$\emptyset$ Consistency& $\emptyset$ No. Full Matches\\
        \midrule
    2 requirements &Small & 0.265s & 0.091s & \textbf{2.9x} & 1.000 & 1.00\\
     &Medium & 0.404s & 0.098s & \textbf{4.1x} & 1.000 & 1.00\\
     &Large & 0.944s & 0.14s & \textbf{6.7x} & 1.000 & 1.00\\
    \midrule
    8 requirements &Small & 0.876s & 0.164s & \textbf{5.3x} & 0.982 & 0.75\\
     &Medium & 1.517s & 0.103s & \textbf{14.7x} & 1.000 & 1.00\\
     &Large & 3.505s & 0.316s & \textbf{11.1x} & 0.981 & 0.50\\
    \midrule
    16 requirements &Small & 1.65s & 0.21s & \textbf{7.9x} & 0.991 & 0.625\\
     &Medium & 2.646s & 0.245s & \textbf{10.8x} & 0.989 & 0.50\\
     &Large & $>$566.636s+\tiny{  3/8 TO} & 0.233s & \textbf{2430.4x} & 0.987 & 0.875\\
    \end{tabular}\end{center}
    \caption{Comparing consistency and synthesis time of our method (Neural) with the SMT-based OSPF synthesis tool NetComplete. The notation {\tiny{n/8 TO}} indicates the number of timed out synthesis runs out of 8 (25+ minutes).}
    \label{fig:evaluation-compare-ospf}
\end{figure*}


\subsection{Comparison to SMT-based Synthesis}
\label{sec:synthesis-vs-smt}

%To provide a comparison of our learned BGP/OSPF synthesizer with SMT-based methods,
We now compare the synthesis time of the learned neural synthesizer with those of NetComplte, a state-of-art configuration synthesis tool based on SMT-solvers \cite{el2018netcomplete}.

\paragraph{Specifications} As the type of supported requirements in NetComplete does not fully align with our model, we restrict this comparison to specifications which only include forwarding paths (i.e. \texttt{fwd} predicates). Further, NetComplete does not support cross-protocol synthesis as in our case and instead requires users to specify for each requirement the protocol to use for its implementation. To bridge this gap, we split the generated forwarding requirements into BGP and OSPF paths for a corresponding NetComplete specification.
%\todo{note on NetComplete installing policies at all routers, not only the edges of the AS}

\paragraph{Methodology} We compare both OSPF synthesis and BGP/OSPF-synthesis. We configure our trained synthesizer model to do OSPF synthesis by only predicting link weights. For each pair of topology and specification, we report the total time of running our synthesizer 4 times using 4-shot sampling, whereas for consistency we report the best out of the 4 runs. For NetComplete, we run the synthesizer with a timeout of 25 minutes. In case a NetComplete attempt times out, we report 25 minutes as a lower bound for its runtime.

\paragraph{OSPF Synthesis Time Results} We document the results of comparing OSPF synthesis time in \cref{fig:evaluation-compare-ospf}. Our synthesizer model achieves a speedup of 2-10x over NetComplete. With 16 requirements and dataset Large this speedup even increases to $2000\times$. Further, our model achieves very high consistency with the provided specification, often producing fully-consistent configurations.

\paragraph{BGP/OSPF Synthesis Time Results} In \cref{fig:evaluation-compare-bgp} we show the comparison of BGP/OSPF synthesis time. Our synthesizer model outperforms NetComplete by multiple orders of magnitude. We observe a speedup of $20-560\times$ which appears to increase with the size of topology and specification. Further, the average specification consistency of the synthesized configurations is greater than $92\%$ across all datasets, even for large topologies. In many cases, our synthesizer model produces fully-consistent configurations, especially with small topologies and specifications. In comparison, NetComplete times out on more than half of the synthesis tasks which means that we can only observe a lower bound of speedup in these cases. Note that our synthesizer model is running on a CPU due to memory restrictions with large topologies. However, running it on a GPU results in even greater speedups (up to $1000\times$, cf. \cref{app:sec:bgp-gpu-performance}). 

==> diff/git-latexdiff.34965/new/sections/5_related_work.tex <==
\section{Related Work}
\label{sec:related-work}

\paragraph{Traditional Configuration Synthesis} 
%A range of existing work is concerned with network configuration synthesis. 
Next to methods based on compilation such as Propane/PropaneAT \cite{beckett2017network}, there are a number of configuration synthesis methods based on constraint solving: Examples include ConfigAssure \cite{narain2008declarative}, SyNet \cite{el2017network} and NetComplete \cite{el2018netcomplete}. Due to their hand-coded nature, these methods are highly protocol-specific and can be very slow due to the solvers they employ. Although some of them allow for cross-protocol reasoning, this is not implemented as transparently as in our framework and users must specify per requirement which protocol to use for its implementation. In contrast, our approach has lower precision but allows for fully transparent cross-protocol reasoning, meaning forwarding requirements are not protocol-bound and the synthesizer chooses how to implement them. Further, our learned BGP/OSPF synthesis tool exhibits much lower synthesis times as compared to an SMT-based tool like NetComplete.

% \begin{itemize}
%     \item NetComplete, SyNet
%     \item Propane, PropaneAT
%     \item DeepBGP
% \end{itemize}

\paragraph{GNNs and Networking} DeepBGP \cite{bahnasy2020deepbgp} relies on GNNs and reinforcement learning to do configuration synthesis. However, it is limited to BGP configuration synthesis and is slower than SMT-based synthesis according to the author's evaluation. In contrast, our learning-based framework is cross-protocol, does not rely on reinforcement learning and provides better synthesis performance. Apart from configuration synthesis, GNNs have also been applied to other problems in the networking domain. For example, the authors of RouteNet \cite{rusek2020routenet} use GNNs to predict performance metrics of network configurations. Other work that is concerned with learning improved protocols includes Q-Routing \cite{boyan1994packet} or more modern approaches such as the Graph-Query Neural Network architecture \cite{geyer2018learning}.

\paragraph{Neural Algorithmic Reasoning} 
Neural algorithmic reasoning (NAR) as proposed in \cite{velivckovic2021neural}, describes the idea of replacing traditional algorithms with neural networks to learn improved algorithmic procedures. Exemplary work includes graph-related algorithms \cite{velivckovic2019neural} or solvers for combinatorial optimization problems \cite{cappart2021combinatorial,joshi2020learning,selsam2019guiding}. Our synthesis framework is the first applications of NAR to the networking domain and relies on the NAR-native encode-process-decode architecture. According to the hierarchy of NAR approaches in \cite{cappart2021combinatorial}, our method is an algorithm-level approach, as we do not supervise on intermediate steps. Although, such step-level methods promise better generalization, it is not clear what an intermediate result of a general synthesis procedure would be. However, future work on a step-level approach may further improve synthesis quality.

% \begin{itemize}
%     \item RouteNet
%     \item GraphNET
%     \item Learning and generating distributed routing protocols using graph-based deep learning
%     \item Unveiling the potential of Graph Neural Networks for network modeling and optimization in SDN
% \end{itemize}

==> diff/git-latexdiff.34965/new/sections/6_conclusion.tex <==
\setlength{\parskip}{6pt plus4mm minus4mm}
\section{Conclusion}
\label{sec:conclusion}
We presented a learning-based framework for configuration synthesis based on the idea of neural algorithmic reasoning. To assess the effectiveness of the system, we instantiated it for the case of BGP/OSPF synthesis. In contrast to traditional synthesis methods, our system supports transparent cross-protocol reasoning and learns synthesis rules only from data. Using our system, synthesis is sped up by a factor of up to $500\times$ when compared to SMT-based methods. Further, our evaluation demonstrates that the resulting synthesis tool provides excellent synthesis quality, producing configurations with high specification consistency. Overall, our results illustrate that exploring the direction of learning-based network configuration synthesis is a promising direction, enabling new cross-protocol reasoning capabilities and great performance improvements. Promising future work includes construction of hybrid systems, integrating both neural models and SMT-based approaches to obtain the best of both worlds.

==> diff/git-latexdiff.34965/old/acronyms.tex <==
\DeclareAcronym{AS}{
    short = AS,
    long = autonomous system,
    short-plural = es ,
    long-plural = s
}

==> diff/git-latexdiff.34965/old/sections/0_abstract.tex <==
% Context
Computer networks employ a number of different protocols to enable efficient routing. However, due to the complexity of multiple interacting protocols, it can be hard for network operators to implement high-level routing policies and requirements. Network configuration synthesis promises to address this situation by automatically generating configurations that satisfy a provided specification. However, existing synthesis methods are often limited to single-protocol reasoning, depend on protocol-specific and hand-coded synthesis rules, and are difficult to scale due to the SMT-based methods they employ. In this work we present a rather different, learning-based method for addressing the configuration synthesis challenge, one based on the recently proposed paradigm of neural algorithmic reasoning. Our framework is protocol-agnostic, enables cross-protocol reasoning and does not depend on any hardcoded synthesis rules. To evaluate, we instantiate our framework for the case of BGP/OSPF synthesis. Our experiments show we can synthesize configurations with a very high degree of specification consistency while observing speedups of up to $500\times$ compared to a state-of-the-art SMT-based synthesis tool.


==> diff/git-latexdiff.34965/old/sections/1_intro.tex <==
\section{Introduction}
\label{sec:introduction}

The backbone of the internet consists of many connected computer networks operated by different internet service providers (ISPs) and other large organizations. These networks rely on a number of protocols to enable effective and policy-driven routing of traffic. Based on router-level configurations, the protocols perform a distributed computation to construct a network's forwarding state. However, the relatively low-level router configuration makes it hard for network operators to directly enforce network-wide policies and requirements. This often leads to misconfiguration, which can cause global outages such as the recent hours-long blackout of the entire Facebook platform \cite{janardhan2021} and comparable events \cite{mccarthy_2019}.
%
\paragraph{Configuration Synthesis} This situation has triggered a number of research efforts regarding the synthesis of network configurations \cite{el2018netcomplete,beckett2017network,narain2008declarative}. Configuration synthesis is concerned with the task of automatically generating router-level configurations given a set of high-level requirements. However, this synthesis problem can be very hard to solve, since network configurations typically consist of a considerable number of tunable parameters, where the execution of several interacting protocols yields the overall forwarding state. An effective synthesis tool must thus account for this fact and be able to reason across multiple protocols.

\paragraph{SMT-based Synthesis} Some of the most successful efforts in providing cross-protocol synthesis capabilities are based on satisfiability modulo theory (SMT) solvers \cite{el2018netcomplete,el2017network}. While SMT-based synthesis is a promising method, it comes with a number of limitations:
% \item protocol-specific
% fully hand-coded synthesis rules, a lot of implementation effort, cross-protocol support extra complicated
(1) SMT-based synthesizers are hand-crafted and highly protocol-specific. To implement synthesis, we must first express our networking model, protocol semantics including vendor and device specific behavior in terms of first-order logic constraints. This is a time-intensive and complicated process, requiring lots of expert knowledge.
%  model-dependent: synthesis is reasoning on the level of some assumed model which may not reflect the real world: even if a configuration is synthesized based on some spec, it may behave differently and violate spec in practice
Further, (2) logic-based modelling introduces a disconnect between the synthesis tool and real-world behavior \cite{birkner2021metha}. More specifically, synthesized configurations may satisfy a provided specification within a formal framework, but may not behave the same way in the real world.
% can be very slow
And, (3) SMT-based synthesis can be very slow or fail to complete, especially when reasoning about large network topologies. In practice however, network operators reconfigure their networks on a daily basis \cite{vissicchio2012improving}, which means an effective synthesis tool must be fast.

% \item fully learned, no hand-coded synthesis rules (model-free), very flexible to adapt to more/new protocols
% \item protocol-agnostic, cross-protocol
\paragraph{Neural Algorithmic Reasoning for Synthesis} Recent work on neural algorithmic reasoning (NAR) proposes to replace traditional algorithms with neural networks to learn improved algorithmic procedures \cite{velivckovic2021neural}.
It has been shown to be a powerful and fast algorithmic approximation method for a number of graph-related \cite{velivckovic2019neural} and combinatorial optimization problems \cite{cappart2021combinatorial}. Further, due to its learned nature, NAR allows for learning procedures directly from (real-world) data, without the need for manual feature extraction. Overall, this positions NAR as an attractive method to obtain a fast, fully-learned synthesis procedure, which entirely avoids the need for a formal model or any hand-crafted synthesis rules. Based on this promising outlook, this paper explores how to apply the NAR paradigm to the problem of network configuration synthesis.

To that end, we propose a \textbf{new learning-based framework for configuration synthesis} as an alternative to SMT-based approaches. Our framework is protocol-agnostic, enables cross-protocol reasoning and avoids the need to manually provide synthesis rules. We build upon the idea of NAR, and train a graph-based processor neural network to learn a synthesis procedure in latent space. A key challenge in a multi-protocol setting is the diversity of different protocols and configuration parameters. To this end, we implement a generic embedding scheme based on Datalog-like facts and program sketching \cite{solar2008program}, which allows us to easily adapt our framework to new protocols. Further, our synthesis processor network produces a whole distribution of network configurations. As a consequence, we can directly sample multiple alternative synthesis outputs, which is not possible with standard SMT solvers. We apply our framework to a non-trivial synthesis setting where both the Border Gateway Protocol (BGP) and the Open Shortest Path First (OSPF) protocol are used. We demonstrate that our learned synthesis tool is up to~$500\times$ faster than a state-of-the-art SMT-based synthesizer, while producing configurations which on average enjoy more than 91\% satisfaction of the provided specification.

\paragraph{Main Contributions} Our core contributions are:
\vspace{-5pt}
\begin{itemize}
    \setlength{\itemsep}{5pt}
    \setlength{\parskip}{0pt}
    \item A learning-based framework for network configuration synthesis based on neural algorithmic reasoning.
    \item A neural network architecture for learning synthesizer models which relies on a generic graph-based encoding of network topologies and configurations.
    \item An extensive evaluation of our learning-based synthesizer, in terms of both precision and scalability, on the challenging setting where both the BGP and OSPF protocols are involved.
\end{itemize}

\section{Overview}
\label{sec:overview}

\begin{figure}
    \begin{center}
        \includegraphics[width=0.45\textwidth]{figures/synthesizer-overview.pdf}
    \end{center}
    \caption{An overview of our learning-based synthesis framework.}
    \label{fig:learning-based-synthesis}
\end{figure}

%As an example, consider \cref{fig:network-fwd-tree} (c) which illustrates the forwarding plane of some traffic class reachable via external peer $E$ or $F$ in our example network. Each router of the network forwards traffic along some of its outgoing links. In practice, a number of protocols are used to populate a router's routing tables. For the instantiation of our synthesis framework however, we focus on OSPF and BGP.

We focus on the \emph{forwarding plane} of a network. This means we are interested in how each router forwards traffic, given packets with certain destination. The forwarding plane is determined by a distributed computation according to the routing protocols' semantics. 
To adapt the forwarding behavior, network operators change configuration parameters at the router-level (e.g. link weights), such that running the protocols results in the desired forwarding plane. 

In our context, the synthesis problem is concerned with automatically generating router-level configurations, given a set of requirements constraining the forwarding plane. Typical requirements include reachability, traffic isolation or enforcing certain forwarding paths. To construct a NAR-based system that solves this synthesis problem, our framework relies on a number of key steps as illustrated in \cref{fig:learning-based-synthesis}.

\paragraph{Dataset} To train a synthesizer model, we first generate a dataset of input/output samples. For this, we rely on a generative pipeline as shown in the top of \cref{fig:learning-based-synthesis}. First, we sample a random network configuration for some topology using a uniform generative process. Then, we simulate the involved protocols to obtain the corresponding forwarding plane. Next, we extract a specification by randomly selecting properties that hold for the computed forwarding plane. This leaves us with a pair of (specification+topology, configuration) added to a dataset of training~samples.

\paragraph{Simulation} Depending on the protocols in use, one implements simulation code to compute the forwarding plane induced by a sampled configuration. Although this step is protocol-specific, the overall implementation effort is much lower compared to SMT-based synthesis. Protocols are typically well-defined algorithms which can be simulated, whereas the alternative of implementing a synthesizer often requires expert knowledge about SMT solvers. In practice, our framework may also be adapted to use a real-world network router to compute the behavior of a configuration, thereby capturing the real-world behavior directly.

\paragraph{Neural Synthesizer Model} Given a dataset of pairs each consisting of a configuration and a specification, we now train a graph neural network on this dataset to perform synthesis: given a specification, it tries to predict the configuration. Following the NAR paradigm, we first encode the synthesizer input (specification) in latent space. Then, we apply an iterative processor network which relies on the graph attention mechanism to propagate information \cite{velivckovic2017graph}. Last, we apply a decoder network to extract the synthesized configuration. To remain protocol-agnostic, our model is generic with respect to the input format, using an intermediate representation based on Datalog-like facts.

%More specifically, we employ a slightly modified variant which operates on a graph-based encoding of a specification, topology and configuration parameters.



 \begin{figure*}
     \centering
     \includegraphics[width=0.85\textwidth]{figures/system-overview.pdf}
     \caption{An overview of our synthesis system: (1) First, we use a generic embedding scheme to transform a network topology, protocol configuration sketches and the specification given as Datalog-like facts to a latent input representation. Next, we apply a learned (2) Processor GNN and obtain a latent synthesis output. Last, we apply a (3) Decoder Network to obtain a distribution over possible values per unknown parameter in our configuration.}
     \label{fig:overview-model}
\end{figure*}

\paragraph{Relaxed Specification Consistency} Parts of the configuration synthesis problems are known to be NP-hard \cite{fortz2000internet}. In contrast, our learning-based framework depends on a fixed-size neural network architecture running in polynomial time. Hence, we expect neural synthesis to be less precise than SMT methods and propose the notion of \emph{relaxed~specification~consistency}. That is, to assess the performance of a neural synthesizer, we not only consider if a configuration satisfies a specification, but also the degree up to which it satisfies a specification (e.g., via the relative number of satisfied requirements). This ``soft'' understanding of a specification allows us to evaluate neural synthesis systems which may not always produce fully specification-consistent configurations. Nonetheless, we argue that configurations with less than $100\%$ consistency are still very useful in practice as they provide a good starting point for further manual adjustment by network operators. Note that a similar adjustment process may also be required with SMT-based synthesizers, due to differences between the formal protocol model and the one running on a given real-world router where the configuration is to be deployed.

Next, we discuss the architecture of our neural synthesis framework. In follow-up sections, we instantiate this framework for the case of BGP/OSPF configuration synthesis, and evaluate the resulting instantiation by comparing it to a state-of-the-art SMT-based synthesizer.

% \begin{itemize}
%     \item effort: need to implement simulation code to generate dataset to learn from (typically well-defined in protocol specs, much easier than implementing synthesis directly)
%     \item can be sampled (multiple alternative solutions, not easily possible with SMT-based methods)
%     \item much faster than SMT-based synthesis
% \end{itemize}

% Requirements:
% \begin{itemize}
%     \item protocol-agnostic
%     \item fully learned, no hand-coded synthesis rules
%     \item define: strict specification vs. relaxed specification
% \end{itemize} 

==> diff/git-latexdiff.34965/old/sections/2_model.tex <==
\section{Neural Synthesis Framework}
\label{sec:model}


We now present the architecture of our graph-based neural synthesizer model, illustrated in \cref{fig:overview-model}. First, in \cref{sec:graph-embedding} we introduce our generic graph-based encoding, which allows us to embed network topologies, protocol configuration and the specification into a latent space. Then, in \cref{sec:graph-transformer} we present the architecture of the processor network which we train to perform the synthesis task. Finally, in \cref{sec:decoding-sampling} we discuss how to sample network configurations from the resulting latent synthesis output.

\begin{figure}
    \begin{minipage}[t]{0.21\textwidth}
    \begin{lstlisting}[basicstyle=\ttfamily\small, escapeinside={(*}{*)}]
router(A)
router(B)
(...)

connected(A,B,2)
connected(A,C,?)(*\blackcircled{1}*)
(...)
    \end{lstlisting}
\end{minipage}
\begin{minipage}[t]{0.21\textwidth}
    \begin{lstlisting}[basicstyle=\ttfamily\small, escapeinside={(*}{*)}]
network(N1)
bgp_route(E,N1,2,3,1,0,1)

fwd(A,B,N1)
not fwd(B,A,N1)
(...)
    \end{lstlisting}
\end{minipage}
    \caption{A snippet of a fact base sketch encoding a network's topology, parameters such as link weights (\texttt{connected} facts) and a specification (\texttt{fwd} facts).}
    \label{fig:datalog-encoding}
\end{figure}

\begin{figure}[t]
    \centering
    \includegraphics[width=0.25\textwidth]{figures/synth-architecture.png}
    \caption{The neural synthesizer model architecture.}
    \label{fig:architecture}
\end{figure}

\subsection{Fact Base Embedding}
\label{sec:graph-embedding}
To remain network protocol-agnostic in our model architecture, we implement a generic graph-based encoding of Datalog-like facts, similar to knowledge graphs \cite{rosso2020beyond}. This means that we first encode topologies, configurations and specifications as a set of Datalog-like facts and then employ a generic embedding.
%We chose Datalog facts as the input format of our synthesis approach for its flexibility, wide-spread use in Program Analysis and use in previous work on configuration synthesis \cite{el2017network}.

\paragraph{Fact Base} A set of Datalog-like facts, as depicted in \cref{fig:datalog-encoding}, serves as the input \emph{fact base} $\mathcal{F}$ to our synthesizer model. $\mathcal{F}$ is a set of facts $f(a_0, \dots, a_n)$ where arguments may be constants (e.g. A or B) or integer literals. Further, each fact in a fact base has a corresponding truth value denoted as $[f(a)]_{\mathcal{B}}$. For instance, from the fact base in \cref{fig:datalog-encoding} we can derive $[fwd(A,B,N1)]_{\mathcal{B}} = \text{\texttt{true}}$ and $[fwd(B,A,N1)]_{\mathcal{B}} = \text{\texttt{false}}$.

\paragraph{Consistency} We represent a network's topology, the protocol configuration and parameters as well as the specification, all in a single fact base. Given the semantics of the protocols in use, we can then check whether the specification encoded in a fact base is satisfied by the provided configuration. To quantify, we define the notion of relaxed specification consistency, as discussed earlier, with respect to a fact base: Given a fact base $\mathcal{F}$, a subset of specification facts $S \subset \mathcal{F}$ and protocol semantics $\mathcal{P}$, the \emph{consistency} of a fact base is defined as the relative number of satisfied facts in $S$ with respect to the forwarding plane obtained via $\mathcal{P}$. The contents of $S$ depend on the concrete instantiation of the synthesizer model. For an example of possible specification facts, see our instantiation of the synthesizer model for BGP/OSPF in \cref{sec:training}.

\begin{figure*}
    \def\arraystretch{1.5}
    \begin{tabular}{lr}
        %$T_f: T_1 \times \dots \times T_n$ & \textit{(fact type declaration)}\\
        $emb(f) := \mathbf{V_f}$ & \textit{(learned fact type embedding)}\\
        $emb(b) := \mathbf{W_{\text{bool}}}\;onehot(b)$ & \textit{(learned boolean embedding)}\\
        $emb(f,i,v) := \mathbf{W_{f_i}}\;onehot(v)$ & \textit{(learned integer embedding)}\\
        $emb(f,i,?) := \mathbf{V_{hole}}$ & \textit{(learned hole embedding)}\vspace{10pt}\\
        $\mathlarger{
        h_c := \sum_{f(c) \in \mathcal{F}}
        emb(f)
        }$ & \textit{(constant embedding)}\vspace{10pt}\\
        $h_{f(a_0, \dots, a_n)} := emb(f) + emb([f(a_0, \dots, a_n)]_{\mathcal{B}}) + \mathlarger{
        \sum_{(i,v) \in \mathcal{I}(f(a_0, \dots, a_n))}
        emb(f, i, v)
        }$\hspace{-1.2cm} & \textit{(fact embedding)}\\
        $\mathcal{I}(f(a_0, \dots, a_n)) := \{(i,v) \; | \; f(a_0, \dots, a_{i-1}, v, \dots, a_n) \in \mathcal{F} \wedge v:Int \wedge i \in \mathbb{N}$ \}& \textit{(integer arguments)}\vspace{10pt}\\
        $N_i(h_c) := \{h_f \; | \; \exists i \in \mathbb{N} . f(a_0, \dots, a_{i-1}, c, a_{i+1}, \dots, a_n) \in \mathcal{F}\}$& \textit{(i-th neighborhood of constant node)} \\
        $N_i(h_f) := \{h_c \; | \; \exists i \in \mathbb{N} . f(a_0, \dots, a_{i-1}, c, a_{i+1}, \dots, a_n) \in \mathcal{F}\}$& \textit{(i-th neighborhood of fact node)} \\
    \end{tabular}
    \caption{Translating a fact base $\mathcal{F}$ to node features. $f$ denotes a predicate, $v$ integer values, $b$ boolean values as 0 or 1, $i$ argument indices and $[f(a)]_{\mathcal{B}}$ the truth value of a fact. }
    \label{fig:graph-embedding}
\end{figure*}

%discuss embedding as shown in \cref{fig:datalog-encoding}. Note how this makes fact bases a suitable input to standard GNN architectures.

\paragraph{Fact Base Sketching} In a synthesis setting, we are confronted with incomplete fact bases, i.e. the specification and topology is given but the network configuration is to be synthesized. For these cases, we also consider fact bases with unknown parameters inspired by the idea of program sketching in program synthesis \cite{solar2008program}. More specifically, users may replace an unknown integer argument of a fact by a \texttt{?} symbol, indicating a value to be synthesized. Using this mechanic, we can represent the synthesis input as an incomplete fact base which encodes to-be-synthesized values as unknown parameters. As an example, consider \cref{fig:datalog-encoding} \blackcircled{1}, where the link weight between router nodes \texttt{A} and \texttt{C} is represented as an unknown parameter.

\paragraph{Embedding} We employ a structurally-defined embedding scheme to transform a fact base into a graph with node features as required for processing with graph neural networks. Given a fact base $\mathcal{F}$, we apply the rules in \cref{fig:graph-embedding} to obtain node features and adjacency information. Both a fact $f$ and a constant $c$ are represented as distinct nodes with features $h_c$ and $h_f$, respectively. The relationships between facts and constants is encoded as node adjacency as defined by the neighborhood functions $N_i$.

We use multiple neighborhood functions, i.e. multiple types of edges, to encode the argument position of a constant occurring in a fact. Hence, the number of neighborhood functions corresponds to the maximum number of arguments in a single fact, e.g. 3 in \cref{fig:datalog-encoding}. Integer arguments and unary facts are directly accounted for in the respective node or fact embedding. To handle unknown parameters, we replace the corresponding $emb(...)$ term with the learned $\mathbf{V_{hole}}$ embedding.

Considering the embedding function $emb$, the learned parameters of our embedding are $\mathbf{V_f} \in \mathbb{R}^D$ per fact type in~$\mathcal{F}$, $\mathbf{W_{\text{bool}}} \in \mathbb{R}^{D \times 2}$ for boolean values, $\mathbf{W_{f_i}} \in \mathbb{R}^{D \times N}$ per integer argument of fact type $f$ and $\mathbf{V_{hole}} \in \mathbb{R}^D$ to represent unknown parameters. Hyperparameter $D$ represents the dimension of the latent space the synthesizer model operates in and $N$ specifies the number of supported integer values. An example of applying this embedding scheme to a simple fact base is given in \cref{fig:graph-encoding-example}.

\begin{figure}
    \begin{minipage}[t]{0.2\textwidth}
        \centering
        \footnotesize
        \textbf{Fact Base}
        \begin{lstlisting}[basicstyle=\ttfamily\small]
router(A)
router(B)

conn(A, B, 12)
        \end{lstlisting}
    \end{minipage}
    \begin{minipage}[t]{0.15\textwidth}
        \centering
        \textbf{Graph}\\
        \vspace{5pt}
        \includegraphics[width=0.7\textwidth]{figures/graph-encoding.pdf}
    \end{minipage}\\
    \centering\\
    \vspace{10pt}
    \textbf{Node Features}\\
    \vspace{10pt}
    \begin{minipage}[t]{0.5\textwidth}
        $\begin{array}{rcl}
        h_A &:=& emb(router) = \mathbf{V_{\text{router}}}\\
        h_B &:=& emb(router) = \mathbf{V_{\text{router}}}\\
        h_{\text{conn(A,B,12)}} &:=& emb(conn) + emb(conn, 2, 12)\\
        &:=& \mathbf{V_{\text{conn}}} + \mathbf{W_{conn_2}} onehot(12)
    \end{array}$
    \end{minipage}
    \caption{An example of embedding a simple fact base using the embedding scheme of \cref{fig:graph-embedding}. The shown graph illustrates the neighborhoods $N_0$ and $N_1$ induced by the \texttt{conn} fact.}
    \label{fig:graph-encoding-example}
\end{figure}

\begin{figure}
    $$
    \begin{array}{rcl}
    z_j &:=& h_j + Drop(\mathlarger{\sum_{N_i}} h'_{GAT_i})\\
    h'_j &:=& FFN(Norm(z_j))\vspace{11pt}\\
    FFN(x_j) &:=& Norm(Lin2(Drop(Lin1(x_j)))))
    \end{array}
    $$
    \caption{
        The recurrence relation of a node $j$'s representation $h_j$. $h'_{GAT_i}$ represents the output of a graph attention layer operating with neighborhood $N_i$ according to \cite{velivckovic2017graph}, $h_j$ the representation of node $j$ at the previous step. $Norm$ refers to batch normalization \cite{ioffe2015batch}, $Drop$ to dropout regularization \cite{hinton2012improving} and $Lin1$ and $Lin2$ to linear layers with an inner dimension of $4N$.
    }
    \label{fig:recurrence}
\end{figure}

\subsection{Synthesizer Model}
\label{sec:graph-transformer}

For an illustration of the synthesizer model's architecture, please see Figure~\ref{fig:architecture}. Given a fact base $\mathcal{F}$ we first apply our embedding scheme as described in \cref{sec:graph-embedding}. We then employ a 2-layer GNN-based encoder network to produce the latent representation of a synthesis input.
Given this representation, a processors network is trained to perform the actual synthesis task in high-dimensional space. Last, we apply a set of decoder networks, to obtain the synthesized values of unknown parameter, given the latent synthesis~output.

%In this context, the synthesis problem for network configurations corresponds to completing partially provided fact bases.

% \paragraph{High-Level Architecture}

% We employ the high-level architecture to obtain the latent synthesis output $y_\mathcal{F}$:
% $$
% \begin{array}{rcl}
%     \mathbf{x_{\mathcal{F}}} &:=& Encoder(Embedding(\mathcal{F}))\\
%     \mathbf{y_{\mathcal{F}}} &:=& Processor(\mathbf{x_{\mathcal{F}}} + \mathbf{z})\\
%     z_i &\sim& \mathcal{N}(0,1)
% \end{array}
% $$
% \todo{z is only added for $i<N/2$}

% $Embedding$ corresponds to the graph-based embedding as discussed in \cref{sec:graph-embedding} and $Encoder$ is a 2-layer graph attention module. $Processor$

\paragraph{Encoding} The encoder GNN operates on the embedded representation of a fact base. It produces the high-dimensional representation of a synthesis input as required for the processor network. We additionally apply noise to the first half of the units of the latent representation via $\mathbf{z}$, as a source of non-determinism. According to our experiments this improves model performance and we hypothesize this is due to the synthesis problem having more than one solution in most cases.

\paragraph{Iterative Processor} The processor network is modelled as an iterative process. For this, we apply the same 6-layer graph attention module for a total of 4 iterations.
In the framework of neural algorithmic reasoning, this iterative computational structure encodes an inductive bias towards an iterative solution to the synthesis problem. Because of this bias, our processor network essentially learns an algorithmic procedure which iteratively synthesizes the values of unknown parameters in a fact base.

\paragraph{Graph Attention Layer} In the GNNs we employ, we rely on a composed variant of the graph attention layer as introduced by \cite{velivckovic2017graph}. We employ multiple graph attention layers in lockstep, one per neighborhood $N_i$ defined by our graph embedding (cf. \cref{sec:graph-embedding}), and combine the intermediate results after each step. Specifically, the recurrence relation of a node $j$'s representation $h_j$ is defined as shown in \cref{fig:recurrence}. These mechanics of combining the results of the different graph attention layers $h'_{GAT_i}$, directly corresponds to how multiple attention heads are combined in the original Transformer architecture \cite{vaswani2017attention}.

\paragraph{Argument Decoder Networks} To synthesize the values of unknown parameters, the model maintains a set of decoder networks. That is, it provides one decoder network per integer argument per fact type in a fact base. When decoding, the network is applied to the latent synthesis output of the corresponding fact node. For example, a synthesizer model which operates on the fact base in \cref{fig:graph-encoding-example}, would provide a decoder network $D_{\text{conn}_2}: \mathbb{R}^D \rightarrow \mathbb{R^N}$ to decode values for the third argument of a \texttt{conn} fact. In our experiments, decoder networks are implemented as simple multi-layer perceptron models.

%The synthesizer model learns a conditional distribution of fact bases which are consistent with respect to the protocols' semantics.

%\todo{introduce synthesis as a completion problem of an encoded fact base (a la BERT). Introduce masking, introduce decoding of integer and truth values. Synthesis is learning a conditional distribution of consistent fact bases.}

%Using this method, we obtain the node features $h_c$ per constant, $h_f$ per fact and adjacency information in terms of node neighborhood functions $N_i(h_c)$ and $N_i(h_f)$. Overall, this encoding makes a fact base suitable for processing using standard graph neural networks.

%- Brief description of the Graph Transformer Model
\subsection{Multi-Shot Sampling}
\label{sec:decoding-sampling}

%Multi-Stage Parameter Sampling (sampling methods: topk, high-temp, low-temp)
To sample concrete values from the output distributions over unknown parameters, we apply a multi-shot sampling strategy. That is, we sample values only for a subset of unknown parameters, insert them in our input fact base and run the synthesis model again. We repeat this process until no more unknown parameters remain. This multi-shot sampling strategy allows the model to incorporate the concrete values of previously synthesized parameters in its computation. In our evaluation in \cref{sec:evaluation}, we include a comparison of how this compares to sampling all unknown parameters at once.

%In a fact base with multiple holes, we apply the corresponding decoder networks to obtain a value distribution for each integer hole. However, instead of sampling all integer holes in one


==> diff/git-latexdiff.34965/old/sections/3_bgp_ospf.tex <==
\section{BGP/OSPF Synthesis}
\label{sec:bgp-ospf}

\newcommand{\as}{\ac{AS}~}
\newcommand{\ases}{\acp{AS}~}

\newcommand{\squareann}{{\tiny$\blacksquare\;$}}
\newcommand{\triangleann}{{\small$\blacktriangle\;$}}

\begin{figure*}
    \centering
    \includegraphics[width=0.95\textwidth]{figures/networks-all.pdf}
    \caption{(a) An illustration of a small AS network, including internal peers (blue), external peers (purple), BGP sessions as well as physical links. (b) The propagation of two BGP announcement across the network. (c) The resulting forwarding plane after applying BGP and OSPF.}
    \label{fig:network-fwd-tree}
\end{figure*}

We now discuss an instantiation of our learning-based framework for the case of BGP and OSPF protocols. In \cref{sec:synthesis-setting} we introduce a basic networking model, BGP and OSPF protocols and the synthesis setting. Given this model, \cref{sec:training} describes how to generate a corresponding dataset of input/output samples and train a synthesizer model.
%This shall serve as a prerequisite to the instantiation of our learning-based synthesis framework for the BGP and OSPF protocol in \cref{sec:training}.

\subsection{Synthesis Setting}
\label{sec:synthesis-setting}

\paragraph{Graphical Model} We assume an abstract network model which can be represented as an undirected graph as shown in \cref{fig:network-fwd-tree} (a). We always consider a set of internal routers (A, B, C, D in \cref{fig:network-fwd-tree}) as well as a set of adjacent external routers (E, F  in \cref{fig:network-fwd-tree}). The group of internal routers forms the \emph{\as} under consideration whereas external routers belong to other adjacent \ases. In practice, an \as represents an administrative domain controlled by a single operator.

\paragraph{Forwarding Plane} We focus on the \emph{forwarding plane} of a network. This means we are interested in how a router forwards packets given incoming traffic of different traffic classes. For this, each router maintains a routing table which determines which of its outgoing edges is used to forward packets of a certain traffic class. As an example, consider \cref{fig:network-fwd-tree} (c) which illustrates the forwarding plane of some traffic class reachable via external peer $E$ or $F$ in our example network. Each router of the network forwards traffic along some of its outgoing links. In practice, a number of protocols are used to populate a router's routing tables. For the instantiation of our synthesis framework however, we focus on OSPF and BGP.

\paragraph{OSPF} The OSPF protocol \cite{moy1994ospf} is a link-state protocol, typically used as an interior gateway protocol~(IGP), i.e., to route traffic within an \ac{AS}. Given link weights per physical link in the network, OSPF simply routes traffic along the shortest path towards the destination.

\paragraph{BGP} The BGP protocol \cite{rekhter1994border} on the other hand is a path-vector protocol used to exchange reachability information mostly on the level of \acp{AS}.
%These are groups of routers typically operated by a single party (e.g. an ISP).
When using BGP, a routing destination announces its existence to other \ases and routers, by sending out a BGP announcement. Receivers of such announcements may then choose to pass them on to other \acp{AS}, redistribute them internally and/or modify them. Instead of communicating along physical links directly, the BGP protocol requires manually configured BGP sessions among routers of the \as and external peers, as indicated by the BGP session edges in \cref{fig:network-fwd-tree}(a).
%\todo{more discussion of eBGP vs iBGP and support for route reflection (more of an implementation detail, maybe only mention in dataset generation where simulation code is discussed)}.

%\paragraph{BGP Decision Procedure}~
%\todo{discuss decision procedure}
In case a router receives more than one announcement for a destination, a designated BGP decision process is applied to determine a single best route. \cref{fig:bgp-decision} shows the ordered list of comparison criteria of this decision process. The different criteria depend different properties of a route announcements, including the IGP cost towards the routing destination. As a consequence, when used together, OSPF as IGP protocol and BGP will interact. %Note also that BGP is an iterative process which needs multiple rounds of propagation to converge.

\paragraph{Example}
%\todo{run through simple BGP+OSPF example of computing the forwarding plane}
To better understand BGP/OSPF routing, consider the simple example given in \cref{fig:network-fwd-tree} (b). Here, our example \as imports BGP announcements \squareann and \triangleann from E and F respectively. Both represent a route to the same destination. As shown, both announcements have a so-called local preference of 2. For simplicity, we ignore other properties such as the AS path length, Origin and MED in this example. The announcements are propagated among BGP neighbors and the best route is selected according to the decision procedure in \cref{fig:bgp-decision}. See \cref{fig:network-fwd-tree} (b) for an illustration of the intermediate states of this propagation process. As both announcements have a local preference of 2, rule 1 of the decision process is not used. Instead, in round 2, node B selects \squareann over \triangleann due to a lower IGP cost of 2 via egress node A as compared to 3 via egress node D (rule 6). Node D selects \triangleann over \squareann, since it learns this route directly from an external peer (rule 5). After Round 3, the BGP propagation process converges to a stable state and we can derive the forwarding plane as shown in \cref{fig:network-fwd-tree} (c).


%, as well as external peers E and F which belong to other \acp{AS}. External peers are routers which are connected via eBGP sessions to routers of the \ac{AS} under consideration. They announce BGP routes to their neighbors, which are propagated within the network

\paragraph{Problem Statement: Configuration Synthesis} We phrase the BGP/OSPF configuration synthesis problem on the level of the forwarding plane. This means that users provide a specification which constraints the set of allowed forwarding planes. This includes predicates which enforce forwarding paths, block forwarding paths or assert higher-level properties like traffic isolation and reachability. Given such a specification, we consider network configuration synthesis as the task of configuring OSPF and BGP in a way that produces a forwarding plane which satisfies the provided specification.

\paragraph{Search Space} To limit the space of candidate configurations, we define the set of synthesized parameters: For OSPF we synthesize link weights as explored in a wide range of existing work (e.g. \cite{el2018netcomplete,fortz2000internet}. BGP parameters on the other hand are not defined as clearly: Depending on the requirements of a network operator, one may employ custom BGP import and export policies at every router of a network to implement complex behavior. However, in this work we focus on a simplified setting, where we assume BGP route announcements to only be modified when imported into the \as from an external peer. Previous work has already pointed out that this is a reasonable assumption which holds for the majority of real-world networks \cite{caesar2005bgp,cittadini2010doing, steffen2020probabilistic}.

\begin{figure}
    \small{
    \begin{enumerate}
        \setlength{\itemsep}{0pt}
        \setlength{\parskip}{0pt}
        \item Highest Local preference
        \item Lowest AS path length
        \item Prefer Origin (IGP $>$ EBGP $>$ INCOMPLETE)
        \item Lowest Multi-exit discriminator (MED)
        \item External over internal announcements
        \item Lowest IGP cost to egress
        \item Lowest BGP peer id (tie breaker)
    \end{enumerate}}
    \vspace{-15pt}
    \caption{The BGP decision process \cite{rekhter1994border}. The shown rules are applied in order until a single best BGP announcements remains.}
    \label{fig:bgp-decision}
\end{figure}

\subsection{Dataset Generation and Training}
\label{sec:training}
To train a synthesizer model, we need a large number of fact bases encoding a variety of network topologies, configurations and forwarding specifications. Further, we must provide the model with target values for unknown parameters as a supervision signal. This section discusses how we construct such a dataset for BGP/OSPF synthesis.
%Further, we provide an example of what a corresponding fact base looks like, including a description of the supported specification language.

\paragraph{Dataset Generation} To obtain network configurations and corresponding forwarding specifications we employ a generative process: We first randomly configure BGP and OSPF parameters for some topology. Then we simulate the OSPF and BGP protocol and compute the resulting forwarding plane. Based on this, we extract a forwarding specification which fixes a random subset of forwarding paths, reachability and isolation properties that are satisfied by the forwarding plane.

\paragraph{Topologies} For training, our dataset is based on random topologies with $16$-$24$ routers. We generate the physical layout of these graphs by triangulation of uniformly sampled points in two-dimensional space.

\paragraph{Simulation} To compute the forwarding plane given an OSPF and BGP configuration, we simulate the protocols. For OSPF, we implement shortest path computation to obtain the forwarding plane. For BGP, we implement the full BGP decision process as shown in \cref{fig:bgp-decision}, except for the MED attribute. In addition to the basic networking model discussed in \cref{sec:synthesis-setting}, we implement support for eBGP and iBGP, fully-meshed BGP session layouts as well as layouts relying on route reflection. For more details of these BGP concepts see \cite{bates2000rr}.

%Note that the synthesizer model will reason on the level of the provided training samples. That is, to improve the overall synthesis quality in a real-world setting, it is helpful to implement simulation code which behaves very similar to real-world networks. Another promising approach would be to extract training samples from real-world networks, thereby circumventing the need for simulation, however, we leave this as future work.

%While this can be a considerable effort, it is typically an easier task than to implement the synthesizer directly. The concrete semantics of protocols and their simulation is a well-defined procedure, whereas implementing efficient synthesis tools is still an open problem.

\paragraph{Fact Base Encoding} We encode synthesis input using a small set of facts. For an example of a corresponding fact base see \cref{fig:bgp-ospf-fact-base}. We use the \texttt{router}, \texttt{external} and \texttt{network} facts to mark routers, external peers and routing destinations respectively. Physical links between routers are encoded as \texttt{connected(R1,R2,W)} facts where \texttt{W} denotes the OSPF link weight. Further, we rely on \texttt{ibgp}, \texttt{ebgp}, \texttt{route\_reflector} and \texttt{bgp\_route} facts to represent different types of BGP sessions and imported routes. Using the notion of unknown parameters as discussed in \cref{sec:graph-embedding}, we encode configuration parameters, e.g., properties of imported routes or OSPF link weights.

\paragraph{Specification Language} We support a small specification language with three types of forwarding predicates:

\begin{itemize}
    \setlength{\itemsep}{0pt}
    \setlength{\parskip}{2pt}
    \item \texttt{fwd(R1, Net, R2)} specifies that router \texttt{R1} forwards traffic destined for \texttt{Net} to its neighbor \texttt{R2}.
    \item \texttt{reachable(R1, Net, R2)} specifies that traffic destined for \texttt{Net} that passes through \texttt{R1} also passes through \texttt{R2} before reaching its destination.
    \item \texttt{trafficIsolation(R1, R2, N1, N2)} specifies that it must not hold that $[fwd(R1,R2,N1)]_{\mathcal{B}} \wedge [fwd(R1,R2,N2)]_{\mathcal{B}}$.
\end{itemize}

In the negative case of each predicate, the opposite must hold true for the fact to be satisfied. This specification language can easily be extended by including new specification predicates in the dataset generation process. One must simply provide a method of extracting positive and negative cases of a specification fact from a given forwarding plane. Once included in the training dataset of a synthesizer model, the resulting synthesis system will be able to consider specifications relying on the new type of predicates.

% \todo{info on loss function, optimizer, etc.}
\paragraph{Training} We generate a dataset of $10,240$ input/output samples and instantiate our synthesizer model with a hidden dimension $D$ of $64$. For optimization, we use the Adam optimizer \cite{kingma2014adam} with a learning rate of $10^{-4}$, applying negative log-likelihood loss to the decoder networks' outputs. We stop training after the specification consistency on a validation dataset no longer increases at around $\sim2800$ epochs.

\begin{figure}
\begin{minipage}[t]{0.22\textwidth}
\begin{lstlisting}[basicstyle=\ttfamily\tiny]
# topology and configuration
router(c5)
router(c3)
router(c1)
router(c0)
network(c6)
network(c7)

external(c8)
external(c9)
external(c10)
external(c11)
external(c12)
external(c13)

route_reflector(c2)
route_reflector(c4)

connected(c2,c4,?)
connected(c2,c5,?)
connected(c2,c3,?)
connected(c4,c5,?)
connected(c4,c3,?)
connected(c4,c0,?)
connected(c5,c1,?)
connected(c5,c0,?)
connected(c3,c0,?)
connected(c3,c1,?)
connected(c1,c0,?)

ibgp(c2,c4)
ibgp(c2,c5)
ibgp(c2,c0)
ibgp(c2,c1)
ibgp(c4,c3)
ibgp(c4,c4)
\end{lstlisting}
\end{minipage}
\begin{minipage}[t]{0.2\textwidth}
\begin{lstlisting}[basicstyle=\ttfamily\tiny]
ebgp(c2,c12)
ebgp(c5,c9)
ebgp(c5,c10)
ebgp(c5,c13)
ebgp(c0,c8)
ebgp(c0,c11)

bgp_route(c8,c6,?,?,1,?,1,8)
bgp_route(c9,c6,?,?,0,?,1,9)
bgp_route(c10,c6,?,?,0,?,1,10)
bgp_route(c11,c7,?,?,0,?,1,11)
bgp_route(c12,c7,?,?,0,?,1,12)
bgp_route(c13,c7,?,?,2,?,1,13)

# forwarding specification
fwd(c0,c6,c3)
fwd(c3,c6,c2)
fwd(c2,c6,c4)
not fwd(c3,c6,c0)
not fwd(c0,c6,c11)
not fwd(c11,c6,c0)

not trafficIsolation(c1,c0,c7,c6)
not trafficIsolation(c1,c0,c7,c6)
trafficIsolation(c0,c3,c6,c7)
trafficIsolation(c0,c3,c6,c7)

reachable(c5,c6,c10)
reachable(c1,c6,c4)
not reachable(c0,c6,c5)
reachable(c5,c6,c10)
\end{lstlisting}
\end{minipage}
\caption{An example of a fact base encoding a topology, a sketch of a BGP and OSPF configuration and a forwarding specification.}
\label{fig:bgp-ospf-fact-base}
\end{figure} 

==> diff/git-latexdiff.34965/old/sections/4_evaluation.tex <==
\section{Evaluation}
\label{sec:evaluation}

We trained a synthesizer model to perform configuration synthesis for BGP and OSPF. We now assess the performance of the resulting neural synthesizer with respect to two core metrics: (1) the quality of synthesized configurations in terms of their consistency with the provided forwarding specifications (\cref{sec:synthesis-quality}), and (ii) the time a learned synthesizer takes when compared to the state-of-the-art SMT-based synthesizer NetComplete \cite{el2018netcomplete} (\cref{sec:synthesis-vs-smt}).

\paragraph{Dataset} We compare across three datasets: Small, Medium and Large. Each dataset represents 8 real-world topologies, sampled from the Topology Zoo \cite{knight2011internet}, where the number of nodes lies between 0-34, 34-68 and 68-170 respectively. To obtain forwarding specifications for the sampled topologies, we use our generative pipeline as discussed in \cref{sec:training}. In each topology, we do synthesis for 4 different traffic classes (routing destinations) at a time.

\paragraph{Experimental Setup} We run all our experiments on an Ubuntu Linux machine with an Intel(R)~Core(TM)~i9-9900X~@~3.50GHz processor, 64GB of system memory and an NVIDIA GeForce RTX 3080 GPU with 10GB of video~memory.

\subsection{Synthesis Quality}
\label{sec:synthesis-quality}
To assess our learned synthesizer, we examine its behavior with increasingly large topologies and specifications.

\paragraph{Specifications} Using the same generative model as described in \cref{sec:training}, we generate forwarding specifications for the topologies in our three datasets with each specification constructed from $3 \times n$ requirements, one per supported predicate type:  \texttt{fwd} requirements correspond to specifying or blocking a forwarding path using multiple \texttt{fwd} predicates whereas \texttt{reachable} and \texttt{trafficIsolation} requirements each translate to a single specification fact. We compare across increasingly large specifications of $3\times 2$, $3\times 8$ and $3 \times 16$ requirements, respectively.

\paragraph{Methodology} For each pair of topology and specification, we run our synthesizer 5 times and report the network configurations with the highest overall consistency value. For sampling, we rely on our multi-shot sampling strategy where we randomly group the unknown parameters of a configuration into 4 groups (4-shot sampling).

\paragraph{Results} We summarize our results in \cref{fig:eval-consistency}. On average, our synthesis model produces network configurations that are $>91\%$ consistent with the provided forwarding specifications across all datasets and sizes of specifications. When only few requirements are given, the synthesizer model even succeeds in producing fully-consistent configurations. We observe a slightly decreasing consistency with increasingly large topologies.

%\texttt{fwd} facts are satisfied more easily, whereas \texttt{reachable} and \texttt{trafficIsolation} facts are violated more often.

\paragraph{Multi-Shot Sampling} In \cref{fig:eval-consistency-baseline}, we report the average specification consistency using our multi-shot sampling strategy as compared to sampling all unknown parameters at once. As a baseline we have also sampled random configurations from a uniform distribution (per parameter) and compute the corresponding specification consistency. Over the baseline, our synthesizer model shows clear improvement and multi-shot sampling further increases consistency.

\begin{figure*}
    \begin{center}
        \textbf{Specification Consistency}\\
        \footnotesize
        \begin{tabular}{rrcccccccccc}
        \toprule
        \multicolumn{2}{c}{Dataset} & \tiny\texttt{fwd} & \tiny\texttt{reachable}  & \tiny\texttt{trafficIsolation} & Overall & $\emptyset$     No. Full Matches & $\emptyset$ No. $>90\%$ Matches\\
        \midrule
        $3\times 2$ requirements & Small & 0.95 & 0.94 & 1.00 & \textbf{0.95} & 0.62 & 0.62\\
& Medium & 0.96 & 1.00 & 0.94 & \textbf{0.96} & 0.88 & 0.88\\
& Large & 0.94 & 0.94 & 1.00 & \textbf{0.93} & 0.62 & 0.62\\
\midrule
$3\times 8$ requirements & Small & 0.97 & 0.98 & 0.97 & \textbf{0.98} & 0.50 & 1.00\\
& Medium & 0.99 & 0.95 & 1.00 & \textbf{0.98} & 0.50 & 1.00\\
& Large & 0.96 & 0.95 & 0.91 & \textbf{0.94} & 0.38 & 0.88\\
\midrule
$3\times 16$ requirements & Small & 0.97 & 0.89 & 0.95 & \textbf{0.94} & 0.38 & 0.75\\
& Medium & 0.98 & 0.97 & 0.97 & \textbf{0.98} & 0.38 & 1.00\\
& Large & 0.92 & 0.88 & 0.95 & \textbf{0.91} & 0.12 & 0.50\\
    \end{tabular}\end{center}
    \caption{Average specification consistency of the network configurations synthesized by our trained synthesizer model. Per sample we run the synthesizer with a specification of $3\times N$ requirements, where the specifications always include $N$ requirements per supported predicate type (\texttt{fwd}, \texttt{reachable}, \texttt{trafficIsolation}).}
    \label{fig:eval-consistency}
\end{figure*}

\begin{figure}
    \begin{center}
        \footnotesize
        \begin{tabular}{rrcccccccccc}
        &  & \multicolumn{2}{c}{Neural}\\
        & Random & 1-Shot & 4-shot\\
        \toprule
        Small & 0.83 & 0.92 & \textbf{0.94} \\
        Medium & 0.88 & 0.95 & \textbf{0.98} \\
        Large & 0.78 & 0.88 & \textbf{0.91} \\
    \end{tabular}\end{center}
    \caption{Average specification consistency with $3\times 16$ requirements when sampling configurations randomly from a uniform distribution and 1-shot/4-shot sampling using our synthesizer model.}
    \label{fig:eval-consistency-baseline}
\end{figure}

\begin{figure*}[ht]
    \footnotesize
    \begin{center}
        \textbf{BGP Synthesis Time}
        \footnotesize
        \begin{tabular}{rrccccccccc}
        \toprule
        &&\multicolumn{3}{c}{Synthesis Time (s)} & \multicolumn{2}{c}{Accuracy (Neural)} \\
        \multicolumn{2}{l}{\# Requirements} & NetComplete & Neural (CPU) & Speedup &$\emptyset$ Consistency& $\emptyset$ No. Full Matches\\
        \midrule
    2 requirements &Small & 18.073s & 0.641s & \textbf{28.2x} & 0.969 & 0.875\\
        &Medium & 60.864s & 2.748s & \textbf{22.2x} & 0.939 & 0.75\\
        &Large & 1389.485s\tiny{  7/8 TO} & 22.301s & \textbf{62.3x} & 0.989 & 0.875\\
    \midrule
    8 requirements &Small & 247.691s & 1.065s & \textbf{232.5x} & 0.96 & 0.75\\
        &Medium & $>$25m\tiny{  8/8 TO} & 3.47s & \textbf{432.2x} & 0.968 & 0.5\\
        &Large & $>$25m\tiny{  8/8 TO} & 30.961s & \textbf{48.4x} & 0.969 & 0.75\\
    \midrule
    16 requirements &Small & 1416.828s\tiny{  7/8 TO} & 2.528s & \textbf{560.5x} & 0.926 & 0.25\\
        &Medium & $>$25m\tiny{  8/8 TO} & 5.481s & \textbf{273.7x} & 0.947 & 0.25\\
        &Large & $>$25m\tiny{  8/8 TO} & 69.092s & \textbf{21.7x} & 0.959 & 0.25\\
    \end{tabular}\end{center}
    \caption{Comparing consistency and synthesis time of our method (Neural) with the SMT-based state-of-art synthesis tool NetComplete. The notation {\tiny{n/8 TO}} indicates the number of timed out synthesis runs out of 8 (25+ minutes).}
    \label{fig:evaluation-compare-bgp}
\end{figure*}

\begin{figure*}[ht]
    \begin{center}
        \footnotesize
        \textbf{OSPF Synthesis Time}\\
        \footnotesize
        \begin{tabular}{rrccccccccc}
        \toprule
        &&\multicolumn{3}{c}{Synthesis Time (s)} & \multicolumn{2}{c}{Accuracy (Neural)} \\
        \multicolumn{2}{l}{} & NetComplete & Neural (GPU) & Speedup &$\emptyset$ Consistency& $\emptyset$ No. Full Matches\\
        \midrule
    2 requirements &Small & 0.265s & 0.091s & \textbf{2.9x} & 1.000 & 1.00\\
     &Medium & 0.404s & 0.098s & \textbf{4.1x} & 1.000 & 1.00\\
     &Large & 0.944s & 0.14s & \textbf{6.7x} & 1.000 & 1.00\\
    \midrule
    8 requirements &Small & 0.876s & 0.164s & \textbf{5.3x} & 0.982 & 0.75\\
     &Medium & 1.517s & 0.103s & \textbf{14.7x} & 1.000 & 1.00\\
     &Large & 3.505s & 0.316s & \textbf{11.1x} & 0.981 & 0.50\\
    \midrule
    16 requirements &Small & 1.65s & 0.21s & \textbf{7.9x} & 0.991 & 0.625\\
     &Medium & 2.646s & 0.245s & \textbf{10.8x} & 0.989 & 0.50\\
     &Large & $>$566.636s+\tiny{  3/8 TO} & 0.233s & \textbf{2430.4x} & 0.987 & 0.875\\
    \end{tabular}\end{center}
    \caption{Comparing consistency and synthesis time of our method (Neural) with the SMT-based OSPF synthesis tool NetComplete. The notation {\tiny{n/8 TO}} indicates the number of timed out synthesis runs out of 8 (25+ minutes).}
    \label{fig:evaluation-compare-ospf}
\end{figure*}


\subsection{Comparison to SMT-based Synthesis}
\label{sec:synthesis-vs-smt}

%To provide a comparison of our learned BGP/OSPF synthesizer with SMT-based methods,
We now compare the synthesis time of the learned neural synthesizer with those of NetComplte, a state-of-art configuration synthesis tool based on SMT-solvers \cite{el2018netcomplete}.

\paragraph{Specifications} As the type of supported requirements in NetComplete does not fully align with our model, we restrict this comparison to specifications which only include forwarding paths (i.e. \texttt{fwd} predicates). Further, NetComplete does not support cross-protocol synthesis as in our case and instead requires users to specify for each requirement the protocol to use for its implementation. To bridge this gap, we split the generated forwarding requirements into BGP and OSPF paths for a corresponding NetComplete specification.
%\todo{note on NetComplete installing policies at all routers, not only the edges of the AS}

\paragraph{Methodology} We compare both OSPF synthesis and BGP/OSPF-synthesis. We configure our trained synthesizer model to do OSPF synthesis by only predicting link weights. For each pair of topology and specification, we report the total time of running our synthesizer 4 times using 4-shot sampling, whereas for consistency we report the best out of the 4 runs. For NetComplete, we run the synthesizer with a timeout of 25 minutes. In case a NetComplete attempt times out, we report 25 minutes as a lower bound for its runtime.

\paragraph{OSPF Synthesis Time Results} We document the results of comparing OSPF synthesis time in \cref{fig:evaluation-compare-ospf}. Our synthesizer model achieves a speedup of 2-10x over NetComplete. With 16 requirements and dataset Large this speedup even increases to $2000\times$. Further, our model achieves very high consistency with the provided specification, often producing fully-consistent configurations.

\paragraph{BGP/OSPF Synthesis Time Results} In \cref{fig:evaluation-compare-bgp} we show the comparison of BGP/OSPF synthesis time. Our synthesizer model outperforms NetComplete by multiple orders of magnitude. We observe a speedup of $20-560\times$ which appears to increase with the size of topology and specification. Further, the average specification consistency of the synthesized configurations is greater than $92\%$ across all datasets, even for large topologies. In many cases, our synthesizer model produces fully-consistent configurations, especially with small topologies and specifications. In comparison, NetComplete times out on more than half of the synthesis tasks which means that we can only observe a lower bound of speedup in these cases. Note that our synthesizer model is running on a CPU due to memory restrictions with large topologies. However, running it on a GPU results in even greater speedups (up to $1000\times$, cf. \cref{app:sec:bgp-gpu-performance}). 

==> diff/git-latexdiff.34965/old/sections/5_related_work.tex <==
\section{Related Work}
\label{sec:related-work}

\paragraph{Traditional Configuration Synthesis} 
%A range of existing work is concerned with network configuration synthesis. 
Next to methods based on compilation such as Propane/PropaneAT \cite{beckett2017network}, there are a number of configuration synthesis methods based on constraint solving: Examples include ConfigAssure \cite{narain2008declarative}, SyNet \cite{el2017network} and NetComplete \cite{el2018netcomplete}. Due to their hand-coded nature, these methods are highly protocol-specific and can be very slow due to the solvers they employ. Although some of them allow for cross-protocol reasoning, this is not implemented as transparently as in our framework and users must specify per requirement which protocol to use for its implementation. In contrast, our approach has lower precision but allows for fully transparent cross-protocol reasoning, meaning forwarding requirements are not protocol-bound and the synthesizer chooses how to implement them. Further, our learned BGP/OSPF synthesis tool exhibits much lower synthesis times as compared to an SMT-based tool like NetComplete.

% \begin{itemize}
%     \item NetComplete, SyNet
%     \item Propane, PropaneAT
%     \item DeepBGP
% \end{itemize}

\paragraph{GNNs and Networking} DeepBGP \cite{bahnasy2020deepbgp} relies on GNNs and reinforcement learning to do configuration synthesis. However, it is limited to BGP configuration synthesis and is slower than SMT-based synthesis according to the author's evaluation. In contrast, our learning-based framework is cross-protocol, does not rely on reinforcement learning and provides better synthesis performance. Apart from configuration synthesis, GNNs have also been applied to other problems in the networking domain. For example, the authors of RouteNet \cite{rusek2020routenet} use GNNs to predict performance metrics of network configurations. Other work that is concerned with learning improved protocols includes Q-Routing \cite{boyan1994packet} or more modern approaches such as the Graph-Query Neural Network architecture \cite{geyer2018learning}.

\paragraph{Neural Algorithmic Reasoning} 
Neural algorithmic reasoning (NAR) as proposed in \cite{velivckovic2021neural}, describes the idea of replacing traditional algorithms with neural networks to learn improved algorithmic procedures. Exemplary work includes graph-related algorithms \cite{velivckovic2019neural} or solvers for combinatorial optimization problems \cite{cappart2021combinatorial,joshi2020learning,selsam2019guiding}. Our synthesis framework is the first applications of NAR to the networking domain and relies on the NAR-native encode-process-decode architecture. According to the hierarchy of NAR approaches in \cite{cappart2021combinatorial}, our method is an algorithm-level approach, as we do not supervise on intermediate steps. Although, such step-level methods promise better generalization, it is not clear what an intermediate result of a general synthesis procedure would be. However, future work on a step-level approach may further improve synthesis quality.

% \begin{itemize}
%     \item RouteNet
%     \item GraphNET
%     \item Learning and generating distributed routing protocols using graph-based deep learning
%     \item Unveiling the potential of Graph Neural Networks for network modeling and optimization in SDN
% \end{itemize}

==> diff/git-latexdiff.34965/old/sections/6_conclusion.tex <==
\setlength{\parskip}{6pt plus4mm minus4mm}
\section{Conclusion}
\label{sec:conclusion}
We presented a learning-based framework for configuration synthesis based on the idea of neural algorithmic reasoning. To assess the effectiveness of the system, we instantiated it for the case of BGP/OSPF synthesis. In contrast to traditional synthesis methods, our system supports transparent cross-protocol reasoning and learns synthesis rules only from data. Using our system, synthesis is sped up by a factor of up to $500\times$ when compared to SMT-based methods. Further, our evaluation demonstrates that the resulting synthesis tool provides excellent synthesis quality, producing configurations with high specification consistency. Overall, our results illustrate that exploring the direction of learning-based network configuration synthesis is a promising direction, enabling new cross-protocol reasoning capabilities and great performance improvements. Promising future work includes construction of hybrid systems, integrating both neural models and SMT-based approaches to obtain the best of both worlds.
